Submodular Matroid Secretary Problem with Shortlists

In the matroid secretary problem, the elements of a matroid $\mathcal{M}$ arrive in random order. Once we observe an item we need to irrevocably decide whether or not to accept it. The set of selected elements should form an independent set of the matroid. The goal is to maximize the total sum of the values assigned to these elements. We introduce a version of this problem motivated by the shortlist model in [Agrawal et al.]. In this setting, the algorithm is allowed to choose a subset of items as part of a shortlist, possibly more than $k=rk(\mathcal{M})$ items. Then, after seeing the entire input, the algorithm can choose an independent subset from the shortlist. Furthermore we generalize the objective function to any monotone submodular function. Is there an online algorithm achieve a constant competitive ratio using a shortlist of size $O(k)$? We design an algorithm that achieves a $\frac{1}{2}(1-1/e^2-\epsilon-O(1/k))$ competitive ratio for any constant $\epsilon>0$, using a shortlist of size $O(k)$. This is especially surprising considering that the best known competitive ratio for the matroid secretary problem is $O(\log \log k)$. An important application of our algorithm is for the random order streaming of submodular functions. We show that our algorithm can be implemented in the streaming setting using $O(k)$ memory. It achieves a $\frac{1}{2}(1-1/e^2-\epsilon-O(1/k))$ approximation. The previously best known approximation ratio for streaming submodular maximization under matroid constraint is 0.25 (adversarial order) due to [Feldman et al.], [Chekuri et al.], and [Chakrabarti et al.]. Moreover, we generalize our results to the case of p-matchoid constraints and give a $\frac{1}{p+1}(1-1/e^{p+1}-\epsilon-O(1/k))$ approximation using $O(k)$ memory, which asymptotically approaches the best known offline guarantee $\frac{1}{p+1}$ [Nemhauser et al.]

==> Impossiblesave.tex <==
%\section{Impossibility Result}

In this section we provide an upper bound showing the following:

\hardness*

%\begin{theorem}
%There is no algorithm achieving asymptotic competitive ratio $7/8+\epsilon$ for submodular secretary problem using $o(n)$ selections. 
%\end{theorem}

%\mcomment{In the following proof we will consider a submodular $k+1$-secretary} problem. 
In the following proof, for simplicity of notation, we prove the desired bound for submodular $k+1$-secretary problem. %Since $k+1=O(k)$, the upper bound derived will imply the stated bound for the  submodular $k$-secretary problem. 
First, we define a monotone submodular function $f$ as follows. 
For $n>0$, the ground set consists of two types of elements, $A$ and  $B$, such that
$f(a)=k$ for $a\in A$ and $f(b)=1$ for $b\in B$. %There are infinitely many elements of $A$ and $B$. 
\scomment{Don't you just need $L$ items of type $A$ and $n-1$ items of type $B$?}
There are $L:=n/2k$ items of type $A$ and
$n-1$ items of type $B$.
Also there is a collection of {\it disjoint} sets $T_{\ell}=\{a_1^{\ell}, b_1^{\ell},\cdots, b^{\ell}_{k}\}$, $\ell=1,2, \ldots L$, such that $a_1^{\ell}\in A$ and $b_j^{\ell}\in B$, and $f(T_{\ell})=2k$.
\scomment{infinite number of such sets? or will $L$ suffice?} 
\mcomment{in the definition of function it should be infinite but in the input we use $n/2k$ of them}
\scomment{After going through the proof, I don't see why you need infinite number, it seems just $L=n/2k$ will suffice. Where are you using that there are infinte number of $T^\ell$?}
\mcomment{
The reason is that you should give one functions $f$ that works for all $n$. Otherwise one may claim that for any given function $f$ there is large enough $N_f$ so that we can go beyond 7/8, for $n>N_f$. 
}

Now define 
$$g(t):=k+k/2+\cdots+ (t-ik)/2^i$$
where $i=\floor{t/k}$. It is easy to see that $g$ is a monotone submodular function.
Now define $f$ as follows:
\begin{itemize}
\item $|S\cap A| \ge 2 \implies f(S):=2k+1$
\item $|S\cap A|=0 \implies f(S):=1+g(|S|-1)$
\item $|S\cap A|=1 :$
\begin{itemize}
\item $S\cap A\notin\{a^{\ell}_1\}_{\ell>0} \implies f(S):=k+\frac{1}{2} g(|S|-1)$
\item $S\cap A= \{a_1^{\ell}\}$ for some $\ell$  $\implies f(S):=\min\{2k+1, k+\frac{1}{2} g(|S|-1)+k'/2^{i+1}\}$, where $k'=|S\cap\{b^{\ell}_1,\cdots, b_k^{\ell}\} |$.
\end{itemize}
\end{itemize}
Note that for any subset $S$, $f(S)\le 2k+1$.
\begin{lemma}
$f$ is a monotone submodular function.
\end{lemma}
\begin{proof}
We have to show that for elements $x$ and subsets $S\subseteq T$, $\Delta_f(x|S) \ge \Delta_f(x|T)$.
We consider the following cases:
\begin{itemize}
\item if $|T\cap A| \ge 2 \implies f_T(x)=0$, so it is trivial.
\item if $|T\cap A| =0 \implies |S\cap A|=0 \implies \Delta_f(x|S) \ge \Delta_f(x|T)$ because of submodularity of $g$.
\item if $|T\cap A|=1 \implies |S\cap A|\le 1$
\begin{itemize}
\item if $|S\cap A|=1 :$
\begin{itemize}
\item $S\cap A = T\cap A = \{a_1^{\ell}\}:$
\begin{itemize}
\item $x\in \{b_1^{\ell},\cdots, b_k^{\ell}\} \implies \Delta_f(x|S)=1/2^i+1/2^i$ and $\Delta_f(x|T)=1/2^j+1/2^j$ for $j\ge i$.
\item $x\notin \{b_1^{\ell},\cdots, b_k^{\ell}\} \implies \Delta_f(x|S)=1/2^i$ and $\Delta_f(x|T)=1/2^j$ for $j\ge i$.
\end{itemize}
\item $S\cap A = T\cap A \notin \{a_1^{\ell}\}_{\ell} \implies \Delta_f(x|S) \ge \Delta_f(x|T)$ because of submodularity of $g$.
\end{itemize}
\item if $|S\cap A|=0 \implies \Delta_f(x|T) \le 1/2^{i+1}+1/2^{i+1}$ and $\Delta_f(x|S)= 1/2^j$ for $j\le i$. Thus $\Delta_f(x|S) \ge \Delta_f(x|T)$.
\end{itemize}
\end{itemize} 
Monotonicity is trivial.
\end{proof}

\toRemove{
Also for any subset of $S$ with at least two elements of $A$, $f(S)=2k$. 
For subset $S$ with no element in $A$, if $i=\floor*{\frac{|S|}{k}}$, 
$f(S)$ is defined as 
\[
f(S)= k+k/2+ \dots +(|S|-ik)/2^{i}.
\]
For subset $S$ with exactly one element $a\in A$ such that $a\neq a_1$, if if $i=\floor*{\frac{|S|-1}{k}}$, 
$f(S)$ is defined as 
\[
f(S)= k+ k/2+ \dots +(|S|-1-ik)/2^{i+1}.
\]
Thus if $|S|=k+1$ and it contains exactly one element of $a\in A$ such that $a\neq a_1$ then $f(S)=k+k/2$.
Now suppose $S$  contains $a'$. 
For $S=T$, $f(S)=2k$.  Suppose $S$ contains $k'<k$ elements of $\{b_1, \dots, b_k\}$  and $\ell$ other elements of $B$. 
Let's $t=k'+\ell$, and $i=\floor*{\frac{t}{k}}$, then
\[
f(S)= \min\{2k, k'/2+(k+ k/2+ \dots +(t-ik)/2^{i+1})\}
\]
}
%\scomment{this proof is very vague, especially the claim any algorithm will select $k/2$ of $B$? Phrases like algorithm is not "aware" of something cannot be stated as a fact. You need to prove that the algorithm will not be able to distinguish between the two scenarios. We need to discuss.}



%Let $ {\cal T}^L$ be a collection of (any) $L=n/2k$ sets from $T^\ell, \ell=1,2, \ldots$. W.l.o.g., let's assume ${\cal T}^\ell = \{T_1, \ldots, T_L\}$.   

Denote $B^{\ell} := T^\ell \cap B = \{b_1^{\ell},\cdots, b_k^{\ell}\}$ for $\ell=1,2, \ldots,$. Also, let 
$B'=B\setminus (\bigcup_{\ell=1}^L B^{\ell})$. % where $L:=n/2k$. 
%\scomment{Do you need $T^\ell, \ell =1,\ldots, L$ to be disjoint?} \mcomment{yes}
% $B'=B\setminus (\bigcup_{\ell }^{L} B^{\ell})$ for $L:=n/2k$.
Now define $L$ input instances $\{I_{\ell}\}_{\ell =1,\ldots, L}$, each of size $n$, as follows. For
any arbitrary subset $\tilde{B}\subseteq B'$ of size $n-Lk-1$, 
%\scomment{Which subset $\tilde{B}$? any arbitrary subset?} \mcomment{arbitrary}
define $I_{i}=\bigcup_{\ell=1,\ldots, L}  B^{\ell} \cup \tilde{B} \cup \{a_1^{i}\}$, for  $i=1,\ldots, L$.
%and $I_2=B^1 \cup B^2 \cup \tilde{B} \cup \{a_1^2\}$ (the difference is $a_1^1$ and $a_1^2$).
%Now suppose the input consists of the following:  $T^{\ell}=\{a_1^{\ell}, b_1^{\ell}, \cdots b_k^{\ell} \}$, no other element of $A$ and the remaining elements are from $B':=B\setminus \{b_1^{\ell}, \cdots, b_k^{\ell}\}$. 
Thus the optimal is $T^{\ell}$ for instance $I_{\ell}$, with $f(T^{\ell})=2k$. 
\scomment{$T^\ell$ is of size $k+1$, optimal should be of size $k$. If making $T_\ell$ to be of size $k$ makes it messy, you can initially state that you will consider submodular $k+1$ secretary problem.}


Now consider any algorithm for the submodular \nameSecSL~,and cardinality constraint $k+1$. We denote by $Alg$ the set of $\eta(k+1)$ items selected by the algorithm as part of the shortlist. % (all elements in the shortlist of size $\eta(k)$).
\scomment{We have  used $A$ to denote shortlist in the algorithm. May be you can use a different symbol instead of type $A$ and $B$. }
Let $\bar I$ denote an instance chosen uniformly at random from $I_\ell, \ell=1,\ldots, L$.  
%We choose one of $I_{\ell}$ randomly. \scomment{randomly or arbitrarily?} 
Let $\pi$ denote a random ordering of $n$ items in $\bar I$. 
%We give a random order of $I_{\ell}$, say $\pi$ to the algorithm as input,
%(note that in the secretary problem the elements of input can be selected adversarially but the order should be random).
We denote by random variable $(\bar{I},\pi)$ the randomly ordered input instance to the algorithm. Also we denote by $\bar{T}, \bar{B}$ and $\bar a$, the corresponding $T^{\ell}$, $B^{\ell}$ and $a_1^\ell$.

Now we claim 

%Note that algorithm is not aware of $\ell$.
%Consider an algorithm $Alg$.
%Suppose $a_1^{\ell}$ is the $t$-th elements in the input, and
%elements of input are ordered as $I=(I_1,\cdots, I_n)$.
%Suppose $Alg$ is the set of elements selected by an algorithm.
%Denote by $\bar{B}=\{b_1,\cdots, b_k\}$.

\begin{lemma}
$\mathbb{E}_{(\bar{I},\pi)}[|Alg\cap \bar{B}|] \le k/2+\eta(k+1)/L$.
\end{lemma}
\begin{proof}
Suppose $(e_1,\cdots, e_n)$ indicates the ordered input according to random ordering $\pi$ on $\bar{I}$. %for some $0<\ell<L$.
Now let $t$ be the random variable indicating the index of $a_1^{\ell}$ in $(e_1,\cdots, e_n)$, i.e., $e_t=a_1^{\ell}$. 
%Define $R:=\mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}|]$.
Then, due to random ordering, and random choice of $\bar I$ from $I_1, \ldots, I_\ell$, we have
$$\mathbb{E}_{(\bar I, \pi)}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap B^1|]= \cdots = \mathbb{E}[|Alg\cap\{e_1,\cdots, e_{t-1}\}\cap B^{L}|]\ .$$
Also, since $B^\ell, \ell=1,\ldots, L$ are disjoint,
$$\sum_{\ell=1}^L \mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap B^{\ell}|] \le \eta(k+1)\ .$$
Since $\bar B=B^\ell$ with probability $1/L$,  we have
$$H:=\mathbb{E}[|Alg\cap\{e_1,\cdots, e_{t-1}\}\cap \bar{B}|]=  \frac{1}{L} \sum_{\ell=1}^L \mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap B^{\ell}|] \le \frac{1}{L} \eta(k+1)\ . $$ 
%\rightarrow 0$ as $n/\eta(k) \rightarrow \infty$.
Now define
$G:=\mathbb{E}[|Alg\cap\{e_t,\cdots, e_{n}\}\cap \bar{B}|]$.
We have
$$G\le \mathbb{E} [|\bar{B}\cap\{e_t,\cdots, e_n\}|]  \le k/2\ .$$
%Also define $H:=\mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\cap \bar{B}\}|]$.
%Also, $H\le k-G$.
Thus $$\mathbb{E}[|Alg\cap \bar{B}|] \le G+H\le k/2+\eta(k+1)/L\ .$$
%\rightarrow G$$
%\le k/2$$
%G+(k-G)/2 \le k/2+G/2\le k/2+k/4=3/4k$$.
\end{proof}
Now on input $\bar{I}$, if the algorithm doesn't select $\bar a$, then $f(Alg)\le k+k/2$. Otherwise, if algorithm selects $\bar a$ then 
$$f(Alg)= k+ \frac{1}{2} g(k)+\frac{1}{2} |Alg\cap \bar{B}|$$ therefore $$\mathbb{E}[f(Alg)] \le k+\frac k 2+ \frac k 4+ \frac{\eta(k+1)}{2L} = \frac{7k}{4} + \frac{k\eta(k+1)}{n} \ .$$
%Hence $\mathbb{E}[f(Alg)]  \rightarrow k+k/2+k/4$ as $n\rightarrow \infty$, since $\eta(k)=o(n)$.
Since the optimal is at least $\Ex[f(\bar T)]=2k$, the competitive ratio is upper bounded by
$$ 
%\left(\frac{7k}{4} + \frac{k\eta(k)}{n}\right)\left/\right. 2k = 
\frac{7}{8} + \frac{\eta(k+1)}{2n} = \frac{7}{8} + o(1)\ ,$$
where we used $\eta(k+1)=o(n)$.
\scomment{I think we need to change the upper bound in theorem statement to $7/8 + o(1)$}
%Before arriving $a_1^{\ell}$ algorithm can not distinguish between elements of $B'=\{b_1^{\ell},\dots, b_k^{\ell}\}$
%and the rest of $B$ thus the expected number of elements in $B'$ selected by algorithm before observing $a_1$ goes to $0$ as $n/k\rightarrow \infty$.

%Therefore an online algorithm would select $k/2$ elements of set $B'$ in expectation and also it selects $a_1^{\ell}$ (and $k/2$ other elements from $B\setminus B'$).  Therefore, its $f$ value is $k+k/2+k/4$.
%Hence the competitive ratio is at most $7/8$.


==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/Impossiblesave.tex <==
%\section{Impossibility Result}

In this section we provide an upper bound showing the following:

\hardness*

%\begin{theorem}
%There is no algorithm achieving asymptotic competitive ratio $7/8+\epsilon$ for submodular secretary problem using $o(n)$ selections. 
%\end{theorem}

%\mcomment{In the following proof we will consider a submodular $k+1$-secretary} problem. 
In the following proof, for simplicity of notation, we prove the desired bound for submodular $k+1$-secretary problem. %Since $k+1=O(k)$, the upper bound derived will imply the stated bound for the  submodular $k$-secretary problem. 
First, we define a monotone submodular function $f$ as follows. 
For $n>0$, the ground set consists of two types of elements, $A$ and  $B$, such that
$f(a)=k$ for $a\in A$ and $f(b)=1$ for $b\in B$. %There are infinitely many elements of $A$ and $B$. 
\scomment{Don't you just need $L$ items of type $A$ and $n-1$ items of type $B$?}
There are $L:=n/2k$ items of type $A$ and
$n-1$ items of type $B$.
Also there is a collection of {\it disjoint} sets $T_{\ell}=\{a_1^{\ell}, b_1^{\ell},\cdots, b^{\ell}_{k}\}$, $\ell=1,2, \ldots L$, such that $a_1^{\ell}\in A$ and $b_j^{\ell}\in B$, and $f(T_{\ell})=2k$.
\scomment{infinite number of such sets? or will $L$ suffice?} 
\mcomment{in the definition of function it should be infinite but in the input we use $n/2k$ of them}
\scomment{After going through the proof, I don't see why you need infinite number, it seems just $L=n/2k$ will suffice. Where are you using that there are infinte number of $T^\ell$?}
\mcomment{
The reason is that you should give one functions $f$ that works for all $n$. Otherwise one may claim that for any given function $f$ there is large enough $N_f$ so that we can go beyond 7/8, for $n>N_f$. 
}

Now define 
$$g(t):=k+k/2+\cdots+ (t-ik)/2^i$$
where $i=\floor{t/k}$. It is easy to see that $g$ is a monotone submodular function.
Now define $f$ as follows:
\begin{itemize}
\item $|S\cap A| \ge 2 \implies f(S):=2k+1$
\item $|S\cap A|=0 \implies f(S):=1+g(|S|-1)$
\item $|S\cap A|=1 :$
\begin{itemize}
\item $S\cap A\notin\{a^{\ell}_1\}_{\ell>0} \implies f(S):=k+\frac{1}{2} g(|S|-1)$
\item $S\cap A= \{a_1^{\ell}\}$ for some $\ell$  $\implies f(S):=\min\{2k+1, k+\frac{1}{2} g(|S|-1)+k'/2^{i+1}\}$, where $k'=|S\cap\{b^{\ell}_1,\cdots, b_k^{\ell}\} |$.
\end{itemize}
\end{itemize}
Note that for any subset $S$, $f(S)\le 2k+1$.
\begin{lemma}
$f$ is a monotone submodular function.
\end{lemma}
\begin{proof}
We have to show that for elements $x$ and subsets $S\subseteq T$, $\Delta_f(x|S) \ge \Delta_f(x|T)$.
We consider the following cases:
\begin{itemize}
\item if $|T\cap A| \ge 2 \implies f_T(x)=0$, so it is trivial.
\item if $|T\cap A| =0 \implies |S\cap A|=0 \implies \Delta_f(x|S) \ge \Delta_f(x|T)$ because of submodularity of $g$.
\item if $|T\cap A|=1 \implies |S\cap A|\le 1$
\begin{itemize}
\item if $|S\cap A|=1 :$
\begin{itemize}
\item $S\cap A = T\cap A = \{a_1^{\ell}\}:$
\begin{itemize}
\item $x\in \{b_1^{\ell},\cdots, b_k^{\ell}\} \implies \Delta_f(x|S)=1/2^i+1/2^i$ and $\Delta_f(x|T)=1/2^j+1/2^j$ for $j\ge i$.
\item $x\notin \{b_1^{\ell},\cdots, b_k^{\ell}\} \implies \Delta_f(x|S)=1/2^i$ and $\Delta_f(x|T)=1/2^j$ for $j\ge i$.
\end{itemize}
\item $S\cap A = T\cap A \notin \{a_1^{\ell}\}_{\ell} \implies \Delta_f(x|S) \ge \Delta_f(x|T)$ because of submodularity of $g$.
\end{itemize}
\item if $|S\cap A|=0 \implies \Delta_f(x|T) \le 1/2^{i+1}+1/2^{i+1}$ and $\Delta_f(x|S)= 1/2^j$ for $j\le i$. Thus $\Delta_f(x|S) \ge \Delta_f(x|T)$.
\end{itemize}
\end{itemize} 
Monotonicity is trivial.
\end{proof}

\toRemove{
Also for any subset of $S$ with at least two elements of $A$, $f(S)=2k$. 
For subset $S$ with no element in $A$, if $i=\floor*{\frac{|S|}{k}}$, 
$f(S)$ is defined as 
\[
f(S)= k+k/2+ \dots +(|S|-ik)/2^{i}.
\]
For subset $S$ with exactly one element $a\in A$ such that $a\neq a_1$, if if $i=\floor*{\frac{|S|-1}{k}}$, 
$f(S)$ is defined as 
\[
f(S)= k+ k/2+ \dots +(|S|-1-ik)/2^{i+1}.
\]
Thus if $|S|=k+1$ and it contains exactly one element of $a\in A$ such that $a\neq a_1$ then $f(S)=k+k/2$.
Now suppose $S$  contains $a'$. 
For $S=T$, $f(S)=2k$.  Suppose $S$ contains $k'<k$ elements of $\{b_1, \dots, b_k\}$  and $\ell$ other elements of $B$. 
Let's $t=k'+\ell$, and $i=\floor*{\frac{t}{k}}$, then
\[
f(S)= \min\{2k, k'/2+(k+ k/2+ \dots +(t-ik)/2^{i+1})\}
\]
}
%\scomment{this proof is very vague, especially the claim any algorithm will select $k/2$ of $B$? Phrases like algorithm is not "aware" of something cannot be stated as a fact. You need to prove that the algorithm will not be able to distinguish between the two scenarios. We need to discuss.}



%Let $ {\cal T}^L$ be a collection of (any) $L=n/2k$ sets from $T^\ell, \ell=1,2, \ldots$. W.l.o.g., let's assume ${\cal T}^\ell = \{T_1, \ldots, T_L\}$.   

Denote $B^{\ell} := T^\ell \cap B = \{b_1^{\ell},\cdots, b_k^{\ell}\}$ for $\ell=1,2, \ldots,$. Also, let 
$B'=B\setminus (\bigcup_{\ell=1}^L B^{\ell})$. % where $L:=n/2k$. 
%\scomment{Do you need $T^\ell, \ell =1,\ldots, L$ to be disjoint?} \mcomment{yes}
% $B'=B\setminus (\bigcup_{\ell }^{L} B^{\ell})$ for $L:=n/2k$.
Now define $L$ input instances $\{I_{\ell}\}_{\ell =1,\ldots, L}$, each of size $n$, as follows. For
any arbitrary subset $\tilde{B}\subseteq B'$ of size $n-Lk-1$, 
%\scomment{Which subset $\tilde{B}$? any arbitrary subset?} \mcomment{arbitrary}
define $I_{i}=\bigcup_{\ell=1,\ldots, L}  B^{\ell} \cup \tilde{B} \cup \{a_1^{i}\}$, for  $i=1,\ldots, L$.
%and $I_2=B^1 \cup B^2 \cup \tilde{B} \cup \{a_1^2\}$ (the difference is $a_1^1$ and $a_1^2$).
%Now suppose the input consists of the following:  $T^{\ell}=\{a_1^{\ell}, b_1^{\ell}, \cdots b_k^{\ell} \}$, no other element of $A$ and the remaining elements are from $B':=B\setminus \{b_1^{\ell}, \cdots, b_k^{\ell}\}$. 
Thus the optimal is $T^{\ell}$ for instance $I_{\ell}$, with $f(T^{\ell})=2k$. 
\scomment{$T^\ell$ is of size $k+1$, optimal should be of size $k$. If making $T_\ell$ to be of size $k$ makes it messy, you can initially state that you will consider submodular $k+1$ secretary problem.}


Now consider any algorithm for the submodular \nameSecSL~,and cardinality constraint $k+1$. We denote by $Alg$ the set of $\eta(k+1)$ items selected by the algorithm as part of the shortlist. % (all elements in the shortlist of size $\eta(k)$).
\scomment{We have  used $A$ to denote shortlist in the algorithm. May be you can use a different symbol instead of type $A$ and $B$. }
Let $\bar I$ denote an instance chosen uniformly at random from $I_\ell, \ell=1,\ldots, L$.  
%We choose one of $I_{\ell}$ randomly. \scomment{randomly or arbitrarily?} 
Let $\pi$ denote a random ordering of $n$ items in $\bar I$. 
%We give a random order of $I_{\ell}$, say $\pi$ to the algorithm as input,
%(note that in the secretary problem the elements of input can be selected adversarially but the order should be random).
We denote by random variable $(\bar{I},\pi)$ the randomly ordered input instance to the algorithm. Also we denote by $\bar{T}, \bar{B}$ and $\bar a$, the corresponding $T^{\ell}$, $B^{\ell}$ and $a_1^\ell$.

Now we claim 

%Note that algorithm is not aware of $\ell$.
%Consider an algorithm $Alg$.
%Suppose $a_1^{\ell}$ is the $t$-th elements in the input, and
%elements of input are ordered as $I=(I_1,\cdots, I_n)$.
%Suppose $Alg$ is the set of elements selected by an algorithm.
%Denote by $\bar{B}=\{b_1,\cdots, b_k\}$.

\begin{lemma}
$\mathbb{E}_{(\bar{I},\pi)}[|Alg\cap \bar{B}|] \le k/2+\eta(k+1)/L$.
\end{lemma}
\begin{proof}
Suppose $(e_1,\cdots, e_n)$ indicates the ordered input according to random ordering $\pi$ on $\bar{I}$. %for some $0<\ell<L$.
Now let $t$ be the random variable indicating the index of $a_1^{\ell}$ in $(e_1,\cdots, e_n)$, i.e., $e_t=a_1^{\ell}$. 
%Define $R:=\mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}|]$.
Then, due to random ordering, and random choice of $\bar I$ from $I_1, \ldots, I_\ell$, we have
$$\mathbb{E}_{(\bar I, \pi)}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap B^1|]= \cdots = \mathbb{E}[|Alg\cap\{e_1,\cdots, e_{t-1}\}\cap B^{L}|]\ .$$
Also, since $B^\ell, \ell=1,\ldots, L$ are disjoint,
$$\sum_{\ell=1}^L \mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap B^{\ell}|] \le \eta(k+1)\ .$$
Since $\bar B=B^\ell$ with probability $1/L$,  we have
$$H:=\mathbb{E}[|Alg\cap\{e_1,\cdots, e_{t-1}\}\cap \bar{B}|]=  \frac{1}{L} \sum_{\ell=1}^L \mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap B^{\ell}|] \le \frac{1}{L} \eta(k+1)\ . $$ 
%\rightarrow 0$ as $n/\eta(k) \rightarrow \infty$.
Now define
$G:=\mathbb{E}[|Alg\cap\{e_t,\cdots, e_{n}\}\cap \bar{B}|]$.
We have
$$G\le \mathbb{E} [|\bar{B}\cap\{e_t,\cdots, e_n\}|]  \le k/2\ .$$
%Also define $H:=\mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\cap \bar{B}\}|]$.
%Also, $H\le k-G$.
Thus $$\mathbb{E}[|Alg\cap \bar{B}|] \le G+H\le k/2+\eta(k+1)/L\ .$$
%\rightarrow G$$
%\le k/2$$
%G+(k-G)/2 \le k/2+G/2\le k/2+k/4=3/4k$$.
\end{proof}
Now on input $\bar{I}$, if the algorithm doesn't select $\bar a$, then $f(Alg)\le k+k/2$. Otherwise, if algorithm selects $\bar a$ then 
$$f(Alg)= k+ \frac{1}{2} g(k)+\frac{1}{2} |Alg\cap \bar{B}|$$ therefore $$\mathbb{E}[f(Alg)] \le k+\frac k 2+ \frac k 4+ \frac{\eta(k+1)}{2L} = \frac{7k}{4} + \frac{k\eta(k+1)}{n} \ .$$
%Hence $\mathbb{E}[f(Alg)]  \rightarrow k+k/2+k/4$ as $n\rightarrow \infty$, since $\eta(k)=o(n)$.
Since the optimal is at least $\Ex[f(\bar T)]=2k$, the competitive ratio is upper bounded by
$$ 
%\left(\frac{7k}{4} + \frac{k\eta(k)}{n}\right)\left/\right. 2k = 
\frac{7}{8} + \frac{\eta(k+1)}{2n} = \frac{7}{8} + o(1)\ ,$$
where we used $\eta(k+1)=o(n)$.
\scomment{I think we need to change the upper bound in theorem statement to $7/8 + o(1)$}
%Before arriving $a_1^{\ell}$ algorithm can not distinguish between elements of $B'=\{b_1^{\ell},\dots, b_k^{\ell}\}$
%and the rest of $B$ thus the expected number of elements in $B'$ selected by algorithm before observing $a_1$ goes to $0$ as $n/k\rightarrow \infty$.

%Therefore an online algorithm would select $k/2$ elements of set $B'$ in expectation and also it selects $a_1^{\ell}$ (and $k/2$ other elements from $B\setminus B'$).  Therefore, its $f$ value is $k+k/2+k/4$.
%Hence the competitive ratio is at most $7/8$.


==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/abstract.tex <==
In the \textit{matroid secretary problem}, which is a generalization of the classic secretary problem,
the elements of a matroid $\mathcal{M}$ arrive in random order. Once we observe an item we need to irrevocably decide 
whether or not to accept it. The set of selected elements should form an independent set of the matroid.
The goal is to maximize the total sum of the values assigned to these elements. The existence of a constant competitive algorithm
is a long standing open problem.

In this paper, we introduce a version of this problem, which we refer to as submodular matroid secretary problem with shortlists (motivated by the \textit{shortlist} model in~\cite{us}). 
In this setting, the algorithm is allowed to choose a subset of items as part of a shortlist, possibly more than $k=rk(\mathcal{M})$ items. Then, after seeing the entire input, the algorithm can choose an independent subset from the shortlist. Furthermore we generalize the objective function to any monotone submodular function.
The main question is that can an online algorithm achieve a constant competitive ratio using a shortlist of size $O(k)$?

We design an algorithm that achieves a $\frac{1}{2}(1-1/e^2-\epsilon-O(1/k))$ competitive ratio for any constant $\epsilon>0$, using a shortlist of size $O(k)$. This is especially surprising considering that the best known competitive ratio for the matroid secretary problem is $O(\log \log k)$. We are also able to get a constant competitive algorithm using shortlist of size  at most $k$ and also a constant competitive algorithm in the preemption model.

 %An important application of our algorithm is for the submodular function maximization in the random order streaming model.
An important application of our algorithm is for the random order streaming of submodular functions.
We show that our algorithm can be implemented in the streaming setting using $O(k)$ memory. It achieves a $\frac{1}{2}(1-1/e^2-\epsilon-O(1/k))$ approximation. 
The previously best known approximation ratio for streaming submodular maximization under matroid constraint  is 0.25 (adversarial order) due to ~\citet{feldman2018streaming},~\citet{Chekuri} and ~\citet{Chakrabarti2015}.
%using $O(k\log k)$ memory.
%Recently, Feldman et al give an algorithm with the same approximation but with improved memory $O(k)$.
Moreover, we generalize our results to the case of $p$-matchoid constraints and give a $\frac{1}{p+1}(1-1/e^{p+1}-\epsilon-O(1/k))$ approximation using $O(k)$ memory,
which asymptotically (as $p$ and $k$ increase) approaches the best known offline guarantee $\frac{1}{p+1}$~\cite{nemhauser1978analysis}. 

%($m$ is a the number of matroids used to define the $p$-matchoid constraint)
%We also empirically evaluate the performance of our algorithm on data summarization tasks and observe that it outperforms the state-of-the-art algorithms.
%\newpage


\toRemove{
In \nameOfProblem, 
the goal is to select $k$ items in a randomly ordered input so as to maximize 
the expected value of a given monotone submodular function on the set of selected items. 
In this paper, we introduce a relaxation of this problem, which we refer to as \nameOfProblemSL.
In the proposed problem setting, the algorithm is allowed to choose more than $k$ items as part of a shortlist. Then, after seeing the entire input, the algorithm can choose a subset of size $k$ from the bigger set of items in the shortlist. We are interested in understanding to what extent this relaxation can improve the achievable competitive ratio for the \nameOfProblem. In particular, using an $O(k)$ shortlist, can an online algorithm achieve a competitive ratio close to the best achievable offline approximation factor for this problem? 

We answer this question affirmatively by giving a polynomial time algorithm that achieves a $1-1/e-\epsilon-O(k^{-1})$ competitive ratio for any constant $\epsilon>0$, using a shortlist of size $\eta_\epsilon(k)=O(k)$. This is especially surprising considering that the best known competitive ratio (in polynomial time) for the \nameOfProblem~is $(1/e-O(k^{-1/2}))(1-1/e)$ \cite{kesselheim}. Further, for the special case of $m$-submodular functions, we demonstrate an algorithm that achieves $1-\epsilon$ competitive ratio for any constant $\epsilon>0$, using an $O(1)$ shortlist.

The proposed algorithm also has significant implications for another important problem of submodular function maximization under random order streaming model and $k$-cardinality constraint. We show that our algorithm can be implemented in the streaming setting using a memory buffer of size $\eta_\epsilon(k)=O(k)$ to achieve a $1-1/e-\epsilon-O(k^{-1})$ approximation. 
%This substantially improves upon the previous work, where the  best known approximation factor was $1/2 + 8\times 10^{-14}$ using $O(k\log k)$ memory\cite{norouzi}.
This substantially improves upon \cite{norouzi}, which achieved the previously best known approximation factor of $1/2 + 8\times 10^{-14}$ using $O(k\log k)$  memory.
Furthermore in the random order streaming setting our algorithm is asymptotically tight due to $1-1/e$ upper bound in~\cite{mcgregor2017better} 

\toRemove{
In \nameOfProblem, 
the goal is to select $k$ items in a randomly ordered input so as to maximize 
the expected value of a given monotone submodular function on the set of selected items. 
%In this paper we only consider monotone submodular functions.
For each element that arrives we have to irrevocably decide whether or not to select it.
The best known result (in polynomial time) is an algorithm with $(1/e-O(k^{-1/2}))(1-1/e)$ asymptotic competitive ratio~\cite{kesselheim}.\newline
%, and $1/e-O(k^{-1/2})$ asymptotic competitive ratio
%by having access to an oracle that optimally solves offline submodular function maximization with cardinality constraint~\cite{kleh}.
In this paper, we introduce a relaxation of We relax the problem by allowing the algorithm to select more than $k$ elements, and return a subset of size $k$
out of selected elements at the end of algorithm. Our main result is that for any $R<1-1/e$ there is an algorithm with asymptotic competitive ratio
$R-O(k^{-1})$ that only selects $O(k)$  elements. The running time is linear in  $n$ the size of input.
\newline
%We relax the problem by allowing the algorithm to select more than $k$ elements, and return a subset of size $k$
%out of selected elements at the end of algorithm. Our main result is that for any $1-1/e-\epsilon$ there is an algorithm with asymptotic competitive ratio
%$R-\epsilon-O(k^{-1})$ that selects $k\log(1/\epsilon) {\frac{1}{\epsilon^3} \log(1/\epsilon)  \choose {\epsilon^2} \log(1/\epsilon)}}$ elements. The running time is linear in  $n$ the size of input.
Our algorithm can also be considered a single pass streaming algorithm on random order inputs. 
%A $0.193$-competitive algorithm is proposed in a recent paper~\cite{recent}, which uses $n$ function evaluations and $O(k)$ memory.
The best known streaming algorithm for adversarial order input is $1/2-\epsilon$ approximation using memory of size $O(\frac{1}{\epsilon}k\log k)$~\cite{Badanidiyuru2014StreamingFly}. No algorithm can achieve better than $1/2+o(1)$ in the adversarial model using $o(n)$ memory~\cite{norouzi}. 
Our algorithm substantially improves~\cite{norouzi}, which uses $O(k\log k)$ memory to get $1/2+8\times 10^{-14}$ approximation in the random order model. % Also it improves~\cite{mirzasoleiman}  on random order inputs. 
We use only $O(k)$  memory to get asymptotic $R$-approximation for any $R<1-1/e$.
Also our algorithm is highly parallel.
%, i.e. the  operations required to make a decision for each item can be divided between available processors. (the running time will be divided by $\min(c,p)$ where $c$ is the hidden constant in $O(k)$ and $p$ the number of processors )

%%Distributed submodular maximization:
%%Faster algorithm for large streams:
%Although the update time in our algorithm is $O(1)$, the constant can be very large. Consequently it may not be desirable for large streams. 
%We take two approaches to deal with it. The first approach is parallel algorithms. The interesting fact about our algorithm is that it is highly parallel, i.e. the  operations required to make a decision for one item can be divided between available processors. 
%%The running time will be divided by the number of processors. 
%In the other approach, %when $n>>k$, 
%we design a simple thresholding algorithm that requires only one function evaluation per element. %time is only one operation.
%It achieves competitive ratio $(1/2-O(k^{-1/2}))(1-1/e)$ by selecting $k\log^2k$ elements.
%% Its guarantee is still better than~\cite{kleh}, and is much faster ( they need $O(n^2)$ update time).
%%It  needs to solve an offline submodular maximization problem on a subset of size $k\log k$ at the end of input.
%%%It needs an extra processing at the end of algorithm which is $O(2^k)$ (It is only reasonable when $n>2^k$).
\newline
We also provide an upper bound showing that it is not possible to achieve any competitive ratio better than $7/8$ by selecting $o(n)$ elements even with unlimited computational power.
%%$O(g(k))$ elements, where $g$ is an arbitrary function, even if we have free computation.
Furthermore, we provide two families of monotone submodular functions that we can asymptotically approach the optimal solution.
}
}

==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/algorithms.tex <==
Before describing our main algorithm we design a subroutine for 
a problem that we call it \textit{secretary problem with replacement}:
we are given a matroid $\mathcal{M}=(\mathcal{E},\mathcal{I})$ and an independent set $S\in \mathcal{I}$.
A pool of items
$I=(a_1,\cdots, a_N)$ arriving sequentially in a uniformly random order,
find an element $e$ from $I$ that can be added to $S$ after removing 
possibly one element $e'$ from $S$ such that the set remains independent, i.e., $S+e-e' \in \mathcal{I}$.
The goal is to choose element $e$ and $e'$ in an online manner with maximum marginal increment $g(e,S)=f(S+e-e')-f(S)$.
%which contains an item with expected value close to the maximum
%marginal increment. 
More precisely define function $g$ as:
\begin{equation}
\label{eq:g}
g(e,S):= f(S+e-\theta(e,S)) - f(S),
\end{equation}
%Now define function 
where $\theta$ is defined as: 
$$ \theta(e,S) := \arg\max_{e'\in S} \{ f(S+e-e')| S+e-e' \in \mathcal{I} \} $$
%Also define $g$ as 
%% $$g(e):=\max_{e': S+e-e' \in \mathcal{I}} F(S+e-e') - F(S)$$
% $$g(e,S):= f(S+e-\theta(e,S)) - f(S)$$
We will consider the variant in which we are allowed to have a shortlist, where the  algorithm can add items to 
a shortlist and choose one item from the shortlist at the end.

For the \textit{secretary problem with replacement}, we give Algorithm~\ref{alg:matroidmax} which is a simple modification of the \textit{online max algorithm} in~\cite{us}.

\begin{lemma}
Algorithm~\ref{alg:matroidmax}, returns  element  $e$ with maximum  $g(e,S)$ with probability $1-\delta$, thus it achieves a  $1-\delta$ competitive ratio for the \textit{secretary problem with replacement}. %with shortlists of size logarithmic in $1/\delta$.
The size of the shortlist that it uses is logarithmic in $1/\delta$.
\end{lemma}

%In the main algorithm, we  remove $g(S_W)$ from $S_{1, \cdots, w-1}$ at the end of window $w$. Note that $T$ and $R$ will remain as before.


%\begin{theorem}
%Algorithm~\ref{alg:replacment} achieves a $1-\delta$ competitive ratio
%for shortlists of size logarithmic in $1/\delta$.
%\end{theorem}








%\section{Algorithms}
%\subsection{Simpler but unimplementable, offline version}
%\subsection{Algorithm description}

%Before giving our algorithm for \nameOfProblemSL, we describe a simple technique for \nameSecSL~
%that achieves a  $1-\delta$ competitive ratio for  with shortlists of size logarithmic in $1/\delta$.
%Recall that in the \nameSec, the aim is to select an item with expected value close to the maximum among a pool of items $I=(a_1, \ldots, a_N)$ arriving sequentially in a uniformly random order. 
%We will consider the variant with shortlists, where we now want to pick a shortlist which contains an item with expected value close to the maximum.
%%\ccomment{why are we using $\epsilon$ in the text and $\delta$ in the Algorithm below}\scomment{fixed}

%We propose the following simple algorithm. 
%Which is a simple modification of the algorithm proposed in~\cite{us}.
%%For the first $n\delta/2$ rounds, don't add any items to the shortlist, but just keep track of the element $e$ with maximum $g(e,S)$ value seen so far.
%%For all subsequent rounds, 
%%for any arriving item $i$ that has a value $g(a_i,S)$ greater than or equal to the maximum $g(.,S)$ value seen so far, add it to the shortlist if the size of shortlist is less than or equal to $L=4\ln(2/\delta)$. This algorithm is summarized as Algorithm \ref{alg:matroidmax}. 
%Clearly, 
%For constant $\delta$, this algorithm uses a shortlist of size $L=O(1)$. Further, under a uniform random ordering of input, we can show that the item with maximum $g$ value  will be part of the shortlist with probability $1-\delta$. (See Proposition \ref{maxanalysis} in Section \ref{sec:analysis}.)
%that the expected number of items in the shortlist $A$ is at most $\log(1/\epsilon)$, i.e., $O(1)$, and the maximum value item will be part of the shortlist with probability $1-\epsilon$. %analysis is presented in Section \ref{sec:max}. 
%--------------------------------------
\begin{algorithm*}[ht]
  %\caption{~\bf{Select-If-it-Improves}($I , u$)}
  \caption{~\bf{Secretary Problem with Replacement}}%Algorithm for finding max matroid replacement   }}
  \label{alg:matroidmax} 
\begin{algorithmic}[1]
\State Inputs: number of items $N$, an independent set $S$, items in $I=\{a_1, \ldots, a_N\}$ arriving sequentially, $\delta \in (0,1]$. 
\State Initialize: $A\leftarrow \emptyset$,  $u=n\delta/2$, $M = -\infty$ %$M\leftarrow \max\{a_1, \cdots, a_{u-1}\}$
\State $L \leftarrow 4\ln(2/\delta)$

\For {$i= 1$ to $N$}
%\If {$F(S\cup \{a_i\}) > F(S) $}
\If {$ g(a_i,S) > M$}
\State $M \leftarrow  g(a_i,S)$
\If {$i \geq u$ and $|A|<L$}
\State $A\leftarrow A\cup \{a_i\}$
\EndIf
\EndIf
\EndFor
%\State return $S\setminus \{a_1,\cdots, a_u\}$
\State return $A$, and $A^*:= \max_{i\in A} g(a_i,S)$
\end{algorithmic}
\end{algorithm*}


\begin{algorithm*}[h!]
  %\caption{~\bf{Select-If-it-Improves}($I , u$)}
  \caption{~\bf{Algorithm for {\bf submodular} matroid secretary with shortlist}}
  \label{alg:main} 
  \label{alg:tmp} 
\begin{algorithmic}[1]
\State Inputs: number of items $n$, submodular function $f$, parameter $\epsilon \in (0,1]$. 
\State Initialize: $S_0 \leftarrow \emptyset, R_0 \leftarrow \emptyset, A \leftarrow \emptyset, A^* \leftarrow \emptyset$, constants $\alpha \ge 1, \beta \ge 1$ which depend on the constant $\epsilon$.
\State Divide indices $\{1,\ldots, n\}$ into $(\alpha, \beta)$ windows. %as prescribed by Definition \ref{def:windows}.
%Divide the sequence of candidates into consecutive groups of $\frac{n}{\beta k}$ candidates, referred to as slots (or buckets). And, divide the sequence of slots into consecutive groups of $\alpha \beta$ slots, referred to as {\it windows}.
%===========================
\For {window $w= 1, \ldots, k/\alpha$} 
%\State For every $\alpha$-length subsequence $\tau=(s_1,\ldots, s_\alpha) \subseteq [\alpha\beta]$ of slots in window $w$, define 
%$$\gamma(\tau):=\{i_1, \ldots, i_\alpha\}$$
%where 
%$$i_j := \arg \max_{i\in V_{s_j,w} \cup R_{1,\ldots, w-1}} f(S_{1,\ldots,w-1} \cup \{i_1\ldots, i_{j-1}\} \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \{i_1\ldots, i_{j-1}\})$$
%\State Define $R_w:=\{\cup_{\tau} \gamma(\tau)\}.$ 
 

%\State Process the online inputs in window $w$ using the subroutine in Algorithm \ref{alg:tmpWindow} to select a subset $H_w$ of items. 
 \For {every slot $s_j$ in window $w$, $j=1,\ldots, \alpha\beta$}
  \State Concurrently for all subsequences of previous slots $\tau\subseteq \{s_1, \ldots, s_{j-1}\}$ of length $|\tau|<\alpha$ \label{li:subb}\\
  \hspace{0.44in} in window $w$, call the online algorithm in Algorithm \ref{alg:matroidmax} with the following inputs: 
  %\begin{center}
  \begin{itemize}%[leftmargin=0.7in]
  \item   number of items $N=|s_j|+1$, $\delta=\frac{\epsilon}{2}$, and
%  \scomment{You have to use $\delta$ smaller than $\epsilon$ to get $1-\frac{1}{e}-\epsilon$ in the final result.}
  \item item values $I=(a_0, a_1, \ldots, a_{N-1})$, with 
   
     \begin{eqnarray*} 
  a_0 & := & \max_{x\in R_{1,\ldots, w-1}} \Delta(x|S_{1,\ldots,w-1} \cup \gamma(\tau)\setminus \zeta(\tau)) \\
  %\max_{x\in R_{1,\ldots, w-1}} f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{x\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\}$
     a_\ell & := & \Delta(s_j(\ell)| S_{1,\ldots,w-1} \cup \gamma(\tau)\setminus \zeta(\tau) ),  \forall 0<\ell\le N-1
     \end{eqnarray*}
    %f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\})$
 where $s_j(\ell)$ denotes the $\ell^{th}$ item in the slot $s_j$. 
% \item $\delta = \frac{\epsilon}{{\alpha \beta \choose \alpha}}$.
  \end{itemize}
   %\end{center}
   %\mcomment{why do you divide by... the erros do not add up}  \scomment{Please add the required theorem showing this}  \mcomment{added lemma~\ref{online}}
\State Let $A_{j}(\tau)$ be the shortlist returned by  Algorithm \ref{alg:matroidmax} for slot $j$ and subsequence $\tau$. Add \\
\hspace{0.44in} all items except the dummy item $0$ to the shortlist $A$. %$H_w$, i.e, for all $\tau$,
 % $$H_w \leftarrow H_w\cup (A_{j}(\tau) \cap s_j)$$
 That is, \label{li:sube}
 $$A\leftarrow A\cup  (A(j)\cap s_j)$$
 \EndFor
%\State return $H_w$
% \State $A\leftarrow A\cup H_w$
 \State After seeing all items in window $w$, compute $R_w, S_w$ and $\bar{S}_w$ as before %defined in \eqref{eq:Rw} and \eqref{eq:Sw} respectively.
 \State $S_{1,\cdots, w} \leftarrow S_{1,\cdots, w-1}\cup S_w \setminus \bar{S}_w$
 \State $A^* \leftarrow A^*\cup (S_w \cap A)\setminus \hat{S}_w$
\EndFor
\State return $A$, $A^*$. %$A=T_1 \cup \cdots  \cup T_{W}$
\end{algorithmic}
\end{algorithm*}

%==========================


%\begin{algorithm*}[ht]
  %\caption{~\bf{Subroutine of Algorithm \ref{alg:tmp} for window $w$}}
  %\label{alg:tmpWindow} 
  \toRemove{
  \begin{algorithmic}[1]
  \For {every slot $s_j$ in window $w$, $j=1,\ldots, \alpha\beta$}
  \State Concurrently for all subsequences of previous slots $\tau\subseteq \{s_1, \ldots, s_{j-1}\}$ in window $w$, of length $|\tau|<\alpha$, call the online algorithm in Algorithm \ref{alg:SIIImax} with the following inputs: number of items $N=|s_j|+1$, $\delta = \frac{\epsilon}{{\alpha \beta \choose \alpha}}$, \mcomment{why do you divide by... the errors do not add up} and values of arriving items $(a_0, a_1, \ldots, a_{N-1})$ defined as 
  $$a_0:=\max_{x\in R_{1,\ldots, w-1}} f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{x\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\}$$
    $$a_i :=f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\})$$
 where $i$ denotes the $i^{th}$ item in slot $s_j$.
  \State Let $A_{j}(\tau)$ be the shortlist returned by  Algorithm \ref{alg:SIIImax} for slot $j$ and subsequence $\tau$. Add all items except the dummy item $0$ to $H_w$, i.e, for all $\tau$,
  $$H_w \leftarrow H_w\cup (A_{j}(\tau) \cap s_j)$$
 \EndFor
\State return $H_w$
\end{algorithmic}
}
%\end{algorithm*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%There are two main difficulties in extending this idea to the \nameOfProblemSL. First, instead of one item, here we aim to select a set $S$ of $k$ items using an $O(k)$ length shortlist. Second, the contribution of each new item $i$ to the objective value, as given by the submodular function $f$, depends on the set of items selected so far. 

%The first main concept we introduce to handle these difficulties  is
%Similar to~\cite{us},
%we divide the input into sequential blocks that we refer to as $(\alpha, \beta)$ windows. 
%You can find the precise definition of $(\alpha, \beta)$ windows in~\cite{us}.
%Below is the precise construction of $(\alpha, \beta)$ windows, for any postivie integers $\alpha$ and $\beta$, such that $k/\alpha$ is an integer.
%\ccomment{This definition is imprecise.  Needs to be made technically crisp.}
%\ccomment{What exactly is this distribution?  Are we drawing with replacement or without and do the $X_i$ sum to $n$?}
%We use a set of random variables $X_1,\ldots,X_m$ defined in the following way.  Throw $n$ balls into $m$ bins uniformly at random.  Then set $X_j$ to be the number of balls in the $j$th bin.  We call the resulting $X_j$'s a {\em $(n,m)$-ball-bin random set}.


Similar to~\cite{us}, we divide the input into sequential blocks that we refer to as $(\alpha, \beta)$ windows.
Here $k=rk(\mathcal{M})$.
\begin{definition}[$(\alpha,\beta)$ windows] \label{def:windows}
Let $X_1,\ldots,X_{k\beta}$ be a $(n,k\beta)$-ball-bin random set.
Divide the indices $\{1,\ldots, n\}$ into $k\beta$ slots, where the $j$-th slot, $s_j$, consists of $X_j$ consecutive indices in the natural way, that is, slot $1$ contains the first $X_1$ indices, slot $2$ contains the next $X_2$, etc.
 %, $X_i$ would be the number of balls in the $i$-th bin.
 Next, we define $k/\alpha$ windows, where window $i$ consists of $\alpha \beta$ consecutive slots, in the same manner as we assigned slots.
\end{definition}
%\ccomment{Would an example or a figure help here to define slots and windows?}

%Thus, $q^{th}$ slot is composed of indices $\{\ell, \ldots, r\}$, where $\ell=X_1+...+X_{q-1}+1$ and  $r=X_1+...+X_q$. 
%Further, if the ordered the input is $\bar a_1, \dots, \bar a_n$ then we say that the items inside the slot $s_q$ are $\bar a_{\ell}, \bar a_{\ell+1}, \dots, \bar a_{r}$ 
%To reduce notation, when clear from context, we will use $s_q$ and $w$ to also indicate the {\it set of items} in the slot $s_q$ and window $w$ respectively.

%The idea is to divide the inputs into $k/\alpha$ blocks (i.e., windows) for a constant $\alpha\ge 1$ such that 
%\ccomment{Shouldn't we say what alpha is because the intuition depends on it}

Intuitively, for large enough $\alpha$ and $\beta$,
roughly $\alpha$ items from the optimal set $S^*$ are likely to lie in each of these windows, and further, it is unlikely that two items from $S^*$ will appear in the same slot. 

The algorithm can focus on identifying a constant number (roughly $\alpha$) of optimal items from each of these windows, with at most one item coming from each of the $\alpha \beta$ slots in a window. 
Similar to~\cite{us}, the core of our algorithm is a subroutine that accomplishes this task in an online manner using a shortlist of constant size in each window. But the difference is that adding items from a new window to the current solution $S$ could make it a non-independent set of $\mathcal{M}$. In order to make the new set independent we have to remove some items from $S$. The removed item corresponding to $e$ will be $\theta(e,S)$. We need to take care of all the removals for newly selected items in a window. Therefore we have to slightly change the definitions in~\cite{us}. We introduce $\zeta(\tau)$ which is counterpart of $\gamma(\tau)$ for the removed elements. 
%To implement this idea, we use a greedy selection method that considers all possible $\alpha$ sized subsequences of the $\alpha\beta$ slots in a window, and aims to identify the subsequence that maximizes the increment over the best items identified so far. Because of the removal of elements in the definition of $g$, we slightly modify the definition of function $\gamma$ compared to its definition in~\cite{us}.
More precisely, for any subsequence $\tau=(s_1,\ldots, s_\ell)$ of the $\alpha\beta$ slots in window $w$, recall the greedy subsequence $\gamma(\tau)$ of items as:
\begin{equation}
\label{eq:gamma}
\gamma(\tau):=\{i_1, \ldots, i_\ell\}
\end{equation}
where
\begin{equation}
\label{eq:ij}
i_j := \arg \max_{i\in s_j \cup R_{1, \ldots, w-1}} g(i, S_{1, \ldots,w-1} \cup \{i_1,\ldots, i_{j-1}\})
%f(S_{1, \ldots,w-1} \cup \{i_1,\ldots, i_{j-1}\} \cup \{i\}) - f(S_{1, \ldots, w-1} \cup \{i_1\ldots, i_{j-1}\}).
\end{equation}
%Also suppose $\theta(E,S):= \cup_{e\in E} \theta(e,s)$. 
now define $\zeta(\tau):=\{c_1, \ldots, c_\ell\}$
where
\begin{equation}
\label{eq:cij}
c_j :=  \theta(i_j, S_{1, \ldots,w-1} \cup \{i_1,\ldots, i_{j-1}\})
%f(S_{1, \ldots,w-1} \cup \{i_1,\ldots, i_{j-1}\} \cup \{i\}) - f(S_{1, \ldots, w-1} \cup \{i_1\ldots, i_{j-1}\}).
\end{equation}
%Note that $T$ and $R$ will remain as before and $S_w=\gamma(\tau^*)$. Define $\bar{S}_w:=\zeta(\tau^*)$.
%\begin{equation}
%\label{eq:Rw}
%R_w = \cup_{\tau: |\tau|=\alpha} \gamma(\tau)
%\end{equation}
%and 
%\begin{equation}
%\label{eq:Sw}
%S_w=\gamma(\tau^*),
%\end{equation} where
%\begin{equation}
%\label{eq:taustar}
%\tau^*:=\arg \max_{\tau: |\tau|=\alpha} f(S_{1,\ldots,w-1} \cup \gamma(\tau)) - f(S_{1,\ldots,w-1}).
%\end{equation}






%More precisely, for any subsequence $\tau=(s_1,\ldots, s_\ell)$ of the $\alpha\beta$ slots in window $w$, we define a `greedy' subsequence $\gamma(\tau)$ of items as:
%\begin{equation}
%\label{eq:gamma}
%\gamma(\tau):=\{i_1, \ldots, i_\ell\}
%\end{equation}
%where
%\begin{equation}
%\label{eq:ij}
%i_j := \arg \max_{i\in s_j \cup R_{1, \ldots, w-1}} f(S_{1, \ldots,w-1} \cup \{i_1,\ldots, i_{j-1}\} \cup \{i\}) - f(S_{1, \ldots, w-1} \cup \{i_1\ldots, i_{j-1}\}).
%\end{equation}
%In ({\ref{eq:ij}) and in the rest of the paper, we use shorthand $S_{1,\ldots, w}$ to denote $S_1\cup \cdots \cup S_{w}$, and $R_{1,\ldots, w}$ to denote $R_1\cup \cdots \cup R_{w}$, etc.  We also will take unions of subsequences, which we interpret as the union of the elements in the subsequences.

%\ccomment{Are we bothered by taking the union of a sequence rather than a set?}
Recall the definition of $R_w$ in~\cite{us}, which is  the union of all greedy subsequences of length $\alpha$, and $S_w$ to be  the best subsequence among those. That is,
\begin{equation}
\label{eq:Rw}
R_w = \cup_{\tau: |\tau|=\alpha} \gamma(\tau)
\end{equation}
and 
\begin{equation}
\label{eq:Sw}
S_w=\gamma(\tau^*),
\end{equation} now define 
\begin{equation}
\label{eq:Swbar}
\bar{S}_w=\zeta(\tau^*),
\end{equation}
where
\begin{equation}
\label{eq:taustar}
\tau^*:=\arg \max_{\tau: |\tau|=\alpha} f((S_{1,\ldots,w-1} \cup \gamma(\tau))\setminus \zeta(\tau)) - f(S_{1,\ldots,w-1}).
\end{equation}
also define
\begin{equation}
\label{eq:Swhat}
\hat{S}_w=\{c_{j_1},\cdots, c_{j_t}\}, \text{where } (S_w\cap A)=  \{i_{j_1},\cdots, i_{j_t}\}
\end{equation}

%Note that $i_j$ (refer to \eqref{eq:ij}) can be set as  either an item in slot $s_j$ or an item {\it from a previous greedy subsequence} in $R_1\cup \cdots \cup R_{w-1}$. The significance of the latter relaxation will become clear in the analysis.
%Here, $s_j \cup R_1 \cup \cdots \cup R_{w-1}$ denotes the union of items in slot $s_j$ and 
In other words, $\hat{S}_w$ is counterpart of elements of $S_w\cap A$ that are removed by $g$. 
Also note that in the main Algorithm~\ref{alg:main}, we  remove $\zeta(\tau^*)$ from $S_{1, \cdots, w-1}\cup S_w$ at the end of window $w$ and make $S_{1,\cdots, w}$ an independent set of $\mathcal{M}$.

%$S_w$ represents the best subsequence among all the subsequences in $R_w$.
%\mcomment{sa}
%As such, identifying the sets $R_w$ and $S_w$ involves looking forward in a slot $s_j$ to 

In order to find the item with the maximum $g$ value \eqref{eq:ij}, among all the items in the slot. 
%To obtain an online implementation of this procedure, 
We use an online subroutine that employs the algorithm (Algorithm \ref{alg:matroidmax}) for the \textit{secretary problem with replacement} described earlier. 
Note that $R_w$, $S_w$ and $\bar{S}_w$ can be computed {\it exactly at the end} of window $w$. 


%This online procedure will result in selection of a set $H_w$ potentially larger than $R_w$, while ensuring that each element from $R_w$ is part of $H_w$ with a high probability $1-\delta$ at the cost of adding extra $\log(1/\delta)$ items to the shortlist. Note that $R_w$ and $S_w$ can be computed {\it exactly at the end} of window $w$. 

%Algorithm \ref{alg:tmp} summarizes the overall structure of our algorithm. 
%The  following notation is used for brevity. For any collection of sets $V_1, \ldots, V_\ell$, we use $V_{1,\ldots, \ell}$ to denote $V_1 \cup \cdots \cup V_\ell$. 
%In the algorithm, for any item $i$ and set $V $, we define $\Delta_f(i|V):=f(V\cup \{i\})- f(V)$.
%The subroutine to compute $H_w$ for window $w$ uses Algorithm \ref{alg:SIImax} for each subsequence $\tau$ and each slot $s_j$ in that subsequence. Consequently, the parameters for Algorithm \ref{alg:SIImax} for slot $j$ are: number of items $X_j$ which is $n/k\beta$ in expectation, $\delta >0$, and value $a_i$ of an item $i\in [X_j]$ is as given by the expression inside maximizer in \eqref{eq:ij}.
%\scomment{I will come back to make this more precise with parameter specifications, after finishing the subroutine description and analysis.}

The algorithm returns both the shortlist $A$ which similar to~\cite{us} is of size $O(k)$ as stated in the following proposition, as well the set $A^*$.
Note that we remove $\hat{S}_w$ from $A^*$ at the end of window $w$.
%as a set $A^*=\cup_w (S_w \cap A)$ of size at most $k$to compete with $S^*$.
In the next section, we will show that $\Ex[f(A^*)] \ge (1-\frac{1}{e^2} - \epsilon -O(\frac{1}{k})) f(S^*)$ to provide a bound on the competitive ratio of this algorithm.  As it is proved in~\cite{us},

\begin{prop}
\label{prop:size}
Given $k,n$, and any constant $\alpha, \beta$ and $\epsilon$, the size of shortlist $A$ selected by Algorithm~\ref{alg:main} is at most $4k \beta {\alpha \beta \choose \alpha}\log(2/\epsilon) = O(k)$. 
%\scomment{proposition about size of shortlist returned by Algorithm \ref{alg:tmp}.}
\end{prop}
%\begin{proof}
%For each window $w=1,\ldots, k/\alpha$, and for each of the $\alpha\beta$ slots in this window, lines \ref{li:subb} through \ref{li:sube} in  Algorithm \ref{alg:main} runs  Algorithm \ref{alg:SIIImax} for ${\alpha \beta \choose \alpha}$ times (for all $\alpha$ length subsequences). By construction of  Algorithm \ref{alg:SIIImax}, for each run it will add at most $L\le 4\log(2/\epsilon)$ items each time to the shortlist. 
%\scomment{Here, we need to fix what $ \delta$ is in terms of $\epsilon$. I have waiting for your precise theorem about this.} \mcomment{lemma~\ref{online}}
%Therefore, over all windows, Algorithm \ref{alg:main} adds at most $ \frac{k}{\alpha} \times \alpha\beta  {\alpha \beta \choose \alpha} L = O(k)$ items to  the shortlist. 
%\end{proof}

%Later, in the proof of Theorem \ref{opttheorem}, we show that we set $\alpha=O(\frac{1}{\epsilon^4}\log(1/\epsilon)), \beta=O(\frac{1}{\epsilon^2})$ to get the desired competitive ratio. This setting of $\alpha, \beta$ results in the specific dependence of function $\eta_\epsilon(k)$ on $\epsilon$, as  stated in Theorem \ref{opttheorem}.
%\scomment{Add some sentences regarding the changes in implementation required for the streaming version.}


%\subsection{Preliminary: Algorithm for finding max online}
%Add details about online Algorithm for picking $\log(1/\delta)$ items from a sequence of $n$ items such that max lies in the picked items with probability $1-\delta$.
%Consider the simple greedy algorithm described in algorithm~\ref{alg:SIIImax}.

%\begin{algorithm*}[ht]
%  \caption{~\bf{Select-If-it-Improves}($I , u$)}
%  \label{alg:SIII} 
%\begin{algorithmic}[1]
%\State $S\leftarrow \emptyset$
%\For {i=0 to n}
%%\If {$\max(S\cup \{a_i\}) > \max(S) $}
%\If {$F(a_i) > \max_{a\in S} F(a) $}
%\State $S\leftarrow S\cup \{a_i\}$
%\EndIf
%\EndFor
%\State return $S\setminus \{a_1,\cdots, a_u\}$
%\end{algorithmic}
%\end{algorithm*}




%\begin{theorem}
%Suppose $S$ is the output of above algorithm on the input $I=\{a_1,\cdots, a_n\}$ then $F(S) = F(I)$
%\end{theorem}
%\begin{proof}

%%Suppose $F(I)=f(T)$,  where $|T|=m$. The above algorithm never miss  any element of $T$.
%%Since $F$ is submodular if the marginal increae

%Suppose $S_i$ is the subset selected at iteration $i$. Since $F$ is submodular, if $F(S_i\cup \{a_i\}) \le F(S_i)$ 
%then $F(S\cup\{a_i\}) \le F(S)$. Therefore every $e\in I\setminus S$ has marginal value 0 with respect to $S$, i.e., $F(S)=F(I)$.
%\end{proof}

%\paragraph{Bounds on size of shortlist maintained by Algorithm \ref{alg:tmp}.}



==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/algorithms1.tex <==
%\section{Algorithms}
%\subsection{Simpler but unimplementable, offline version}
%\subsection{Algorithm description}

Before giving our algorithm for \nameOfProblemSL, we describe a simple technique for \nameSecSL~
that achieves a  $1-\delta$ competitive ratio for  with shortlists of size logarithmic in $1/\delta$.
Recall that in the \nameSec, the aim is to select an item with expected value close to the maximum among a pool of items $I=(a_1, \ldots, a_N)$ arriving sequentially in a uniformly random order. 
We will consider the variant with shortlists, where we now want to pick a shortlist which contains an item with expected value close to the maximum.
%\ccomment{why are we using $\epsilon$ in the text and $\delta$ in the Algorithm below}\scomment{fixed}
We propose the following simple algorithm. For the first $n\delta/2$ rounds, don't add any items to the shortlist, but just keep track of the maximum value seen so far.
For all subsequent rounds, 
for any arriving item $i$ that has a value $a_i$ greater than or equal to the maximum value seen so far, add it to the shortlist if the size of shortlist is less than or equal to $L=4\ln(2/\delta)$. This algorithm is summarized as Algorithm \ref{alg:SIIImax}. Clearly, for contant $\delta$, this algorithm uses a shortlist of size $L=O(1)$. Further, under a uniform random ordering of input, we can show that the maximum value item will be part of the shortlist with probability $1-\delta$. (See Proposition \ref{maxanalysis} in Section \ref{sec:analysis}.)
%that the expected number of items in the shortlist $A$ is at most $\log(1/\epsilon)$, i.e., $O(1)$, and the maximum value item will be part of the shortlist with probability $1-\epsilon$. %analysis is presented in Section \ref{sec:max}. 
%--------------------------------------
\begin{algorithm*}[ht]
  %\caption{~\bf{Select-If-it-Improves}($I , u$)}
  \caption{~\bf{Algorithm for secretary with shortlist} (finding max online)}
  \label{alg:SIIImax} 
\begin{algorithmic}[1]
\State Inputs: number of items $N$, items in $I=\{a_1, \ldots, a_N\}$ arriving sequentially, $\delta \in (0,1]$. 
\State Initialize: $A\leftarrow \emptyset$,  $u=n\delta/2$, $M = -\infty$ %$M\leftarrow \max\{a_1, \cdots, a_{u-1}\}$
%\scomment{Should initialization of $u$ be changed to $n\delta/2$?}
%\mcomment{yes}
\State $L \leftarrow 4\ln(2/\delta)$ %\scomment{I changed (3+$\sqrt{2}$) to $4$}

\For {$i= 1$ to $N$}
%\If {$F(S\cup \{a_i\}) > F(S) $}
\If {$ a_i > M$}
\State $M \leftarrow  a_i$
\If {$i \geq u$ and $|A|<L$}
\State $A\leftarrow A\cup \{a_i\}$
\EndIf
\EndIf
\EndFor
%\State return $S\setminus \{a_1,\cdots, a_u\}$

%\mcomment{
%cleaner:
%\For {$i= u$ to $N$}
%\If {$ a_i > \max_{1\le j <i} a_j$ and $|A|<L$}
%\State $A\leftarrow A\cup \{a_i\}$
%\EndIf
%\EndFor
%}

\State return $A$, and $A^*:= \max_{i\in A} a_i$
\end{algorithmic}
\end{algorithm*}
%--------------------------------------------

%-----------------------------------------
\begin{algorithm*}[h!]
  %\caption{~\bf{Select-If-it-Improves}($I , u$)}
  \caption{~\bf{Algorithm for {\bf submodular} $k$-secretary with shortlist}}
  \label{alg:main} 
  \label{alg:tmp} 
\begin{algorithmic}[1]
\State Inputs: set $\bar I=\{\bar{a}_1,\ldots, \bar{a}_n\}$ of $n$ items arriving sequentially, submodular function $f$, parameter $\epsilon \in (0,1]$. 
\State Initialize: $S_0 \leftarrow \emptyset, R_0 \leftarrow \emptyset, A \leftarrow \emptyset, A^* \leftarrow \emptyset$, constants $\alpha \ge 1, \beta \ge 1$ which depend on the constant $\epsilon$.
\State Divide indices $\{1,\ldots, n\}$ into $(\alpha, \beta)$ windows as prescribed by Definition \ref{def:windows}.
%Divide the sequence of candidates into consecutive groups of $\frac{n}{\beta k}$ candidates, referred to as slots (or buckets). And, divide the sequence of slots into consecutive groups of $\alpha \beta$ slots, referred to as {\it windows}.
%===========================
\For {window $w= 1, \ldots, k/\alpha$} 
%\State For every $\alpha$-length subsequence $\tau=(s_1,\ldots, s_\alpha) \subseteq [\alpha\beta]$ of slots in window $w$, define 
%$$\gamma(\tau):=\{i_1, \ldots, i_\alpha\}$$
%where 
%$$i_j := \arg \max_{i\in V_{s_j,w} \cup R_{1,\ldots, w-1}} f(S_{1,\ldots,w-1} \cup \{i_1\ldots, i_{j-1}\} \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \{i_1\ldots, i_{j-1}\})$$
%\State Define $R_w:=\{\cup_{\tau} \gamma(\tau)\}.$ 
 

%\State Process the online inputs in window $w$ using the subroutine in Algorithm \ref{alg:tmpWindow} to select a subset $H_w$ of items. 
 \For {every slot $s_j$ in window $w$, $j=1,\ldots, \alpha\beta$}
  \State Concurrently for all subsequences of previous slots $\tau\subseteq \{s_1, \ldots, s_{j-1}\}$ of length $|\tau|<\alpha$ \label{li:subb}   \hspace{0.44in} in window $w$, call the online algorithm in Algorithm \ref{alg:SIIImax} with the following inputs: 
  %\begin{center}
  \begin{itemize}[leftmargin=0.7in]
  \item   number of items $N=|s_j|+1$, $\delta=\frac{\epsilon}{2}$, and
%  \scomment{You have to use $\delta$ smaller than $\epsilon$ to get $1-\frac{1}{e}-\epsilon$ in the final result.}
  \item item values $I=(a_0, a_1, \ldots, a_{N-1})$, with 
     \begin{eqnarray*} 
  a_0 & := & \max_{x\in R_{1,\ldots, w-1}} \Delta(x|S_{1,\ldots,w-1} \cup \gamma(\tau)) \\
  %\max_{x\in R_{1,\ldots, w-1}} f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{x\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\}$
     a_\ell & := & \Delta(s_j(\ell)| S_{1,\ldots,w-1} \cup \gamma(\tau) ),  \forall \ell=1,\ldots, N-1
     \end{eqnarray*}
    %f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\})$
 where $s_j(\ell)$ denotes the $\ell^{th}$ item in the slot $s_j$. 
% \item $\delta = \frac{\epsilon}{{\alpha \beta \choose \alpha}}$.
  \end{itemize}
   %\end{center}
   %\mcomment{why do you divide by... the erros do not add up}  \scomment{Please add the required theorem showing this}  \mcomment{added lemma~\ref{online}}
\State Let $A_{j}(\tau)$ be the shortlist returned by  Algorithm \ref{alg:SIIImax} for slot $j$ and subsequence $\tau$. Add 
\label{li:tmp} \hspace{0.44in} all items except the dummy item $0$ to the shortlist $A$. Let's $A(j)=\bigcup_{\tau} A_j(\tau)$.
%for all $\tau$,
%  $$A(j) \leftarrow A(j)\cup (A_{j}(\tau))$$
%$H_w$, i.e, for all $\tau$,
 % $$H_w \leftarrow H_w\cup (A_{j}(\tau) \cap s_j)$$
 That is, \label{li:sube}
 $$A\leftarrow A\cup  (A(j)\cap s_j)$$
 \EndFor
%\State return $H_w$
% \State $A\leftarrow A\cup H_w$
 \State \label{li:Rw} After seeing all items in window $w$, compute $R_w, S_w$ as defined in \eqref{eq:Rw} and \eqref{eq:Sw} respectively.
 \State $A^* \leftarrow A^*\cup (S_w \cap A)$
\EndFor
\State return $A$, $A^*$. %$A=T_1 \cup \cdots  \cup T_{W}$
\end{algorithmic}
\end{algorithm*}

%==========================


%\begin{algorithm*}[ht]
  %\caption{~\bf{Subroutine of Algorithm \ref{alg:tmp} for window $w$}}
  %\label{alg:tmpWindow} 
  \toRemove{
  \begin{algorithmic}[1]
  \For {every slot $s_j$ in window $w$, $j=1,\ldots, \alpha\beta$}
  \State Concurrently for all subsequences of previous slots $\tau\subseteq \{s_1, \ldots, s_{j-1}\}$ in window $w$, of length $|\tau|<\alpha$, call the online algorithm in Algorithm \ref{alg:SIIImax} with the following inputs: number of items $N=|s_j|+1$, $\delta = \frac{\epsilon}{{\alpha \beta \choose \alpha}}$, \mcomment{why do you divide by... the errors do not add up} and values of arriving items $(a_0, a_1, \ldots, a_{N-1})$ defined as 
  $$a_0:=\max_{x\in R_{1,\ldots, w-1}} f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{x\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\}$$
    $$a_i :=f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\})$$
 where $i$ denotes the $i^{th}$ item in slot $s_j$.
  \State Let $A_{j}(\tau)$ be the shortlist returned by  Algorithm \ref{alg:SIIImax} for slot $j$ and subsequence $\tau$. Add all items except the dummy item $0$ to $H_w$, i.e, for all $\tau$,
  $$H_w \leftarrow H_w\cup (A_{j}(\tau) \cap s_j)$$
 \EndFor
\State return $H_w$
\end{algorithmic}
}
%\end{algorithm*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
There are two main difficulties in extending this idea to the \nameOfProblemSL. First, instead of one item, here we aim to select a set $S$ of $k$ items using an $O(k)$ length shortlist. Second, the contribution of each new item $i$ to the objective value, as given by the submodular function $f$, depends on the set of items selected so far. 

The first main concept we introduce to handle these difficulties  is that of dividing the input into sequential blocks that we refer to as $(\alpha, \beta)$ windows. Below is the precise construction of $(\alpha, \beta)$ windows, for any postivie integers $\alpha$ and $\beta$, such that $k/\alpha$ is an integer.
%\ccomment{This definition is imprecise.  Needs to be made technically crisp.}
%\ccomment{What exactly is this distribution?  Are we drawing with replacement or without and do the $X_i$ sum to $n$?}

We use a set of random variables $X_1,\ldots,X_m$ defined in the following way.  Throw $n$ balls into $m$ bins uniformly at random.  Then set $X_j$ to be the number of balls in the $j$th bin.  We call the resulting $X_j$'s a {\em $(n,m)$-ball-bin random set}.


\begin{definition}[$(\alpha,\beta)$ windows]
\label{def:windows}
Let $X_1,\ldots,X_{k\beta}$ be a $(n,k\beta)$-ball-bin random set.
Divide the indices $\{1,\ldots, n\}$ into $k\beta$ slots, where the $j$-th slot, $s_j$, consists of $X_j$ consecutive indices in the natural way, that is, slot $1$ contains the first $X_1$ indices, slot $2$ contains the next $X_2$, etc.
 %, $X_i$ would be the number of balls in the $i$-th bin.
 Next, we define $k/\alpha$ windows, where window $i$ consists of $\alpha \beta$ consecutive slots, in the same manner as we assigned slots.
\end{definition}
%\ccomment{Would an example or a figure help here to define slots and windows?}
Thus, $q^{th}$ slot is composed of indices $\{\ell, \ldots, r\}$, where $\ell=X_1+...+X_{q-1}+1$ and  $r=X_1+...+X_q$. 
Further, if the ordered the input is $\bar a_1, \dots, \bar a_n$ then we say that the items inside the slot $s_q$ are $\bar a_{\ell}, \bar a_{\ell+1}, \dots, \bar a_{r}$ 
To reduce notation, when clear from context, we will use $s_q$ and $w$ to also indicate the {\it set of items} in the slot $s_q$ and window $w$ respectively.

%The idea is to divide the inputs into $k/\alpha$ blocks (i.e., windows) for a constant $\alpha\ge 1$ such that 
%\ccomment{Shouldn't we say what alpha is because the intuition depends on it}
When $\alpha$ and $\beta$ are large enough constants, some useful properties can be obtained from the construction of these windows and slots. First, roughly $\alpha$ items from the optimal set $S^*$ are likely to lie in each of these windows; and further, it is unlikely that two items from $S^*$ will appear in the same slot. (These statements will be made more precise in the analysis where precise setting of $\alpha,\beta$ in terms of $\epsilon$ will be provided.) Consequently, our algorithm can focus on identifying a constant number (roughly $\alpha$) of optimal items from each of these windows, with at most one item coming from each of the $\alpha \beta$ slots in a window. The core of our algorithm is a subroutine that accomplishes this task in an online manner using a shortlist of constant size in each window. 

To implement this idea, we use a greedy selection method that considers all possible $\alpha$ sized subsequences of the $\alpha\beta$ slots in a window, and aims to identify the subsequence that maximizes the increment over the best items identified so far. 
More precisely, for any subsequence $\tau=(s_1,\ldots, s_\ell)$ of the $\alpha\beta$ slots in window $w$, we define a `greedy' subsequence $\gamma(\tau)$ of items as:
\begin{equation}
\label{eq:gamma}
\gamma(\tau):=\{i_1, \ldots, i_\ell\}
\end{equation}
where
\begin{equation}
\label{eq:ij}
i_j := \arg \max_{i\in s_j \cup R_{1, \ldots, w-1}} f(S_{1, \ldots,w-1} \cup \{i_1,\ldots, i_{j-1}\} \cup \{i\}) - f(S_{1, \ldots, w-1} \cup \{i_1\ldots, i_{j-1}\}).
\end{equation}
In ({\ref{eq:ij}) and in the rest of the paper, we use shorthand $S_{1,\ldots, w}$ to denote $S_1\cup \cdots \cup S_{w}$, and $R_{1,\ldots, w}$ to denote $R_1\cup \cdots \cup R_{w}$, etc.  We also will take unions of subsequences, which we interpret as the union of the elements in the subsequences.
%\ccomment{Are we bothered by taking the union of a sequence rather than a set?}
We also define $R_w$ to be  the union of all greedy subsequences of length $\alpha$, and $S_w$to be  the best subsequence among those. That is,
\begin{equation}
\label{eq:Rw}
R_w = \cup_{\tau: |\tau|=\alpha} \gamma(\tau)
\end{equation}
and 
\begin{equation}
\label{eq:Sw}
S_w=\gamma(\tau^*),
\end{equation} where
\begin{equation}
\label{eq:taustar}
\tau^*:=\arg \max_{\tau: |\tau|=\alpha} f(S_{1,\ldots,w-1} \cup \gamma(\tau)) - f(S_{1,\ldots,w-1}).
\end{equation}
Note that $i_j$ (refer to \eqref{eq:ij}) can be set as  either an item in slot $s_j$ or an item {\it from a previous greedy subsequence} in $R_1\cup \cdots \cup R_{w-1}$. The significance of the latter relaxation will become clear in the analysis.
%Here, $s_j \cup R_1 \cup \cdots \cup R_{w-1}$ denotes the union of items in slot $s_j$ and 

%$S_w$ represents the best subsequence among all the subsequences in $R_w$.
As such, identifying the sets $R_w$ and $S_w$ involves looking forward in a slot $s_j$ to find the best item (according to the given criterion in \eqref{eq:ij}) among all the items in the slot. To obtain an online implementation of this procedure, we use an online subroutine that employs the algorithm (Algorithm \ref{alg:SIIImax}) for the basic secretary problem described earlier. This online procedure will result in selection of a set $H_w$ potentially larger than $R_w$, while ensuring that each element from $R_w$ is part of $H_w$ with a high probability $1-\delta$ at the cost of adding extra $\log(1/\delta)$ items to the shortlist. Note that $R_w$ and $S_w$ can be computed {\it exactly at the end} of window $w$. 

Algorithm \ref{alg:tmp} summarizes the overall structure of our algorithm. 
%The  following notation is used for brevity. For any collection of sets $V_1, \ldots, V_\ell$, we use $V_{1,\ldots, \ell}$ to denote $V_1 \cup \cdots \cup V_\ell$. 
In the algorithm, for any item $i$ and set $V $, we define $\Delta_f(i|V):=f(V\cup \{i\})- f(V)$.
%The subroutine to compute $H_w$ for window $w$ uses Algorithm \ref{alg:SIImax} for each subsequence $\tau$ and each slot $s_j$ in that subsequence. Consequently, the parameters for Algorithm \ref{alg:SIImax} for slot $j$ are: number of items $X_j$ which is $n/k\beta$ in expectation, $\delta >0$, and value $a_i$ of an item $i\in [X_j]$ is as given by the expression inside maximizer in \eqref{eq:ij}.
%\scomment{I will come back to make this more precise with parameter specifications, after finishing the subroutine description and analysis.}

The algorithm returns both the shortlist $A$ which we show to be  of size $O(k)$ in the following proposition, as well as a set $A^*=\cup_w (S_w \cap A)$ of size at most $k$ to compete with $S^*$. In the next section, we will show that $\Ex[f(A^*)] \ge (1-\frac{1}{e} - \epsilon -O(\frac{1}{k})) f(S^*)$ to provide a bound on the competitive ratio of this algorithm. 

\begin{prop}
\label{prop:size}
Given $k,n$, and any constant $\alpha, \beta$ and $\epsilon$, the size of shortlist $A$ selected by Algorithm~\ref{alg:main} is at most $4k \beta {\alpha \beta \choose \alpha}\log(2/\epsilon) = O(k)$. 
%\scomment{proposition about size of shortlist returned by Algorithm \ref{alg:tmp}.}
\end{prop}
\begin{proof}
For each window $w=1,\ldots, k/\alpha$, and for each of the $\alpha\beta$ slots in this window, lines \ref{li:subb} through \ref{li:sube} in  Algorithm \ref{alg:main} runs  Algorithm \ref{alg:SIIImax} for ${\alpha \beta \choose \alpha}$ times (for all $\alpha$ length subsequences). By construction of  Algorithm \ref{alg:SIIImax}, for each run it will add at most $L\le 4\log(2/\epsilon)$ items each time to the shortlist. 
%\scomment{Here, we need to fix what $ \delta$ is in terms of $\epsilon$. I have waiting for your precise theorem about this.} \mcomment{lemma~\ref{online}}
Therefore, over all windows, Algorithm \ref{alg:main} adds at most $ \frac{k}{\alpha} \times \alpha\beta  {\alpha \beta \choose \alpha} L = O(k)$ items to  the shortlist. 
\end{proof}
%Later, in the proof of Theorem \ref{opttheorem}, we show that we set $\alpha=O(\frac{1}{\epsilon^4}\log(1/\epsilon)), \beta=O(\frac{1}{\epsilon^2})$ to get the desired competitive ratio. This setting of $\alpha, \beta$ results in the specific dependence of function $\eta_\epsilon(k)$ on $\epsilon$, as  stated in Theorem \ref{opttheorem}.
%\scomment{Add some sentences regarding the changes in implementation required for the streaming version.}


%\subsection{Preliminary: Algorithm for finding max online}
%Add details about online Algorithm for picking $\log(1/\delta)$ items from a sequence of $n$ items such that max lies in the picked items with probability $1-\delta$.
%Consider the simple greedy algorithm described in algorithm~\ref{alg:SIIImax}.

%\begin{algorithm*}[ht]
%  \caption{~\bf{Select-If-it-Improves}($I , u$)}
%  \label{alg:SIII} 
%\begin{algorithmic}[1]
%\State $S\leftarrow \emptyset$
%\For {i=0 to n}
%%\If {$\max(S\cup \{a_i\}) > \max(S) $}
%\If {$F(a_i) > \max_{a\in S} F(a) $}
%\State $S\leftarrow S\cup \{a_i\}$
%\EndIf
%\EndFor
%\State return $S\setminus \{a_1,\cdots, a_u\}$
%\end{algorithmic}
%\end{algorithm*}




%\begin{theorem}
%Suppose $S$ is the output of above algorithm on the input $I=\{a_1,\cdots, a_n\}$ then $F(S) = F(I)$
%\end{theorem}
%\begin{proof}

%%Suppose $F(I)=f(T)$,  where $|T|=m$. The above algorithm never miss  any element of $T$.
%%Since $F$ is submodular if the marginal increae

%Suppose $S_i$ is the subset selected at iteration $i$. Since $F$ is submodular, if $F(S_i\cup \{a_i\}) \le F(S_i)$ 
%then $F(S\cup\{a_i\}) \le F(S)$. Therefore every $e\in I\setminus S$ has marginal value 0 with respect to $S$, i.e., $F(S)=F(I)$.
%\end{proof}

%\paragraph{Bounds on size of shortlist maintained by Algorithm \ref{alg:tmp}.}



==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/analysis.tex <==
\newcommand{\settinga}{\mbox{$k \ge \alpha\beta$}, \settingb}
\newcommand{\settingb}{\mbox{$\beta\ge \frac{8}{(\delta')^2}$}, $\alpha\ge 8\beta^2 \log(1/\delta')$}

In this section we show that for any $\epsilon \in (0,1)$, Algorithm \ref{alg:tmp} with an appropriate choice of constants $\alpha, \beta$, achieves the competitive ratio claimed in Theorem \ref{opttheorem} for the \nameOfProblemMatroidSL.  

%Recall the following notation defined in the previous section.  For any collection of sets $V_1, \ldots, V_\ell$, we use $V_{1,\ldots, \ell}$ to denote $V_1 \cup \cdots \cup V_\ell$. Also, recall that for any item $i$ and set $V $, we denote $\Delta_f(i|V):=f(V\cup \{i\})- f(V)$.
\toRemove{
\paragraph{Proof overview.} The proof is divided into two parts. We first  show a lower bound on the ratio $\Ex[f(S_{1,\cdots,W})]/{\OPT}$ in Proposition~\ref{prop:first}, where $S_w$ is the subset of items as defined in \eqref{eq:Sw} for every window $w$. Later in Proposition~\ref{prop:online}, we use the said  bound to derive a lower bound on the ratio $\Ex[f(A^*)]/\OPT$, where $A^*=A\cap (S_{1,\cdots, W})$ is the subset of shortlist returned by Algorithm~\ref{alg:main}. %This will complete the proof of Theorem \ref{opttheorem}.

Specifically, in Proposition \ref{prop:first}, we provide settings of parameters $\alpha, \beta$ such that of $\Ex[f(S_{1,\cdots, W})] \ge \left(1-\frac{1}{e}-\frac{\epsilon}{2} - O(\frac{1}{k})\right)\OPT$.  A central idea in the proof of this result is to show that for every window $w$, given $R_{1,\ldots, w-1}$,  the items tracked from the previous windows, any of the $k$ items from the optimal set $S^*$ (if the independent set has less than $k$ items extend it by adding some dummy items) has at least $\frac{\alpha}{k}$ probability to appear either in window $w$, or among the tracked items $R_{1,\ldots, w-1}$. Further, the items from $S^*$ that appear in window $w$, appear  independently, and in a uniformly at random slot in this window. (See Lemma \ref{lem:pijBound}.)  This observation allows us to show that, in each window, there exists a subsequence $\tilde \tau_w$ of close to $\alpha$ slots, such that the greedy sequence of items $\gamma(\tilde \tau_w)$ will be almost ``as good as" a randomly chosen sequence of $\alpha$ items from $S^*$. More precisely, denoting $\gamma(\tilde \tau_s)=(i_1,\ldots, i_t)$, in Lemma \ref{lem:asGoodas}, for all $j=1,\ldots, t$, we lower bound the increment in function value $f(\cdots)$ on adding $i_j$ over the items in $S_{1, \ldots, w-1} \cup i_{1,\ldots, j-1}$ as:
{\small $$\Ex[\Delta_f(i_j|S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\})|T_{1,\ldots, w-1}, i_1, \ldots, i_{j-1}] \ge \frac{1}{k}\left((1-\frac{\alpha}{k})f(S^*)-f(S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\})\right)\ . $$}
We then deduce (using standard techniques for the analysis of greedy algorithm for submodular functions) that 
{\small $$\Ex[\left(1-\frac{\alpha}{k}\right) f(S^*) - f(S_{1,\ldots, w-1}\cup \gamma(\tilde \tau_w)) | S_{1,\ldots, w-1}] \le e^{-t/k} \left(\left(1-\frac{\alpha}{k}\right) f(S^*)-f(S_{1,\ldots, w-1})\right)\ .$$}
%Further, we show that $t$ is close to $\alpha$ with high probability (refer to Lemma \ref{lem:}). 
Now, since the length $t$ of $\tilde \tau_w$ is close to $\alpha$ (as we show in Lemma \ref{lem:lengthtau}) and since  $S_w=\gamma(\tau^*)$ with $\tau^*$ defined as the ``best"  subsequence of length $\alpha$ (refer to definition of $\tau^*$ in \eqref{eq:taustar}), we can show that a similar inequality holds for {\small $S_w=\gamma(\tau^*)$, i.e.,
$$\left(1-\frac{\alpha}{k}\right) f(S^*) - \Ex[f(S_{1,\ldots, w-1}\cup S_w)|S_{1,\ldots, w-1}] \le e^{-\alpha/k} \left(1-\delta'\right)\left(\left(1-\frac{\alpha}{k}\right) f(S^*)-f(S_{1,\ldots, w-1})\right)\ ,$$}
where $\delta'\in (0,1)$ depends on the setting of $\alpha, \beta$. (See   Lemma~\ref{lem:Sw}.)  Then repeatedly applying this inequality for $w=1, \ldots, k/\alpha$, and setting $\delta, \alpha, \beta$ appropriately in terms of $\epsilon$, we can obtain $\Ex[f(S_{1,\ldots, W})] \ge \left(1-\frac{1}{e^2} - \frac{\epsilon}{2} -\frac{1}{k}\right) f(S^*)$, completing  the proof of Proposition \ref{prop:first}.

However, a remaining difficulty is that while the algorithm keeps a track of the set $S_w$ for every window $w$, it may not have been able to add all the items in $S_w$ to the shortlist $A$ during the online processing of the inputs in that window. In the proof of Proposition \ref{prop:online}, we show that in fact the algorithm will add most of the items in $\cup_w S_w$ to the short list. More precisely, we show that given that an item $i$ is in $S_w$, it will be in shortlist $A$ with probability $1-\delta$, where $\delta$ is the parameter used while calling Algorithm \ref{alg:SIIImax} in Algorithm \ref{alg:main}. Therefore, using properties of submodular functions it follows  that with $\delta=\epsilon/2$, $\Ex[f(A^*)] = \Ex[f( S_{1,\cdots, W} \cap A)] \ge (1-\frac{\epsilon}{2})\Ex[f(S_{1,\cdots, W})]$ (see Proposition \ref{prop:online}). Combining this with the lower bound $\frac{\Ex[f(S_{1,\cdots, W})]}{\OPT} \ge (1-\frac{1}{e^2}-\frac{\epsilon}{2} - O(\frac{1}{k}))$ mentioned earlier, we complete the proof of competitive ratio bound stated in Theorem \ref{opttheorem}.
%The set $A^*$ returned by Algorithm \ref{alg:tmp} is $\cup_w (S_w\cap H_w)$. we complete the proof of Theorem \ref{opttheorem} by showing that each item in $S_w$ will appear in $H_w$ with a high enough probability,

}




%\subsection{Bounding $\Ex[f( S_{1,\cdots, W})]/\OPT$}
 
%%%%%%%%%%%%%%%%%%%%
\input{newProof.tex}
%%%%%%%%%%%%%%%%%%%%%%%%%%



%\subsection{Bounding $\Ex[f(A^*)]/\OPT$}

\toRemove{
\begin{proof}
%Because of Theorem~\ref{maxanalysis},
%each element of $S_{1,\cdots, W}$ will be selected by the online max algorithm~\ref{alg:SIIImax} (or equivalently it is in $H_{1,\cdots, W}$)  with probability at least $1-\delta$.
From the previous lemma, given any configuration $Y$, we have that each item of $S_{1,\cdots, W}$ is in $A$ with probability at least $1-\delta$, where $\delta=\epsilon/2$ in Algorithm \ref{alg:main}.  
Therefore using Lemma~\ref{sample}, the expected value of $f(S_{1,\cdots, W}\cap A)$ 
is at least $(1-\delta)\mathbb{E}[F(S_{1,\cdots, W})]$.
\end{proof}
}


\toRemove{
\begin{theorem} \label{opttheorem}
For any constant $\epsilon>0$, there exists an online algorithm (Algorithm \ref{alg:main}) for the \nameOfProblemMatroidSL\ that achieves a competitive ratio of $\frac{1}{2}(1-\frac{1}{e^2} -\epsilon -O(\frac{1}{k}))$, with shortlist of size $\eta_\epsilon(k)=O(k)$. Here,  $\eta_\epsilon(k)=O(2^{poly(1/\epsilon)}k)$. The running time of this online algorithm is $O(n)$.
\end{theorem}
}
%\paragraph{Proof of Theorem \ref{opttheorem}.} 

\toRemove{
\begin{proof}
Now, we can show that Algorithm \ref{alg:main} provides the results claimed in Theorem \ref{opttheorem} for appropriate settings of $\alpha, \beta$ in terms of $\epsilon$. 
Specifically for $\delta'=\epsilon/4$, set $\alpha,\beta$ as smallest integers satisfying  \settingb. Then, using Proposition \ref{prop:first} and Proposition \ref{prop:online}, for $k\ge \alpha\beta$ we obtain:
$$\Ex[f(A^*)] \ge (1-\frac{\epsilon}{2})(1-\delta')^2 (\frac{1}{2}(1-1/e^2)) \OPT \ge \frac{1}{2}(1-\epsilon)(1-1/e^2) \OPT.$$
This implies a lower bound of $\frac{1}{2}(1-\epsilon - 1/e^2 - \alpha\beta/k) =\frac{1}{2}( 1-\epsilon-1/e^2 - O(1/k))$ on the competitive ratio.
The $O(k)$ bound on the size of the shortlist was  demonstrated in Proposition \ref{prop:size}.

%Now by slightly modify the algorithm to get a more efficient one.
%The idea is that in each window after computing $R_w$ we reassign each element of $R_w$ uniformly at random to a new slot (among all $k\beta$ slots).
%Then to find argmax in each slot we only look at  $V_{s_j,w}$ instead of  $V_{s_j,w} \cup R_{1,\ldots, w-1}$.



%\subsection{Matroid secretary problem with shortlist of size $k$}

\end{proof}
}

\subsection{Preemption model and  Shorlitst of size at most $k$}
Finally we focus on the special case where the size of shortlist is at most $k$. We can get a constant competitive algorithm even with the slight relaxation of the \textit{matroid secretary problem} 
to the case that we allow the algorithm to select a shortlist of size at most $k=rk(\mathcal{M})$. 
The algorithm finally outputs an independent subset of this shortlist of size $k$. There was no constant compettetive algorithm even for this natural relaxation of \textit{matroid secretary problem}.
Also we are not aware of any direct way to prove a constant factor guarantee for this simple relaxation without using the techniques that we develop using $(\alpha,\beta)$-windows. 


%The Algorithm~\ref{alg:main}s becomes very simple in this case:



\toRemove{
\begin{algorithm*}[h!]
  %\caption{~\bf{Select-If-it-Improves}($I , u$)}
  \caption{~\bf{Algorithm for {\bf submodular} matroid secretary with shortlist of size $k$}}
  \label{alg:simple} 
\begin{algorithmic}[1]
\State Inputs: number of items $n$, submodular function $f$, parameter $\epsilon \in (0,1]$. 
\State Initialize: $S_0 \leftarrow \emptyset, R_0 \leftarrow \emptyset, A \leftarrow \emptyset, A^* \leftarrow \emptyset$, constants $\alpha \ge 1, \beta \ge 1$ which depend on the constant $\epsilon$.
\State Divide indices $\{1,\ldots, n\}$ into $(\alpha, \beta)$ windows. %as prescribed by Definition \ref{def:windows}.
%Divide the sequence of candidates into consecutive groups of $\frac{n}{\beta k}$ candidates, referred to as slots (or buckets). And, divide the sequence of slots into consecutive groups of $\alpha \beta$ slots, referred to as {\it windows}.
%===========================
\For {window $w= 1, \ldots, k/\alpha$} 
%\State For every $\alpha$-length subsequence $\tau=(s_1,\ldots, s_\alpha) \subseteq [\alpha\beta]$ of slots in window $w$, define 
%$$\gamma(\tau):=\{i_1, \ldots, i_\alpha\}$$
%where 
%$$i_j := \arg \max_{i\in V_{s_j,w} \cup R_{1,\ldots, w-1}} f(S_{1,\ldots,w-1} \cup \{i_1\ldots, i_{j-1}\} \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \{i_1\ldots, i_{j-1}\})$$
%\State Define $R_w:=\{\cup_{\tau} \gamma(\tau)\}.$ 
 

%\State Process the online inputs in window $w$ using the subroutine in Algorithm \ref{alg:tmpWindow} to select a subset $H_w$ of items. 
 \For {every slot $s_j$ in window $w$, $j=1,\ldots, \alpha\beta$}
  \State Concurrently for all subsequences of previous slots $\tau\subseteq \{s_1, \ldots, s_{j-1}\}$ of length $|\tau|<\alpha$ \label{li:subb}\\
  \hspace{0.44in} in window $w$, call the online algorithm in Algorithm \ref{alg:matroidmax} with the following inputs: 
  %\begin{center}
  \begin{itemize}%[leftmargin=0.7in]
  \item   number of items $N=|s_j|+1$, $\delta=\frac{\epsilon}{2}$, and
%  \scomment{You have to use $\delta$ smaller than $\epsilon$ to get $1-\frac{1}{e}-\epsilon$ in the final result.}
  \item item values $I=(a_0, a_1, \ldots, a_{N-1})$, with 
   
     \begin{eqnarray*} 
  a_0 & := & \max_{x\in R_{1,\ldots, w-1}} \Delta(x|S_{1,\ldots,w-1} \cup \gamma(\tau)\setminus \zeta(\tau)) \\
  %\max_{x\in R_{1,\ldots, w-1}} f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{x\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\}$
     a_\ell & := & \Delta(s_j(\ell)| S_{1,\ldots,w-1} \cup \gamma(\tau)\setminus \zeta(\tau) ),  \forall 0<\ell\le N-1
     \end{eqnarray*}
    %f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\})$
 where $s_j(\ell)$ denotes the $\ell^{th}$ item in the slot $s_j$. 
% \item $\delta = \frac{\epsilon}{{\alpha \beta \choose \alpha}}$.
  \end{itemize}
   %\end{center}
   %\mcomment{why do you divide by... the erros do not add up}  \scomment{Please add the required theorem showing this}  \mcomment{added lemma~\ref{online}}
\State Let $A_{j}(\tau)$ be the shortlist returned by  Algorithm \ref{alg:matroidmax} for slot $j$ and subsequence $\tau$. Add \\
\hspace{0.44in} all items except the dummy item $0$ to the shortlist $A$. %$H_w$, i.e, for all $\tau$,
 % $$H_w \leftarrow H_w\cup (A_{j}(\tau) \cap s_j)$$
 That is, \label{li:sube}
 $$A\leftarrow A\cup  (A(j)\cap s_j)$$
 \EndFor
%\State return $H_w$
% \State $A\leftarrow A\cup H_w$
 \State After seeing all items in window $w$, compute $R_w, S_w$ as before %defined in \eqref{eq:Rw} and \eqref{eq:Sw} respectively.
 \State $S_{1,\cdots, w} \leftarrow S_{1,\cdots, w-1}\cup S_w \setminus \bar{S}_w$
 \State $A^* \leftarrow A^*\cup (S_w \cap A)\setminus \hat{S}_w$
\EndFor
\State return $A$, $A^*$. %$A=T_1 \cup \cdots  \cup T_{W}$
\end{algorithmic}
\end{algorithm*}
}




%If the size of shortlist is exactly $k$ we get the following.

%\preemption

\thmpreemption

\begin{proof}
We show that  algorithm~\ref{alg:main} 
with parameter $\alpha=\beta=1$ satisfies the above mentioned properties. Firstly,  algorithm~\ref{alg:main} (with $\alpha=1$, and $\beta=1$) uses shortlist of size $\eta(k)\le k$.
The reason is that the algorithm divides the input into exactly $k$ slots.
Also each window contains exactly one slot. 
The function $\gamma$ tries all $\alpha$-subsequences of a window which is exactly one slot. Thus $\gamma$ returns one element in that slot with hight value of $g(e,S)$ as defined in~\ref{eq:g}, which might cause removal of at most one element $\theta(S,e)$ from the current solution $S$. Therefore the algorithm has shortlist size at most $k$ and also satisfies the preemption model. Now by setting $\alpha=1, \beta=1$ we can get a constant compettetive ratio that  the error rate comes from lemma~\ref{lem:Sw}.

\toRemove{
Given that $|OPT|\le k$, we can extend the size of $OPT$ to a set of size exactly $k$, by adding some dummy elements.
Let's call that set $OPT'$.
In order to calculate the competitive ratio, we first compute the probability that one slot contains an element of optimal solution $OPT'$, i.e., the probability that $s\cap OPT'\neq \emptyset$, for a slot $s$ in window $w$. Since all $k$ elements of $OPT'$ are uniformly distributed, 
$$
Pr[s\cap OPT' \neq \emptyset | T_{1,\cdots, w-1} ] \ge 1- (1-1/k)^k.
$$
Therefore in lemma~\ref{cor:lengthtau}, $|\bar{\tau}_{w}|\ge 1$ with probability $1-1/e$. Hence 
$\mathbb{E}[f(S_{1,\ldots, W})] \ge \frac{1}{2}(1-1/e) (1-1/e^2)  \OPT.$
Thus by Lemma~\ref{cor:lengthtau} and~\ref{lem:Sw}, 
$$\mathbb{E}[f(A^*)] \ge  \frac{1}{2} (1-\epsilon)(1-1/e) (1-1/e^2)  \OPT.$$
}
\end{proof}


==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/bib.tex <==
@misc{kazemi2019submodular,
    title={Submodular Streaming in All its Glory: Tight Approximation, Minimum Memory and Low Adaptive Complexity},
    author={Ehsan Kazemi and Marko Mitrovic and Morteza Zadimoghaddam and Silvio Lattanzi and Amin Karbasi},
    year={2019},
    eprint={1905.00948},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}
\bibitem{kleinberg} R. Kleinberg, A Multiple-Choice Secretary Algorithm with Applications to Online Auctions
\bibitem{vondrak} V. Feldman, J. Vondrak, Optimal Bounds on Approximation of Submodular and XOS Functions by Juntas
\bibitem{kleh} T. Kesselheim, A. Tönnis, Submodular Secretary Problems: Cardinality, Matching, and Linear Constraints
\bibitem{mirzasoleiman} A. Badanidiyuru, B. Mirzasoleiman, A. Karbasi, A. Krause, Streaming Submodular Maximization: Massive Data Summarization on the Fly
\bibitem{bateni} M. Bateni, M. Hajiaghayi, M, Zadimoghaddam,  Submodular Secretary Problem and Extensions
%\bibitem{distr} B. Mirzasoleiman, A. Karbasi, R. Sarkar, A. Krause, Distributed Submodular Maximization
\bibitem{recent}  T. Hess, S. Sabato, The monotone submodular secretary problem under a cardinality constraint with limited resources
\bibitem{norouzi} Beyond 1/2-Approximation for Submodular Maximization on Massive Data Streams
\bibitem{linear} B. Mirzasoleiman, A. Badanidiyuru, A Karbasi, J. Vondrak, A. Krause, Lazier Than Lazy Greedy
%\bibitem{swm} M. Kapralov, I. Post, J. Vondrak, Online Submodular Maximization: Beating 1/2 Made Simple
\bibitem{vahab} N. Korula, V. Mirrokni, M. Zadimoghaddam, Online Submodular Welfare Maximization Greedy Beats 1/2 in random order



@article{buchbinder2018online,
  title={Online Submodular Maximization: Beating 1/2 Made Simple},
  author={Buchbinder, Niv and Feldman, Moran and Garg, Mohit},
  journal={arXiv preprint arXiv:1807.05529},
  year={2018}
}


==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/conclusion.tex <==
In this paper, we defined a relaxation of the submodular secretary problem with cardinality constraint. We allow the algorithm
to select more than $k$ elements, and the algorithm should output a subset of size $k$ among selected items.
We designed an algorithm with asymptotic
competitive ratio $R$ for any $R<1-1/e$. The total number of selections is only $O(k)$ elements. 
It is open  whether we can generalize this result to more general constraints such as matroid constraints.


==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/impossible.tex <==
%\section{Impossibility Result}

In this section we provide an upper bound showing the following:

\hardness*

%\begin{theorem}
%There is no algorithm achieving asymptotic competitive ratio $7/8+\epsilon$ for submodular secretary problem using $o(n)$ selections. 
%\end{theorem}

%\mcomment{In the following proof we will consider a submodular $k+1$-secretary} problem. 
In the following proof, for simplicity of notation, we prove the desired bound for submodular $(k+1)$-secretary problem. %Since $k+1=O(k)$, the upper bound derived will imply the stated bound for the  submodular $k$-secretary problem. 
For any given $n, k$, we construct a set of instances of the  \nameOfProblemSLplus~such that any online algorithm that uses a shortlist of size $\eta(k+1)$ will have competitive ratio of at most $\frac{7}{8} + \frac{\eta(k+1)}{2n}$ on a randomly selected instance from this set. 

First, we define a monotone submodular function $f$ as follows. 
%For $n>0$, we define a  monotone submodular function $f$. 
The ground set consists of $\frac{n}{2k}+n-1$ items. There are two types of items, $C$ and  $D$, with $L:=n/2k$ items of type $C$ and
$n-1$ items of type $D$. We define $f(\phi):=0$, $f(\{c\}):=k$ for $c\in C$, and $f(\{d\}):=1$ for all $d\in D$. 
%There are infinitely many elements of $C$ and $D$. 
%\scomment{Don't you just need $L$ items of type $C$ and $n-1$ items of type $D$?}
%There are
Also there is a collection of $L$ {\it disjoint} sets $T_{\ell}=\{c^{\ell}, d_1^{\ell},\cdots, d^{\ell}_{k}\}$, $\ell=1,2, \ldots L$, such that $c^{\ell}\in C$ and $d_j^{\ell}\in D$. We define $f(T_{\ell}):=2k$ for all $\ell=1,\ldots, L$.
%\scomment{infinite number of such sets? or will $L$ suffice?} 
%\mcomment{in the definition of function it should be infinite but in the input we use $n/2k$ of them}
%\scomment{After going through the proof, I don't see why you need infinite number, it seems just $L=n/2k$ will suffice. Where are you using that there are infinte number of $T^\ell$?}
%\mcomment{
%The reason is that you should give one functions $f$ that works for all $n$. Otherwise one may claim that for any given function $f$ there is large enough $N_f$ so that we can go beyond 7/8, for $n>N_f$. 
%}
Now, let
$$g(t):=k+\frac{k}{2}+\cdots+ \frac{k}{2^{i-1}} + \frac{(t-ik)}{2^i},$$
where $i=\floor{t/k}$. It is easy to see that $g$ is a monotone submodular function. 

Now, define $f$ on the remaining subsets of the ground set as follows. For all $S$ with $|S|\ge 1$, 
\begin{itemize}
\item $|S\cap C| \ge 2 \implies f(S):=2k+1$
\item $|S\cap C|=0 \implies f(S):=1+g(|S|-1)$
\item $|S\cap C|=1$ $\implies S\cap C=\{c^\ell\}$ for some $\ell\in [L]$   $\implies$
%$$f(S):=\min\{2k+1, k+\frac{1}{2} g(|S|-1)+\frac{k'}{2} (g(|S|-1)-g(|S|-2))\},$$ 
%$$f(S):=\min\{2k+1, k+\frac{1}{2} g(|S|-1)+\frac{k'}{2^{i+1}}\},$$ 
$$f(S):= \min\{2k+1, k+\frac{1}{2} g(|S|-1)+\frac{k'}{2^{i+1}}\},$$ 
%\mcomment{so can we remove min above? }\scomment{yes, actually, you don't use $f(S)\le 2k+1$ anywhere, do you?} 
where $k'=|S\cap\{d^{\ell}_1,\cdots, d_k^{\ell}\} |$, $i=\lfloor(|S|-1)/k\rfloor$.
\end{itemize}

%\scomment{$i$ was not defined in above, please check if I defined it correctly.}
%\mcomment{yes}
%\scomment{isn't the first case in the below gone now?}
%\mcomment{no why?} \scomment{because all items in $C$ are $c^\ell$ for some $\ell$}
%\mcomment{yes correct}
%\scomment{removed below
%\begin{itemize}
%\item ..
%\begin{itemize}
%\item $S\cap C\notin\{c^{\ell}\}_{\ell=1, \ldots, L} \implies f(S):=k+\frac{1}{2} g(|S|-1)$
%\item $S\cap C= \{c_1^{\ell}\}$ for some $\ell$  $\implies f(S):=\min\{2k+1, k+\frac{1}{2} g(|S|-1)+k'/2^{i+1}\}$, where $k'=|S\cap\{d^{\ell}_1,\cdots, d_k^{\ell}\} |$.
%\end{itemize}
%\end{itemize}
%}
%Observe that for any subset $S$, $f(S)\le 2k+1$. 
Observe that since $g(k)=k$, for any subset $S$ of size at most $k+1$, we have $f(S)\le k+\frac{k}{2} + \frac{k}{2} = 2k$.

\begin{lemma}
$f$ is a monotone submodular function.
\end{lemma}
\begin{proof}
We have to show that for any item $x$ and subsets $S\subseteq T$, $\Delta_f(x|S) \ge \Delta_f(x|T)$.
We consider the following cases:
\begin{itemize}
\item if $|T\cap C| \ge 2 \implies \Delta_f(x|T)=0$, so it is trivial.
\item if $|T\cap C| =0 \implies |S\cap C|=0 \implies \Delta_f(x|S) \ge \Delta_f(x|T)$ because of submodularity of $g$.
\item if $|T\cap C|=1 \implies |S\cap C|\le 1$
\begin{itemize}
\item if $|S\cap C|=1 $ then $S\cap C = T\cap C = \{c^{\ell}\}$ for some $\ell$:
\begin{itemize}
\item $x\in \{d_1^{\ell},\cdots, d_k^{\ell}\} \implies \Delta_f(x|S)=1/2^{i+1}+1/2^{i+1}$ for $i=\lfloor (|S|-1)/k\rfloor$, and $\Delta_f(x|T)=1/2^j+1/2^j$ for some $j=\lfloor (|T|-1)/k\rfloor$ and $j\ge i+1$.
\item $x\notin \{d_1^{\ell},\cdots, d_k^{\ell}\} \implies \Delta_f(x|S)=1/2^{i+1}$ for $i=\lfloor (|S|-1)/k\rfloor$ and $\Delta_f(x|T)=1/2^j$ for some $j\ge i+1$.
\end{itemize} 
%\item $S\cap C = T\cap C \notin \{c_1^{\ell}\}_{\ell} \implies \Delta_f(x|S) \ge \Delta_f(x|T)$ because of submodularity of $g$.

\item if $|S\cap C|=0 \implies \Delta_f(x|T) \le 1/2^{j+1}+1/2^{j+1}$ for $j=\lfloor (|T|-1)/k\rfloor$ and $\Delta_f(x|S)= 1/2^i$ for some $i\le j$. 
\end{itemize}
Thus $\Delta_f(x|S) \ge \Delta_f(x|T)$.
\end{itemize} 
Monotonicity follows trivially from the definition of $f$.
\end{proof}

\toRemove{
Also for any subset of $S$ with at least two elements of $C$, $f(S)=2k$. 
For subset $S$ with no element in $C$, if $i=\floor*{\frac{|S|}{k}}$, 
$f(S)$ is defined as 
\[
f(S)= k+k/2+ \dots +(|S|-ik)/2^{i}.
\]
For subset $S$ with exactly one element $c\in C$ such that $c\neq c_1$, if if $i=\floor*{\frac{|S|-1}{k}}$, 
$f(S)$ is defined as 
\[
f(S)= k+ k/2+ \dots +(|S|-1-ik)/2^{i+1}.
\]
Thus if $|S|=k+1$ and it contains exactly one element of $c\in C$ such that $c\neq c_1$ then $f(S)=k+k/2$.
Now suppose $S$  contains $c'$. 
For $S=T$, $f(S)=2k$.  Suppose $S$ contains $k'<k$ elements of $\{b_1, \dots, b_k\}$  and $\ell$ other elements of $D$. 
Let's $t=k'+\ell$, and $i=\floor*{\frac{t}{k}}$, then
\[
f(S)= \min\{2k, k'/2+(k+ k/2+ \dots +(t-ik)/2^{i+1})\}
\]
}
%\scomment{this proof is very vague, especially the claim any algorithm will select $k/2$ of $D$? Phrases like algorithm is not "aware" of something cannot be stated as a fact. You need to prove that the algorithm will not be able to distinguish between the two scenarios. We need to discuss.}



%Let $ {\cal T}^L$ be a collection of (any) $L=n/2k$ sets from $T^\ell, \ell=1,2, \ldots$. W.l.o.g., let's assume ${\cal T}^\ell = \{T_1, \ldots, T_L\}$.   

Now, denote $D^{\ell} := T^\ell \cap D = \{d_1^{\ell},\cdots, d_k^{\ell}\}$ for $\ell=1,2, \ldots, L$. Also, let 
$D'=D\setminus (\bigcup_{\ell=1}^L D^{\ell})$. % where $L:=n/2k$. 
%\scomment{Do you need $T^\ell, \ell =1,\ldots, L$ to be disjoint?} \mcomment{yes}
% $B'=B\setminus (\bigcup_{\ell }^{L} B^{\ell})$ for $L:=n/2k$.
Now define $L$ input instances $\{I_{\ell}\}_{\ell =1,\ldots, L}$, each of size $n$, as follows. For
any arbitrary subset $\tilde{D}\subseteq D'$ of size $n-Lk-1$, 
%\scomment{Which subset $\tilde{B}$? any arbitrary subset?} \mcomment{arbitrary}
define $I_{\ell}=\bigcup_{i=1,\ldots, L}  D^{i} \cup \tilde{D} \cup \{c^{\ell}\}$, for  $\ell=1,\ldots, L$.
%and $I_2=B^1 \cup B^2 \cup \tilde{B} \cup \{a_1^2\}$ (the difference is $a_1^1$ and $a_1^2$).
%Now suppose the input consists of the following:  $T^{\ell}=\{a_1^{\ell}, b_1^{\ell}, \cdots b_k^{\ell} \}$, no other element of $C$ and the remaining elements are from $B':=B\setminus \{b_1^{\ell}, \cdots, b_k^{\ell}\}$. 
Thus, for instance $I_{\ell}$, the the optimal $k+1$ subset is $T^\ell$ with value $f(T^{\ell})=2k$. 
%\scomment{earlier we stated $T^\ell$ is optimal, but we have never proven that none of the $k+1$ subset can take value $2k+1$. We actually do not need to show $T^\ell$ is optimal.}
%\scomment{$T^\ell$ is of size $k+1$, optimal should be of size $k$. If making $T_\ell$ to be of size $k$ makes it messy, you can initially state that you will consider submodular $k+1$ secretary problem.}


Now consider any algorithm for the submodular \nameSecSL\ and cardinality constraint $k+1$. We denote by $Alg$ the set of $\eta(k+1)$ items selected by the algorithm as part of the shortlist. % (all elements in the shortlist of size $\eta(k)$).
%\scomment{We have  used $C$ to denote shortlist in the algorithm. May be you can use a different symbol instead of type $A$ and $B$. }
Let $\bar I$ denote an instance chosen uniformly at random from $I_\ell, \ell=1,\ldots, L$.  
%We choose one of $I_{\ell}$ randomly. \scomment{randomly or arbitrarily?} 
Let $\pi$ denote a random ordering of $n$ items in $\bar I$. 
%We give a random order of $I_{\ell}$, say $\pi$ to the algorithm as input,
%(note that in the secretary problem the elements of input can be selected adversarially but the order should be random).
We denote by random variable $(\bar{I},\pi)$ the randomly ordered input instance to the algorithm. Also we denote by $\bar{T}, \bar{D}$ and $\bar c$, the corresponding $T^{\ell}$, $D^{\ell}$ and $c^\ell$.

Now we claim 

%Note that algorithm is not aware of $\ell$.
%Consider an algorithm $Alg$.
%Suppose $a_1^{\ell}$ is the $t$-th elements in the input, and
%elements of input are ordered as $I=(I_1,\cdots, I_n)$.
%Suppose $Alg$ is the set of elements selected by an algorithm.
%Denote by $\bar{B}=\{b_1,\cdots, b_k\}$.

\begin{lemma}
$\mathbb{E}_{(\bar{I},\pi)}[|Alg\cap \bar{D}|] \le k/2+\eta(k+1)/L$.
\end{lemma}
\begin{proof}
Suppose $(e_1,\cdots, e_n)$ indicates the ordered input according to random ordering $\pi$ on $\bar{I}$. %for some $0<\ell<L$.
Now let $t$ be the random variable indicating the index of $c^{\ell}$ in $(e_1,\cdots, e_n)$, i.e., $e_t=c^{\ell}$. 
%Define $R:=\mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}|]$.
Then, due to random ordering, and random choice of $\bar I$ from $I_1, \ldots, I_\ell$, we have
$$\mathbb{E}_{(\bar I, \pi)}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap D^1|]= \cdots = \mathbb{E}[|Alg\cap\{e_1,\cdots, e_{t-1}\}\cap D^{L}|]\ .$$
Also, since $D^\ell, \ell=1,\ldots, L$ are disjoint,
$$\sum_{\ell=1}^L \mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap D^{\ell}|] \le \eta(k+1)\ .$$
Since $\bar D=D^\ell$ with probability $1/L$,  we have
$$H:=\mathbb{E}[|Alg\cap\{e_1,\cdots, e_{t-1}\}\cap \bar{D}|]=  \frac{1}{L} \sum_{\ell=1}^L \mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap D^{\ell}|] \le \frac{1}{L} \eta(k+1)\ . $$ 
%\rightarrow 0$ as $n/\eta(k) \rightarrow \infty$.
Now define
$G:=\mathbb{E}[|Alg\cap\{e_t,\cdots, e_{n}\}\cap \bar{D}|]$.
We have
$$G\le \mathbb{E} [|\bar{D}\cap\{e_t,\cdots, e_n\}|]  \le k/2\ .$$
%Also define $H:=\mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\cap \bar{B}\}|]$.
%Also, $H\le k-G$.
Thus $$\mathbb{E}[|Alg\cap \bar{D}|] \le G+H\le k/2+\eta(k+1)/L\ .$$
%\rightarrow G$$
%\le k/2$$
%G+(k-G)/2 \le k/2+G/2\le k/2+k/4=3/4k$$.
\end{proof}
Now on input $\bar{I}$, if the algorithm doesn't select $\bar c$ as part of shortlist $Alg$, then by definition of $f$ for sets that do not contain any item of type $C$, we have 
$$f(A^*):=\max_{S \subseteq Alg:|S|\le k+1} f(S) \le 1+ g(k) = k+ \frac{k}{2}$$ 

Otherwise, if algorithm selects $\bar c$ then by definition of $f$ 
$$f(A^*):=\max_{S \subseteq Alg:|S|\le k+1} f(S) \le \max_{S \subseteq Alg \backslash (\bar D \cup \{\bar c\}):|S|\le k-|Alg \cap \bar D|} f(S \cup \bar D \cup \{\bar c\}) 
= k+ \frac{k}{2} +\frac{1}{2} |Alg\cap \bar{D}|$$ 
therefore $$\mathbb{E}[f(A^*)] \le k+\frac k 2+ \frac k 4+ \frac{\eta(k+1)}{2L} = \frac{7k}{4} + \frac{k\eta(k+1)}{n} \ .$$

%Hence $\mathbb{E}[f(Alg)]  \rightarrow k+k/2+k/4$ as $n\rightarrow \infty$, since $\eta(k)=o(n)$.
Since the optimal is equal to $\Ex[f(\bar T)]=2k$, the competitive ratio is upper bounded by
$$ 
%\left(\frac{7k}{4} + \frac{k\eta(k)}{n}\right)\left/\right. 2k = 
\frac{7}{8} + \frac{\eta(k+1)}{2n}$$

This proves competitive ratio upper bound of $\frac{7}{8} + o(1)$ when $\eta(k+1)=o(n)$, to complete the proof of Theorem \ref{hardness}.
%\scomment{I think we need to change the upper bound in theorem statement to $7/8 + o(1)$}
%Before arriving $a_1^{\ell}$ algorithm can not distinguish between elements of $B'=\{b_1^{\ell},\dots, b_k^{\ell}\}$
%and the rest of $D$ thus the expected number of elements in $B'$ selected by algorithm before observing $a_1$ goes to $0$ as $n/k\rightarrow \infty$.

%Therefore an online algorithm would select $k/2$ elements of set $B'$ in expectation and also it selects $a_1^{\ell}$ (and $k/2$ other elements from $B\setminus B'$).  Therefore, its $f$ value is $k+k/2+k/4$.
%Hence the competitive ratio is at most $7/8$.


==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/introduction.tex <==
%\section{Introduction}



In the classic \textit{secretary problem}, 
$n$ items appear in random order.  We know $n$, but don't know the value of an item until it appears.   
Once an item arrives we have to irrevocably and immediately decide whether or not to select it. Only one item is allowed to be selected, and the objective is to  select the most valuable item, or perhaps to 
%\ccomment{Is this really equivalent, or just related}
%\mcomment{not equivalent but related. }
maximize the expected value of the selected item  
%The origin of the secretary problem is hard to track
~\cite{Dynkin:SovMath:1963,ferguson1989solved, 10.2307/2985407}. 
It is well known that the optimal policy is to observe the first $n/e$ items without making any selection and then select the first item whose value is larger than the value of the best item in the first $n/e$ items~\cite{Dynkin:SovMath:1963}. This algorithm, given by ~\citet{Dynkin:SovMath:1963},
is asymptotically optimal, and hires the best secretary with probability at least $1/e$. Hence it
is also $1/e$-competitive for the expected value of the chosen item, and
%\ccomment{Is this true?}
%\mcomment{Yes, but the original paper shows the probability not the expectation Dynkin provided an asympotically optimal algorithm for this problem, which hires the best secretary with probability at least 1/e}
it can be shown that no algorithm can beat $1/e$-competitive ratio in expectation.
%

Many variants and generalizations of the secretary problem have been studied in the literature, see e.g., \cite{Ajtai:2001,WILSON1991325,vanderbei1980optimal, wilson1991optimal, kleinberg, Babaioff:2008}.  
%\ccomment{We should have more variants hear} The secretary problem has been generalized.  
\cite{kleinberg, Babaioff:2008} introduced a 
{multiple choice secretary problem}, where the goal is to select $k$ items in a randomly ordered input so as to maximize  the {\it sum} of their values; and  \citet{kleinberg} gave an algorithm with an asymptotic competitive ratio of $1-O(1/\sqrt{k})$. Thus as $k\to \infty$, the competitive ratio approaches  1. Recent literature studied several generalizations of this setting to multidimensional knapsacks \cite{moser1997algorithm}, and proposed algorithms for which the expected online solution approaches the best offline solution as the knapsack sizes becomes large~(e.g., \cite{FHKMS10, devanur-hayes, AgrawalWY14}). 
%\scomment{add citations, Cliff's paper, Devanur and Hayes, my paper on online linear programming etc.}
%\ccomment{I added some of these references to bibtex to the bib file because I had it handy.  Mohammad, you need to add the text and references.}
%\ccomment{Does multiple choice secretary only refer to the case of sum?}
%\mcomment{no it can be any function}


In another variant of multiple-choice secretary problem, \citet{Bateni} and ~\citet{Gupta:2010} introduce 
the \textit{\nameOfProblem}. In this secretary problem, the algorithm again selects $k$ items, but 
the value of the selected items is given by a monotone submodular function 
%It is an online variant of monotone submodular maximization subject to cardinality constraints. 
%The objective function is designed by an adversary, but the order of the items is uniformly at random.
$f$. The algorithm has a value oracle access to the function, i.e., for any given set $T$, an algorithm can query an oracle to find its value $f(T)$~\cite{oracle}.
The algorithm can select at most $k$ items $a_1 \cdots, a_k$, from a randomly ordered sequence of $n$ items. The goal is to maximize $f(\{a_1,\cdots, a_k\})$.
%Now imagine we are allowed to select several items instead of one item. Would that let us to improve $1/e$?
%Assuming a value oracle access to the submodular function; i.e., for a given set $T$, an algorithm can query an oracle to find its value $f(T)$~\cite{oracle}.
Currently, the best result for this setting is due to ~\citet{kesselheim}, who achieve a $1/e$-competitive ratio in exponential time, or $\frac{1}{e}(1-\frac{1}{e})$ in polynomial time. In this case, the offline problem is NP-hard and hard-to approximate beyond the factor of $1-1/e$ achieved by the greedy algorithm \cite{nemhauser1978best}. 
%\scomment{need a reference for lower bound of $1-1/e$ for offline monotone submodular maximization}
However, it is unclear if a competitive ratio of $1-1/e$ can be achieved by an online algorithm for the {\nameOfProblem} even when $k$ is large. 

\paragraph{Our model: \nameSecSL.}
In this paper, we consider a relaxation of the secretary problem 
%.  What if  the online algorithm for secretary problem 
where the algorithm is allowed to  select a {\it shortlist} of items that is larger than the number of items that ultimately need to be selected. That is, in a multiple-choice secretary problem with cardinality constraint $k$, the algorithm is allowed to choose more than $k$ items as part of a shortlist. Then, after seeing the entire input, the algorithm can choose a subset of size $k$ from the bigger set of items in the shortlist. 
%when seeing items online, and ultimately maximizes a function of $k$ elements, 
%we are allowed to choose more than $k$ elements, and then after seeing the entire input, choose a  a subset of size $k$ from our bigger set.  

This new model is motivated by some practical applications of secretary problems, such as hiring (or assignment problems),  where in some cases it may be possible to tentatively accept a larger number of candidates (or requests), while deferring the choice of the final $k$-selections to after all the candidates have been seen. Since there may be a penalty for declining candidates who were part of the shortlist, one would prefer that the shortlist is not much larger than $k$.

Another important motivation is theoretical: we wish to understand to what extent this relaxation of the secretary problem can improve the achievable competitive ratio. This question is in the spirit of several other methods of analysis that allow an online algorithm to have additional power, such as {\em resource augmentation} \cite{KalyanasundaramP00,PhillipsSTW97}.

The potential of this relaxation is illustrated by the basic secretary problem, where the aim is to select the item of maximum value among randomly ordered inputs. There, it is not difficult to show that if an algorithm  picks every item that is better than the items seen so far, the true maximum will be found, while the expected number of items picked under randomly ordered inputs will be $\log(n)$. Further, we show that this approach can be easily modified to get the maximum with $1-\epsilon$ probability while picking at most  $O(\ln(1/\epsilon))$ items for any constant $\epsilon>0$. Thus, with just a constant size shortlist, we can break the $1/e$ barrier for the secretary problem and achieve a competitive ratio that is arbitrarily close to $1$.

%For the secretary problem, we can imagine choosing not one secretary, but several, and then taking the best one at the end.  
Motivated by this observation, we ask if a similar improvement can be achieved by relaxing the \nameOfProblem~to allow a shortlist. That is, instead of choosing $k$ items, the algorithm is allowed to chose  $\eta(k)$ items as part of a shortlist, for some function $\eta$;
and at the end of all inputs, the algorithm chooses $k$ items from the $\eta(k)$ selected items. Then, what is the relationship between $\eta(\cdot)$ and the competitive ratio for this problem? Can we achieve a solution close to the best offline solution when $\eta(k)$ is not much bigger than $k$, for example  when 
 $\eta(k)=O(k)$?  

%We answer this question affirmatively in this paper, and provide an algorithm 
%What is the relationship between $\eta$ and the competitive ratio. 
%In other words, we have a {\em shortlist} of size $\eta(k)$, where $\eta(k)$ is independent of $n$, and the output is subset of this shortlist.
%We wish to understand how much this relaxation can improve the competitive ratio.   In other words, what is the relationship between $\eta$ and the competitive ratio.
 
%For exmaple, when the  it is possible to approach the optimal offline solution by some function $\eta$ as $k\to \infty$.  Can we obtain a similar results for the \nameOfProblemSL.


%\ccomment{Is there a practical-ish motivation for this model?}
%A motivation for this model is that for the $k$-secretary problem instead of restricting ourselves to make irrevocable decisions for each item, we may add items to a shortlist and defer the final decision to the end (choosing $k$ elements from shortlist). We want the size of shortlist to be as small as possible.

In this paper, we answer this question affirmatively by giving a polynomial time algorithm that achieves $1-1/e-\epsilon-O(k^{-1})$ competitive ratio for the \nameOfProblem~using a shortlist of size $\eta(k)=O(k)$. This is surprising since $1-1/e$ is the best achievable approximation (in polynomial time) for the offline problem. Further, for some special cases of submodular functions, we demonstrate that an $O(1)$ shortlist allows us to achieve a $1-\epsilon$ competitive ratio. These results demonstrate the power of (small) shortlists for closing the gap between online and offline (polynomial time) algorithms. 
%size we give a new algorithm and show several positive (and one negative) results that capture the power of these shortlists and  show that they are (surprisingly) powerful. 

We also discuss connections of {\nameSecSL} to the related streaming settings. While a streaming algorithm does not qualify as an online algorithm (even when a shortlist is allowed), we show that our algorithm can in fact be implemented in a streaming setting to use $\eta(k)=O(k)$ memory buffer; and our results significantly  improve  the available results for the \streamingProblem.
Furthermore since the upperbound given in ~\cite{mcgregor2017better} holds for random order streams, our result is asymptotically tight in this setting.

\subsection{Problem Definition}
%In the well-studied submodular $k$-secretary problem, applicants from a set ${\cal U} = \{a_1, a_2, \ldots, a_n\}$  (pool of applicants) arrive in a uniformly random order over $n$ sequential rounds. In each round, an online algorithm irrevocably decides whether to select an applicant or not. The algorithm can select at most $k$ applicant. The goal is to maximize the value of the selected $k$ applicants, as given by a submodular function $f$. 

%More formally, let $S, |S|\le k$ denote the subset of candidates selected by the algorithm, then the expected utility of the algorithm is given by $\ALG:=\Ex[f(S)]$, where $f$ is a monotone submodular function, and the expectation taken both over random order and possible randomness in the algorithm's selection of subset $A$ given an order. The competitive ratio of the online algorithm is then defined as $\frac{\ALG}{\OPT}$, where $\OPT$ is the optimal offline utility defined as 
%$$\OPT=f(S^*), \text{ where, } S^*=\arg \max_{S \subseteq [n], |S|\le k} f(S).$$

%\scomment{edited by me on 8/21}
We now give a more formal definition.
Items from a set ${\cal U} = \{a_1, a_2, \ldots, a_n\}$  (pool of items) arrive in a uniformly random order over $n$ sequential rounds. The set ${\cal U}$ is apriori fixed but unknown to the algorithm, and the total number of items $n$ is known to the algorithm. In each round, the algorithm irrevocably decides whether to add the arriving item to a {\it shortlist} $A$ or not. %The goal is to return,  at the end of $n$ rounds, a shortlist $A$ of size at most $\eta(k) \ge k$ to maximize the  `value' of best $k$ subset of this shortlist. More formally, 
%We are given a monotone submodular function $f:2^{\cal U} \rightarrow \mathbb{R}$, in a value oracle model. %Let the set $A \subseteq {\cal U}, |A|\le \eta(k)$ denote the shortlist of items selected by the online algorithm,  then 
The algorithm's value at the end of $n$ rounds is given by 
$$\ALG = \Ex[\max_{S\subseteq A, |S|\le k} f(S)]$$ 
where $f(\cdot)$ is a monotone submodular function. The algorithm has value oracle access to this function.

The optimal offline utility is given by
$$\OPT:=f(S^*), \text{ where } S^*=\arg \max_{S \subseteq [n], |S|\le k} f(S).$$ 
We say that an algorithm for this problem achieves a competitive ratio  $c$ using shortlist of size $\eta(k)$, if at the end of $n$ rounds, $|A|\le \eta(k)$ and $\frac{\ALG}{\OPT}\ge c$.

Given the shortlist $A$, since the problem of computing the solution $\arg \max_{S\subseteq A, |S|\le k} f(S)$ can itself be computationally intensive, our algorithm will also track and output a subset $A^* \subseteq A, |A^*| \le k$. We will lower bound  the competitive ratio by bounding $\frac{f(A^*)}{f(S^*)}$.

The above problem definition has connections to some existing problems studied in the literature. The well-studied online \nameOfProblem~described earlier is obtained from the above definition by setting $\eta(k)=k$, i.e., it is same as the case when no extra items can be selected as part of a shortlist. 
%\scomment{Did a pass on the para below on 8/30 after our discussion regarding streaming problem}
Another related problem is {\it  \streamingProblem}~studied in~\cite{norouzi}. In this problem, items from a set $\cal U$ arrive online in random order and the algorithm aims to select a subset $S \subseteq {\cal U}, |S|\le k$ in order to maximize $f(S)$. The streaming algorithm is allowed to maintain a {\it buffer} of size $\eta(k)\ge k$. 
However, this streaming problem is distinct from the \nameOfProblemSL\ in several important ways. On one hand, since an item previously selected in the memory buffer can be discarded and replaced by a new items, a memory buffer of size $\eta(k)$ does not imply a shortlist of size at most $\eta(k)$. On the other hand, in the secretary setting, we are allowed to memorize/store more than $\eta(k)$ items without adding them to the shortlist. Thus an algorithm for \nameOfProblem with shortlist of size $\eta(k)$ may potentially use a buffer of size larger than $\eta(k)$. 
Our algorithms, as described in the paper, do use a large buffer, but we will show
%\ccomment{Where do we show that the streaming actually works}
that the algorithm presented in this paper can in fact be implemented to use only $\eta(k)=O(k)$ buffer, thus obtaining matching results for the streaming problem. 
%imply the same competitive ratio for random order streaming problem with buffer of size $\eta(k)$, but not vice-versa. We will discuss the corollary of our algorithm design and analysis for the  submodular random order streaming problem. 
%Because shortlists can be used as a buffer for memory but not vice versa. ( we are allowed to delete from memory and reduce the size but we can not remove from a shortlist)







%In the new `submodular $k$-secretary with shortlist' problem considered in this paper, we allow the online algorithm to select a shortlist of more than $k$ candidates, and pick the final subset of $k$ candidates from this shortlist at the end. Specifically,  we allow the online algorithm to select a subset $A$ of size $|A|\le \eta(k)$, where $\eta(k)\ge k$. The competitive ratio of the online algorithm is then defined with respect to the best $k$-subset of $A$. That is, competitive ratio is given by $ \frac{\ALG_{\eta}}{\OPT}$, where $\OPT$ as defined before, and 
%$$\ALG_\eta = \Ex[\max_{S\subseteq A, |S|\le k} f(S)],$$ 
%with $A$ being the subset of items selected by the online algorithm, of size at most $\eta(k)$. 

\subsection{Our Results}
Our main result is an online algorithm  for \nameOfProblemSL\ that, for any constant $\epsilon>0$, achieves a competitive ratio of $1-\frac{1}{e} - \epsilon-O(\frac{1}{k})$ with $\eta(k) = O(k)$. 
Note that for \nameOfProblem\ there is an upper bound of $1-1/e$ on the achievable aproximation factor, even in the offline setting, and this upper bound applies to our problem for arbitrary size $\eta(\cdot)$ of shortlists. On the other hand for online monotone \nameOfProblem, i.e., when $\eta(k)=k$, the best competitive ratio achieved in the literature is $1/e-O(k^{-1/2})$~\cite{kesselheim} 
%\scomment{is there an upper bound? } \mcomment{ No} 
Remarkably, with only an $O(k)$ size shortlist, our online algorithm is able to achieve a competitive ratio that is arbitrarily close to the offline upper bound of $1-1/e$.

In the theorem statements below, big-Oh notation $O(\cdot)$ is used to represent asymptotic behavior with respect to $k$ and $n$. We assume the standard  value oracle model:  the only access to the submodular function is through a black box
returning $f(S)$ for a given set $S$, and  each such queary can be done in $O(1)$ time. 
%\ccomment{Define value oracle model and state thm.1 appropriately}
\begin{theorem} \label{opttheorem}
For any constant $\epsilon>0$, there exists an online algorithm (Algorithm \ref{alg:main}) for the \nameOfProblemMatroidSL\ that achieves a competitive ratio of $1-\frac{1}{e} -\epsilon -O(\frac{1}{k})$, with shortlist of size $\eta_\epsilon(k)=O(k)$. Here,  $\eta_\epsilon(k)=O(2^{poly(1/\epsilon)}k)$.  
%$$\eta_\epsilon(k) =c k\log(1/\epsilon) {\frac{1}{\epsilon^3} \log(1/\epsilon)  \choose {\frac{1}{\epsilon^2} \log(1/\epsilon)}} =O(2^{poly(1/\epsilon)}) \ ,$$
%for some absolute constant $c$.
% for submodular secretary problem with cardinality constraints, such that it selects $O(k)$ elements. %, where $C(a)$ is a constant depending only on $a$.
  The running time of this online algorithm is $O(n)$.
\end{theorem}
%\scomment{Can we add a compact description of dependence of  $\eta_\epsilon(k)$ on $\epsilon$ in this theorem statement? What is this function: exponential or super-exponential in $1/\epsilon$?}
%\scomment{Should we say $O(n)$ evaluations of the objective function instead of time?}
%\scomment{After fixing the proof in section 3, I am getting a different (much bigger) dependence on $1/\epsilon$. Mohammad, can you check? May be considering this, we should leave it here as $\eta_\epsilon(k)=O(2^{poly(1/\epsilon)}$?}
%\scomment{I see that the theorem statement was changed, but we still need to provide the exact function, may be right after the theorem statement. Adding below:}

%Specifically, we have $\eta_\epsilon(k)=$\etaMacro$k$ for some constant $c$.
%The running time  of our algorithm is linear in $n$, the size of the input, which 
%is significant as, until recently, it was not known if there exists a linear time algorithm achieving a $1-1/e-\epsilon$ approximation even for the offline monotone submodular maximization problem under cardinality constraint\cite{linear}. 
Similar to~\cite{us}, an interesting aspect of our algorithm is that it is highly parallel. Even though the decision for each arriving item may take time that is exponential in $1/\epsilon$ (roughly  $\eta_\epsilon(k)/k$), it can be readily parallelized among multiple (as many as $\eta_\epsilon(k)/k$) processors. 
%The  operations required to make a decision for each item can be divided between available processors. (the running time will be divided by $\min(c,p)$ where $c=k\log(1/\delta) {\frac{1}{\delta^3} \log(1/\delta)  \choose {\frac{1}{\delta^2} \log(1/\delta)}}$ is the hidden constant in $O(k)$ and $p$ the number of processors )


%More precisely, we design a $1-1/e-\epsilon-O(k^{-1})$ competitive algorithm that selects $O(k\log(1/\delta) {\frac{1}{\delta^3} \log(1/\delta)  \choose {\frac{1}{\delta^2} \log(1/\delta)}})$ elements, i.e., the dependency on $k$ is linear and on $\delta$ is exponential.



%\scomment{Add a formal corollary of Theorem 1 for random-order streaming problem here. Also, will be good to add a few lines in problem definition section describing how our problem relates to random order streaming.} \mcomment{done done}


%As discussed earlier, by definition, a corollary of our results is an algorithm for the submodular random order streaming problem with the same competitive ratio.
Further, we show an implementation of Algorithm 2 that uses a memory buffer of size at most $\eta_\epsilon(k)$ to get the following result for the problem of {\it \streamingProblem} described in the previous section. 
%\ccomment{Make terminology for evaluations consistent with previous work}
\begin{restatable}{theorem}{thmStreaming}
\label{thm:streaming}
For any constant $\epsilon\in (0,1)$, there exists an algorithm for the \streamingProblem  that achieves $1-\frac{1}{e} -\epsilon -O(\frac{1}{k})$ approximation to $\OPT$ while using a memory buffer of size at most $\eta_\epsilon(k)=O(k)$. Also, the number of objective  function evaluations for each item, amortized over $n$ items, is $O(1+\frac{k^2}{n})$.
%Also, decision for each arriving item requires $O(1)$ evaluations of the objective function.
%Also in amortized time, it processes each arriving item with $O(1+\frac{k^2}{n})$ evaluations of the objective function.
%Also the amortized time to processes each arriving item requires $O(1+\frac{O(k^2)}{n})$ evaluations of the objective function.
% The running time of this online algorithm is $O(n)$.
\end{restatable}
%The above result significantly improves over the state-of-the-art results in random order streaming model \cite{norouzi}, which are an approximation ratio of $\frac 1 2+8\times 10^{-14}$ using a memory of size $O(k\log k)$. 
%uses $O(k)$ memory and achieves asymptotic $R<1-1/e$ approximation.

%\scomment{I don't understand the upper bound stated below - by arbitrary $\eta$, couldn't we get at best the the offline problem. I can just select everything into shortlist. So, is the below giving an upper bound for the offline problem?  } \mcomment{using $o(n)$ selections. No it is for online problem}

%As a result, we show that in our model $\eta(k)=\gamma.k$, where $\gamma$ is a constant. It is optimal up to a constant factor.
%The constant factor $\gamma$ is growing as the competitive ratio gets closer to $1-1/e$. 
%Because of the known upper bound for offline submodular maximization with cardinality constraint.
%It is obvious that we can not get better than $1-1/e$ competitive algorithm if we only consider  polynomial time algorithms. 

%It is natural to ask whether these $k$-lists are, in fact, too powerful.  Maybe they could actually allow us to always match the best offline algorithm.  We give a negative result in this direction and 
%show that even if we have unlimited computation power, for any function $\eta(k)=o(n)$, we can get no better than $7/8$-competitive algorithm using a shortlist of size $\eta(k)$. Note that with unlimited computational power, the offline problem can be solved exactly. This result demonstrates that 
%having a shortlist does not make the online problem too easy - 
%even with a shortlist (of size $o(n)$) there is an information theoretic gap between the online and offline problem. Note that the $1-1/e$ upperbound for streaming model~\cite{mcgregor2017better} 
%does not imply an upper bound for the shortlist model.

\toRemove{
%\mcomment{we should emphasize the upper bound is for any $k$, i.e., it holds asymptotically}
\begin{restatable}{theorem}{hardness}
%\begin{theorem} 
\label{hardness}
No online algorithm (even with unlimited computational power)   can achieve a competitive ratio better than $7/8+o(1)$ for the \nameOfProblemSL, while using a shortlist of size $\eta(k)=o(n)$.
%by selecting $\eta(k)$ elements for any function $\eta$ (independent of $n$).
\end{restatable}
%\end{theorem}

%\scomment{By independent of $n$, do you mean $\eta(k)$ does not grow with $n$, i.e., $\eta(k)=O(1)$ if $O(\cdot)$ denotes asymptotic with respect to $n$? This is not same as $o(n)$, e.g.. $\eta(k)=\sqrt{n}$ would also be $\eta(k)=o(n)$.} \scomment{We need to discuss this issue}
 
 % It also improves~\cite{Badanidiyuru2014StreamingFly} on random order inputs.
%(Note that in our algorithm we keep extra items in the shortlist only for a limited time $O(n/k)$, and then we are able to release them.
%That is why the extra memory is $O(1)$ instead of $O(k)$).

%Another interesting aspect of our algorithm is that it is highly parallel. In order to decide whether or not to select an item in a slot $s_i$ in window $W$ which consists of $\{s_1, \dots, s_{\alpha \beta}\}$,
%the algorithm concurrently run several online maximum algorithms to find the maximum marginal value with respect to %different subsets.
% $S\cup \gamma(\tau)$, where $\tau$ is a subset of slots $\{s_1,\dots, s_{i-1}\}$ with $|\tau|<\alpha$.
%We select a new item if any of the maximum algorithms (for some $\tau$) select it, otherwise we do not select it. All the maximum algorithms for different subsets $\tau$ can be run in parallel. 

%Although the update time in our algorithm is $O(1)$, the constant can be very large. Consequently it may not be desirable for large streams. 
%We take two approaches to improve it. The first approach is parallel algorithms. The interesting fact about our algorithm is that it is highly parallel, i.e. the  operations required for each element can be divided between as many processor as it is available. 
%The running time will be divided by the number of processors. 

%In addition, we design a fast  thresholding algorithm that requires only one function evaluation per element.
%It achieves competitive ratio $1/2-O(1/\sqrt{k})$ by selecting $k\log^2k$ elements. The competitive ratio and the update time of this algorithm is still better than~\cite{kesselheim} and~\cite{Hess}. In ~\cite{kesselheim}  update time is $O(n^2)$. 
%In terms of memory, our thresholding algorithm uses less memory than~\cite{Badanidiyuru2014StreamingFly} but more than~\cite{Hess}.


%We also provide an upper bound showing that it is not possible to achieve any competitive ratio better than $7/8$ by selecting $O(g(k))$ elements, where $g$ is an arbitrary function, even if we have free computation.
%\scomment{Can you add a theorem statement for the results discussed below?} \mcomment{added}
Finally, for some special cases of monotone submodular functions, we can asymptotically approach the optimal solution.
%\ccomment{Don't mention this as a thm.}
%\begin{theorem}
%Suppose $F$ is a monotone submodular function and $F(a_1,\cdots, a_i+\alpha,\cdots, a_k)  \ge  F(a_1, \cdots, a_i, \cdots, a_k  )$, for any  $\alpha >0$ and $1\le i \le k$.
%Let $S$ be the elements selected by Kleinberg's algorithm~\cite{kleinberg}, then
%$E[F(S)]>(1-5/\sqrt{k})OPT$.
%%Let $T$ be the $k$ largest elements of $S$, and $OPT=f(T)$.
%The expected number of elements of $T$ selected by the algorithm is at least $(1 -5/\sqrt{k})k$.
%\end{theorem}
%\begin{enumerate}
%\item $F$ is a monotone submodular function, and $F(a_1,\cdots, a_i+\alpha,\cdots, a_k)  \ge  F(a_1, \cdots, a_i, \cdots, a_k  )$, for $\alpha >0$ and $1\le i \le k$.
%\end{enumerate}
%We show Kleinberg's algorithm asymptotically approaches optimal solution.
%We prove that the Kleinberg algorithm works under this assumption which means that the competitive ratio of the algorithm asymptotically approaches 1.
The first one is the family of functions we call $m$-submdular. 
A function $f$ is $m$-submodular if it is submodular and there exists a submodular function $F$ such that for all $S$:
%\begin{itemize}
%\item 
\[ 
f(S)= \max_{T\subseteq S, |T|\le m} F(T) \ .
\]
%\end{itemize}
\scomment{This needs to be rewritten, I don't have time right now, so removing: Example of $m$-submodular functions are   maximum node weighted bipartite matching and  maximum edge weighted bipartite matching defined on $G=(X\times Y)$ with $|Y|=m$.  (the assignments will be done at the end of algorithm after all the selections are made).}

%\scomment{
%What is $\epsilon, \delta$? I removed this and restated inline with our rest of the results.
%\begin{theorem}
%For any $m$-submodular function $F$ there is an Algorithm that selects a set $S$ with $|S|<m\ln (1/\epsilon)+\ln(1/\delta)+\sqrt{\ln^2{1/\delta}+2m\ln(1/\delta)\ln(1/\epsilon)}$ and $E[F(S)]=(1-\epsilon-\delta)OPT$.
%\end{theorem}
%}
%\begin{restatable}{theorem}{msub}
\begin{theorem}
\label{thm:msub}
If $f$ is an $m$-submodular function, there exists an online algorithm for the \nameOfProblemSL~that achieves a competitive ratio of $1-\epsilon$ with shortlist of size $\eta_{\epsilon,m}(k)=O(1)$. Here, 
$\eta_{\epsilon,m}(k) = (2m+3) \ln(2/\epsilon)$.
\end{theorem}
%\end{restatable}
A proof of Theorem~\ref{thm:msub} along with the relevant algorithm (Algorithm \ref{alg:SIII}) appears in the appendix.

Another special case  is  monotone submodular functions $f$ satisfying the following property:
$f(\{a_1,\cdots, a_i+\alpha,\cdots, a_k\})  \ge  f(\{a_1, \cdots, a_i, \cdots, a_k \})$, for any $\alpha >0$ and $1\le i \le k$.
We can show that the algorithm by \citet{kleinberg} asymptotically approaches optimal solution for such functions, but we omit the details.

}





%We call an algorithm $ALG$ c-competitive if for any objective function $F$ chosen by the adversary, the
%set of selected items $ALG$ satisfies $E [F(ALG)] \ge (c ? o(1)) · OPT$, where $OPT$ is a feasible
%(offline) solution that maximizes v and the o(1)-term is asymptotical with respect to the length of
%the sequence n. 










%What is the minimum size shortlist to get a  $c$-competitive algorithm?
%These are questions that we consider in this paper.



%The submodular secretary problem, introduced by Bateni2013SubmodularExtensions et al. and Gupta et al., is an
%online variant of monotone submodular maximization subject to cardinality constraints. In this
%problem, we are allowed to select up to k items from a set of n items.
%The value of a set is represented by a monotone, submodular function.
%The values of the submodular function are only known on subsets of the items that have already arrived.
%The objective function is designed by an adversary, but the order of the items is uniformly at random.




%It is well-known since 1963 [10]
%that the optimal policy is to interview the first t ? 1 applicants, then hire the next one whose quality exceeds that of
%the first t ? 1 applicants, where t is defined by ; as $n \to \infty$, the probability of hiring
%the best applicant approaches 1/e, as does the ratio t/n.
%Note that a solution to the secretary problem immediately
%yields an algorithm for a slightly different objective function optimizing the expected value of the chosen element.





%In secretary problem, we are given a random order input and we are going to select the maximum element.
%In the classic secretary problem, one is presented a sequence of items with different scores online in
%random order. Upon arrival of an item, one has to decide immediately and irrevocably whether to
%accept or to reject the current item.  The objective is to accept the best of these items. 




%Multiple Choice secretary problem:


%Submodular Secretary problem:



%Our extension


%Streaming model:





% Imagine that you
%manage a company, and you want to hire a secretary from a pool of n applicants. You are very keen on hiring only
%the best and brightest. Unfortunately, you cannot tell how good a secretary is until you interview him, and you must
%make an irrevocable decision whether or not to make an offer at the time of the interview. The problem is to design
%a strategy which maximizes the probability of hiring the most qualified secretary. It is well-known since 1963 [10]
%that the optimal policy is to interview the first t ? 1 applicants, then hire the next one whose quality exceeds that of
%the first t ? 1 applicants, where t is defined by ; as $n \to \infty$, the probability of hiring
%the best applicant approaches 1/e, as does the ratio t/n. Note that a solution to the secretary problem immediately
%yields an algorithm for a slightly different objective function optimizing the expected value of the chosen element.




%In this paper, we consider general monotone submodular functions.



%The submodular secretary problem, introduced by Bateni2013SubmodularExtensions et al. and Gupta et al., is an
%online variant of monotone submodular maximization subject to cardinality constraints. In this
%problem, we are allowed to select up to k items from a set of n items.
%The value of a set is represented by a monotone, submodular function.
%The values of the submodular function are only known on subsets of the items that have already arrived.
%The objective function is designed by an adversary, but the order of the items is uniformly at random.

%We call an algorithm c-competitive if for any objective function v chosen by the adversary, the
%set of selected items ALG satisfies $E [v(ALG)] \ge (c ? o(1)) · v(OPT)$, where $OPT$ is a feasible
%(offline) solution that maximizes v and the o(1)-term is asymptotical with respect to the length of
%the sequence n. 

\scomment{The susection "Our techniques" was describing analysis and algorithm design techniques that are not being used in the proof anymore, there is no time to revise it, so I am removing it. Most of this intuition appears in algorithm description and proof overview anyway.}
\toRemove{
\subsection{Our techniques}
First we design a simple algorithm for the classic secretary problem  (finding the maximum element) that achieves a competitive ratio  of $1-\epsilon$ (for any $\epsilon>0$)  using a shortlist of size $O(\log(1/\epsilon))$.
%for a class of submodular functions that we call them $m$-submodular,
%for any $m>0$. 
The algorithm  ignores an $\epsilon$-fraction of the input and then selects an item if it is greater than the maximum element seen so far. 
We show that with probability $1-\epsilon$, the total number of selections made by this algorithm is at most $O(\log (1/\epsilon))$.
%A special $m$-submodular function for $m=1$ is the function $\max$. 
%As a result we 
We will use this online algorithm as a subroutine in our proposed algorithm for \nameOfProblemSL, for repeatedly finding (with probability $1-\epsilon$) the  item with maximum marginal value with respect to a subset of items, under submodular function $f$.  %It requires $\log(1/\epsilon)$ selections.
The main idea of the algorithm for \nameOfProblemSL\ is to divide the input into some blocks that we call them $(\alpha,\beta)$ \textit{windows}.  In this procedure, we partition the input into slots, where the sizes of the slots follow a balls-and-bins distribution.  We then group these slots into windows.
%Divide the input into $k\beta$ slots. The $i$-th slot, $s_i$, consists of $X_i$ consecutive elements of the input.
%Random variables $\{X_i\}$  for $i\in [k\beta]$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
%A \textit{window}, represented by parameters $(\alpha,\beta)$, consists of $\alpha \beta$ consecutive slots.
%\begin{definition} 
%A \textit{window}, represented by parameters $(\alpha,\beta)$, consists of $\alpha$ consecutive intervals, 
%of length $n/k$. 
%each interval is divided into $\beta$ slots. The length of $i$-th slot is a random variable denoted by $X_i$.
%Random variables $\{X_i\}$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
%random sample from the binomial distribution $B(n,\frac{1}{k\beta})$.
%of length $\frac{n}{k\beta}$.
%\end{definition}
%It consists of $\alpha$ consecutive intervals, 
%%of length $n/k$. 
%each interval is divided into $\beta$ slots. The length of $i$-th slot is a random variable denoted by $X_i$.
%Random variables $\{X_i\}$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
%%random sample from the binomial distribution $B(n,\frac{1}{k\beta})$.
%%of length $\frac{n}{k\beta}$.
%%Each window consists of smaller subintervals that we call them \textit{slots}.
Applying concentration inequalities for each {window}, and show that each window  has  roughly $\alpha$ elements of $OPT$ (the optimal solution), w.h.p.,
%the probability increases as $\alpha$ increases.
and that the fraction of elements of $OPT$ in a window that lie in different slots is at least $1-1/\beta$.
Therefore by choosing $\beta$ large enough most of the items in a window are in different slots, roughly speaking.\newline
For each window $w$ the algorithm \textit{guesses} the slots in which elements of $OPT$ in  $w$ lie in. 
By \text{guess} we mean that the algorithm enumerates over all subsets of size $\alpha$ of all $\alpha\beta$  slots in  $w$, and choose 
the one with the maximum marginal gain with respect to previously selected items. This can be done in an online manner.\newline
In the analysis of the algorithm for each window $w$,
we define an event $T_{1,\cdots, w-1}$ which conditions on the elements selected by the algorithm and also the positions in which they get selected by the algorithm. 
By conditioning on $T_{1,\cdots, w-1}$, we prove a lower bound for the expected marginal gain in the next window $w$.
Suppose $S_{1,\cdots, w-1}$ is output of the algorithm in windows $1,\cdots ,w-1$.
The crucial idea is that we show  conditioned on $T_{1,\cdots, w-1}$, each element $e\in OPT\setminus S_{1,\cdots, w-1}$
is more likely to appear in a slot in $w$ than in a slot in $1,\cdots, w-1$. 

We then have a normalization step in which we make all the elements of $OPT\setminus S_{1,\cdots, w-1}$ "appear" with the same probability in $w$. 
Therefore given that one slot in window $w$ contains an element of $OPT$, it can be any of $OPT\setminus S_{1,\cdots, w-1}$ with probability at least $1/k$. Hence the marginal gain for that slot is at least $\frac{1}{k}(OPT-F(S))$. 
We then repeat the argument for all the slots in window $w$  containing elements of the normalized sample.
\newline
The algorithm we describe uses $O(n)$ memory, in addition to the shortlist, but we can show how to modify the algorithm so that the amount of memory used is roughly the same as the size of the shortlist, and therefore the algorithm can be implemented in a streaming model.
} 

\subsection{Comparison to related work}
%There are two main frameworks  for \nameOfProblem: online algorithms and streaming algorithms.
%In the online framework,  we assume the input has random order. %(in adversarial order we can not guarantee anything)
%All of the previous algorithms in this framework irrevocably select a subset of size $k$, whose value is close to OPT~\cite{Bateni, kesselheim,Naor,smspm}.
We compare our results (Theorem \ref{opttheorem} and Theorem \ref{thm:streaming}) to the best known results for {\it \nameOfProblem}~and {\it \streamingProblem}, respectively.

The best known algorithm so far for \nameOfProblem~is by \citet{kesselheim}, with asymptotic competitive ratio of $1/e-O(k^{-1/2})$. 
In their algorithm, after observing each element, they use an oracle to compute optimal offline solution on the elements seen so far.
Therefore it requires exponential time in $n$. The best competitive ratio that they can get in polynomial time is 
$\frac{1}{e}(1-\frac{1}{e})-O(k^{-1/2})$.
In comparison, by using a shortlist of size $O(k)$ our (polynomial time) algorithm achieves a competitive ratio of $1-\frac{1}{e}-\epsilon-O(k^{-1})$. In addition to substantially improves the above-mentioned results for \nameOfProblem, this closely matches the best possible offline approximation ratio of $1-1/e$ in polynomial time. Further, our algorithm is linear time. Table \ref{table:t1} summarizes this comparison. 
Here, $O_\epsilon(\cdot)$ hides the dependence on the constant $\epsilon$. The hidden constant in $O_{\epsilon}(.)$ is %$c\frac{\log(1/\epsilon)}{\epsilon^2}  {\frac{1}{\epsilon^6} \log(1/\epsilon)  \choose {\frac{1}{\epsilon^4} \log(1/\epsilon)}}$ 
\etaMacro for some absolute constant $c$.
%~\cite{Badanidiyuru2014StreamingFly} and~\cite{kesselheim}.

\begin{table}[h!]
\centering
\begin{tabular}{ |c c c c c| }
\hline
 & \#selections & Comp ratio & Running time & Comp ratio in poly(n) \\%&  Comp ratio in poly(n,k)  \\ 
\hline
\cite{kesselheim} & $k$ & $1/e-O(k^{-1/2})$ & $exp(n)$ & $\frac{1}{e}(1-1/e)$ \\ %& $(1-1/e)1/e$ \\ 
this & $O_{\epsilon}(k)$ & $1-1/e-\epsilon-O(1/k) $ & $O_{\epsilon}(n)$ &  $1-1/e-\epsilon-O(1/k)$ \\%&  $1-1/e-\epsilon$ \\
%2nd & $k\log^2 k$ & $1/2-O(k^{-1/4})$ & $poly(n), exp(k)$ & $1/2-O(k^{-1/4})$ & $(1/2-O(k^{-1/4}))(1-1/e)$ \\
\hline    

\end{tabular}
\caption{\nameOfProblem~settings}
\label{table:t1}
\end{table}
%On the other hand, in the streaming framework the decision to select an element is not irrevocable, and there is a buffer of limited size and you can add or remove elements from the buffer, i.e., you can deselect some elements that you have already selected. The random order assumption in this model is not necessary.
In the streaming setting, \citet{Chakrabarti2015} provided a single pass streaming algorithm for monotone submodular function maximization under $k$-cardinality constraint, that achieves a $0.25$ approximation under adversarial ordering of input. Further, their algorithm requires $O(1)$ function evaluations per arriving item and $O(k)$ memory.
The currently best known approximation  under  adversarial order streaming model is by~\citet{Badanidiyuru2014StreamingFly}, who achieve a $1/2-\epsilon$ approximation with a memory of size $O(\frac{1}{\epsilon}k\log k)$. 
%\scomment{no known? or is it not possible?}\mcomment{not possible}
%Any algorithm for streaming submodular
%maximization that only queries the value of the
%submodular function on feasible sets (i.e., sets of cardinality
%at most k) and is an α-approximation for a
%constant α > 0.5 must use Ω(n/k) memory, where n is
%the length of the stream.
There is an upper bound of $1/2+o(1)$ on the competitive ratio achievable by 
any algorithm for streaming submodular
maximization that only queries the value of the submodular function on feasible sets while using $o(n)$ memory~\cite{norouzi}.
%any streaming algorithm for this problem under adversarial order, while using $o(n)$ memory~\cite{norouzi}.
%It does not need random order assumption. 
%Also note that this algorithm can not be converted into an online algorithm. 
%Streaming algorithm with random order assumption has been considered for other problems. 
%But nothing better than~\cite{Badanidiyuru2014StreamingFly} is known for this problem under random order setting. 

\citet{Hess} initiated the study of  \streamingProblem.
Their algorithm uses $O(k)$ memory and a total of $n$ function evaluations to achieve $0.19$ approximation. 
%This result is  worse than the result of~\cite{kesselheim}  in the stricter online model. But note that~\cite{kesselheim} requires $\Omega(nk)$ function evalutation and $\Omega(n)$ memory.
The state of the art result in the random order input model is due to \citet{norouzi} who achieve a $1/2+8\times 10^{-14}$ approximation, while using a memory buffer of size $O(k\log k)$.
%Badanidiyuru et al.~\cite{Badanidiyuru2014StreamingFly} design the first efficient streaming algorithm
%with constant factor $1/2-\epsilon$ approximation guarantee, requiring only a single pass through the data, and memory $O(\frac{1}{\epsilon}k\log k )$.
%Recently~\cite{norouzi} showed that it is impossible to get ratio better than $1/2+o(1)$ in the adversarial order input using memory $o(n)$.
%Our algorithm is in the intersection of the above frameworks. 
%It generalizes the online framework in the way that we are allowed to select more than $k$ elements. 
%We generalize the online model in the way that we are allowed to select more than $k$ elements, and output a subset of size $k$ whose  value is close to OPT.  Note that we are only interested in returning a subset of size at most $k$ as our output.  
%In algorithms like ~\cite{Vondrak}, although the output is close to OPT, it is not restricted to $k$ elements, and we can't guarantee that it contains a subset of size $k$ whose value is close to OPT.
%In comparison, our algorithm selects $O(k)$ elements and guarantees that there is a subset of size $k$ whose value is $R-O(k^{-1})$ times $OPT$, for $R<1-1/e$.Thus by relaxing the number of selections we improve upon the best competitive ratio $1/e$, while only using $O(n)$ running time.  These bounds compare favorably to~\cite{kesselheim}, which  needs to find the optimal offline solution $n$ times, or to use an $1-1/e$ approximation to find each offline optimal solution. In the latter case, the running time is  $O(n^2)$ and the competitive ratio is  $\frac{1}{e} (1-1/e)$.
 
%It is asymptotically a $1/2-O(k^{-1/4})$ approximation algorithm.
%In terms of memory size, it improves upon the previous $k\log k$~\cite{norouzi}. %$\frac{1}{\epsilon}k\log k$.%, for $k>(1/\epsilon)^4$.
%(Note that the approximation ratio of our algorithm is asymptotic and for a fixed $k$ we can not decrease error more than $k^{-1/4}$)
%Also in terms of running time it is polynomial in $n$, but it requires exponential time in $k$.
%Also note that the online algorithm~\cite{kesselheim} can not be converted into a streaming algorithm with nontrivial memory size.

%The goal is to partition the items between agents so as to maximize the sum of their valuation functions.
%The well known greedy algorithm gives a 1/2 approximation for this problem. Also for the adversarial order 1/2 is the best we can achieve~\cite{Kapralov:2013}.
%\cite{vahab},~\cite{swm}  slightly improve the analysis of the greedy algorithm to just above 1/2 for  random order input (0.505, 0.509 competitive ratio respectively). The later result can be generalized to maximizing monotone sumobular functions subject to  a partition matroid. It is incomparable with \nameOfProblemSL.

%Table~\ref{table:t1} and 
Table~\ref{table:t2} provides a detailed comparison of our result in Theorem \ref{thm:streaming} to the 
%, we compare our algorithm to some of the previous works to show the tradeoffs in the various parameters for both the online algorithms model and the streaming model.
above-mentioned results for  \streamingProblem, showing that our algorithm substantially improves the existing results on most aspects of the problem. 

\begin{table}[h!]
\centering
\begin{tabular}{ |c c c c c | }
\hline
 & Memory size & Approximation ratio & Running time & update time \\ 
 \hline
\cite{Hess} & $O(k)$ &  $0.19$ & $O(n)$ & O(1) \\ 
\cite{norouzi} & $O(k\log k)$ &  $1/2+8\times 10^{-14}$ & $O(n\log k)$ & $O(\log k)$ \\ 
\cite{Badanidiyuru2014StreamingFly} & $O(\frac{1}{\epsilon}k\log k)$ & $1/2-\epsilon$ & $poly(n,k, 1/\epsilon)$ & $O(\frac{1}{\epsilon}\log k)$ \\ 
this & $O_{\epsilon}(k)$ & $1-1/e-\epsilon-O(1/k)$ & $O_{\epsilon}(n)$ & amortized $O_{\epsilon}(1+\frac{k^2}{n})$ \\
%2nd & $k\log^2 k$ & $1/2-O(k^{-1/4})$ & $poly(n), exp(k)$ &  \text{amortize one operation}\\
\hline    
\end{tabular}
\caption{\streamingProblem
}
%$\log(1/\epsilon) {\frac{1}{\epsilon^3} \log(1/\epsilon)  \choose {\frac{1}{\epsilon^2} \log(1/\epsilon)}}$.}
\label{table:t2}
\end{table}



There is also a line of work studying the online variant of the submodular welfare maximization problem (e.g., \cite{vahab,swm,Kapralov:2013}). In this problem, 
the items arrive online, and each arriving item should be allocated  to one of $m$ agents with a submodular valuation functions $w_i(S_i)$ where $S_i$ is the subset of items allocated to $i$-th agent). The goal is to partition the arriving items into $m$ sets to be allocated to $m$ agents, so that the sum of valuations over all agents is maximized. This setting is incomparable with the \nameOfProblem~setting considered here.

==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/maxanalysis.tex <==
%\subsection{Analysis of Algorithm \ref{alg:} for the basic secretary problem with shortlist}
\scomment{Can we add a lemma showing that expected number of items selected will be $\log(1/\delta)$ when $u=N\delta$}
\mcomment{same as previous comment}
\scomment{Also we need to discuss that when we say shortlist of size $\eta(k)$, is that expected number of items or high probability? If it is high probability, we need to define what it means to say shortlist of size $\eta(k)$. Does it mean $\eta(k)$ with prescribed probability $1-\epsilon'$?}
\scomment{the results here will move to the previous section, and proofs for high prob bound will go to appendix}

\begin{theorem}
$\mathbb{E}[|S|] = \ln n$.
\end{theorem}
\begin{proof}
%Suppose $F(S_i) = f(T)$, where $|T|=m$. If $a_i \notin T$ then it is not selected. 
%Because if $a_i\notin T$ and is selected then it should have positive $F$ marginal value, which means $F(S_i) = F(S_{i-1} \cup \{a_i\} ) > F(S_{i-1}) =  f(T) $, it is a contradiction. 
%Thus only elements in $T$ will be selected at position $\ell$.  
Suppose $S_i=\{a_1, \cdots, a_i\}$.
Consider all permutations of $S_i$, an element will be selected at position $i$ if it is equal to $\max_{a\in S_i} F(a)$, thus the probability that it gets selected is $1/i$. Therefore the expected number of selections will be at most $\sum_{i=1}^{n} \frac{1}{i}  = \ln n $
%The expected number of elements selected at position $\ell$ is at most $\frac{m}{\ell}$. 
\end{proof}


%In the rest we will make the following assumption:\\
%\textbf{Assumption. } %There is a unique $m$-tuple $OPT$ with maximum $f(OPT)$ in the input. 
%There is a unique maximum element.


\scomment{What is $\delta$ in the theorem below? The proof below seems to suggest it is high probability statement, not exact.}
\begin{theorem}\label{maxanalysis}
Algorithm~\ref{alg:SIIImax}, with parameter $u=n\epsilon$,  selects a set $S$ with 
$$|S|<\ln (1/\epsilon)+\ln(1/\delta)+\sqrt{\ln^2{1/\delta}+2m\ln(1/\delta)\ln(1/\epsilon)}$$ 
and $\mathbb{E}[\max_{a\in S} a]=(1-\epsilon-\delta)OPT$, where $OPT$ is the max element in the input.
\end{theorem}
\begin{proof}
We use Freedman's inequality.
 If $\{a_1,\cdots, a_i\}$ has a unique maximum, % subset of size $m$, 
define $Y_i$ to be a random variable indicating whether the algorithm has selected $a_i$  or not, where $Y_i=1-\frac{1}{i}$ if $a_i$ is selected and $Y_i=-\frac{1}{i}$ otherwise. 
 If it has not unique solution define $Y_i=0$. ($a_i$ will not be selected)
 Also define $\mathcal{F}_i=\{Y_{n},Y_{n-1}, \cdots, Y_{n-i+1}\}$.

Let $X_i=\sum_{j=n-i+1}^{n} Y_j$,
then $\{X_i\}$ is a martingle, 
because $E[X_{i+1}|\mathcal{F}_{i}] = X_i+E[Y_{n-i}|\mathcal{F}_i]$.
 If $\{a_1,\cdots, a_i\}$ has a unique maximum element, $E[Y_{n-i}|\mathcal{F}_i]=(1/i)(1-1/i)+(1-1/i)(-1/i)=0$,
 otherwise $E[Y_{n-i}|\mathcal{F}_i]=0$. So in both cases $E[X_{i+1}|\mathcal{F}_{i}] =X_i$.
%X_i+E[Y_{n-i}]=X_i$. Also $|X_{i+1}-X_i| < 1$.
%frac{m}{i} (1-\frac{m}{i}) +(1-\frac{m}{i})\frac{m}{i} 
As in the Freedman's inequality, let $L=\sum_{i=n\epsilon}^{n} Var(Y_i| F_{i-1})$. 
\begin{align*}
L  =  \sum_{i=n\epsilon}^{n} \frac{1}{i}  (1-\frac{1}{i})^2 + (1-\frac{1}{i}) (\frac{1}{i})^2 
< \sum_{i=n\epsilon}^{n} \frac{1}{i} =\ln (1/\epsilon)
\end{align*}
Therefore,
\[
Pr(X_{n-n\epsilon}\ge \alpha \text{ and }  L\le \ln (1/\epsilon) ) \le exp(-\frac{\alpha^2}{\ln (1/\epsilon)+ 2\alpha })   < \delta 
\]
Thus we get $\alpha > \ln(1/\delta)+\sqrt{\ln^2{1/\delta}+2\ln(1/\delta)\ln(1/\epsilon)}$.
%Thus we get $\alpha > \ln(1/\epsilon)(1+\sqrt{1+2m})$. 
Also $|S| = X_{n-n\epsilon} + \ln(1/\epsilon)$. Therefore 
\[
Pr(|S| \ge  \ln (1/\epsilon)+\ln(1/\delta)+\sqrt{\ln^2{1/\delta}+2\ln(1/\delta)\ln(1/\epsilon)}  )  \le \delta
\]
So with probability $(1-\delta)$, $|S| \le \ln (1/\epsilon)+\ln(1/\delta)+\sqrt{\ln^2{1/\delta}+2\ln(1/\delta)\ln(1/\epsilon)} $.  %\frac{m\ln c}{\sqrt{\epsilon}} + m\ln c $ .
%Suppose $OPT$ is the optimal solution, i.e $|OPT|=m$ and  $f(OPT)$ is maximum in subsets of $I$.
%Since $\max $ is a submodular function, 
Also $\mathbb{P}(OPT \in\{a_{n\epsilon},\cdots, a_n \}  ) =(1-\epsilon)$.
%$E[f(OPT\cap \{a_{n\epsilon},\cdots, a_n \} )] = (1-\epsilon)OPT$.
Therefore $E[\max_{a\in S} a] \ge (1-\epsilon)OPT-\delta OPT$. 
%By setting $1/c=\epsilon$, $|S|=m\ln (1/\epsilon)+ \sqrt{2m \log (1/\epsilon)} $ and $E[F(S)]=(1-2\epsilon)OPT$.
\end{proof}

\begin{theorem}
Any online algorithm needs to select at least $\frac{1}{2}\log(1/\epsilon)-\frac{1}{2}$ elements, in expectation, to select the maximum element  with probability at least $(1-\epsilon)$ in a random permutation. (we assume $n> 1/\epsilon$)
\end{theorem}
\begin{proof}
Let $I_i=\{a_1,\cdots, a_{n/2^{i-1}}\}$, $T_i=\{a_{n/2^i+1}, \cdots, a_{n/2^{i-1}}\}$, and $R_i=I_1\setminus I_i$, for $i=1, \cdots, \log(1/\epsilon)$. Suppose $M_i$ is the maximum element in $I_i$. Let $S$  be the set of selected elements by algorithm at the end of execution.
Suppose $\epsilon_i= E[M_i\notin S| M_i\in T_i]$,
then $E[|S\cap T_i|] \ge \frac{1}{2} (1-\epsilon_i)$.
Therefore $E[|S|] \ge \sum_{i=1}^{\log(1/\epsilon)} \frac{1}{2} (1-\epsilon_i) $. Also w.p. $\frac{1}{2^{i}}$, $M_1 \in T_i$, 
thus $\sum_{i=1}^{\log(1/\epsilon)} \frac{1}{2^{i}} \epsilon_i  \le \epsilon$. 
(Note that we use the fact $ E[M_i\notin S| M_i\in T_i \text{ and }  M_i=M_1] \le \epsilon_i$, i.e, if algorithm selects one element it will select 
it even if we increase its value and keep the rest untouched) 
Now $E[|S|]$ is minimized under above constraint if $\frac{1}{2^{\log(1/\epsilon)}}\epsilon_{\log(1/\epsilon)} = \epsilon$ and the rest are zero.
Hence $E[|S|] \ge \frac{1}{2}\log(1/\epsilon)-\frac{1}{2}$.
\end{proof}

%\begin{prop}
%For a m-submodular function $f$, any online algorithm needs to select at least $\frac{m}{2}\log(m/\epsilon)-\frac{m}{2}$ elements, in expectation, to select a set $S$, with $|S|\le m$  such that  $E[f(S)] \ge (1-\epsilon)OPT$, in a random permutation. 
%\end{prop}
%\begin{proof}
%Apply previous theorem on m separate 1 to n matching.
%\end{proof}




==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/mmatroids.tex <==
In this section, we present  algorithms
for monotone submodular function maximization subject to $p$-matchoid constraints.
These constraints generalize many basic combinatorial constraints such as the cardinality constraint, the intersection of $p$ matroids, and matchings in graphs. 
Throughout this section,  $k$ would refer to the size of the largest feasible set.
A formal definition of
a $p$-matchoid is as follows:

\begin{definition} \label{def:matchoid}
(\textbf{Matchoids}). Let $\mathcal{M}_1 = (\mathcal{N}_1, \mathcal{I}_1), \cdots ,\mathcal{M}_q = (\mathcal{N}_q, \mathcal{I}_q)$ be $q$ matroids over overlapping groundsets. Let $\mathcal{N} = \mathcal{N}_1\cup  \cdots \cup \mathcal{N}_q$ and $\mathcal{I} = \{S\subseteq \mathcal{N} : S\cap \mathcal{N} \in \mathcal{I}_{\ell},
 \forall \ell\}$. The finite set system
$\mathcal{M}_p = (\mathcal{N} , \mathcal{I})$ is a $p$-matchoid if for every element $e \in \mathcal{N}$ , $e$ is a member of $\mathcal{N}$ for at most $p$ indices $\ell \in [q]$.
\end{definition}

%p-matchoids generalizes matchings and intersections of matroids, among
%others






There are some subtle differences in the algorithm as well as in the analysis.
The main difference in the algorithm is that instead of removing one item from the current independent set $S$, we might remove up to $p$ items form  $S$. Each removed item corresponds to different ground sett $N_i$, in which the new item lies (based on the definition of $p$-matchoid constraints, Definition~\ref{def:matchoid}, there are at most $p$ such elements).

For each index $\ell\in [q]$  define:
\begin{equation}
\Omega_{\ell}(e,S):= \{e'\in S| S+e-e' \in \mathcal{I}_{\ell} \} 
\end{equation}
For an element $e$ in the input, suppose $e\in N_{\ell_i}$, for $i=1,\cdots, p$.
Define 
\begin{equation}
\lambda(e,S):= \prod_{i=1}^{p} {\Omega_{\ell_i}(e,S)}
\end{equation}
For a combination vector 
$r=(r_1,\cdots, r_p)\in \lambda(e,S)$, where
$r_i \in \Omega_{\ell_i}(e,S)$,
define:
\begin{equation}
\mu(r):=  \{r_1,\cdots, r_p\}
\end{equation}
\begin{equation}
g_r(e,S):= f(S+e-\mu(r))-f(S)
\end{equation}
Also define:
\begin{equation}
\theta(e,S):= \mu( \arg\max_{r\in \lambda(e,S) } g_r(e,S))
\end{equation}
%Thus, $\theta(e,S) \in \lambda(e,S)$.
Furthermore define,
\begin{equation}
\label{eq:newg}
g(e,S):= \max_{r\in \lambda(e,S) } g_r(e,S)
\end{equation}

\toRemove{
For each index $\ell\in [q]$  define the following functions as before:
%$\theta$ as: 
$$ \theta_{\ell}(e,S) := \arg\max_{e'\in S} \{ f(S+e-e')| S+e-e' \in \mathcal{I}_{\ell} \} $$
Also define $g_{\ell}$ as 
% $$g(e):=\max_{e': S+e-e' \in \mathcal{I}} F(S+e-e') - F(S)$$
 $$g_{\ell}(e,S):= f(S+e-\theta_{\ell}(e,S)) - f(S)$$
and
$$g(e,S):= f(S+e-\bigcup_{i}\theta_i(e,S)) - f(S)$$
 }
As in the online subroutine for the main algorithm, we run Algorithm~\ref{alg:matroidmax} with the new function $g$ defined in equation~\ref{eq:newg}. It returns  element  $e$ with maximum  $g(e,S)$, and it achieves a  $1-\delta$ competitive ratio   with shortlists of size logarithmic in $1/\delta$.

Additionally, we  make some changes in the main algorithm~\ref{alg:main}. In particular, we define $\gamma$ similar to equation~\ref{eq:gamma} but using the new definition of $g$ in equation~\ref{eq:newg}.
%$\zeta(\tau):=\{C_1, \ldots, C_\ell\}$
Moreover, for a subsequence $\tau=(s_1,\ldots, s_\ell)$
define 
\begin{equation}
\zeta(\tau):=\bigcup_{j=1}^{\ell} C_j
\end{equation}
where each $C_j$ is a set defined as
\begin{equation}
\label{eq:cij}
C_j :=  
%\bigcup_{i_j \in N_\ell}
\theta(i_j, S_{1, \ldots,w-1} \cup \{i_1,\ldots, i_{j-1}\})
\end{equation}
Note that in contrast with the definition of $\zeta(\tau)$ for the matroid constraints equation~\ref{eq:cij}, in which $c_j$ is only one item, now each $C_j$ is a subset of the current independent set $S$. Further, the definition of $\bar{S}_w$, in equation~\ref{eq:Swbar}, will be updated accordingly using the new definition of $\zeta(\tau)$.

Now we can generalize Lemma~\ref{replaced} to $p$-matchoid constraints.
%First we use Brualdi lemma~\ref{lem:Brualdi} to define the following:
%\begin{definition}
%For any $j\in \{1,\ldots, t\}$, 
%let $S'_{\ell}$ be the extension of $S_{1,\cdots, w-1}\cup \{i_1, \cdots, i_{j-1}\}\setminus\bigcup_{r\le j-1} C_r$ to an independent set in $\mathcal{M}_{\ell}$, and $\pi_{\ell}$ be the bijection from Brualdi lemma (refer to Lemma~\ref{lem:Brualdi}) from $S^*$ to $S'_{\ell}$.
%\end{definition}

\begin{lemma}\label{replacedMatchoid}
%At the end of window $w$, 
Suppose the sequence $\tilde \tau_w=(s_1, \ldots, s_t)$ defined as in Definition \ref{def:tauw}, let $\gamma(\tilde \tau_s)=(i_1,\ldots, i_t)$, with $\gamma(\cdot)$ as defined in \eqref{eq:gamma}. 
For any $j\in \{1,\ldots, t\}$, and element $b\in \mathcal{N}_{\ell}$, 
let $S'_{\ell}$ be the extension of $S_{1,\cdots, w-1}\cup \{i_1, \cdots, i_{j-1}\}\setminus\bigcup_{r\le j-1} C_r$ to an independent set in $\mathcal{M}_{\ell}$, and $\pi_{\ell}$ be the bijection from Brualdi lemma (refer to Lemma~\ref{lem:Brualdi}) from $S^*$ to $S'_{\ell}$. 
Further, let's denote by $\pi(b):=\{\pi_{\ell}(b)|b \in \mathcal{N}_{\ell}\}$, then
{\small \begin{eqnarray*}
\Ex[f(S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus (\bigcup_{r\le j-1} C_r \cup \pi(a)|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}]\\
 \ge (1-\frac{p}{k})f(S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots,c_{j-1}\})\
\end{eqnarray*}}
%{\small \begin{eqnarray*}
%\Ex[f(S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus (\bigcup_{r\le j-1} C_r \cup \bigcup_{\ell} \pi_{\ell}(a))|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}]\\
% \ge (1-\frac{p}{k-\alpha})f(S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots,c_{j-1}\})\
%\end{eqnarray*}}
\end{lemma}
\begin{proof}
%It follows from Brualdi lemma and lemma~\ref{sample}.

%where each element has probability at least $p$ to appear in $A$ (not necessarily independently)
The proof is similar to the proof of Lemma~\ref{replaced}. 
For $\ell \in [q]$,
since $\pi_{\ell}$ is a bijection from $S^*\cap \mathcal{N}_{\ell}$ to $S'_{\ell}$, from Brualdi's lemma (lemma~\ref{lem:Brualdi}), there is an onto mapping $\pi'_{\ell}$ from $S^*\cap \mathcal{N}_{\ell}$ %$OPT$ 
 to $S_{1,\cdots, w-1}\cup \{i_1, \cdots, i_{j-1}\}\setminus (\bigcup_{r\le j-1} C_r \cup \pi(a))\cup \{\emptyset\}$ 
such that %$S_{1,\cdots, w-1}\cup \{i_1, \ldots, i_{j-1}\} - \pi(a) +a \in M$ for all $a \in S^*$.
$S_{1,\cdots, w-1}\cup \{i_1, \cdots, i_{j-1}\}\setminus (\bigcup_{r\le j-1} C_r \cup \pi(a))- \pi'_{\ell}(a) +a \in M_{\ell}$, for all $a \in S^*$. Further, $\pi'_{\ell}(a)=\pi_{\ell}(a)$ if $\pi_{\ell}(a)\in  S_{1,\cdots, w-1}\cup \{i_1, \cdots, i_{j-1}\}\setminus \bigcup_{r\le j-1} C_r$ and $\pi'_{\ell}(a)=\emptyset$ otherwise.

Recall the definition of $Z_{s_j}$ (refer to definition~\ref{def:tauw}).
Suppose $a$ is a randomly picked item from $S^*\cap Z_{s_j}$.
Note that from Lemma~\ref{lem:Zs}, conditioned on $T_{1,\cdots, w-1}$, the element $a$ can be equally any element of %$S^*$ 
$S^*\backslash  \{Z_1,\ldots Z_{s_{j-1}}\}$
with probability at least $1/k$.
Therefore, $\pi'_{\ell}(a)$ would be any of $S_{1,\cdots, w-1}\cup \{i_1, \cdots, i_{j-1}\}\setminus \bigcup_{r\le j-1} C_r $ with probability at most $1/k$ 
(since $\pi'_{\ell}$ might map some elements of $S^*$ to the empty set).

For  element $e\in S_{1,\cdots, w-1}\cup \{i_1, \cdots, i_{j-1}\}\setminus \bigcup_{r\le j-1} C_r$, let $\mathcal{N}(e)$ be the set of indices $\ell$ such that $e\in \mathcal{N}_{\ell}$. Because of the $p$-matchoid constraint, we have $|\mathcal{N}(e)|\le p$.
Define 
$$
\pi^{-1}(e):=\{t | t\in \mathcal{N}_{\ell}, \text{ for some }  \ell\in \mathcal{N}(e) \text{ and }  \pi_{\ell}(t)=e \} 
$$
we have also $|\pi^{-1}(e)|\le p$. Thus, each element $e \in S_{1,\cdots, w-1}\cup \{i_1, \cdots, i_{j-1}\}\setminus \bigcup_{r\le j-1} C_r$ belongs to %$\bigcup_{\ell} \pi_{\ell}(a)$
$\pi(a)$ with probability at most $p/k$:
$$
\Pr(e\in \pi(a) | a\in S^{*}\cap Z_{s_j} ) = \Pr(a\in S^{*}\cap Z_{s_j}\cap \pi^{-1}(a) ) \le \frac{p}{k} 
$$
 Now we apply Lemma~\ref{sample}.
It is crucial to note that in Lemma~\ref{sample}  each element do not need to be selected necessarily independently.
Definition of $\pi$ and lemma~\ref{sample} imply the lemma.
\end{proof}

Furthermore the main difference in the analysis is that instead of recursion~\ref{recursion}, we get the following new recursion:
\toRemove{
\begin{align}\label{matchoidRecursion}
f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j}\} \setminus \bigcup_{r\le j} C_r )  
%f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}, a\} \setminus \{c_1,\cdots, c_{j-1}, \pi(a) \} )\ge 
- f(S_{1,\cdots, w-1}\cup \{i_1, \ldots, i_{j-1}\} \setminus \bigcup_{r\le j-1} C_r )\\
\ge
{ \frac{1}{k}\left((1-\frac{\alpha}{k})f(S^*)-pf({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\})\right)\ . }
\end{align}
}

\begin{lemma}\label{exgmatchoid}
%We can show that:
%\begin{align}\label{recursion}
Suppose function $g$ is as defined in equation~\ref{eq:newg}.
For the sequence $\tilde \tau_w=(s_1, \ldots, s_t)$, and $\gamma(\tilde \tau_s)=(i_1,\ldots, i_t)$. Then, for all $j=1,\ldots, t$, \\
{\small \begin{eqnarray*}
\Ex \left[g(i_j,S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus \bigcup_{r\le j-1} C_r)|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}\right]\\
 \ge 
 %(1-\frac{1}{k-\alpha})
 \frac{1}{k}
 \left(
 (1-\frac{\alpha}{k})f(S^*)-(p+1) f(S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\bigcup_{r\le j-1} C_r)\right)\
\end{eqnarray*}}
\end{lemma}
%\begin{proof}
%The proof is based on lemma~\ref{replacedMatchoid} for matchoids and is similar to the proof of lemma~\ref{exg} for matroids.
%\end{proof}

%\begin{theorem}
%$$ \mathbb{E}[f(S_{1,\cdots, W})] \ge \frac{1}{p} (1-1/e) (1-\frac{\alpha}{k}) OPT$$
%\end{theorem}


\begin{proof}
The proof is similar to the proof of Lemma~\ref{exg} with some changes regarding matchoid constraints.
In the algorithm~\ref{alg:main}, at the end of window $w$, we set %$S_{1,\cdots, w-1} = {S}_{1,\cdots, w-1} \setminus \bar{S}_w$.
$S_{1,\cdots, w} = S_{1,\cdots, w-1}\cup S_w \setminus \bar{S}_w$.
Suppose $a\in s_j\cap S^*$. 
Moreover, let $S'_{\ell}$ be the extension of $S_{1,\cdots, w-1}\cup \{i_1, \cdots, i_{j-1}\}\setminus \bigcup_{r\le j-1} C_r$ to an independent set in $\mathcal{M}_{\ell}$, and $\pi_{\ell}$ be the bijection in Brualdi lemma (refer to Lemma~\ref{lem:Brualdi}) from $S^*_{\ell}$ to $S'_{\ell}$.
Thus the expected value of the function $g$ on the element selected by the algorithm in slot $s_j$ (the element with maximum $g$ in the slot $s_j$) would be
\begin{eqnarray*}
%\begin{align}
%g(i_j,{S}_{1,\ldots, w-1} \cup \{i_1,\cdots,i_{j-1}\}\setminus \{c_1,\cdots, c_{j-1}\})
%= 
&\Ex[f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j}\} \setminus \bigcup_{r\le j} C_r)|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}]  %- f(S_{1,\cdots, w-1}\cup \{i_1, \ldots, i_{j-1}\} \setminus \{c_1,\cdots, c_{j-1}\}) 
\\\ge&
\Ex[f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}, a\} \setminus \bigcup_{r\le j-1} C_r \cup \pi(a)  |T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}] %- f(S_{1,\cdots, w-1}\cup \{i_1, \ldots, i_{j-1}\} \setminus \{c_1,\cdots, c_{j-1} \}) 
\\\ge&
%f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}, a\} \setminus \{c_1,\cdots, c_{j-1}, \pi(a) \} )-
\Ex[f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\} \setminus \bigcup_{r\le j-1} C_r \cup \pi(a) )|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}]
\\&+\Ex[\Delta_f(a|S_{1,\cdots,w-1}\cup\{i_1,\cdots,i_{j-1}\}\setminus \bigcup_{r\le j-1} C_r \cup \pi(a) )|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}] \\
\ge&
\Ex[f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\} \setminus \bigcup_{r\le j-1} C_r \cup  \pi(a) )|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}]
\\&+\Ex[\Delta_f(a|S_{1,\cdots,w-1}\cup\{i_1,\cdots,i_{j-1}\}\setminus \bigcup_{r\le j-1} C_r )|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}]
%\end{align}
\end{eqnarray*}
The first inequality is from the definition of function $g$ as it is defined in equation~\ref{eq:newg} and the fact that the algrotihm selects an element in slot $s_j$ with maximum value of $g$. The second inequality is from submodularity and the last inequality is from monotonicity of $f$.
Now from the last inequality  and Lemma~\ref{exgmatchoid}, we can show,
\begin{align*}
&\Ex[f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j}\} \setminus \bigcup_{r\le j} C_r) |T_{1,\ldots, w-1}, i_{1,\ldots, j-1}]& \\ &\ge
%f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}, a\} \setminus \{c_1,\cdots, c_{j-1}, \pi(a) \} )\ge 
(1-\frac{p}{k} ) f(S_{1,\cdots, w-1}\cup \{i_1, \ldots, i_{j-1}\} \setminus \bigcup_{r\le j-1} C_r )&\\
&+ \Ex[ \Delta_f(a|{S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\} \setminus\bigcup_{r\le j-1} C_r )||T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}] &
\end{align*}
Now from lemma~\ref{lem:asGoodas} and the above inequality we can show
\begin{align*}
&\Ex[f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j}\} \setminus \bigcup_{r\le j} C_r) |T_{1,\ldots, w-1}, i_{1,\ldots, j-1}]& \\  &\ge
%f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}, a\} \setminus \{c_1,\cdots, c_{j-1}, \pi(a) \} )\ge 
(1-\frac{p}{k} ) f(S_{1,\cdots, w-1}\cup \{i_1, \ldots, i_{j-1}\} \setminus \bigcup_{r\le j-1} C_r )&\\
&+ { \frac{1}{k}\left((1-\frac{\alpha}{k})f(S^*)-f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\} \setminus\bigcup_{r\le j-1} C_r ) \right)\ . }&
\end{align*}
Thus,
\begin{align}\label{newrecursion}
f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j}\} \setminus \bigcup_{r\le j} C_r )  
%f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}, a\} \setminus \{c_1,\cdots, c_{j-1}, \pi(a) \} )\ge 
- f(S_{1,\cdots, w-1}\cup \{i_1, \ldots, i_{j-1}\} \setminus \bigcup_{r\le j-1} C_r )\\
\ge
{ \frac{1}{k}\left((1-\frac{\alpha}{k})f(S^*)-(p+1)f({S}_{1,\ldots, w-1} \cup \{i_1,\cdots,i_{j-1}\}\setminus \bigcup_{r\le j-1}C_r)\right)\ . }
\end{align}

\end{proof}





By solving the recursion and similar to the analysis for matroid constraints we can show the following theorem:


\matchoidThm



==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/newIntroduction.tex <==
%\section{Introduction}


\toRemove{
In the classic \textit{secretary problem}, 
$n$ items appear in random order.  We know $n$, but don't know the value of an item until it appears.   
Once an item arrives we have to irrevocably and immediately decide whether or not to select it. Only one item is allowed to be selected, and the objective is to  select the most valuable item, or perhaps to 
%\ccomment{Is this really equivalent, or just related}
%\mcomment{not equivalent but related. }
maximize the expected value of the selected item  
%The origin of the secretary problem is hard to track
~\cite{Dynkin:SovMath:1963,ferguson1989solved, 10.2307/2985407}. 
It is well known that the optimal policy is to observe the first $n/e$ items without making any selection and then select the first item whose value is larger than the value of the best item in the first $n/e$ items~\cite{Dynkin:SovMath:1963}. This algorithm, given by ~\citet{Dynkin:SovMath:1963},
is asymptotically optimal, and hires the best secretary with probability at least $1/e$. Hence it
is also $1/e$-competitive for the expected value of the chosen item, and
%\ccomment{Is this true?}
%\mcomment{Yes, but the original paper shows the probability not the expectation Dynkin provided an asympotically optimal algorithm for this problem, which hires the best secretary with probability at least 1/e}
it can be shown that no algorithm can beat $1/e$-competitive ratio in expectation.
%

Many variants and generalizations of the secretary problem have been studied in the literature, see e.g., \cite{Ajtai:2001,WILSON1991325,vanderbei1980optimal, wilson1991optimal, kleinberg, Babaioff:2008}.  
%\ccomment{We should have more variants hear} The secretary problem has been generalized.  
\cite{kleinberg, Babaioff:2008} introduced a 
{multiple choice secretary problem}, where the goal is to select $k$ items in a randomly ordered input so as to maximize  the {\it sum} of their values; and  \citet{kleinberg} gave an algorithm with an asymptotic competitive ratio of $1-O(1/\sqrt{k})$. Thus as $k\to \infty$, the competitive ratio approaches  1. Recent literature studied several generalizations of this setting to multidimensional knapsacks \cite{moser1997algorithm}, and proposed algorithms for which the expected online solution approaches the best offline solution as the knapsack sizes becomes large~(e.g., \cite{FHKMS10, devanur-hayes, AgrawalWY14}). 
%\scomment{add citations, Cliff's paper, Devanur and Hayes, my paper on online linear programming etc.}
%\ccomment{I added some of these references to bibtex to the bib file because I had it handy.  Mohammad, you need to add the text and references.}
%\ccomment{Does multiple choice secretary only refer to the case of sum?}
%\mcomment{no it can be any function}
}
%In another variant of multiple-choice secretary problem, \citet{Bateni} and ~\citet{Gupta:2010} introduce 
%the \textit{\nameOfProblem}. In this secretary problem, 
In recent years, submodular optimization has found
%identified as a powerful tool
 applications 
for different 
machine learning and data mining  applications including data summarization,
  sparsity,  active learning, recommendation,  high-order graphical model inference, determinantal point processes~\cite{feldman2018streaming, Badanidiyuru2014StreamingFly,kazemi2019submodular}, network inference, network design~\cite{ghugequasi,friggstad2014linear},  and influence
maximization in social networks~\cite{kazemi2019submodular}.
%Submodularity characterizes a wide variety of discrete optimization problems that naturally occur in machine learning and artificial intelligence [Bilmes and Bai, 2017]. Of particular interest is ubmodular maximization, which captures many novel instances of data summarization such as active set selection in non-parametric learning [Mirzasoleiman et al., 2016b]

In these applications,  the data is generated in a real time, 
and it is important to keep track of the data that is seen so far. Consequently, a line of recent papers studied streaming algorithms for maximizing a submodular function.
%and it is important to maintain at real time a summary of the part of the collection generated so far.
%Submodular maximization has found several new applications in recent years. Some of these include data summarization [LB11, SSSJ12, DKR13], influence
%maximization in social networks [KKT03, CWY09, CWW10, GBL11, SS13], generalized
%assignment[CCPV07], mechanism design [BIK07], and network monitoring [LKG+07].
The first  one-pass streaming algorithm for maximizing a monotone submodular function subject to a $k$-cardinality constraint is due to ~\citet{Badanidiyuru2014StreamingFly}, who propose a ($1/2-\epsilon$)-approximation streaming algorithm, 
with a memory of size $O(\frac{1}{\epsilon}k\log k)$.
Recently,~\citet{kazemi2019submodular} proposed a new algorithm with the same approximation ratio but with improved memory $O(k)$. 

\citet{norouzi} give an upper bound of $1/2+o(1)$ on the approximation ratio achievable by
any algorithm for streaming submodular
maximization that only queries the value of the submodular function on feasible sets (sets of size at most $k$) while using $o(n)$ memory.
Consequently, they initiate the study of the random order streaming model in order to go beyond this worst case analysis for the adversarial order inputs. They achieve a $1/2+8\times 10^{-14}$ approximation for maximizing a monotone submodular function in the random order model, using a memory buffer of size $O(k\log k)$.
Subsequently, \citet{us} substantially improve their result to  $1-1/e-\epsilon-O(1/k)$ approximation which is close to the best possible guarantee in the offline setting, i.e., $1-1/e$ (assuming $P\neq NP$). Furthermore, they improve the required memory buffer to only $O(k)$. 

%In the streaming setting, \citet{Chakrabarti2015} provided a single pass streaming algorithm for monotone submodular function maximization under $k$-cardinality constraint, that achieves a $0.25$ approximation under adversarial ordering of input. Further, their algorithm requires $O(1)$ function evaluations per arriving item and $O(k)$ memory.
%The currently best known approximation  under  adversarial order streaming model is by~\citet{Badanidiyuru2014StreamingFly}, who achieve a $1/2-\epsilon$ approximation with a memory of size $O(\frac{1}{\epsilon}k\log k)$. 
In addition to the simple cardinality constraint, more general constraints
have been studied in the literature.
%For more general constraints than the simple cardinality constraint,
~\citet{Chakrabarti2015} give a $1/4p$ approximation algorithm for streaming monotone submodular functions maximization subject to the intersection of $p$ matroid constraints.  
\citet{Chekuri}
extend it to $p$-matchoids constraints.  A precise definition of
a $p$-matchoid is given in Section~\ref{sec:matchoid}. 
These constraints are generalization of   constraints such as the cardinality constraint,
the intersection of $p$ matroids, and matchings in graphs and hyper-graphs~\cite{Chekuri}.
%A formal definition of a $p$-matchoid is given in Section~\ref{sec:matchoid}. 
Recently,~\citet{feldman2018streaming} designed a more efficient algorithm with lower number of function evaluations achieving  the same approximation $1/4p$.

%value oracle independence oracle
 %Given access to these oracles, 
The algorithms
of~\citet{feldman2018streaming},
%~\citet{Chakrabarti2015} and %~\citet{Chekuri} 
for monotone submodular objective
functions require only $O(k)$ memory ($k$ is the size of the largest feasible
set) and using only $O(kq)$ value and independence oracle queries for processing  each element of the stream ($q$ is a the number of matroids used to define the $p$-matchoid constraint).

Moreover, the greedy algorithm achieves a  $1/(p + 1)$ approximation for $p$-independent systems~\cite{nemhauser1978analysis},  which is tight for all $p$, even for the case of $p$-matroid constraints. Also it is $NP$-hard to approximate the $p$-dimensional matching
within an $\Omega(\log p/p)$ approximation for large but fixed $p$~\cite{hazan2006complexity}.

%The offline greedy algorithm is optimal for submodular function maximization subject to a matroid constraint
%and achieves a
%$1/p$-approximation for $p$-matroid constraints.
%It achieves a
%$1/(p+1)$-approximation for $p$-matroid constraints; for these
%two cases, it is known that it is NP-hard to achieve an approximation factor better than $1-1/e$ and $\Omega(\log p/p)$, respectively.

\toRemove{
\paragraph{Random-order streaming model.}
The {\it  \streamingProblem}~studied in~\cite{norouzi}. In this problem, items from a set $\cal U$ arrive online in random order and the algorithm aims to select a subset $S \subseteq {\cal U}, |S|\le k$ in order to maximize $f(S)$. The streaming algorithm is allowed to maintain a {\it buffer} of size $\eta(k)\ge k$. 

\citet{Hess} initiated the study of  \streamingProblem.
Their algorithm uses $O(k)$ memory and a total of $n$ function evaluations to achieve $0.19$ approximation. 
The state of the art result in the random order input model is due to \citet{norouzi} who achieve a $1/2+8\times 10^{-14}$ approximation, while using a memory buffer of size $O(k\log k)$.
They also give an upper bound of $1/2+o(1)$ on the competitive ratio achievable by  any algorithm for streaming submodular
maximization that only queries the value of the submodular function on feasible sets while using $o(n)$ memory~\cite{norouzi}.
}
\paragraph{\textbf{The shortlist model}.}
%\paragraph{The \nameSecSL.}
%\paragraph{The \nameOfProblemSL.}
In~\cite{us}, a relaxation of the secretary problem  is introduced
%.  What if  the online algorithm for secretary problem
where the algorithm is allowed to  select a {\it shortlist} of items that is larger than the number of items that ultimately need to be selected. after seeing the entire input, the algorithm can choose from the bigger set of items in the shortlist. 
%That is, in a {\nameOfProblem}, the algorithm is allowed to choose more than $k$ items as part of a shortlist. Then, after seeing the entire input, the algorithm can choose a subset of size $k$ from the bigger set of items in the shortlist. 
%when seeing items online, and ultimately maximizes a function of $k$ elements, 
%we are allowed to choose more than $k$ elements, and then after seeing the entire input, choose a  a subset of size $k$ from our bigger set. 
This model is closely related to the random order streaming model. A comprehensive comparison between these two models can be found in~\cite{us}.
The main result of~\cite{us} is an online algorithm  for \nameOfProblemSL\ that, for any constant $\epsilon>0$, achieves a competitive ratio of $1-\frac{1}{e} - \epsilon-O(\frac{1}{k})$ with shortlist of size $ O(k)$. They also provide an implementation of their algorithm in the streaming setting with the same approximation ratio and memory $O(k)$. 
\toRemove{
This new model is motivated by some practical applications of secretary problems, such as hiring (or assignment problems),  where in some cases it may be possible to tentatively accept a larger number of candidates (or requests), while deferring the choice of the final $k$-selections to after all the candidates have been seen. Since there may be a penalty for declining candidates who were part of the shortlist, one would prefer that the shortlist is not much larger than $k$.
}
\toRemove{
Another important motivation is theoretical: we wish to understand to what extent this relaxation of the secretary problem can improve the achievable competitive ratio. This question is in the spirit of several other methods of analysis that allow an online algorithm to have additional power, such as {\em resource augmentation} \cite{KalyanasundaramP00,PhillipsSTW97}.


The potential of this relaxation is illustrated by the basic secretary problem, where the aim is to select the item of maximum value among randomly ordered inputs. There, it is not difficult to show that if an algorithm  picks every item that is better than the items seen so far, the true maximum will be found, while the expected number of items picked under randomly ordered inputs will be $\log(n)$. Further, we show that this approach can be easily modified to get the maximum with $1-\epsilon$ probability while picking at most  $O(\ln(1/\epsilon))$ items for any constant $\epsilon>0$. Thus, with just a constant size shortlist, we can break the $1/e$ barrier for the secretary problem and achieve a competitive ratio that is arbitrarily close to $1$.

%For the secretary problem, we can imagine choosing not one secretary, but several, and then taking the best one at the end.  
}
\paragraph{\textbf{The \nameOfProblemMatroidSL}.} Motivated by the improvements achieved for the competitive ratio of  \nameOfProblem\ in the \textit{shortlist} model, we ask if similar improvements can be achieved by relaxing the \nameOfProblemMatroid~to have a shortlist. That is, instead of choosing an independent set of a matroid $\mathcal{M}$ with $rk(\mathcal{M})=k$, the algorithm is allowed to chose  $\eta(k)$ items as part of a shortlist, for some function $\eta$;
and at the end of all inputs, the algorithm chooses an independent subset of items from the $\eta(k)$ selected items. Then what is the best competetive ratio that we can achieve 
in this model for example  when 
 $\eta(k)=O(k)$? Is it possible to improve the best known competetive ratio for matroid secretary problem in this model? 
%Then, what is the relationship between $\eta(\cdot)$ and the competitive ratio for this problem? Can we achieve a solution close to the best offline solution when $\eta(k)$ is not much bigger than $k$, for example  when  $\eta(k)=O(k)$?  
%We answer this question affirmatively in this paper, and provide an algorithm 
%What is the relationship between $\eta$ and the competitive ratio. 
%In other words, we have a {\em shortlist} of size $\eta(k)$, where $\eta(k)$ is independent of $n$, and the output is subset of this shortlist.
%We wish to understand how much this relaxation can improve the competitive ratio.   In other words, what is the relationship between $\eta$ and the competitive ratio.
 %For exmaple, when the  it is possible to approach the optimal offline solution by some function $\eta$ as $k\to \infty$.  Can we obtain a similar results for the \nameOfProblemSL.
%\ccomment{Is there a practical-ish motivation for this model?}
%A motivation for this model is that for the $k$-secretary problem instead of restricting ourselves to make irrevocable decisions for each item, we may add items to a shortlist and defer the final decision to the end (choosing $k$ elements from shortlist). We want the size of shortlist to be as small as possible.

%\paragraph{\textbf{Problem definition.}}
\subsection{Problem definition}
We now give a more formal definition. We are given matroid $\mathcal{M}=(\mathcal{N},\mathcal{I})$, with $rk(\mathcal{M})=k$.
Items from a set ${\mathcal{ U}} = \{a_1, a_2, \ldots, a_n\}$  (pool of items) arrive in a uniformly random order over $n$ sequential rounds. The set ${\mathcal U}$ is apriori fixed but unknown to the algorithm, and the total number of items $n$ is known to the algorithm. In each round, the algorithm irrevocably decides whether to add the arriving item to a { shortlist} $A$ or not. %The goal is to return,  at the end of $n$ rounds, a shortlist $A$ of size at most $\eta(k) \ge k$ to maximize the  `value' of best $k$ subset of this shortlist. More formally, 
%We are given a monotone submodular function $f:2^{\cal U} \rightarrow \mathbb{R}$, in a value oracle model. %Let the set $A \subseteq {\cal U}, |A|\le \eta(k)$ denote the shortlist of items selected by the online algorithm,  then 
The algorithm's value at the end of $n$ rounds is given by 
$$\ALG = \Ex[\max_{S\subseteq A, S\in \mathcal{I}} f(S)]$$ 
where $f(\cdot)$ is a monotone submodular function. The algorithm has value oracle access to this function.
The optimal offline utility is given by
$$\OPT:=f(S^*), \text{ where } S^*=\arg \max_{S \subseteq [n], S\in \mathcal{I}} f(S).$$ 
We say that an algorithm for this problem achieves a competitive ratio  $c$ using shortlist of size $\eta(k)$, if at the end of $n$ rounds, $|A|\le \eta(k)$ and $\frac{\ALG}{\OPT}\ge c$.

Given the shortlist $A$, since the problem of computing the solution $\arg \max_{S\subseteq A, S\in \mathcal{I}} f(S)$ can itself be computationally intensive, our algorithm will also track and output a subset $A^* \subseteq A, |A^*| \le k$. %We will lower bound  the competitive ratio by bounding $\frac{f(A^*)}{f(S^*)}$.


%\paragraph{\textbf{Our results.}}
\subsection{Our Results}
We design an algorithm that achieves a $\frac{1}{2}(1-1/e^2-\epsilon-O(1/k))$ competitive ratio for any constant $\epsilon>0$, using a shortlist of size $O(k)$ for the matroid secretary problem with shortlists. This is especially surprising considering that the best known competitive ratio for the matroid secretary problem is $O(\log \log k)$. We are also able to get a constant competitive algorithm using shortlist of size  at most $k$ and also a constant competitive algorithm in the preemption model.



\begin{restatable*}{theorem}{matroidThm} \label{opttheorem}
For any constant $\epsilon>0$, there exists an online algorithm (Algorithm \ref{alg:main}) for the \nameOfProblemMatroidSL\ that achieves a competitive ratio of $\frac{1}{2}(1-\frac{1}{e^2} -\epsilon -O(\frac{1}{k}))$, with shortlist of size $\eta_\epsilon(k)=O(k)$. Here,  $\eta_\epsilon(k)=O(2^{poly(1/\epsilon)}k)$. The running time of this online algorithm is $O(nk)$.
\end{restatable*}

\begin{restatable*}{theorem}{thmpreemption} \label{thm:preemption}
For the matroid secretary problem in the preemption model, and matroid secretary problem 
that uses shortlist of size at most $\eta(k)=k$,
there is an algorithm 
%the algorithm~\ref{alg:main} 
%(with $\alpha=\beta=1$) 
that achieves a constant competitive ratio. %$\frac{1}{2} (1-1/e) (1-1/e^2-\epsilon)$.
\end{restatable*}

Furthermore,  for a more general constraint, namely $p$-matchoid constraints (defined in section~\ref{sec:matchoid}) we prove:

\begin{restatable*}{theorem}{matchoidThm} \label{opttheoremmatchoid}
For any constant $\epsilon>0$, there exists an online algorithm for the submodular secretary problem with $p$-matchoid constraints that achieves a competitive ratio of $\frac{1}{p+1}(1-\frac{1}{e^{p+1}} -\epsilon -O(\frac{1}{k}))$, with shortlist of size $\eta_\epsilon(k)=O(k)$. Here,  $\eta_\epsilon(k)=O(2^{poly(1/\epsilon)}k)$. The running time of this online algorithm is $O(n\kappa^{p})$, where $\kappa= \max_{i\in[q]} rk(\mathcal{M}_i)$.
\end{restatable*}


The  proposed  algorithm  also  has  implications  for  another  important  problem
of submodular function maximization under random order streaming model and matchoid constraints.
%We show that our algorithm can be implemented in the streaming setting using $O(k)$ memory. It achieves 
%$\frac{1}{2}(1-1/e^2-\epsilon-O(1/k))$ 
$\frac{1}{p+1}(1-1/e^{p+1}-\epsilon-O(1/k))$
approximation. 
%The previously best known approximation ratio for streaming submodular maximization under matroid constraint  is 0.25 (adversarial order) due to Chekuri et al. and Chakrabarti et al. 
%using memory buffer of $O(k\log k)$.
%Recently, Feldman et al give an algorithm with the same approximation but with improved memory $O(k)$.
%Furthermore, we generalize our results to the case of p-matchoid constraints and give a $\frac{1}{p+1}(1-1/e^{p+1}-\epsilon-O(1/k))$ approximation using $O(k)$ memory.


\begin{restatable*}{theorem}{thmStreamingMatroid}
\label{thm:streamingMatroid}
For any constant $\epsilon\in (0,1)$, there exists an algorithm for the \streamingProblem\ with matroid constraints  that achieves $\frac{1}{2}( 1-\frac{1}{e} -\epsilon -O(\frac{1}{k}))$ approximation to $\OPT$ while using a memory buffer of size at most $\eta_\epsilon(k)=O(k)$. Also, the number of objective  function evaluations for each item, amortized over $n$ items, is $O(pk+\frac{k^2}{n})$.
\end{restatable*}



\begin{restatable*}{theorem}{thmStreamingMatchoid}
\label{thm:streamingMatcoid}
For any constant $\epsilon>0$, there exists an algorithm for the \streamingProblem\ with $p$-matchoid constraints  that achieves $\frac{1}{p+1}(1-\frac{1}{e^{p+1}} -\epsilon -O(\frac{1}{k}))$ approximation to $\OPT$ while using a memory buffer of size at most $\eta_\epsilon(k)=O(k)$. Also, the number of objective  function evaluations for each item, amortized over $n$ items, is $O(p\kappa+\kappa^p+\frac{k^2}{n})$, where $\kappa= \max_{i\in[q]} rk(\mathcal{M}_i)$.
\end{restatable*}


\toRemove{
In this paper, we answer this question affirmatively by giving a polynomial time algorithm that achieves $1-1/e-\epsilon-O(k^{-1})$ competitive ratio for the \nameOfProblem~using a shortlist of size $\eta(k)=O(k)$. This is surprising since $1-1/e$ is the best achievable approximation (in polynomial time) for the offline problem. Further, for some special cases of submodular functions, we demonstrate that an $O(1)$ shortlist allows us to achieve a $1-\epsilon$ competitive ratio. These results demonstrate the power of (small) shortlists for closing the gap between online and offline (polynomial time) algorithms. 
%size we give a new algorithm and show several positive (and one negative) results that capture the power of these shortlists and  show that they are (surprisingly) powerful. 
}
\toRemove{
We also discuss connections of {\nameSecSL} to the related streaming settings. While a streaming algorithm does not qualify as an online algorithm (even when a shortlist is allowed), we show that our algorithm can in fact be implemented in a streaming setting to use $\eta(k)=O(k)$ memory buffer; and our results significantly  improve  the available results for the \streamingProblem.
Furthermore since the upperbound given in ~\cite{mcgregor2017better} holds for random order streams, our result is asymptotically tight in this setting.
}
\toRemove{
\subsection{Problem Definition}
%In the well-studied submodular $k$-secretary problem, applicants from a set ${\cal U} = \{a_1, a_2, \ldots, a_n\}$  (pool of applicants) arrive in a uniformly random order over $n$ sequential rounds. In each round, an online algorithm irrevocably decides whether to select an applicant or not. The algorithm can select at most $k$ applicant. The goal is to maximize the value of the selected $k$ applicants, as given by a submodular function $f$. 

%More formally, let $S, |S|\le k$ denote the subset of candidates selected by the algorithm, then the expected utility of the algorithm is given by $\ALG:=\Ex[f(S)]$, where $f$ is a monotone submodular function, and the expectation taken both over random order and possible randomness in the algorithm's selection of subset $A$ given an order. The competitive ratio of the online algorithm is then defined as $\frac{\ALG}{\OPT}$, where $\OPT$ is the optimal offline utility defined as 
%$$\OPT=f(S^*), \text{ where, } S^*=\arg \max_{S \subseteq [n], |S|\le k} f(S).$$

%\scomment{edited by me on 8/21}
We now give a more formal definition.
Items from a set ${\cal U} = \{a_1, a_2, \ldots, a_n\}$  (pool of items) arrive in a uniformly random order over $n$ sequential rounds. The set ${\cal U}$ is apriori fixed but unknown to the algorithm, and the total number of items $n$ is known to the algorithm. In each round, the algorithm irrevocably decides whether to add the arriving item to a {\it shortlist} $A$ or not. %The goal is to return,  at the end of $n$ rounds, a shortlist $A$ of size at most $\eta(k) \ge k$ to maximize the  `value' of best $k$ subset of this shortlist. More formally, 
%We are given a monotone submodular function $f:2^{\cal U} \rightarrow \mathbb{R}$, in a value oracle model. %Let the set $A \subseteq {\cal U}, |A|\le \eta(k)$ denote the shortlist of items selected by the online algorithm,  then 
The algorithm's value at the end of $n$ rounds is given by 
$$\ALG = \Ex[\max_{S\subseteq A, |S|\le k} f(S)]$$ 
where $f(\cdot)$ is a monotone submodular function. The algorithm has value oracle access to this function.

The optimal offline utility is given by
$$\OPT:=f(S^*), \text{ where } S^*=\arg \max_{S \subseteq [n], |S|\le k} f(S).$$ 
We say that an algorithm for this problem achieves a competitive ratio  $c$ using shortlist of size $\eta(k)$, if at the end of $n$ rounds, $|A|\le \eta(k)$ and $\frac{\ALG}{\OPT}\ge c$.

Given the shortlist $A$, since the problem of computing the solution $\arg \max_{S\subseteq A, |S|\le k} f(S)$ can itself be computationally intensive, our algorithm will also track and output a subset $A^* \subseteq A, |A^*| \le k$. We will lower bound  the competitive ratio by bounding $\frac{f(A^*)}{f(S^*)}$.

The above problem definition has connections to some existing problems studied in the literature. The well-studied online \nameOfProblem~described earlier is obtained from the above definition by setting $\eta(k)=k$, i.e., it is same as the case when no extra items can be selected as part of a shortlist. 
%\scomment{Did a pass on the para below on 8/30 after our discussion regarding streaming problem}
Another related problem is {\it  \streamingProblem}~studied in~\cite{norouzi}. In this problem, items from a set $\cal U$ arrive online in random order and the algorithm aims to select a subset $S \subseteq {\cal U}, |S|\le k$ in order to maximize $f(S)$. The streaming algorithm is allowed to maintain a {\it buffer} of size $\eta(k)\ge k$. 
However, this streaming problem is distinct from the \nameOfProblemSL\ in several important ways. On one hand, since an item previously selected in the memory buffer can be discarded and replaced by a new items, a memory buffer of size $\eta(k)$ does not imply a shortlist of size at most $\eta(k)$. On the other hand, in the secretary setting, we are allowed to memorize/store more than $\eta(k)$ items without adding them to the shortlist. Thus an algorithm for \nameOfProblem with shortlist of size $\eta(k)$ may potentially use a buffer of size larger than $\eta(k)$. 
Our algorithms, as described in the paper, do use a large buffer, but we will show
%\ccomment{Where do we show that the streaming actually works}
that the algorithm presented in this paper can in fact be implemented to use only $\eta(k)=O(k)$ buffer, thus obtaining matching results for the streaming problem. 
%imply the same competitive ratio for random order streaming problem with buffer of size $\eta(k)$, but not vice-versa. We will discuss the corollary of our algorithm design and analysis for the  submodular random order streaming problem. 
%Because shortlists can be used as a buffer for memory but not vice versa. ( we are allowed to delete from memory and reduce the size but we can not remove from a shortlist)







%In the new `submodular $k$-secretary with shortlist' problem considered in this paper, we allow the online algorithm to select a shortlist of more than $k$ candidates, and pick the final subset of $k$ candidates from this shortlist at the end. Specifically,  we allow the online algorithm to select a subset $A$ of size $|A|\le \eta(k)$, where $\eta(k)\ge k$. The competitive ratio of the online algorithm is then defined with respect to the best $k$-subset of $A$. That is, competitive ratio is given by $ \frac{\ALG_{\eta}}{\OPT}$, where $\OPT$ as defined before, and 
%$$\ALG_\eta = \Ex[\max_{S\subseteq A, |S|\le k} f(S)],$$ 
%with $A$ being the subset of items selected by the online algorithm, of size at most $\eta(k)$. 

\subsection{Our Results}
Our main result is an online algorithm  for \nameOfProblemSL\ that, for any constant $\epsilon>0$, achieves a competitive ratio of $1-\frac{1}{e} - \epsilon-O(\frac{1}{k})$ with $\eta(k) = O(k)$. 
Note that for \nameOfProblem\ there is an upper bound of $1-1/e$ on the achievable approximation factor, even in the offline setting, and this upper bound applies to our problem for arbitrary size $\eta(\cdot)$ of shortlists. On the other hand for online monotone \nameOfProblem, i.e., when $\eta(k)=k$, the best competitive ratio achieved in the literature is $1/e-O(k^{-1/2})$~\cite{kesselheim} 
%\scomment{is there an upper bound? } \mcomment{ No} 
Remarkably, with only an $O(k)$ size shortlist, our online algorithm is able to achieve a competitive ratio that is arbitrarily close to the offline upper bound of $1-1/e$.

In the theorem statements below, big-Oh notation $O(\cdot)$ is used to represent asymptotic behavior with respect to $k$ and $n$. We assume the standard  value oracle model:  the only access to the submodular function is through a black box
returning $f(S)$ for a given set $S$, and  each such queary can be done in $O(1)$ time. 
%\ccomment{Define value oracle model and state thm.1 appropriately}
\begin{theorem} \label{opttheorem}
For any constant $\epsilon>0$, there exists an online algorithm (Algorithm \ref{alg:main}) for the \nameOfProblemMatroidSL\ that achieves a competitive ratio of $1-\frac{1}{e} -\epsilon -O(\frac{1}{k})$, with shortlist of size $\eta_\epsilon(k)=O(k)$. Here,  $\eta_\epsilon(k)=O(2^{poly(1/\epsilon)}k)$.  
%$$\eta_\epsilon(k) =c k\log(1/\epsilon) {\frac{1}{\epsilon^3} \log(1/\epsilon)  \choose {\frac{1}{\epsilon^2} \log(1/\epsilon)}} =O(2^{poly(1/\epsilon)}) \ ,$$
%for some absolute constant $c$.
% for submodular secretary problem with cardinality constraints, such that it selects $O(k)$ elements. %, where $C(a)$ is a constant depending only on $a$.
  The running time of this online algorithm is $O(n)$.
\end{theorem}
%\scomment{Can we add a compact description of dependence of  $\eta_\epsilon(k)$ on $\epsilon$ in this theorem statement? What is this function: exponential or super-exponential in $1/\epsilon$?}
%\scomment{Should we say $O(n)$ evaluations of the objective function instead of time?}
%\scomment{After fixing the proof in section 3, I am getting a different (much bigger) dependence on $1/\epsilon$. Mohammad, can you check? May be considering this, we should leave it here as $\eta_\epsilon(k)=O(2^{poly(1/\epsilon)}$?}
%\scomment{I see that the theorem statement was changed, but we still need to provide the exact function, may be right after the theorem statement. Adding below:}

%Specifically, we have $\eta_\epsilon(k)=$\etaMacro$k$ for some constant $c$.
%The running time  of our algorithm is linear in $n$, the size of the input, which 
%is significant as, until recently, it was not known if there exists a linear time algorithm achieving a $1-1/e-\epsilon$ approximation even for the offline monotone submodular maximization problem under cardinality constraint\cite{linear}. 
Similar to~\cite{us}, an interesting aspect of our algorithm is that it is highly parallel. Even though the decision for each arriving item may take time that is exponential in $1/\epsilon$ (roughly  $\eta_\epsilon(k)/k$), it can be readily parallelized among multiple (as many as $\eta_\epsilon(k)/k$) processors. 
%The  operations required to make a decision for each item can be divided between available processors. (the running time will be divided by $\min(c,p)$ where $c=k\log(1/\delta) {\frac{1}{\delta^3} \log(1/\delta)  \choose {\frac{1}{\delta^2} \log(1/\delta)}}$ is the hidden constant in $O(k)$ and $p$ the number of processors )


%More precisely, we design a $1-1/e-\epsilon-O(k^{-1})$ competitive algorithm that selects $O(k\log(1/\delta) {\frac{1}{\delta^3} \log(1/\delta)  \choose {\frac{1}{\delta^2} \log(1/\delta)}})$ elements, i.e., the dependency on $k$ is linear and on $\delta$ is exponential.



%\scomment{Add a formal corollary of Theorem 1 for random-order streaming problem here. Also, will be good to add a few lines in problem definition section describing how our problem relates to random order streaming.} \mcomment{done done}


%As discussed earlier, by definition, a corollary of our results is an algorithm for the submodular random order streaming problem with the same competitive ratio.
Further, we show an implementation of Algorithm 2 that uses a memory buffer of size at most $\eta_\epsilon(k)$ to get the following result for the problem of {\it \streamingProblem} described in the previous section. 
%\ccomment{Make terminology for evaluations consistent with previous work}
\begin{restatable}{theorem}{thmStreaming}
\label{thm:streaming}
For any constant $\epsilon\in (0,1)$, there exists an algorithm for the \streamingProblem  that achieves $1-\frac{1}{e} -\epsilon -O(\frac{1}{k})$ approximation to $\OPT$ while using a memory buffer of size at most $\eta_\epsilon(k)=O(k)$. Also, the number of objective  function evaluations for each item, amortized over $n$ items, is $O(1+\frac{k^2}{n})$.
%Also, decision for each arriving item requires $O(1)$ evaluations of the objective function.
%Also in amortized time, it processes each arriving item with $O(1+\frac{k^2}{n})$ evaluations of the objective function.
%Also the amortized time to processes each arriving item requires $O(1+\frac{O(k^2)}{n})$ evaluations of the objective function.
% The running time of this online algorithm is $O(n)$.
\end{restatable}
%The above result significantly improves over the state-of-the-art results in random order streaming model \cite{norouzi}, which are an approximation ratio of $\frac 1 2+8\times 10^{-14}$ using a memory of size $O(k\log k)$. 
%uses $O(k)$ memory and achieves asymptotic $R<1-1/e$ approximation.

%\scomment{I don't understand the upper bound stated below - by arbitrary $\eta$, couldn't we get at best the the offline problem. I can just select everything into shortlist. So, is the below giving an upper bound for the offline problem?  } \mcomment{using $o(n)$ selections. No it is for online problem}

%As a result, we show that in our model $\eta(k)=\gamma.k$, where $\gamma$ is a constant. It is optimal up to a constant factor.
%The constant factor $\gamma$ is growing as the competitive ratio gets closer to $1-1/e$. 
%Because of the known upper bound for offline submodular maximization with cardinality constraint.
%It is obvious that we can not get better than $1-1/e$ competitive algorithm if we only consider  polynomial time algorithms. 

%It is natural to ask whether these $k$-lists are, in fact, too powerful.  Maybe they could actually allow us to always match the best offline algorithm.  We give a negative result in this direction and 
%show that even if we have unlimited computation power, for any function $\eta(k)=o(n)$, we can get no better than $7/8$-competitive algorithm using a shortlist of size $\eta(k)$. Note that with unlimited computational power, the offline problem can be solved exactly. This result demonstrates that 
%having a shortlist does not make the online problem too easy - 
%even with a shortlist (of size $o(n)$) there is an information theoretic gap between the online and offline problem. Note that the $1-1/e$ upperbound for streaming model~\cite{mcgregor2017better} 
%does not imply an upper bound for the shortlist model.

\toRemove{
%\mcomment{we should emphasize the upper bound is for any $k$, i.e., it holds asymptotically}
\begin{restatable}{theorem}{hardness}
%\begin{theorem} 
\label{hardness}
No online algorithm (even with unlimited computational power)   can achieve a competitive ratio better than $7/8+o(1)$ for the \nameOfProblemSL, while using a shortlist of size $\eta(k)=o(n)$.
%by selecting $\eta(k)$ elements for any function $\eta$ (independent of $n$).
\end{restatable}
%\end{theorem}

%\scomment{By independent of $n$, do you mean $\eta(k)$ does not grow with $n$, i.e., $\eta(k)=O(1)$ if $O(\cdot)$ denotes asymptotic with respect to $n$? This is not same as $o(n)$, e.g.. $\eta(k)=\sqrt{n}$ would also be $\eta(k)=o(n)$.} \scomment{We need to discuss this issue}
 
 % It also improves~\cite{Badanidiyuru2014StreamingFly} on random order inputs.
%(Note that in our algorithm we keep extra items in the shortlist only for a limited time $O(n/k)$, and then we are able to release them.
%That is why the extra memory is $O(1)$ instead of $O(k)$).

%Another interesting aspect of our algorithm is that it is highly parallel. In order to decide whether or not to select an item in a slot $s_i$ in window $W$ which consists of $\{s_1, \dots, s_{\alpha \beta}\}$,
%the algorithm concurrently run several online maximum algorithms to find the maximum marginal value with respect to %different subsets.
% $S\cup \gamma(\tau)$, where $\tau$ is a subset of slots $\{s_1,\dots, s_{i-1}\}$ with $|\tau|<\alpha$.
%We select a new item if any of the maximum algorithms (for some $\tau$) select it, otherwise we do not select it. All the maximum algorithms for different subsets $\tau$ can be run in parallel. 

%Although the update time in our algorithm is $O(1)$, the constant can be very large. Consequently it may not be desirable for large streams. 
%We take two approaches to improve it. The first approach is parallel algorithms. The interesting fact about our algorithm is that it is highly parallel, i.e. the  operations required for each element can be divided between as many processor as it is available. 
%The running time will be divided by the number of processors. 

%In addition, we design a fast  thresholding algorithm that requires only one function evaluation per element.
%It achieves competitive ratio $1/2-O(1/\sqrt{k})$ by selecting $k\log^2k$ elements. The competitive ratio and the update time of this algorithm is still better than~\cite{kesselheim} and~\cite{Hess}. In ~\cite{kesselheim}  update time is $O(n^2)$. 
%In terms of memory, our thresholding algorithm uses less memory than~\cite{Badanidiyuru2014StreamingFly} but more than~\cite{Hess}.


%We also provide an upper bound showing that it is not possible to achieve any competitive ratio better than $7/8$ by selecting $O(g(k))$ elements, where $g$ is an arbitrary function, even if we have free computation.
%\scomment{Can you add a theorem statement for the results discussed below?} \mcomment{added}
Finally, for some special cases of monotone submodular functions, we can asymptotically approach the optimal solution.
%\ccomment{Don't mention this as a thm.}
%\begin{theorem}
%Suppose $F$ is a monotone submodular function and $F(a_1,\cdots, a_i+\alpha,\cdots, a_k)  \ge  F(a_1, \cdots, a_i, \cdots, a_k  )$, for any  $\alpha >0$ and $1\le i \le k$.
%Let $S$ be the elements selected by Kleinberg's algorithm~\cite{kleinberg}, then
%$E[F(S)]>(1-5/\sqrt{k})OPT$.
%%Let $T$ be the $k$ largest elements of $S$, and $OPT=f(T)$.
%The expected number of elements of $T$ selected by the algorithm is at least $(1 -5/\sqrt{k})k$.
%\end{theorem}
%\begin{enumerate}
%\item $F$ is a monotone submodular function, and $F(a_1,\cdots, a_i+\alpha,\cdots, a_k)  \ge  F(a_1, \cdots, a_i, \cdots, a_k  )$, for $\alpha >0$ and $1\le i \le k$.
%\end{enumerate}
%We show Kleinberg's algorithm asymptotically approaches optimal solution.
%We prove that the Kleinberg algorithm works under this assumption which means that the competitive ratio of the algorithm asymptotically approaches 1.
The first one is the family of functions we call $m$-submdular. 
A function $f$ is $m$-submodular if it is submodular and there exists a submodular function $F$ such that for all $S$:
%\begin{itemize}
%\item 
\[ 
f(S)= \max_{T\subseteq S, |T|\le m} F(T) \ .
\]
%\end{itemize}
\scomment{This needs to be rewritten, I don't have time right now, so removing: Example of $m$-submodular functions are   maximum node weighted bipartite matching and  maximum edge weighted bipartite matching defined on $G=(X\times Y)$ with $|Y|=m$.  (the assignments will be done at the end of algorithm after all the selections are made).}

%\scomment{
%What is $\epsilon, \delta$? I removed this and restated inline with our rest of the results.
%\begin{theorem}
%For any $m$-submodular function $F$ there is an Algorithm that selects a set $S$ with $|S|<m\ln (1/\epsilon)+\ln(1/\delta)+\sqrt{\ln^2{1/\delta}+2m\ln(1/\delta)\ln(1/\epsilon)}$ and $E[F(S)]=(1-\epsilon-\delta)OPT$.
%\end{theorem}
%}
%\begin{restatable}{theorem}{msub}
\begin{theorem}
\label{thm:msub}
If $f$ is an $m$-submodular function, there exists an online algorithm for the \nameOfProblemSL~that achieves a competitive ratio of $1-\epsilon$ with shortlist of size $\eta_{\epsilon,m}(k)=O(1)$. Here, 
$\eta_{\epsilon,m}(k) = (2m+3) \ln(2/\epsilon)$.
\end{theorem}
%\end{restatable}
A proof of Theorem~\ref{thm:msub} along with the relevant algorithm (Algorithm \ref{alg:SIII}) appears in the appendix.

Another special case  is  monotone submodular functions $f$ satisfying the following property:
$f(\{a_1,\cdots, a_i+\alpha,\cdots, a_k\})  \ge  f(\{a_1, \cdots, a_i, \cdots, a_k \})$, for any $\alpha >0$ and $1\le i \le k$.
We can show that the algorithm by \citet{kleinberg} asymptotically approaches optimal solution for such functions, but we omit the details.

}





%We call an algorithm $ALG$ c-competitive if for any objective function $F$ chosen by the adversary, the
%set of selected items $ALG$ satisfies $E [F(ALG)] \ge (c ? o(1)) · OPT$, where $OPT$ is a feasible
%(offline) solution that maximizes v and the o(1)-term is asymptotical with respect to the length of
%the sequence n. 










%What is the minimum size shortlist to get a  $c$-competitive algorithm?
%These are questions that we consider in this paper.



%The submodular secretary problem, introduced by Bateni2013SubmodularExtensions et al. and Gupta et al., is an
%online variant of monotone submodular maximization subject to cardinality constraints. In this
%problem, we are allowed to select up to k items from a set of n items.
%The value of a set is represented by a monotone, submodular function.
%The values of the submodular function are only known on subsets of the items that have already arrived.
%The objective function is designed by an adversary, but the order of the items is uniformly at random.




%It is well-known since 1963 [10]
%that the optimal policy is to interview the first t ? 1 applicants, then hire the next one whose quality exceeds that of
%the first t ? 1 applicants, where t is defined by ; as $n \to \infty$, the probability of hiring
%the best applicant approaches 1/e, as does the ratio t/n.
%Note that a solution to the secretary problem immediately
%yields an algorithm for a slightly different objective function optimizing the expected value of the chosen element.





%In secretary problem, we are given a random order input and we are going to select the maximum element.
%In the classic secretary problem, one is presented a sequence of items with different scores online in
%random order. Upon arrival of an item, one has to decide immediately and irrevocably whether to
%accept or to reject the current item.  The objective is to accept the best of these items. 




%Multiple Choice secretary problem:


%Submodular Secretary problem:



%Our extension


%Streaming model:





% Imagine that you
%manage a company, and you want to hire a secretary from a pool of n applicants. You are very keen on hiring only
%the best and brightest. Unfortunately, you cannot tell how good a secretary is until you interview him, and you must
%make an irrevocable decision whether or not to make an offer at the time of the interview. The problem is to design
%a strategy which maximizes the probability of hiring the most qualified secretary. It is well-known since 1963 [10]
%that the optimal policy is to interview the first t ? 1 applicants, then hire the next one whose quality exceeds that of
%the first t ? 1 applicants, where t is defined by ; as $n \to \infty$, the probability of hiring
%the best applicant approaches 1/e, as does the ratio t/n. Note that a solution to the secretary problem immediately
%yields an algorithm for a slightly different objective function optimizing the expected value of the chosen element.




%In this paper, we consider general monotone submodular functions.



%The submodular secretary problem, introduced by Bateni2013SubmodularExtensions et al. and Gupta et al., is an
%online variant of monotone submodular maximization subject to cardinality constraints. In this
%problem, we are allowed to select up to k items from a set of n items.
%The value of a set is represented by a monotone, submodular function.
%The values of the submodular function are only known on subsets of the items that have already arrived.
%The objective function is designed by an adversary, but the order of the items is uniformly at random.

%We call an algorithm c-competitive if for any objective function v chosen by the adversary, the
%set of selected items ALG satisfies $E [v(ALG)] \ge (c ? o(1)) · v(OPT)$, where $OPT$ is a feasible
%(offline) solution that maximizes v and the o(1)-term is asymptotical with respect to the length of
%the sequence n. 

\scomment{The susection "Our techniques" was describing analysis and algorithm design techniques that are not being used in the proof anymore, there is no time to revise it, so I am removing it. Most of this intuition appears in algorithm description and proof overview anyway.}
\toRemove{
\subsection{Our techniques}
First we design a simple algorithm for the classic secretary problem  (finding the maximum element) that achieves a competitive ratio  of $1-\epsilon$ (for any $\epsilon>0$)  using a shortlist of size $O(\log(1/\epsilon))$.
%for a class of submodular functions that we call them $m$-submodular,
%for any $m>0$. 
The algorithm  ignores an $\epsilon$-fraction of the input and then selects an item if it is greater than the maximum element seen so far. 
We show that with probability $1-\epsilon$, the total number of selections made by this algorithm is at most $O(\log (1/\epsilon))$.
%A special $m$-submodular function for $m=1$ is the function $\max$. 
%As a result we 
We will use this online algorithm as a subroutine in our proposed algorithm for \nameOfProblemSL, for repeatedly finding (with probability $1-\epsilon$) the  item with maximum marginal value with respect to a subset of items, under submodular function $f$.  %It requires $\log(1/\epsilon)$ selections.
The main idea of the algorithm for \nameOfProblemSL\ is to divide the input into some blocks that we call them $(\alpha,\beta)$ \textit{windows}.  In this procedure, we partition the input into slots, where the sizes of the slots follow a balls-and-bins distribution.  We then group these slots into windows.
%Divide the input into $k\beta$ slots. The $i$-th slot, $s_i$, consists of $X_i$ consecutive elements of the input.
%Random variables $\{X_i\}$  for $i\in [k\beta]$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
%A \textit{window}, represented by parameters $(\alpha,\beta)$, consists of $\alpha \beta$ consecutive slots.
%\begin{definition} 
%A \textit{window}, represented by parameters $(\alpha,\beta)$, consists of $\alpha$ consecutive intervals, 
%of length $n/k$. 
%each interval is divided into $\beta$ slots. The length of $i$-th slot is a random variable denoted by $X_i$.
%Random variables $\{X_i\}$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
%random sample from the binomial distribution $B(n,\frac{1}{k\beta})$.
%of length $\frac{n}{k\beta}$.
%\end{definition}
%It consists of $\alpha$ consecutive intervals, 
%%of length $n/k$. 
%each interval is divided into $\beta$ slots. The length of $i$-th slot is a random variable denoted by $X_i$.
%Random variables $\{X_i\}$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
%%random sample from the binomial distribution $B(n,\frac{1}{k\beta})$.
%%of length $\frac{n}{k\beta}$.
%%Each window consists of smaller subintervals that we call them \textit{slots}.
Applying concentration inequalities for each {window}, and show that each window  has  roughly $\alpha$ elements of $OPT$ (the optimal solution), w.h.p.,
%the probability increases as $\alpha$ increases.
and that the fraction of elements of $OPT$ in a window that lie in different slots is at least $1-1/\beta$.
Therefore by choosing $\beta$ large enough most of the items in a window are in different slots, roughly speaking.\newline
For each window $w$ the algorithm \textit{guesses} the slots in which elements of $OPT$ in  $w$ lie in. 
By \text{guess} we mean that the algorithm enumerates over all subsets of size $\alpha$ of all $\alpha\beta$  slots in  $w$, and choose 
the one with the maximum marginal gain with respect to previously selected items. This can be done in an online manner.\newline
In the analysis of the algorithm for each window $w$,
we define an event $T_{1,\cdots, w-1}$ which conditions on the elements selected by the algorithm and also the positions in which they get selected by the algorithm. 
By conditioning on $T_{1,\cdots, w-1}$, we prove a lower bound for the expected marginal gain in the next window $w$.
Suppose $S_{1,\cdots, w-1}$ is output of the algorithm in windows $1,\cdots ,w-1$.
The crucial idea is that we show  conditioned on $T_{1,\cdots, w-1}$, each element $e\in OPT\setminus S_{1,\cdots, w-1}$
is more likely to appear in a slot in $w$ than in a slot in $1,\cdots, w-1$. 

We then have a normalization step in which we make all the elements of $OPT\setminus S_{1,\cdots, w-1}$ "appear" with the same probability in $w$. 
Therefore given that one slot in window $w$ contains an element of $OPT$, it can be any of $OPT\setminus S_{1,\cdots, w-1}$ with probability at least $1/k$. Hence the marginal gain for that slot is at least $\frac{1}{k}(OPT-F(S))$. 
We then repeat the argument for all the slots in window $w$  containing elements of the normalized sample.
\newline
The algorithm we describe uses $O(n)$ memory, in addition to the shortlist, but we can show how to modify the algorithm so that the amount of memory used is roughly the same as the size of the shortlist, and therefore the algorithm can be implemented in a streaming model.
} 

\subsection{Comparison to related work}
%There are two main frameworks  for \nameOfProblem: online algorithms and streaming algorithms.
%In the online framework,  we assume the input has random order. %(in adversarial order we can not guarantee anything)
%All of the previous algorithms in this framework irrevocably select a subset of size $k$, whose value is close to OPT~\cite{Bateni, kesselheim,Naor,smspm}.
We compare our results (Theorem \ref{opttheorem} and Theorem \ref{thm:streaming}) to the best known results for {\it \nameOfProblem}~and {\it \streamingProblem}, respectively.

The best known algorithm so far for \nameOfProblem~is by \citet{kesselheim}, with asymptotic competitive ratio of $1/e-O(k^{-1/2})$. 
In their algorithm, after observing each element, they use an oracle to compute optimal offline solution on the elements seen so far.
Therefore it requires exponential time in $n$. The best competitive ratio that they can get in polynomial time is 
$\frac{1}{e}(1-\frac{1}{e})-O(k^{-1/2})$.
In comparison, by using a shortlist of size $O(k)$ our (polynomial time) algorithm achieves a competitive ratio of $1-\frac{1}{e}-\epsilon-O(k^{-1})$. In addition to substantially improves the above-mentioned results for \nameOfProblem, this closely matches the best possible offline approximation ratio of $1-1/e$ in polynomial time. Further, our algorithm is linear time. Table \ref{table:t1} summarizes this comparison. 
Here, $O_\epsilon(\cdot)$ hides the dependence on the constant $\epsilon$. The hidden constant in $O_{\epsilon}(.)$ is %$c\frac{\log(1/\epsilon)}{\epsilon^2}  {\frac{1}{\epsilon^6} \log(1/\epsilon)  \choose {\frac{1}{\epsilon^4} \log(1/\epsilon)}}$ 
\etaMacro for some absolute constant $c$.
%~\cite{Badanidiyuru2014StreamingFly} and~\cite{kesselheim}.

\begin{table}[h!]
\centering
\begin{tabular}{ |c c c c c| }
\hline
 & \#selections & Comp ratio & Running time & Comp ratio in poly(n) \\%&  Comp ratio in poly(n,k)  \\ 
\hline
\cite{kesselheim} & $k$ & $1/e-O(k^{-1/2})$ & $exp(n)$ & $\frac{1}{e}(1-1/e)$ \\ %& $(1-1/e)1/e$ \\ 
this & $O_{\epsilon}(k)$ & $1-1/e-\epsilon-O(1/k) $ & $O_{\epsilon}(n)$ &  $1-1/e-\epsilon-O(1/k)$ \\%&  $1-1/e-\epsilon$ \\
%2nd & $k\log^2 k$ & $1/2-O(k^{-1/4})$ & $poly(n), exp(k)$ & $1/2-O(k^{-1/4})$ & $(1/2-O(k^{-1/4}))(1-1/e)$ \\
\hline    

\end{tabular}
\caption{\nameOfProblem~settings}
\label{table:t1}
\end{table}
%On the other hand, in the streaming framework the decision to select an element is not irrevocable, and there is a buffer of limited size and you can add or remove elements from the buffer, i.e., you can deselect some elements that you have already selected. The random order assumption in this model is not necessary.
In the streaming setting, \citet{Chakrabarti2015} provided a single pass streaming algorithm for monotone submodular function maximization under $k$-cardinality constraint, that achieves a $0.25$ approximation under adversarial ordering of input. Further, their algorithm requires $O(1)$ function evaluations per arriving item and $O(k)$ memory.
The currently best known approximation  under  adversarial order streaming model is by~\citet{Badanidiyuru2014StreamingFly}, who achieve a $1/2-\epsilon$ approximation with a memory of size $O(\frac{1}{\epsilon}k\log k)$. 
%\scomment{no known? or is it not possible?}\mcomment{not possible}
%Any algorithm for streaming submodular
%maximization that only queries the value of the
%submodular function on feasible sets (i.e., sets of cardinality
%at most k) and is an α-approximation for a
%constant α > 0.5 must use Ω(n/k) memory, where n is
%the length of the stream.
There is an upper bound of $1/2+o(1)$ on the competitive ratio achievable by 
any algorithm for streaming submodular
maximization that only queries the value of the submodular function on feasible sets while using $o(n)$ memory~\cite{norouzi}.
%any streaming algorithm for this problem under adversarial order, while using $o(n)$ memory~\cite{norouzi}.
%It does not need random order assumption. 
%Also note that this algorithm can not be converted into an online algorithm. 
%Streaming algorithm with random order assumption has been considered for other problems. 
%But nothing better than~\cite{Badanidiyuru2014StreamingFly} is known for this problem under random order setting. 

\citet{Hess} initiated the study of  \streamingProblem.
Their algorithm uses $O(k)$ memory and a total of $n$ function evaluations to achieve $0.19$ approximation. 
%This result is  worse than the result of~\cite{kesselheim}  in the stricter online model. But note that~\cite{kesselheim} requires $\Omega(nk)$ function evalutation and $\Omega(n)$ memory.
The state of the art result in the random order input model is due to \citet{norouzi} who achieve a $1/2+8\times 10^{-14}$ approximation, while using a memory buffer of size $O(k\log k)$.
%Badanidiyuru et al.~\cite{Badanidiyuru2014StreamingFly} design the first efficient streaming algorithm
%with constant factor $1/2-\epsilon$ approximation guarantee, requiring only a single pass through the data, and memory $O(\frac{1}{\epsilon}k\log k )$.
%Recently~\cite{norouzi} showed that it is impossible to get ratio better than $1/2+o(1)$ in the adversarial order input using memory $o(n)$.
%Our algorithm is in the intersection of the above frameworks. 
%It generalizes the online framework in the way that we are allowed to select more than $k$ elements. 
%We generalize the online model in the way that we are allowed to select more than $k$ elements, and output a subset of size $k$ whose  value is close to OPT.  Note that we are only interested in returning a subset of size at most $k$ as our output.  
%In algorithms like ~\cite{Vondrak}, although the output is close to OPT, it is not restricted to $k$ elements, and we can't guarantee that it contains a subset of size $k$ whose value is close to OPT.
%In comparison, our algorithm selects $O(k)$ elements and guarantees that there is a subset of size $k$ whose value is $R-O(k^{-1})$ times $OPT$, for $R<1-1/e$.Thus by relaxing the number of selections we improve upon the best competitive ratio $1/e$, while only using $O(n)$ running time.  These bounds compare favorably to~\cite{kesselheim}, which  needs to find the optimal offline solution $n$ times, or to use an $1-1/e$ approximation to find each offline optimal solution. In the latter case, the running time is  $O(n^2)$ and the competitive ratio is  $\frac{1}{e} (1-1/e)$.
 
%It is asymptotically a $1/2-O(k^{-1/4})$ approximation algorithm.
%In terms of memory size, it improves upon the previous $k\log k$~\cite{norouzi}. %$\frac{1}{\epsilon}k\log k$.%, for $k>(1/\epsilon)^4$.
%(Note that the approximation ratio of our algorithm is asymptotic and for a fixed $k$ we can not decrease error more than $k^{-1/4}$)
%Also in terms of running time it is polynomial in $n$, but it requires exponential time in $k$.
%Also note that the online algorithm~\cite{kesselheim} can not be converted into a streaming algorithm with nontrivial memory size.

%The goal is to partition the items between agents so as to maximize the sum of their valuation functions.
%The well known greedy algorithm gives a 1/2 approximation for this problem. Also for the adversarial order 1/2 is the best we can achieve~\cite{Kapralov:2013}.
%\cite{vahab},~\cite{swm}  slightly improve the analysis of the greedy algorithm to just above 1/2 for  random order input (0.505, 0.509 competitive ratio respectively). The later result can be generalized to maximizing monotone sumobular functions subject to  a partition matroid. It is incomparable with \nameOfProblemSL.

%Table~\ref{table:t1} and 
Table~\ref{table:t2} provides a detailed comparison of our result in Theorem \ref{thm:streaming} to the 
%, we compare our algorithm to some of the previous works to show the tradeoffs in the various parameters for both the online algorithms model and the streaming model.
above-mentioned results for  \streamingProblem, showing that our algorithm substantially improves the existing results on most aspects of the problem. 

\begin{table}[h!]
\centering
\begin{tabular}{ |c c c c c | }
\hline
 & Memory size & Approximation ratio & Running time & update time \\ 
 \hline
\cite{Hess} & $O(k)$ &  $0.19$ & $O(n)$ & O(1) \\ 
\cite{norouzi} & $O(k\log k)$ &  $1/2+8\times 10^{-14}$ & $O(n\log k)$ & $O(\log k)$ \\ 
\cite{Badanidiyuru2014StreamingFly} & $O(\frac{1}{\epsilon}k\log k)$ & $1/2-\epsilon$ & $poly(n,k, 1/\epsilon)$ & $O(\frac{1}{\epsilon}\log k)$ \\ 
this & $O_{\epsilon}(k)$ & $1-1/e-\epsilon-O(1/k)$ & $O_{\epsilon}(n)$ & amortized $O_{\epsilon}(1+\frac{k^2}{n})$ \\
%2nd & $k\log^2 k$ & $1/2-O(k^{-1/4})$ & $poly(n), exp(k)$ &  \text{amortize one operation}\\
\hline    
\end{tabular}
\caption{\streamingProblem
}
%$\log(1/\epsilon) {\frac{1}{\epsilon^3} \log(1/\epsilon)  \choose {\frac{1}{\epsilon^2} \log(1/\epsilon)}}$.}
\label{table:t2}
\end{table}



There is also a line of work studying the online variant of the submodular welfare maximization problem (e.g., \cite{vahab,swm,Kapralov:2013}). In this problem, 
the items arrive online, and each arriving item should be allocated  to one of $m$ agents with a submodular valuation functions $w_i(S_i)$ where $S_i$ is the subset of items allocated to $i$-th agent). The goal is to partition the arriving items into $m$ sets to be allocated to $m$ agents, so that the sum of valuations over all agents is maximized. This setting is incomparable with the \nameOfProblem~setting considered here.
}

\subsection{ Related Work}
In this section, we overview some of the related online problems.
%\paragraph{The \text{\nameOfProblem}.}
In the \textit{\nameOfProblem} introduced by \citet{Bateni} and ~\citet{Gupta:2010},
the algorithm selects $k$ items, but 
the value of the selected items is given by a monotone submodular function 
%It is an online variant of monotone submodular maximization subject to cardinality constraints. 
%The objective function is designed by an adversary, but the order of the items is uniformly at random.
%$f$. The algorithm has a value oracle access to the function, i.e., for any given set $T$, an algorithm can query an oracle to find its value $f(T)$~\cite{oracle}.
The algorithm can select at most $k$ items $S=\{a_1 \cdots, a_k\}$, from a randomly ordered sequence of $n$ items. The goal is to maximize
$f(S)$.
%$f(\{a_1,\cdots, a_k\})$.
%Now imagine we are allowed to select several items instead of one item. Would that let us to improve $1/e$?
%Assuming a value oracle access to the submodular function; i.e., for a given set $T$, an algorithm can query an oracle to find its value $f(T)$~\cite{oracle}.
Currently, the best result for this setting is due to ~\citet{kesselheim}, who achieve a $1/e$-competitive ratio in exponential time in $k$, or $\frac{1}{e}(1-\frac{1}{e})$ in polynomial time in $n$ and $k$.
Submodular functions also has been used in the network design problems~\cite{ghugequasi,friggstad2016logarithmic}. 
%~\cite{ghugequasi,shadravan2014integrality,friggstad2016logarithmic}. 
There are also some related online coloring problems in the literature~\cite{gijswijt2007clique,abam2014online}.
%In this case, the offline problem is NP-hard and hard-to approximate beyond the factor of $1-1/e$ achieved by the greedy algorithm \cite{nemhauser1978best}. 

%\scomment{need a reference for lower bound of $1-1/e$ for offline monotone submodular maximization}
\toRemove{
However, it is unclear if a competitive ratio of $1-1/e$ can be achieved by an online algorithm for the {\nameOfProblem} even when $k$ is large. 
}

%\paragraph{The matroid secretary problem.}
In the \textit{matroid secretary problem}, the elements of a matroid $\mathcal{M}$ arrive in random order. Once we observe an item we need to irrevocably decide 
whether or not to accept it. The set of selected elements should form an independent set of the matroid.
The goal is to maximize the total sum of the values assigned to these elements.
It has applications in online mechanism design, in particular when the set of acceptable agents form a matroid~\cite{Babaioff:2008}. 
%It has applications in welfare maximizing online mechanism design for domains in which
%the sets of simultaneously satisfiable agents form a matroid~\cite{Babaioff:2008}.

The existence of a constant competitive algorithm is a long-standing open problem.
~\citet{Lachish14} provides  the first $O(\log \log(k))$- competitive algorithm (the hidden constant is $2^{2^{34}}$).
~\citet{feldman2014simple} give a simpler  order-oblivious 
$2560 (\log\log 4k+5)$-competitive algorithm for the matroid secretary problem, by knowing only  the cardinality of the matroid in advance.
There are some $O(1)$-competitive algorithms for special variants
of the matroid secretary problem. 
For example, the elements of the ground set are assigned to a set of  weights uniformly at random hen a $5.7187$-competitive algorithm is possible for any matroid~\cite{soto2013matroid}.
%For example, if a set of $n$ weights is assigned uniformly at random to the elements of the ground set, then a $5.7187$-competitive algorithm can be obtained for any matroid~\cite{soto2013matroid}. 
Furthermore, a $16(1-1/e)$-competitive algorithm can be achieved as long as the weight assignment is  done at random,  even if we assume the adversarial arrival order.


%\paragraph{Preemption Model}
 Recently,~\citet{Buchbinder:2014} considered a
different relaxation which is called preemptions model. In this model, elements added
to $S$ can be discarded later.
The main result of~\cite{Buchbinder:2014},  is a randomized $0.0893$-competitive
algorithm for cardinality constraints using $O(k)$ memory.

%chekuri et al. obtain a
%(1 − )/(2 + e)-competitive algorithm for this case using O(k log k/2)-space



==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/newProof.tex <==
%\scomment{Begin:Trying out something------------------------}

%\begin{lemma}
%\label{lem:indepi}
%For any window $w$, slot $s,s'$ in window %$w, \ldots, W$, and $i\in S^*$, 
%$$\mathbb{P}(Y_i=s | T_{1,\ldots, w-1})=\mathbb{P}(Y_i=s' | T_{1,\ldots, w-1})$$
%\end{lemma}
%\begin{proof}
%By applying Bayes rule to Lemma \ref{afterw}.
%\end{proof}



%In this section, 
First, we use the observations from the previous sections to show the existence of a random subsequence of slots $\tilde \tau_w$ of window $w$ such that we can lower bound $f((S_{1,\ldots, w-1}\cup \gamma(\tilde \tau_w))\setminus \zeta(\tilde \tau_w))- f(S_{1,\ldots, w-1})$ in terms of $\OPT -f(S_{1,\ldots, w-1})$. This will be used to lower bound  increment %$\Delta_f(S_w|S_{1,\ldots, w-1}) = 
$f(S_{1,\ldots, w-1}\cup \gamma(\tau^*)\setminus \zeta(\tau^*)) -f(S_{1,\ldots, w-1})$ in every window.

%For any item $i\in S^*$, window $w \in \{1,\ldots, W\}$, and slot $s$ in window $w$, define
%\begin{equation}
%\label{eq:pijBound}
%p_{is}:=\mathbb{P}(i \in s \cup Supp(T) | T_{1,\ldots, w-1}=T).
%\end{equation}

\begin{definition}[$Z_s$ and $\tilde \gamma_w$]
\label{def:tauw}
Create sets of items $Z_s, \forall s\in w$  as follows: for every slot $s$, add every item from $i\in S^*\cap s$ independently with probability $\frac{1}{k \beta p_{is}}$ to $Z_s$. Then, for every item $i\in S^*\cap T$, with probability $\alpha/k$, add $i$ to $Z_s$ for a randomly chosen slot $s$ in $w$. Define subsequence $\tilde \tau_w$ as the sequence of 
slots with $Z_s\ne \emptyset$. 

%(at most) $\alpha$ slots chosen uniformly at random from 
%Also, define a designated item $a_s$ for every slot $s$ as a randomly chosen item from $Z_s$ ( if $Z_s=\phi$, we set $a_s=0$, denoting a null item).
%Also, define a designated item $a_s$ for every slot $s$ as follows: if $Z_s=\phi$, set $a_s=0$, otherwise, set $a_s$ to be a random item from $Z_s$.  
%define a subsequence $\tilde \tau_w$  of slots in window $w$ by selecting  $\min\{\alpha, |S^*\cap (s\cup Supp(T))|\}$ slots uniformly at random from all slots with  $S^*\cap (s\cup Supp(T)) \ne \phi$ Now, for all $i\in S^*\cap (s\cup Supp(T))$, let $Z_{is}$ be the outcome of an independent  coin toss with probability $\frac{1}{k p_{i}}$ of success. Set $a_s=i$ randomly from all $\{i:i\in S^*\cap (s\cup Supp(T)), Z_{is}=1\}$.

%For every $i\in S^*$ and every slot $s$ in window $w$, let $Z_{is}$ be the outcome of an independent  coin toss with probability $\frac{1}{k\beta p_{is}}$ of success, with $p_{is}$ as defined in Lemma \ref{lem:pijBound}. Now, 
%Consider every slot $s$ in window $w$ such that $S^*\cap \{s\cup Supp(T)\}$ is not empty. Let $i$ be a uniformly at random item from $S^*\cap \{s\cup Supp(T)\}$.  With probability $\frac{1}{k\beta p_{i}}$, add slot $s$ to $\tilde \tau_w$ and set $a_s=i$. 
%Define $\tilde \gamma_w$ as the sequence of all slots $s$ such that for \emph{some} $i\in S^*$, we have $i\in s\cup Supp(T_{1,\ldots, w-1})$ and $Z_{is}=1$.
%onsider the sequence $\Gamma$ of 
%If $|\Gamma|>\alpha$, generate $\tilde \tau_w$  as a random subsequence of $\Gamma$ of length $\alpha$, otherwise set $\tilde \tau_w=\Gamma$.
\end{definition}
Similar to~\cite{us}, we have the following property for $Z_s$:
\begin{lemma}
\label{lem:Zs}
Given any $T_{1,\ldots, w-1}=T$, for any slot $s$ in window $w$, all $i, i' \in S^*, i\ne i'$ will appear in $Z_s$ independently with probability $\frac{1}{k\beta}$. Also, given $T$, for every $i \in S^*$, the probability to appear in $Z_s$ is equal for all slots $s$ in window $w$. Further, each $i\in S^*$ occurs in  $Z_s$ of at most one slot $s$.
\end{lemma}
\toRemove{
\begin{proof}
First consider $i\in S^*\cap Supp(T)$. Then, $\Pr(i\in Z_s|T) = \frac{\alpha}{k}\times \frac{1}{\alpha \beta} = \frac{1}{k\beta}$ by construction. Also, the event $i\in Z_s|T$ is independent from $i'\in Z_s|T$ for any $i'\in S^*$ as $i$ is independently assigned to a $Z_s$ in construction. Further, every $\in S^*\cap T$ is assigned with equal probability to every slot in $s$.

Now, consider $i\in S^*, i\notin Supp(T)$. Then, for all slots $s$ in window $w$,
$$\Pr(i \in Z_s|T) =\Pr(Y_i=s | T) \frac{1}{p_{is}k\beta} =  p_{is}\times \frac{1}{p_{is}k\beta} = \frac{1}{k\beta},$$
where $p_{is}$ is defined in \eqref{eq:pijBound}. We used that 
$p_{is}=\Pr(Y_i=s|T)$ for $i\notin Supp(T)$. 
Independence of events  $i\in Z_s|T$ for items in $S^*\backslash Supp(T)$ follows from Lemma \ref{lem:ijindep}, which ensures $Y_i=s|T$ and  $Y_j=s|T$ are independent for $i\ne j$; and from independent selection among items with $Y_i=s$ into $Z_s$. 

The fact that every $i\in S^*$ occurs in at most one $Z_s$ follows from construction: $i$ is assigned to $Z_s$ of only one slot if $i\in Supp(T)$; and for $i\notin Supp(T)$, it can only appear in $Z_s$ if $i$ appears in slot $s$.
%(Note that the events $Y_i=s, Y_i=s'$ are exclusive for $i\notin T$, therefore we can take a sum of the probabilities)
%Therefore for all $i\in S^*$, we have that $\Pr(i\in \cup_{s\in w} Z_s|T)=\frac{\alpha}{k}$. The lemma statement then follows from the standard results for submodular functions.
\end{proof}
}

% We will show that the subsequence $(a_1, \ldots, a_{\alpha \beta})$ has close to $\alpha$ non-zero  items, and will lower bound the increment provided by the greedy subsequence $S_w=\gamma(\tau^*)$ over $f(S_{1,\ldots, w-1})$ by the increment provided by this subsequence. 

%\begin{lemma}
%For any slot $s$ in $w$, given $T_{1,\ldots, w-1}=T$, variables $\mathbf{1}(i\in Z_s|T_{1,\ldots, w-1}=T)$ for $i\in S^*$ are i.i.d. with probability $\frac{1}{k\beta}$ to be true. 
%\end{lemma}
%\begin{proof}
%\scomment{Should be straightforward by previous lemmas}
%\end{proof}

\begin{lemma}
We can show that for all $i, i' \in S^*\backslash \{Z_{s_1} \cup \ldots \cup Z_{s_{j-1}}\}$,
\begin{equation} 
\label{eq:pk}
\Pr(i\in Z_{s_j}| Z_{s_1} \cup \ldots \cup Z_{s_{j-1}}) = \Pr(i'\in Z_{s_j}| Z_{s_1} \cup \ldots \cup Z_{s_{j-1}})  \ge \frac{1}{k} \ .
\end{equation}
\end{lemma}
\begin{proof}
The proof is similar to Lemma 12 in~\cite{us}, and it is based on Lemma \ref{lem:Zs},
\end{proof}

In the following lemma we lower bound the marginal gain of a randomly picked element of optimal solution in slot $s_j$ with respect to previously selected items.

\begin{lemma}
\label{lem:asGoodas}
%For every slot $s$ in $\tilde \tau_s$, define $a_s$ as the   from slots $1,\ldots, {s-1}$ or $T_{1,\ldots, w-1}$,
%define $a$

Suppose the sequence $\tilde \tau_w=(s_1, \ldots, s_t)$ defined as in Definition \ref{def:tauw}, let $\gamma(\tilde \tau_s)=(i_1,\ldots, i_t)$, with $\gamma(\cdot)$ as defined in \eqref{eq:gamma}. Then, for all $j=1,\ldots, t$, 
%given $a\in S^*\cap Z_{s_j}$.

{\small \begin{eqnarray*}
\Ex[\Delta_f(a|S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots, c_{j-1}\})|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}]\\
 \ge \frac{1}{k}\left((1-\frac{\alpha}{k})f(S^*)-f(S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots,c_{j-1}\})\right)\
\end{eqnarray*}}
%{\small
%$$\Ex[\Delta_f(i_j|S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots, c_{j-1}\})|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}] \ge \frac{1}{k}\left((1-\frac{\alpha}{k})f(S^*)-f(S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdot,c_{j-1}\})\right)\ .$$}
\end{lemma}
\begin{proof}
\toRemove{
For any slot $s'$ in window $w$, let $\{s:s \succ_w s'\}$ denote all the slots $s'$ in the sequence of slots in window $w$. 

Now, using Lemma \ref{lem:Zs}, for any slot $s$ such that $s \succ_w s_{j-1}$, 
%\mcomment{is $s_i$ a number? did we say how slots are assigned to number ids so that we have an ordering of slots}\scomment{fixed it.}
we have that the random variables  $\mathbf{1}(i\in Z_s | Z_{s_1} \cup \ldots \cup Z_{s_{j-1}})$ are i.i.d. for all $i \in S^*\backslash \{Z_{s_1} \cup \ldots \cup Z_{s_{j-1}}\}$. 
Next, we show that the probabilities $\Pr(i\in Z_{s_j}| Z_{s_1} \cup \ldots \cup Z_{s_{j-1}})$ are identical for all $i\in S^*\backslash \{Z_{s_1} \cup \ldots \cup Z_{s_{j-1}}\}$:
{\small \begin{eqnarray*}
\Pr(i\in Z_{s_j}| Z_{s_1} \cup \ldots \cup Z_{s_{j-1}}) & = & \sum_{s:s\succ_w s_{j-1}} \Pr(i\in Z_s, s=s_j | Z_{s_1} \cup \ldots \cup Z_{s_{j-1}})\\
& = & \sum_{s: s\succ_w s_{j-1}} \Pr(i\in Z_s| s=s_j, Z_{s_1} \cup \ldots \cup Z_{s_{j-1}}) \Pr(s=s_j|Z_{s_1} \cup \ldots \cup Z_{s_{j-1}}) \ .\\
\end{eqnarray*}}
Now, from Lemma \ref{lem:Zs}, the probability $\Pr(i\in Z_s| s=s_j, Z_{s_1} \cup \ldots \cup Z_{s_{j-1}}) $ must be  identical for all $i\notin  Z_{s_1} \cup \ldots \cup Z_{s_{j-1}}$. Therefore, from above we have that for all $i, i' \in S^*\backslash \{Z_{s_1} \cup \ldots \cup Z_{s_{j-1}}\}$,
\begin{equation} 
\label{eq:pk}
\Pr(i\in Z_{s_j}| Z_{s_1} \cup \ldots \cup Z_{s_{j-1}}) = \Pr(i'\in Z_{s_j}| Z_{s_1} \cup \ldots \cup Z_{s_{j-1}})  \ge \frac{1}{k} \ .
\end{equation}
%(The lower bound of $1$ on total probability follows from the fact that 
The lower bound of $1/k$ followed from the fact that at least one of the items from $S^*\backslash \{Z_{s_1} \cup \ldots \cup Z_{s_{j-1}}\}$ must appear in $Z_{s_j}$ for $s_j$ to be included in $\tilde \tau_w$. Thus, each of these probabilities is at least $1/k$. 
%$$\Pr(i\in Z_{s_j}| Z_{s_1} \cup \ldots \cup Z_{s_{j-1}}) \ge \frac{1}{k}, \forall i\in S^*\backslash \{Z_{s_1} \cup \ldots \cup Z_{s_{j-1}}\}$$
In other words, if an item is randomly picked from $Z_{s_j}$, it will be $i$ with probability at least $1/k$, for all $i\in S^*\backslash \{Z_{s_1} \cup \ldots \cup Z_{s_{j-1}}\}$.
%with probaility $\frac{1}{k\beta}$. %Since $a_s$ is  a randomly chosen item from $Z_s$, this implies $a_s=i$ independently with probability $1/k\beta$ for all $i \in S^*\backslash Z_{1,\ldots, s-1}$.
}

\toRemove{
Now similar to Lemma 12 in ~\cite{us}, and based on Lemma \ref{lem:Zs}, we can show:
\begin{equation} 
\label{eq:pk}
\Pr(i\in Z_{s_j}| Z_{s_1} \cup \ldots \cup Z_{s_{j-1}}) = \Pr(i'\in Z_{s_j}| Z_{s_1} \cup \ldots \cup Z_{s_{j-1}})  \ge \frac{1}{k} \ .
\end{equation}
}


%Now, by definition of $\gamma(\cdot)$ (refer to \eqref{eq:gamma}), $i_j$ is chosen greedily to maximize the increment 
%$g(i, S_{1, \ldots,w-1} \cup \{i_1,\ldots, i_{j-1}\}\setminus \{c_1,\cdots, c_{j-1}\})$ 
%$\Delta_f(i|S_{1,\ldots, w-1} \cup i_{1,\ldots, s-1})$ 
%over all $i\in s_j \cup Supp(T_{1,\ldots, w-1}) \supseteq Z_{s_j}$. Therefore, 
%we can lower bound the increment provided by $i_j$ by that provided by a randomly picked item from $Z_{s_j}$.
We can lower bound the increment assuming $a$ is randomly picked item from $Z_{s_j}\cap S^*$:
\begin{eqnarray*} 
%\Ex[\Delta_f(a_s|S_{1,\ldots, w-1} \cup S)|T_{1,\ldots, w-1} =T] & \ge & \Ex[\Ex[\frac{1}{k} \left(f(S^*\backslash  S)-f(S_{1,\ldots, w-1} \cup S)\right) | S, T]]\\
%& \ge & \Ex[\frac{1}{k\beta} \left(f(S^*\backslash  \cup_{s'\in w} Z_{s'})-f(S_{1,\ldots, w-1} \cup a_{1,\ldots, s-1})\right)]\\
%& \ge & \frac{1}{k\beta} \left(\left(1-\frac{\Ex[|\cup_{s'\in w} Z_{s'}|]}{k}\right)f(S^*) -f(S_{1,\ldots, w-1} \cup a_{1,\ldots, s-1})\right))\\
%& = & \frac{1}{k\beta} \left(\left(1-\frac{\alpha}{k}\right)f(S^*) -f(S_{1,\ldots, w-1} \cup a_{1,\ldots, s-1})\right)
%& & \Ex[\Delta_f(i_j|S_{1,\ldots, w-1} \cup \{i_1,\ldots, i_{j-1}\})|T_{1,\ldots, w-1} =T] \\
%& = & 
%& & \Ex[\Delta_f(i_j|S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}|T_{1,\ldots, w-1}=T, i_1, \ldots, i_{j-1}] \\
& & \Ex[\Delta_f(a,S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots,c_{j-1}\})|T_{1,\ldots, w-1}=T, i_1, \ldots, i_{j-1},a\in S^*\cap Z_{s_j}] \\
%(\text{using }\eqref{eq:pk})
& \ge & \frac{1}{k} \Ex[\sum_{a\in S^*\backslash \{Z_1,\ldots Z_{s_{j-1}}\}} \Ex[\Delta_f(a,S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots,c_{j-1}\})|T, i_1, \ldots, i_{j-1}]] \\
%(\text{using  Lemma~\ref{marginalsum}, monotonicity of $f$} ) 
& \ge & \frac{1}{k} \Ex[ \left(f(S^*\backslash  \{Z_1,\ldots Z_{s_{j-1}}\})-f(S_{1,\ldots, w-1} \cup i_{1,\ldots, s-1}\setminus\{c_1,\cdots,c_{j-1}\})\right) | T]\\
%(\text{using  monotonicity of }f) 
& \ge & \frac{1}{k}  \Ex[\left(f(S^*\backslash  \cup_{s'\in w} Z_{s'})-f(S_{1,\ldots, w-1} \cup i_{1,\ldots, s-1}\setminus\{c_1,\cdots,c_{j-1}\})\right)| T]\\
%(\text{using  Lemma \ref{lem:Zs} and Lemma~\ref{sample}}) & \ge & \frac{1}{k} \left(\left(1-\frac{\Ex[|\cup_{s'\in w} Z_{s'}|]}{k}\right)f(S^*) -f(S_{1,\ldots, w-1} \cup i_{1,\ldots, s-1})\right))\\
%(\text{using  Lemma~\ref{lem:Zs} and Lemma~\ref{sample}})  
& \geq & \frac{1}{k} \left(\left(1-\frac{\alpha}{k}\right)f(S^*) -f(S_{1,\ldots, w-1} \cup i_{1,\ldots, s-1}\setminus \{c_1,\cdots, c_{j-1}\})\right)
\end{eqnarray*}
%Here, we used the submodularity of $f$ and 
The last inequality uses 
Lemma \ref{sample} for submodular function $f$. 
and the observation from Lemma \ref{lem:Zs} that given $T$, every $i\in S^*$ appears in $\cup_{s'\in w} Z_{s'}$ independently with probability $\alpha/k$, so that every $i\in S^*$ appears in $S^*\backslash\cup_{s'\in w} Z_{s'}$ independently with probability $1-\frac{\alpha}{k}$; %along with Lemma \ref{sample} for submodular function $f$. 
%so that $\Ex[|\cup_{s'\in w} Z_{s'}|] \le {\alpha}$.
\end{proof}


\begin{lemma}\label{replaced}
%At the end of window $w$, 
Suppose the sequence $\tilde \tau_w=(s_1, \ldots, s_t)$ defined as in Definition \ref{def:tauw}, let $\gamma(\tilde \tau_s)=(i_1,\ldots, i_t)$, with $\gamma(\cdot)$ as defined in \eqref{eq:gamma}. 
Moreover, let $S'$ be the extension of $S_{1,\cdots, w-1}\cup \{i_1, \cdots, i_{j-1}\}\setminus \{c_1,\cdots, c_{j-1}\}$ to an independent set in $\mathcal{M}$, and $\pi$ be the bijection from Brualdi lemma (refer to Lemma~\ref{lem:Brualdi}) from $S^*$ to $S'$.
Then, for all $j=1,\ldots, t$, \\
{\small \begin{eqnarray*}
\Ex[f(S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots, c_{j-1},\pi(a)\})|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}]\\
 \ge (1-\frac{1}{k-\alpha})f(S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots,c_{j-1}\})\
\end{eqnarray*}}
\toRemove{
{\small \begin{eqnarray*}
\Ex[\Delta_f(a|S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots, c_{j-1},\pi(a)\})|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}]\\
 \ge (1-\frac{1}{k})f(S^*)-f(S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots,c_{j-1}\}\
\end{eqnarray*}}
}
%$\mathbb{E}[f(S_{1,\cdots, w-1}\cup \{i_1, \ldots, i_{j-1}\} \setminus \{c_1,\cdots, c_{j-1}, \pi(a)\} ] \ge (1-\frac{1}{k}) f(S_{1,\cdots, w-1}\cup \{i_1, \ldots, i_{j-1}\} \setminus \{c_1, \cdots, c_{j-1}\} )$$
\end{lemma}
\begin{proof}
%It follows from Brualdi lemma and lemma~\ref{sample}.
Since $\pi$ is a bijection from $S^*$ to $S'$, from Brualdi's lemma (lemma~\ref{lem:Brualdi}), there is an onto mapping $\pi'$ from $S^*$ %$OPT$ 
 to $S_{1,\cdots, w-1}\cup \{i_1, \cdots, i_{j-1}\}\setminus \{c_1,\cdots, c_{j-1}\}\cup \{\emptyset\}$ 
such that %$S_{1,\cdots, w-1}\cup \{i_1, \ldots, i_{j-1}\} - \pi(a) +a \in M$ for all $a \in S^*$.
$S_{1,\cdots, w-1}\cup \{i_1, \cdots, i_{j-1}\}\setminus \{c_1,\cdots, c_{j-1}\}- \pi'(a) +a \in M$, for all $a \in S^*$. Further, $\pi'(a)=\pi(a)$ if $\pi(a)\in  S_{1,\cdots, w-1}\cup \{i_1, \cdots, i_{j-1}\}\setminus \{c_1,\cdots, c_{j-1}\}$ and $\pi'(a)=\emptyset$ otherwise.

%Note that $\pi$ maps some $a \in S^*$, to the empty set, i.e., we set $\pi(a)=\emptyset$.

Recall the definition of $Z_{s_j}$.
%Recall the definition $Z_{s_j}$ defined in the last paper.
%\begin{definition}[$Z_s$ and $\tilde \gamma_w$]
%\label{def:tauw}
%Create sets of items $Z_s, \forall s\in w$  as follows: for every slot $s$, add every item from $i\in S^*\cap s$ independently with probability $\frac{1}{k \beta p_{is}}$ to $Z_s$. Then, for every item $i\in S^*\cap T$, with probability $\alpha/k$, add $i$ to $Z_s$ for a randomly chosen slot $s$ in $w$. 
%Define subsequence $\tilde \tau_w$ as the sequence of slots with $Z_s\ne \phi$. 
%Suppose $|Z_{s_j}|=1$ and $S^*\cap Z_{s_j}=a$.
Suppose $a$ is a randomly picked item from $S^*\cap Z_{s_j}$.
%(in terms of notation defined in last paper $Z_{s_j}=1$)
Note that from Lemma~\ref{lem:Zs}, conditioned on $T_{1,\cdots, w-1}$, the element $a$ can be equally any element of %$S^*$ 
$S^*\backslash  \{Z_1,\ldots Z_{s_{j-1}}\}$
with probability at least $1/(k-\alpha)$.
Therefore, $\pi'(a)$ would be any of $S_{1,\cdots, w-1}\cup \{i_1, \cdots, i_{j-1}\}\setminus \{c_1,\cdots, c_{j-1}\}$ with probability at most $1/(k-\alpha)$ %(note that $|S_{1,\cdots, w-1}\cup \{i_1, \cdots, i_{j-1}\}\setminus \{c_1,\cdots, c_{j-1}\}| < k$, thus sometimes $\pi(a)$ might not be defined).
(since $\pi'$ might map some elements of $S^*$ to the empty set).
Now based on the definition of $\pi$ and lemma~\ref{sample} we have:

{\small \begin{eqnarray*}
\Ex_a[f(S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots, c_{j-1},\pi(a)\})|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}]\\
 \ge (1-\frac{1}{k-\alpha})f(S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots,c_{j-1}\})\
\end{eqnarray*}}

\toRemove{
{\small \begin{eqnarray*}
\Ex_a[\Delta_f(a|S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots, c_{j-1},\pi(a)\})|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}]\\
 \ge (1-\frac{1}{k})f(S^*)-f(S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots,c_{j-1}\}\
\end{eqnarray*}}
}
%$$ \mathbb{E}[f(S_{1,\cdots, w-1} \cup \{i_1, \cdots, i_{j-1}\} \setminus \{c_1, \cdots, c_{j-1} , \pi(a)\} )] \ge (1-1/k) f(S_{1,\cdots, w-1} \cup \{i_1, \cdots, i_{j-1}\} \setminus \{c_1, \cdots, c_{j-1}\} ) $$


%Note that $g(e,S) \ge \Delta_f(e|S) $.
%Note that $g(e,S) \ge f(S+e-\pi(e) )  -f(S)$.
%Therefore 
%Note that $\bar{S}_w:=\zeta(\tau^*)=\{c_1, \cdots, c_{\ell}\}$.
\end{proof}

\begin{lemma}\label{exg}
%We can show that:
%\begin{align}\label{recursion}
Suppose function $g$ is as defined in equation~\ref{eq:g}.
For the sequence $\tilde \tau_w=(s_1, \ldots, s_t)$, and $\gamma(\tilde \tau_s)=(i_1,\ldots, i_t)$. Then, for all $j=1,\ldots, t$, \\
{\small \begin{eqnarray*}
\Ex[g(i_j,S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots, c_{j-1}\})|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}]\\
 \ge 
 %(1-\frac{1}{k-\alpha})
 \frac{1}{k}
 \left(
 (1-\frac{\alpha}{k-\alpha})f(S^*)-
 2f(S_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\}\setminus\{c_1,\cdots,c_{j-1}\})\right)\
\end{eqnarray*}}

\toRemove{
$$ 
\Ex[g(i_j,{S}_{1,\ldots, w-1} \cup \{i_1,\cdots,i_{j-1}\}\setminus \{c_1,\cdots, c_{j-1}\})|T_{1,\cdots, w-1},i_{1,\cdots, j-1}]
$$
$$
\ge
{ \frac{1}{k}\left((1-\frac{\alpha}{k})f(S^*)-2f({S}_{1,\ldots, w-1} \cup \{i_1,\cdots,i_{j-1}\}\setminus \{c_1,\cdots, c_{j-1}\})\right)\ . }
$$  
}
%\end{align}
\end{lemma}


\begin{proof}
In the algorithm~\ref{alg:main}, at the end of window $w$, we set %$S_{1,\cdots, w-1} = {S}_{1,\cdots, w-1} \setminus \bar{S}_w$.
$S_{1,\cdots, w} = S_{1,\cdots, w-1}\cup S_w \setminus \bar{S}_w$.
Suppose $a\in s_j\cap S^*$. 
Moreover, let $S'$ be the extension of $S_{1,\cdots, w-1}\cup \{i_1, \cdots, i_{j-1}\}\setminus \{c_1,\cdots, c_{j-1}\}$ to an independent set in $\mathcal{M}$, and $\pi$ be the bijection from Brualdi lemma (refer to Lemma~\ref{lem:Brualdi}) from $S^*$ to $S'$.
Thus the expected value of the function $g$ on the element selected by the algorithm in slot $s_j$ (the element with maximum $g$ in the slot $s_j$) would be
\begin{eqnarray*}
%\begin{align}
%g(i_j,{S}_{1,\ldots, w-1} \cup \{i_1,\cdots,i_{j-1}\}\setminus \{c_1,\cdots, c_{j-1}\})
%= 
&\Ex[f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j}\} \setminus \{c_1,\cdots, c_j \}|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}]  %- f(S_{1,\cdots, w-1}\cup \{i_1, \ldots, i_{j-1}\} \setminus \{c_1,\cdots, c_{j-1}\}) 
\\\ge&
\Ex[f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}, a\} \setminus \{c_1,\cdots, c_{j-1}, \pi(a) \} |T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}] %- f(S_{1,\cdots, w-1}\cup \{i_1, \ldots, i_{j-1}\} \setminus \{c_1,\cdots, c_{j-1} \}) 
\\\ge&
%f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}, a\} \setminus \{c_1,\cdots, c_{j-1}, \pi(a) \} )-
\Ex[f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\} \setminus \{c_1,\cdots, c_{j-1}, \pi(a) \} )|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}]
\\&+\Ex[\Delta_f(a|S_{1,\cdots,w-1}\cup\{i_1,\cdots,i_{j-1}\}\setminus \{c_1,\cdots, c_{j-1},\pi(a)\} )|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}] \\
\ge&
\Ex[f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\} \setminus \{c_1,\cdots, c_{j-1}, \pi(a) \} )|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}]
\\&+\Ex[\Delta_f(a|S_{1,\cdots,w-1}\cup\{i_1,\cdots,i_{j-1}\}\setminus \{c_1,\cdots, c_{j-1}\} )|T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}]
%\end{align}
\end{eqnarray*}
The first inequality is from the definition of function $g$ as it is defined in equation~\ref{eq:g}. The last inequality from submoularity of $f$.
Now from the last inequality  and lemma~\ref{replaced} we have
\begin{align*}
&\Ex[f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j}\} \setminus \{c_1,\cdots, c_j \} |T_{1,\ldots, w-1}, i_{1,\ldots, j-1})]& \\ &\ge
%f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}, a\} \setminus \{c_1,\cdots, c_{j-1}, \pi(a) \} )\ge 
(1-\frac{1}{k-\alpha} ) f(S_{1,\cdots, w-1}\cup \{i_1, \ldots, i_{j-1}\} \setminus \{c_1, \cdots, c_{j-1}\} )&\\
&+ \Ex[ \Delta_f(a|{S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\} \setminus\{c_1,\cdots, c_{j-1}\} \})||T_{1,\ldots, w-1}, i_{1,\ldots, j-1}, a\in S^*\cap Z_{s_j}] &
\end{align*}
Now from lemma~\ref{lem:asGoodas} and the above inequality we can show
\begin{align*}
&\Ex[f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j}\} \setminus \{c_1,\cdots, c_j \} |T_{1,\ldots, w-1}, i_{1,\ldots, j-1})]& \\  &\ge
%f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}, a\} \setminus \{c_1,\cdots, c_{j-1}, \pi(a) \} )\ge 
(1-\frac{1}{k-\alpha} ) f(S_{1,\cdots, w-1}\cup \{i_1, \ldots, i_{j-1}\} \setminus \{c_1, \cdots, c_{j-1}\} )&\\
&+{ \frac{1}{k}\left((1-\frac{\alpha}{k})f(S^*)-f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}\} \setminus\{c_1,\cdots, c_{j-1}\})\right)\ . }&
\end{align*}
Thus,
\begin{align}\label{recursion}
f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j}\} \setminus \{c_1,\cdots, c_j \} )  
%f({S}_{1,\ldots, w-1} \cup \{i_1, \ldots, i_{j-1}, a\} \setminus \{c_1,\cdots, c_{j-1}, \pi(a) \} )\ge 
- f(S_{1,\cdots, w-1}\cup \{i_1, \ldots, i_{j-1}\} \setminus \{c_1, \cdots, c_{j-1}\} )\\
\ge
{ \frac{1}{k}\left((1-\frac{\alpha}{k})f(S^*)-2f({S}_{1,\ldots, w-1} \cup \{i_1,\cdots,i_{j-1}\}\setminus \{c_1,\cdots, c_{j-1}\})\right)\ . }
\end{align}

\end{proof}



Using standard techniques for the analysis of greedy algorithm, the following corollary of the previous lemma can be derived, 
\begin{lemma}
\label{cor:asGoodas}
$$\Ex\left[\left(1-\frac{\alpha}{k}\right) f(S^*) - 2f(S_{1,\ldots, w-1}\cup \gamma(\tilde \tau_w)\setminus \zeta(\tilde{\tau}_{w})) | T\right]\le \Ex\left[e^{-\frac{2|\tilde \tau_w|}{k}} \left|\right. T\right] \left(\left(1-\frac{\alpha}{k}\right) f(S^*)-2f(S_{1,\ldots, w-1})\right)$$
%where $t=|\tilde \tau_w|$.
\end{lemma}
\begin{proof}
Let $\pi_0= (1-\frac{\alpha}{k}) f(S^*) - 2\Ex[f(S_{1,\ldots, w-1}) | T_{1,\ldots, w-1}=T]$, and for $j \ge 1$,
$$\pi_j:=(1-\frac{\alpha}{k}) f(S^*) - 2\Ex[f(S_{1,\ldots, w-1}\cup \{i_1, \ldots, i_j\}\setminus\{c_1,\cdots,c_j\}) | T_{1,\ldots, w-1}=T, i_1,\ldots, i_{j-1}],$$
Then, subtracting and adding $\frac{1}{2}(1-\frac{\alpha}{k}) f(S^*)$ from the left hand side of lemma~\ref{exg}, and taking expectation conditional on $T_{1,\ldots, w-1}=T, i_1, \ldots, i_{j-2}$, we get
$$-\frac{1}{2} ( \Ex[\pi_{j} | T, i_1, \ldots, i_{j-2}] + \pi_{j-1} ) \ge \frac{1}{k} \pi_{j-1}$$
which implies
$$\Ex[\pi_j|T, i_1, \ldots, i_{j-2}] \le \left(1-\frac{2}{k}\right) \pi_{j-1} \le \left(1-\frac{2}{k}\right)^j \pi_0\ .$$
By martingale stopping theorem, this implies:
$$\Ex[\pi_t|T] \le \Ex\left[\left(1-\frac{2}{k}\right)^t \left| T\right. \right] \pi_0 \le \Ex\left[e^{-2t/k}| T\right] \pi_0\ .$$
where stopping time $t=|\tilde{\tau}_w|$. ($t=|\tilde \tau_w| \le \alpha\beta$ is bounded, therefore, martingale stopping theorem can be applied).

\end{proof}


Next, we compare $\gamma(\tilde \tau_w)$ to $S_w=\gamma(\tau^*)$ . Here, $\tau^*$ was defined has the `best' greedy subsequence of length $\alpha$ (refer to \eqref{eq:Sw} and \eqref{eq:taustar}). To compare it with $\tilde \tau_w$, we need a bound on size of $\tilde \tau_w$. We use concentration inequalities proved in~\cite{us}:

\toRemove{
\begin{lemma}
\label{lem:lengthtau}
For any real $\delta\in (0,1)$, 
and if $k \ge \alpha\beta$, $\alpha \ge 8\log(\beta)$ and $\beta \ge 8$, 
%$\beta \ge \frac{3}{\delta}$, $\alpha \ge 4 \log(3\beta/\delta)$, and $\frac{2\alpha}{k} \le \frac{\delta}{3}$, 
then given any $T_{1,\ldots, w-1}=T$,
$$(1-\delta)\left(1-\frac{4}{\beta}\right)\alpha \le |\tilde \tau_w| \le (1+\delta)\alpha,$$
with probability $1-\exp(-\frac{\delta^2\alpha}{8\beta})$.
\end{lemma}
}
\toRemove{
\begin{proof}
By definition,
$$|\tilde \tau_w| = |s\in w: Z_s\ne \phi|\ .$$
Again, we use $s'\prec_w s$ to denote all slots before $s$ in window $w$. Then, from Lemma \ref{lem:Zs}, given $T_{1,\ldots, w-1}=T$, for all $i\cap S^*$ and slot $s$ in window $w$, $\Pr[i\in Z_s | Z_{s'}, s'\prec_w s, T]$ is either $0$ or $1/(k\beta)$. Therefore,
$$\Pr[Z_s \ne \phi | T, Z_{s'}, s'\prec_w s]\le \sum_{i\in S^*}  \frac{1}{k\beta} = \frac{1}{\beta}\ .$$
Therefore $X_s=|s'\preceq_w s: Z_{s'}\ne \phi| - \frac{s}{\beta}$ is a super-martingale, with $X_s-X_{s-1}\le 1$. Since there are $\alpha \beta$ slots in window $w$, $X_{\alpha\beta}=|s\in w: Z_{s}\ne \phi| - \alpha$.  Applying Azuma-Hoeffding inequality to  $X_{\alpha\beta}$ (refer to Lemma \ref{lem:azuma}) we get that 
\begin{equation}
\label{eq:upper}
\Pr\left( |s\in w: Z_s \ne \phi| \ge (1+\delta) \alpha |T\right) \le \exp\left(-\frac{\delta^2\alpha}{2\beta}\right)
\end{equation}
which proves the desired upper bound. 


For lower bound, first observe that every $i\in S^*$ appears in $\cup_{s\in w} Z_s$ independently with probability $\frac{\alpha}{k}$. Using Chernoff bound for Bernoulli random variables (Lemma \ref{lem:Chernoff}),  for any $\delta\in(0,1)$
\begin{equation}
\label{eq:lower1}
\Pr(||\cup_{s\in w}Z_s| -\alpha| > \delta\alpha) \le \exp(-\delta^2\alpha/3) \ .
\end{equation}
%\begin{equation}
%\label{eq:lower15}
%\Pr\left(||S^* \cap Z_s| - \frac{1}{\beta}| \ge \frac{\delta}{\beta} |T\right) \le \exp(\frac{-\delta^2}{2k\beta^2})
%\end{equation}

Also, from independence of $i\in Z_s|T$ and  $i'\in Z_s|T$ for any $i,i'\in S^*, i\ne i'$ (refer to Lemma \ref{lem:Zs}),
$$\Pr(i,i'\in Z_s|T, i,i'\notin Z_{s'} \text{ for any } s'\prec_w s) \le  \frac{1}{k^2\beta^2}$$
for any $s\in w$; so that
\begin{equation}
\label{eq:lower10}
\Pr\left(|Z_s|=1|T,  Z_{s'}, s'\prec_w s\right) \ge  \frac{k-|Z_{s'}: s'\prec_w s|}{k\beta}-\frac{1}{\beta^2} \ge \left(1-\frac{2\alpha}{k} \right)\frac{1}{\beta} - \frac{1}{\beta^2}- e^{-\frac{\alpha}{4}} =:p \ .
\end{equation}
where in the last inequality we substituted the upper bound  on $ |Z_{s'}: s'\prec_w s|$ from \eqref{eq:lower1}. 
Specifically, using  \eqref{eq:lower1} with $\delta=3/4$, we obtained  that $|Z_{s'}: s'\prec_w s|\le (1+\frac{3}{4})\alpha \le 2\alpha$ with probability $\exp(-\alpha/4)$. 
%Then, substituing 
%$$\Pr(|Z_s|>1|T, i,i'\notin Z_{s'} \text{ for any } s'\prec_w s) \le  \frac{1}{\beta^2}$$
%Also if  $\beta\ge \frac{3}{\delta'}$, $\alpha \ge  4 \log(3\beta/\delta')$, and $\frac{2\alpha}{k}\le \frac{\delta'}{3}$,  we have $ p :=\left(1-\frac{2\alpha}{k} - \frac{1}{\beta}\right)\frac{1}{\beta} - e^{-\frac{\alpha}{4}} \ge  (1-\delta')\frac{1}{\beta}$.
Also if $\alpha \ge  8 \log(\beta)$, and $k\ge \alpha\beta$,  we have $ p :=\left(1-\frac{2\alpha}{k} - \frac{1}{\beta}\right)\frac{1}{\beta} - e^{-\frac{\alpha}{4}} \ge  (1-\frac{4}{\beta})\frac{1}{\beta}$.

Now, applying Azuma-Hoeffding inequality (Lemma \ref{lem:azuma}), the total number of slots (out of $\alpha\beta$ slots) for which $|Z_s|=1$ can be lower bounded by:

 %we can bound the probability of another item from $S^*$ appearing in the same slot as item $i$. %
%That is, for any $i\in S^*$, %in $Z_s$ for some slot $s$: 
%$$\Pr(Y_i\in w, |Z_{Y_i}|>1, |T) \le \sum_{s\in w} \sum_{i'\in S^*, i'\ne i} \Pr(i,i'\in Z_s| T) = k \alpha\beta\frac{1}{(k\beta)^2} \le \frac{\alpha}{k\beta}$$
%$$\Pr(i: |Z_s|>1 for Y_i=s) \le \alpha\beta \frac{1}{(k\beta)^2} = \frac{\alpha}{k^2\beta}$$
%of these items appearing together in $S^*$, to get
%$$\Pr[i,i'\in Z_s] \le \sum_{i\in S^*, i'\in S^*}  \frac{1}{(k\beta)^2} = \frac{1}{\beta^2}$$

%$$\Pr[|Z_s|>1 | T, Z_{s'}, s'\prec_w s]\le \sum_{i\in S^*, i'\in S^*}  \frac{1}{(k\beta)^2} = \frac{1}{\beta^2}$$

%Therefore, Chernoff bound, 
%applying Azuma-Hoeffding inequality (for super-martingales), 
%the total number of items from $S^*$ who are not alone in their slots in $w$ can be bounded by:
\begin{equation}
\label{eq:lower2}
%\Pr(|\{i: Y_i\in w \text{ and } |Z_{Y_i}|>1\}| \le (1-\delta) \frac{\alpha}{\beta}) \le \exp(-\frac{\delta^2\alpha}{2\beta})
\Pr\left(|\{s \in w:|Z_s|=1\}| \le (1-\delta)p\alpha\beta|T\right) \le \exp\left(-\frac{\delta^2 p^2 \alpha \beta}{2}\right) \ .
\end{equation}
 Substituting $p\ge  (1-\frac{4}{\beta})\frac{1}{\beta}$,
$$\Pr\left(|\{s \in w:|Z_s|=1\}| \le (1-\delta)(1-\frac{4}{\beta})\alpha|T\right) \le \exp\left(-\frac{\delta^2 (1-4/\beta)^2 \alpha}{2\beta}\right)\ . $$
We further substitute $\beta \ge 8$ in the right hand side of the above inequality, to bound the probability by $\exp(-\delta^2\alpha/8\beta)$.
%$$\Pr(|\{s \in w:|Z_s|=1\}| \ge (1-\delta)(1-\delta')\alpha|T) \le \exp(-\frac{\delta^2 (1-\delta')^2 \alpha}{2\beta})$$
%The desired lower bound on $\tilde \tau_w$ is then obtained by using $\delta'=\delta$.
%$$\Pr[|Z_s|\ge 1 | T, Z_{s'}, s'<s, s'\in w]\ge \sum_{i\in S^*\cup_{s'<s} Z_s'}  \frac{1}{k\beta} = \frac{k-|\cup_{s'<s} Z_s'|}{k\beta} =:x_s$$

%Since $k\ge \alpha\beta$, 
%Using \eqref{eq:lower1} and \eqref{eq:lower2}, and taking union bound, we have that for any $\delta\in(0,1)$, with probability at least $1-\exp(\frac{-\delta^2 \alpha}{2}) - \exp(\frac{-\delta^2\alpha}{\beta^3})$, at least $(1-\delta)\alpha$ items from $S^*$ are part of $\cup_{s\in w} Z_s$,  and further at most  $(1-\delta)\frac{\alpha}{\beta}$ slots contain multiple of these items. Therefore, $Z_s$ must be non-empty in at least $\left(1-\frac{1}{\beta}\right)(1-\delta)\alpha$ slots. This proves the required lower bound

%\scomment{using deviation bounds as in the earlier proofs}
\end{proof}
}

\begin{lemma}
%[Corollary of Lemma \ref{lem:lengthtau}]
[proved in~\cite{us}]
\label{cor:lengthtau}
For any real $\delta'\in (0,1)$,  if parameters $k,\alpha, \beta$ satisfy \settinga, then given any $T_{1,\ldots, w-1}=T$, with probability at least $1-\delta' e^{-\alpha/k}$,
$$|\tilde \tau_w| \ge (1-\delta') \alpha\ . $$
%are such that $\alpha \ge 4 \log(36\alpha^2/\delta'^2)$, $\beta \ge 6\alpha/\delta'$, and $k\ge 12\alpha^2/\delta'$,
%$\frac{2\alpha}{k} \le \frac{\delta'}{6\alpha}$,
%$$e^{-|\tilde \tau_w|/k} \le e^{-(1-\delta') \alpha/k}.$$

\end{lemma}
\toRemove{
\begin{proof}
We use the previous lemma with $\delta=\delta'/2$ to get lower bound of $(1-\delta')\alpha$ with probability $1-\exp(-(\delta')^2\alpha/32\beta)$. Then, substituting 
%$\alpha \ge 8\beta^2$,
$ k\ge \alpha\beta \ge \frac{64\beta}{(\delta')^2} \log(1/\delta')$ so that using $\beta \le \frac{k(\delta')^2}{64 \log(1/\delta')}$ we can bound the violation probability by
$$\exp(-(\delta')^2 \alpha/32\beta)\le \exp(-(\delta')^2 \alpha/64\beta)\exp(-\alpha/k) \le \delta' e^{-\alpha/k}.$$
where the last inequality uses $\alpha\ge 8\beta^2 \log(1/\delta')$ and $\beta \ge 8/(\delta')^2$.
%$\delta :=\frac{\log(1-\delta')}{2\alpha}$. Note that $\delta \ge \frac{\delta'}{2\alpha}$. 
\end{proof}
}

\begin{lemma}
\label{lem:Sw}
%For any $\delta'\in (0,1)$,  if parameters $k, \alpha\ge 1, \beta\ge 1$ are such that 
%$\alpha \ge 4 \log(36\alpha^2/\delta'^2)$, $\beta \ge 6\alpha/\delta'$, and $k\ge 12\alpha^2/\delta'$, then
For any real $\delta'\in (0,1)$, if parameters 
$k,\alpha, \beta$ satisfy \settinga, then
%\mbox{$k \ge \alpha\beta$}, \mbox{$\beta\ge \frac{8}{(\delta')^2}$}, $\alpha\ge 8\beta^2 \log(1/\delta')$, then %probability at least $1-\delta'$,
$$\Ex\left[\frac{k-\alpha}{k} \OPT -2f(S_{1,\ldots, w})|T_{1,\ldots, w-1}\right] \le (1-\delta') e^{-2\alpha/k} \left(\frac{k-\alpha}{k} \OPT - 2f(S_{1,\ldots, w-1})\right)\ .$$
\end{lemma}
\begin{proof}
The lemma follows from substituting Lemma \ref{cor:lengthtau} in Lemma \ref{cor:asGoodas}.
%Using previous lemma with $\delta:=\delta'/2$ we get $|\tilde \tau_w|\ge (1-\delta')\alpha$ with probability at least $1-\delta'$. Therefore, we can derive
%Since $e^{-t/k}$ is a convex decreasing function in $t$,
%$$\Ex[e^{-|\tilde \tau_w|/k} |T ] \le (1-\frac{}{})e^{-(1-\delta')\alpha/k}$$
\end{proof}

\matroidThm

\begin{proof}




Now from Lemma~\ref{lem:Sw}, we have,
%\begin{prop}
%\label{prop:first}
for any real $\delta'\in (0,1)$, if parameters 
$k,\alpha, \beta$ satisfy \settinga, then the set $S_{1,\ldots, W}$ tracked by Algorithm \ref{alg:main} satisfies
$$\mathbb{E}[f(S_{1,\ldots, W})] \ge (1-\delta')^2 (\frac{1}{2}(1-1/e^2) ) \OPT.$$
%\end{prop}
\toRemove{
\begin{proof}
By multiplying the inequality Lemma \ref{lem:Sw} from $w=1, \ldots, W$, where $W=k/\alpha$, we get 
$$\mathbb{E}[f(S_{1,\ldots, W})] \ge (1-\delta')(\frac{1}{2}(1-1/e^2)) (1-\frac{\alpha}{k}) \OPT.$$
Then, using $1-\frac{\alpha}{k}\ge 1-\delta'$ because $k\ge \alpha \beta \ge \frac{\alpha}{\delta'}$, we obtain the desired statement.
\end{proof}
}
%\begin{lemma}
%$$\Ex[f(S_{1,\ldots, w-1} \cup_{s\in w} Z_s) - f(S_{1,\ldots,w-1})|T_{1,\ldots, w-1} =T] \ge \frac{\alpha}{k}\Ex[f(S^*)-f(S_{1,\ldots, w-1})|T_{1,\ldots, w-1} =T]$$
%\end{lemma}

%------------------




%\scomment{End:Trying out something------------------------} 




Now, we compare $f(S_{1\ldots, W})$ to $f(A^*)$, where $A^*=S_{1\ldots, W} \cap A$, with $A$ being the shortlist returned by Algorithm \ref{alg:main}. The main difference between the two sets is that in construction of shortlist $A$, Algorithm \ref{alg:matroidmax} is being used to compute the argmax in the definition of $\gamma(\tau)$, in an online manner. This argmax may not be computed exactly, so that some items from $S_{1\ldots, W}$ may not be part of the shortlist $A$. 

\toRemove{
We use the following guarantee for Algorithm~\ref{alg:matroidmax} to bound the probability of this event.
}

%\begin{prop}
%\label{maxanalysis}
%Algorithm~\ref{alg:SIIImax}, with parameter $u=n\epsilon/2$,  and shortlist of size $L= (2+\sqrt{3})\ln(2/\epsilon)$ selects the maximum element with probability $(1-\epsilon)$, \end{prop}

%\scomment{I thought I changed the statement of the above proposition, did you change it back? Algorithm~\ref{alg:SIIImax}  only takes inputs $N, \delta$, the setting of $u, L$ is fixed in Algorithm~\ref{alg:SIIImax}  so it should not be mentioned in the proposition, replace the following:
%}
%\mcomment{No I just changed the format of inequality from $1-\epsilon-\delta$ to $1-\epsilon$}

\toRemove{
\begin{restatable}{prop}{maxanalysis}
\label{maxanalysis}
For any $\delta\in (0,1)$, and input $I=(a_1,\ldots, a_N)$, Algorithm~\ref{alg:matroidmax}
returns $A^*:= \max_{i\in A} g(a_i,S)$ with 
probability $(1-\delta)$. 
\end{restatable}

The proof is similar to Proposition 3 in~\cite{us}.
}
%\scomment{where is the proof of this? add intuition and reference to proof}
%The proof of the above proposition appears in Appendix \ref{app:msubm}. Intuitively, it follows from the observation that if we select every item that improves the maximum of items seen so far, we would have selected $\log(N)$ items in expectation. The exact proof involves showing that on waiting $n\delta/2$ steps and then selecting maximum of every item that improves the maximum of items seen so far, we miss the maximum item with at most $\delta$ probability, and select at most $O(\log(1/\delta))$ items with probability $1-\delta$.
%\scomment{Removed:We prove a more general theorem in the Appendix (Theorem~\ref{hprob}).}
%\scomment{There are some todos with respect to this proof. Please check the comments in appendix.}

Similar to Lemma 16 in~\cite{us}, we can show that each element in $A$ gets selected by the algorithm with probability at least $1-\delta$. More precisely,
%\begin{lemma}
%\label{online}
let $A$ be the shortlist returned by Algorithm \ref{alg:main}, and $\delta$ is the parameter used to call Algorithm \ref{alg:matroidmax} in Algorithm \ref{alg:main}. Then, for given configuration $Y$, for any item $a$, we have $$Pr(a\in A|Y, a\in S_{1,\cdots, w}) \ge 1-\delta\ .$$
%\end{lemma}

\toRemove{
\begin{proof}
From Lemma~\ref{config} by conditioning on $Y$, the set $S_{1,\cdots, W}$ is determined. Now if $a\in S_{1,\dots, w}$, 
%$a=argmax \gamma(\tau)$
then for some slot $s_j$ in an $\alpha$ length subsequence $\tau$ of some window $w$, we must have 
%$$a = \arg \max_{i\in s_j \cup R_{1, \ldots, w-1}} f(S_{1, \ldots,w-1} \cup \gamma(\tau) \cup \{i\}) - f(S_{1, \ldots, w-1} \cup \gamma(\tau)).$$
$$a = \arg \max_{i\in s_j \cup R_{1, \ldots, w-1}} g(i,S_{1, \ldots,w-1} \cup \gamma(\tau) \setminus \zeta(\tau)).$$ 

Note that in contrast with the algorithm for cardinality constraints, now one element can be removed from $S_{1,\cdots, w-1}$
and added back in the next windows. 
Let $w'$ be the first window that $a$ has been added to $S_{1,\cdots, w'}$ and has not been removed later on in the next windows $w',\cdots, w$.
%Let $w'$ be the first such window, 
Also let $\tau', s_{j'}$ be the corresponding subsequence and slot. Then, it must be true that 
%$$a = \arg \max_{i\in s_{j'}} f(S_{1, \ldots,w'-1} \cup \gamma(\tau') \cup \{i\}) - f(S_{1, \ldots, w'-1} \cup \gamma(\tau')).$$
$$a = \arg \max_{i\in s_{j'}} g(i,S_{1, \ldots,w'-1} \cup \gamma(\tau')\setminus \zeta(\tau') ).$$ 
(Note that the argmax in above is not defined on $R_{1,\cdots, w'-1}$).
The configuration $Y$ only determines the set of items in the items in slot $s_{j'}$, the items in $s_{j'}$ are still randomly ordered (refer to Lemma \ref{config}). Therefore, from Proposition~\ref{maxanalysis}, with probability $1-\delta$, $a$ will be added to the shortlist $A_{j'}(\tau')$ by Algorithm~\ref{alg:matroidmax}. Thus $a\in A \supseteq A_{j'}(\tau')$ with probability at least $1-\delta$.
\toRemove{If $a\in R_{1,\cdots, w-1}$ then $a$ has appeared in a window before $w$ for the first time, say $w'$. Since $a\in R_{1,\cdots, w-1}$ there is $\tau'$, such that
$a := \arg \max_{i\in s_{\ell}} f(S_{1, \ldots,w'-1} \cup \gamma(\tau') \cup \{i\}) - f(S_{1, \ldots, w'-1} \cup \gamma(\tau'))$ 
(Note that the argmax in above is not defined on $R_{1,\cdots, w'-1}$).
The configuration $Y$ only determines the set of items in the items in slot $s_{j'}$, the items in $s_{j'}$ are still randomly ordered (refer to Lemma \ref{..}).
The permutation of elements in $s_{\ell}$ defines whether or not the online Algorithm~\ref{alg:SIIImax} selects $a$ or not. 
Therefore, from Theorem~\ref{maxanalysis}, with probability $1-\delta$, $a$ will be added to the shortlist $A_{j'}(\tau')$ by Algorithm~\ref{alg:matroidmax}. Thus $a\in A \supseteq A_{j'}(\tau')$ with probability at least $1-\delta$.
Thus $a\in H_{1,\cdots, w'-1}$ with probability at least $1-\delta$.
Now If $a \notin R_{1,\cdots, w-1}$ and $a\in s_j$, then the permutation of elements in $s_{j}$ defines whether or not the online Algorithm~\ref{alg:matroidmax} selects $a$ or not.
Therefore again from theorem~\ref{maxanalysis}, 
$a\in H_{1,\cdots, w'-1}$ with probability at least  $1-\delta$.}
\end{proof}
}
Therefore using Lemma~\ref{sample},
%\begin{prop}
\label{prop:online}
$$\Ex[f(A^*)] := \mathbb{E}[f(S_{1,\cdots, W} \cap A)] \ge (1-\frac{\epsilon}{2})\mathbb{E}[f(S_{1,\cdots, W})]$$
where $A^*:= S_{1,\cdots, W} \cap A$ is the %size $k$ 
subset of shortlist $A$ returned by Algorithm \ref{alg:main}.
%\end{prop}
%\begin{proof}
The proof is similar to the proof in~\cite{us}.
%\end{proof}


\end{proof}

==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/olderProof.tex <==
\begin{lemma}
\label{lem:piBound}
For any element $i\in S^*$, and $w \in \{1,\ldots, W\}$
\begin{equation}
p_i:=\mathbb{P}(i\in U_w \cup Supp(T_{1,\ldots, w-1}) | T_{1,\ldots, w-1}=T) \ge \frac{\alpha}{k}
\end{equation}
\end{lemma}
\begin{proof}
%Remember that from lemma~\ref{eqprob}, for every configuration $Y \in [k\beta]^n$, we have $\mathbb{P}(Y)=(k\beta)^{-n}$.
%Also from above lemma, for $1\le w\le W$,  $T_{1,\ldots, w}$ and $S_{1, \ldots, w}$ are uniquely defined for each configuration $Y$.
%Suppose $T_{1,\cdots, w-1}=T$ and 
Let $s$ be a slot in the first $w-1$ windows and $s'$ be a slot in window $w$.
If $i\in Supp(T)$ then the statement of the lemma is trivial, so suppose $i\notin Supp(T)$.
By applying Bayes' rule to equation~\ref{eq1} we have
\[
\mathbb{P} (Y_i=s  | T_{1,\ldots, w-1}=T) \frac{ \mathbb{P}(T_{1,\ldots, w-1}=T) }{\mathbb{P}(Y_i=s) } 
\le \mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) \frac{ \mathbb{P}(T_{1,\ldots, w-1}=T) }{\mathbb{P}(Y_i=s') } 
\]
Also from Lemma~\ref{indep}, $\mathbb{P}(Y_i=s)  = \mathbb{P}(Y_i=s')$ thus 
\[
\mathbb{P} (Y_i=s  | T_{1,\ldots, w-1}=T) 
\le \mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) 
\]
Furthermore, for slot $s"$ in  windows $w, w+1, \cdots, W$, by applying Bayes' rule to lemma~\ref{afterw}
we have $\mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) =\mathbb{P} (Y_i=s"  | T_{1,\ldots, w-1}=T)$.
As a result $\mathbb{P}(i \in U_w \cup R_{1,\ldots, w-1} | T_{1,\ldots, w-1}) \ge \frac{\alpha}{k}$.

\end{proof}
%And, for every  $i\in S^*$, define
%\begin{equation}
%p_i :=\mathbb{P}(i\in U_w \cup R_{1,\ldots, w-1} | T_{1,\ldots, w-1})
%\end{equation}
%Then, a corollary of Lemma \ref{lem:piBound} is that $p_i \ge \alpha/k$. 

\begin{lemma}
\label{JIN}
Fix a window $w$. Now, given $U_w, T_{1, \ldots, w-1}$, create $\tilde{S}$ by accepting each item $i\in S^* \cap (U_w \cup R_{1,\ldots, w-1})$ independently with probability $\alpha/(kp_i)$. Then,
the indicator random variables $\{{\mathbf 1}(i\in \tilde S)|T_{1,\ldots, w-1} \}$ for all $i\in S^*$ are independent with  expected value $\alpha/k$.
\end{lemma}
\begin{proof}
Using Lemma \ref{lem:piBound}, the expected value can be derived as
$$\mathbb{P}(i\in \tilde{S}| T_{1, \ldots, w-1}) = \mathbb{P}(i\in \tilde{S}| i\in U_w\cup R_{1,\ldots, w-1},T_{1, \ldots, w-1} )\mathbb{P}(i\in U_w\cup R_{1,\ldots, w-1}| T_{1, \ldots, w-1}) = \alpha/(kp_i) \times p_i = \alpha/k.$$
Next, we show that for any $i,j\in S^*$, random variables ${\mathbf 1}(i\in \tilde S)|T_{1,\ldots, w-1}$ and ${\mathbf 1}(j\in \tilde S)|T_{1,\ldots, w-1}$ are independent. Given the construction of $\tilde S$, it suffices to prove that the random variables ${\mathbf 1}(i\in U_w \cap R_{1,\ldots, w})|T_{1,\ldots, w-1}$ and ${\mathbf 1}(j\in U_w \cap R_{1,\ldots, w})|T_{1,\ldots, w-1}$ are independent. Now, given $T_{1,\ldots, w-1}=T$, if $i \in Supp(T)$ then this is trivial since $R_{1,\ldots, w} =Supp(T)$ so that $\mathbb{P}(i\in U_w \cap R_{1,\ldots, w} | T_{1,\ldots, w-1}=T)=1$. Similarly for $j\in Supp(T)$.

So, assume $i,j  \notin Supp(T)$. Then, the problem reduces to proving that  ${\mathbf 1}(i\in U_w)|T$ and ${\mathbf 1}(j\in U_w)|T$ are independent, i.e., given $T$, $i$ and $j$ will appear in the window $w$ independently. 
To prove this, we show that $\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T)=\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T \text{ and } Y_j =s')$, i.e., slot assignment of $i$ is independent of the slot assignment of $j$. 

Suppose $Y'$ is a configuration such that $Y'_i=s$ and $Y'_j=s'$, and $T_{1,\cdots, w-1}(Y')=T$. To show the required independence, we show that for every other feasible slot assignment of $j$, there exists a feasible configuration where slot assignment of $i$ is $s$.
More precisely, consider any configuration $Y''$ such that $T_{1,\cdots, w-1} (Y'') =T$ and $Y''_j=s''$ where $s''\ne s'$. (If no such configuration $Y''$ exists, then $Y_j|T$ is always $s'$ so that $s'$ is the only feasible assignment of $j$ given $T$, and the desired statement is trivially true.)
Then by changing $Y_j$ from $s'$ to $s''$ in $Y'$, we can obtain another configuration $\bar{Y}$. In Lemma~\ref{addtoslot}, we show that this change will not effect $T_{1,\cdots, w-1}$, i.e., $T_{1,\cdots, w-1} (\bar Y)=T $. 
Thus configuration $\bar Y$ satisfies the desired statement.
\end{proof}
\scomment{I replaced the proof below with the proof of Lemma 7}
\toRemove{
\begin{proof}
Suppose $i,j \in S^*$. 
If $i \in Supp(T) $ then this is trivial since $\mathbf{1}(i\in \tilde S) | T=1$. \scomment{the preceding statement is not correct, in that case, we just have $p_i=1$.}
So suppose $i,j  \notin Supp(T)$. 
%Now we show that $\mathbb{P}(J_i=1|T_{1,\cdots, w-1}=T)=\mathbb{P}(J_i=1|T_{1,\cdots, w-1}=T \text{ and } J_j =s')$.
Now we show that $\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T)=\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T \text{ and } Y_j =s')$.
Suppose $Y$ is a configuration in which $Y_i=s$ and $Y_j=s'$, and $T_{1,\cdots, w-1} (Y)=T$.
Also suppose there exists at least one configuration $\bar{Y}$ such that $T_{1,\cdots, w-1} (\bar{Y}) =T$ and $\bar{Y}_j=s"$. \scomment{what if no such configuration exists?}
Then by changing $Y_j$ from $s'$ to $s"$ we obtain a configuration $Y'$. Also from lemma~\ref{addtoslot}, we have  $T_{1,\cdots, w-1} (Y')=T $. 
%It is because in configuration $Y$, $j$ has not been selected in slot $s'$ and its removal will not change $T_{1,\cdots, w-1}$.
%Furthermore since there is a configuration $\bar{Y}$ as described above, adding $j$ to $s"$ will not change $T_{1,\cdots, w-1}$.
Hence the mapping from $Y$ to $Y'$ proves lemma.
\end{proof}
}

\begin{lemma} \label{addtoslot}
Fix a slot $s'$, $T$, $j\notin Supp(T)$. Suppose that there exists  some configuration  $Y'$ such that $T_{1,\cdots, w-1} (Y') =T$ and $Y_j'=s'$. Then, given any configuration $Y''$ with $T_{1,\ldots, w-1}(Y'')=T$, we can replace  $Y''_j$ with $s'$ to obtain a new configuration $\bar Y$ that also satisfies $T_{1,\ldots, w-1}(\bar Y)=T$.
\toRemove{
Suppose there exists at least one configuration $\bar{Y}$ such that   $T_{1,\cdots, w-1} (\bar{Y}) =T$ and $\bar{Y}_j=s$ for $j\notin Supp(T)$.
Then for any configuration $Y$ with  $T_{1,\cdots, w-1} (Y) =T$, by setting $Y_j=s$, we get a new configuration $Y'$
such that $T_{1,\cdots, w-1} (Y') =T$.}
\end{lemma}
\begin{proof}
%Suppose $Y$ is a configuration such that $T_{1,\cdots, w-1} (Y) =T$. 
Suppose the slot $s'$ lies in window $w'$.
If $w' \ge w$ then the statement is trivial. So suppose $w' < w$.
Create an intermediate configuration by {\it removing} the item $j$ from $Y''$, call it $Y^-$. Since $j\notin Supp(T_{1,\cdots, w-1}(Y'')) = Supp(T)$ we have $T_{1,\cdots, w-1} (Y^-) =T$. In fact, for every subsequence $\tau$, the greedy subsequence for $Y''$, will be same as that for $Y^-$, i.e.,   $\gamma_{Y''}(\tau) = \gamma_{Y^-}(\tau)$.
Now add item $j$ to slot $s'$ in $Y^-$, to obtain configuration $\bar Y$. We claim $T_{1,\cdots, w-1} (\bar Y) =T$.
%We only need to show that $j$ will not get selected in slot $s$ in configuration $Y'$.
%Suppose not, then there is a subsequence $\tau$  in the algorithm ending in slot $s$ such that $\gamma_{Y'} (\tau) =\{i_1, \cdots, i_{t-1}, j\}$


By construction of $T_{1,\ldots, w}$, we only need to show that $j$ will not be part of the greedy subsequence $\gamma_{\bar Y}(\tau)$ for any subsequence $\tau, |\tau| = \alpha$ containing the slot $s'$ when the input is in configuration $\bar Y$. To prove by contradiction, suppose that $j$ is part of greedy subesquence for some $\tau$ ending in the slot $s'$. \toRemove{We only need to show that $j$ will not get selected in slot $s$ in configuration $Y'$.
Suppose $j$ gets selected in slot $s$ for some subsequence $\tau$ ending in slot $s$.}
%Thus $\gamma_{Y'}(\tau) = \{i_1, \cdots, i_{t-1}, j\}$. Note that since slots before $s$ are the same as $Y^-$ and $T_{1,\cdots, w-1} (Y^-) =T$, $\gamma_{Y^-}(\tau) = \{i_1, \cdots, i_{t-1}, i_t\}$.
\toRemove{Suppose that $\gamma_{Y^-}(\tau)  := \{i_1, \cdots, i_{t-1}, i_t\} = \gamma_{Y''}(\tau) $.} 
For this $\tau$, let $\gamma_{Y^-}(\tau)  := \{i_1, \cdots, i_{\alpha-1}, i_\alpha\} = \gamma_{Y''}(\tau) $. Note that since the items in the  slots  before $s'$ are identical for $\bar Y$ and $Y^-$, \toRemove{and $T_{1,\cdots, w-1} (Y^-) =T$,} we must have that $\gamma_{\bar Y}(\tau) = \{i_1, \cdots, i_{\alpha-1}, j\}$, i.e.,
$\Delta_f(j | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{\alpha-1}\} ) \ge \Delta_f(i_\alpha | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{\alpha-1}\} ) $.
%$j=\arg \max_{i\in j\cup U_s \cup T_{1, \ldots, w-1}} \Delta_f(i | S_{1,\ldots,w-1} \cup \{i_1,\ldots, i_{t-1}\} \cup \{i\}) $
%$i_t=\arg \max_{i\in U_s \cup T_{1, \ldots, w-1}} \Delta_f(i | S_{1,\ldots,w-1} \cup \{i_1,\ldots, i_{t-1}\} \cup \{i\}) $
On the other hand, since $T_{1,\cdots, w'-1} (Y') = T_{1, \cdots, w'-1}(Y'') = T (\text{restricted to $w'-1$ windows})$,  we have that $\gamma_{Y'} (\tau) =\{i_1, \cdots, i_\alpha\}$.
However, $Y'_j=s'$. Therefore $j$ was not part of the greedy subsequence $\gamma_{Y'}(\tau)$ even though it was in the last slot in $\tau$, implying $\Delta_f(j | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{t-1}\} ) < \Delta_f(i_t | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{t-1}\} ) $. This is  is a contradiction to the earlier observation.


\end{proof}
%Now let  indicator random variable $J_i$ for $i\in S^*$ indicates whether or not $i \in \tilde{S}$ 
%indicates whether or not $e$ appears in $U_w$, i.e., whether or not $U_i^e\in W_{i+1}$.



%Also if $V_e$ is a random variable indicating whether or not $e\in \mathcal{A}$ for $e\in OPT'$,
%we show $\{V_e|Snapshot(i)\}_{e\in OPT'}$ are i.i.d.  with $\mathbb{P}[V_e=1] = \alpha/k$.

%\begin{lemma}
 % %$\mathbb{P}[e=b_j| e\in \mathcal{A}]=1/k$ for $j\in[k]$.
% Random variables $\{V_e|Snapshot(i)\}$,  $ \forall e\in OPT'$ are i.i.d. with $\mathbb{P}[V_e=1]=\alpha/k$.
%\end{lemma}

%\begin{prop}\label{uni}
% Given $i \in \tilde{S}$, we have $\mathbb{P}(i=j)=1/k$, $\forall j\in S^*$.
%\end{prop}

%\scomment{The lemma statement below is not precise- it seems you actually mean uniformly at  random over $\tilde S|T_{1,\ldots, w-1}$, i.e., random also over $U_w$, but given $T_{1, \ldots, w-1}$. We can discuss.}
\begin{prop}\label{uni}
For element $i$ drawn uniformly at random from $\tilde{S}$, we have $\mathbb{P}(i=e)=1/k$, $\forall e\in S^*$.
\end{prop}




Now each element in $\tilde{S}\cap U_w$ has a unique slot in $w$. 
\begin{prop}
Suppose $p_1, \dots, p_{\ell}$ are the slots in $w$ containing at least one element of $\tilde{S}\cap U_w$ (in the same order that they appear in $w$). 
In addition, suppose $b_j\in p_j\cap \tilde{S}$, is the element of $\tilde{S}\cap U_w$ in slot $p_j$ (in case there are more than one element choose one randomly).
%$a_1 ,\cdots, a_t$ are $t$ samples without replacement drawn uniformly at random from $\tilde{S}$.
Then $b_1, \cdots, b_{\ell}$ is a random order of $\{b_1, \cdots, b_{\ell}\}$, and $\{b_1, \cdots, b_{\ell}\}$ are drawn uniformly at random from $\tilde{S}\cap U_w$.
\end{prop}
\scomment{Is Proposition 3 same as saying that $\{Y_i, i\in \tilde S\cap U_w\}$ are i.i.d. and uniformly distributed over slots in $w$? Where is the proof of this proposition?}
\mcomment{Yes, it follows from lemma 7 and the fact that we showed in lemma 6: for slot $s"$ in  windows $w$, by applying Bayes' rule to lemma~\ref{afterw}
we have $\mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) =\mathbb{P} (Y_i=s"  | T_{1,\ldots, w-1}=T)$.}
%\begin{prop}\label{rord}
%%$a_1 ,\cdots, a_t$ are $t$ samples without replacement drawn uniformly at random from $\tilde{S}$.
%$a_1, \cdots, a_t$ is a random order of $\{a_1, \cdots, a_t\}$, and $\{a_1, \cdots, a_t\}$ are drawn uniformly at random from $\tilde{S}$.
%\end{prop}

On the other hand, elements of $\tilde{S}\cap R_{1,\ldots, w-1}$ 
are not assigned to a  unique slot in $w$ (in the algorithm they were compared against the maximum marginal value in all the slots of $w$).
So we can assign each of them to a unique random slot in $w$.

\begin{prop}
Suppose $q_1, \dots, q_{m}$ are the slots in $w$ assigned to at least one element of $\tilde{S} \cap R_{1,\ldots, w-1}$ (in the same order that they appear in $w$). 
Furthermore, suppose $c_j\in q_j\cap \tilde{S}$, is the element of $\tilde{S}\cap R_{1,\ldots, w-1}$ in slot $q_j$ (in case there are more than one element choose one randomly).
%$a_1 ,\cdots, a_t$ are $t$ samples without replacement drawn uniformly at random from $\tilde{S}$.
Then $c_1, \cdots, c_m$ is a random order of $\{c_1, \cdots, c_m\}$, and $\{c_1, \cdots, c_m\}$ are drawn uniformly at random from $\tilde{S}\cap R_{1,\ldots, w-1} $.
\end{prop}


Now suppose $\{i_1, \cdots, i_t\}=\{p_1, \dots, p_{\ell}\} \cup \{q_1, \dots, q_{m}\}$ (in the same order that they appear in $w$).
From above propositions we have
\begin{prop}\label{rord}
Suppose $a_j \in i_j$  is an element of $i_j \cap (\{p_1, \dots, p_{\ell}\} \cup \{q_1, \dots, q_{m}\})$ (in case there are more than one element choose one randomly).Then
% $a_1, \cdots, a_m$ is a random order of $\{c_1, \cdots, c_m\}$, and $\{c_1, \cdots, c_m\}$ are drawn uniformly at random from $\tilde{S}\cap R_{1,\ldots, w-1} $.
%$a_1 ,\cdots, a_t$ are $t$ samples without replacement drawn uniformly at random from $\tilde{S}$.
$a_1, \cdots, a_t$ is a random order of $\{a_1, \cdots, a_t\}$, and $\{a_1, \cdots, a_t\}$ are drawn uniformly at random from $\tilde{S}$.
\end{prop}





%Consider the set $\mathcal{A}$ we create using the blackbox algorithm. It is a set that we create only for the purpose of argument. Algorithm~\ref{alg:khod} is not aware of this set. 
%Its existence is enough for the algorithm.
The algorithm \textit{guess} the position of elements of $\tilde{S}$, %$OPT\cap W_{i+1}$, 
i.e., slots $i_1, \cdots, i_t$. %, where $t \ge (1-\delta)\alpha$ w.h.p.
In other words, for some $\tau$ in the enumeration of algorithm,  the elements of $\tilde{S}$ lie in the slots of $\tau$. i.e., $\{i_1, \cdots, i_t\} \subseteq \tau$.
%Suppose $a_j\in i_j\cap \tilde{S}$, is the element of $\tilde{S}$ in slot $i_j$.
Suppose $s_j$ is the maximum element selected by the algorithm in $i_j$.
i.e., %$s_j=\omega(\{i_1,\dots,i_j\})$.
$s_j=argmax_{a\in i_j} \Delta_F(a| \gamma{(i_1,\ldots, i_{j-1})})$.
Also let's define $A(j)=\{a_1, \cdots, a_j\} $ and $S(w,j)= S_{1,\ldots, w-1} \cup \{s_1,\cdots, s_j\}$.

\begin{lemma}
%$\mathbb{E}[\Delta_F(S_w | S_{1,\ldots, w-1})] \ge \frac{t}{k} (\frac{k-\alpha}{k}OPT-\mathbb{E}[F(S_{1,\ldots, w-1})])$.
$\mathbb{E}[\Delta_F(s_{j+1}|S(w,j))] \ge \frac{1}{k} (\frac{k-\alpha}{k}OPT-\mathbb{E}[F(S(w,j))])$
\end{lemma}

\begin{proof}
\scomment{What is $OPT'$? What is $P$?}
\mcomment{$P:=S^*\setminus S_{1,\dots, w-1}$, Replaced}
From proposition~\ref{uni} and~\ref{rord}, $a_1$ can be any element in $S^*$, % $OPT\setminus P$, 
w.p. at least $1/k$.
Thus,
\[
\mathbb{E}[\Delta_F(a_1|S_{1,\ldots, w-1}) | T_{1,\ldots, w-1}] \ge \frac{1}{k} \sum_{e\in S^*} \Delta_F(e|S_{1,\ldots, w-1}) %=\frac{1}{k} \sum_{e\in OPT\setminus %P} \Delta_F(e|S_{1,\ldots, w-1}).
\]

%\[
%\mathbb{E}[\Delta_F(a_1|S_{1,\ldots, w-1}) | T_{1,\ldots, w-1}] \ge \frac{1}{k} \sum_{e\in OPT'} \Delta_F(e|S_{1,\ldots, w-1}) =\frac{1}{k} \sum_{e\in OPT\setminus P} \Delta_F(e|S_{1,\ldots, w-1}).
%\]
% (OPT-F(S(i)))$.


Now we use the following well known lemma:
\begin{lemma}%\label{marginalsum}
For any set $A$ and $B$, $\Delta_F(A|B) \le \sum_{a\in A\setminus B} \Delta_F(a|B)$
\end{lemma}
%(Note that in the original version of this lemma the sum is over $A$ instead of $A\setminus B$. But the above format is  stronger if  $A$ and $B$ have intersection. It is the reason we can assign value zero to dummy elements which represent the intersection).
Therefore,
\[
%OPT-F(S(i)) \le \sum_{e\in OPT} \Delta_F(e|S(i)) = \sum_{e\in OPT\setminus P} \Delta_F(e|S(i)) 
OPT-F(S_{1,\ldots, w-1}) \le  \sum_{e\in S^*}  %OPT\setminus P} 
\Delta_F(e|S_{1,\ldots, w-1})  %=  \sum_{e\in OPT'} \Delta_F(e|S(i)) 
\]
Hence,  
\[
\mathbb{E}[\Delta_F(a_1|S_{1,\ldots, w-1})|T_{1,\ldots, w-1}] \ge \frac{1}{k} (OPT-F(S_{1,\ldots, w-1})).
\]
%Now let's define $A(j)=\{a_1, \cdots, a_j\} $ and $S(w,j)= S_{1,\ldots, w-1} \cup \{s_1,\cdots, s_j\}$.
%denote $S(i)\cup \{s_1, \cdots, s_j\} $ by $S(i,j)$. 
Similarly, we can see that 
%$E[\Delta_F(a_{j+1}|S(i,j))] \ge \frac{1}{k} (OPT-F(S(i,j)))$.
\[
\mathbb{E}[\Delta_F(a_{j+1}|S(w,j)) | T_{1,\ldots, w-1}] \ge  \frac{1}{k} \sum_{e\in S^*\setminus A(j)} \Delta_F(e|S(w,j)) 
%=\frac{1}{k} \sum_{e\in OPT\setminus (P\cup A(j))} \Delta_F(e|S(w,j)) 
%\ge \frac{1}{k} \sum_{e\in OPT\setminus (P\cup A)} \Delta_F(e|S(i,j))
\]
Also we have,
\begin{align*} %\label{eq1}
%\begin{split}
%A & = \frac{\pi r^2}{2} \\
% & = \frac{1}{2} \pi r^2
\sum_{e\in S^*\setminus A(j) } %OPT\setminus {(P\cup A(j))}} 
\mathbb{E}[\Delta_F(e|S(w,j)) | T_{1,\ldots, w-1}]  %= \sum_{e\in OPT\setminus P} \Delta_F(e|S(i,j)) 
&\ge \mathbb{E}[F(S^*\setminus A(j)) | T_{1,\ldots, w-1}]-\mathbb{E}[F(S(w,j)) | T_{1,\ldots, w-1}] \\
&\ge \frac{k-\alpha}{k}OPT-\mathbb{E}[F(S(w,j)) | T_{1,\ldots, w-1}] 
%\end{split}
\end{align*}
The last inequality coming from the fact that given $T_{1,\ldots, w-1}$, the set $A(j)$ is a random subset of $S^*$ of size at most  $\alpha$,
so we can apply the following lemma%~\ref{randomsubset}.
\begin{lemma}\label{randomsubset}
For a random subset $A$ of $R$, the expected value of $f(A)$ is at least $\frac{|A|}{k}.f(R)$.
\end{lemma}
Thus 
\[
\mathbb{E}[F(S^*\setminus A(j)) | T_{1,\ldots, w-1}] \ge \frac{k-\alpha}{k}OPT .
\]
Hence, 
\begin{align*}
\mathbb{E}[\Delta_F(s_{j+1}|S(w,j)) | T_{1,\ldots, w-1}] &\ge \mathbb{E}[\Delta_F(a_{j+1}|S(w,j)) | T_{1,\ldots, w-1}] \\
& \ge \frac{1}{k} (\frac{k-\alpha}{k}OPT-\mathbb{E}[F(S(w,j)) | T_{1,\ldots, w-1}]) 
\end{align*}
Now by taking expectation over all possible realizations of $T_{1,\ldots, w-1}$,
\[
\mathbb{E}[\Delta_F(s_{j+1}|S(w,j))] \ge \frac{1}{k} (\frac{k-\alpha}{k}OPT-\mathbb{E}[F(S(w,j))])
\]
%Now by standard techniques we can deduce that $\mathbb{E}[F(S_{1,\ldots, W})] \ge (1-1/e)(\frac{k-\alpha}{k})(1-\delta) OPT$.

 \end{proof}

 
 
Now we prove 
elements of $\tilde{S}$ cover at least  $(1-\delta)\alpha$ slots in $w$, w.h.p. Let $t_w$  denote the number of these slots in $w$.

\begin{theorem}
%Elements of $\tilde{S}$ cover at least  $(1-\delta)\alpha$ slots in $w$, w.h.p.
$(1-\delta)\alpha \le t_w \le (1+\delta)\alpha$, w.h.p. 
\end{theorem}


%Therefore,
%$$\Ex[f(\tilde S \cup S_{1,\ldots, w-1}) - f(S_{1,\ldots, w-1})] \ge \frac{\alpha}{k} f(S^* \cup S_{1,\ldots, w-1}) - f(S_{1,\ldots, w-1}) $$
%INCOMPLETE: the expected size of $\tilde{S}$ is $\alpha$, but the realized size could be larger, and will be truncated to $\alpha$. We need to account for the decrease in objective due to this truncation.
By Chernouf bound, we can show that with high probability each window contains roughly $\alpha$ elements of $\tilde{S}$.

\begin{lemma}\label{bern}
%Suppose $W$ is a $(\alpha,\beta)$ window then
For window $w$
\[
\mathbb{P}(|\tilde{S}| < (1-\delta)\alpha ) %\le exp(-\frac{ (1/2)\alpha^{3/2}}{\alpha+1}) \le exp(-\sqrt{\alpha}/4)
\le \exp(-\delta^2 \alpha/2)
\]
\end{lemma}

Also we can show that roughly $\alpha-2\alpha/\beta$ slots in a window contain at least one element of $\tilde{S}$.

\begin{lemma}\label{slotlemma}
%The probability that one slot has two or more elements is at most $1-e^{-1/\beta}$.
%The fraction of nonempty slots with more than one elements of $OPT$ is at most $\beta(1-e^{1/\beta})$.
%The total number of slots  with more than one element of $OPT$  is at most $2\alpha/\beta$, w.h.p.
Given $|\tilde{S}|=r$,
the total number of slots in $W$ containing at least one element of $\tilde{S}$ is greater than %\alpha-2\alpha/\beta$  w.h.p.
$r(1-r/\alpha \beta)$  w.h.p.
%The total number of elements $e\in OPT\cap W$ such that $Y_e\cap OPT=\{e\}$ is at least $\alpha-2\alpha/\beta$.
%with more than one element of $OPT$  is at most $2\alpha/\beta$, w.h.p.
%$\beta(1-e^{1/\beta})$, w.h.p.
\end{lemma}
\begin{proof}

Suppose $\tilde{S}=\{a_1,\dots, a_r\}$.
%From previous lemma $r\le 2\alpha$, w.p. at least $1-\exp(-\sqrt{\alpha}/3)$.
Let $Z_i$ be a random variable indicating whether or not %$Y_{a_j}\cap OPT\neq \{a_j\}$.
$|Y_{a_j}\cap \{a_1,\dots, a_{j-1}\}| \ge 1$.
%indicating whether $a_k$ is alone in its slot or not.
We have at most $r$ occupied slots, thus the probability that $Z_i=1$ is at most $ r/(\alpha \beta) $ or $\mathbb{E}[Z_i]\le r/\alpha\beta$. Furthermore let $X_i=\sum_{j=1}^{i} Z_j$, then $\mathbb{E}[X_i] \le ri/\alpha\beta$.
%Also let $\mathcal{F}_i$ be the slots elements $1,\cdots, i$  are in, then $L\le \alpha/\beta$. 
Also define the set of filtration $\{\mathcal{F}_i\}$ to be the slots containing elements $\{a_1,\cdots, a_i\}$.
Then $\mathcal{F}_0 \subseteq \dots \subseteq \mathcal{F}_r$.
In addition, $L=\sum_{i\le r}  Var(Z_i|\mathcal{F}_{i-1}) \le r^2/\alpha\beta$.
By Freedman's inequality $\mathbb{P}( X_r > r^2/\alpha\beta + \epsilon )  \le exp(-\frac{\epsilon^2}{4r^2/\alpha\beta +2\epsilon})$.
\end{proof}

Suppose $\delta=1-1/e-R$.
From the above lemmas there are large enough constants $\alpha$ and $\beta$ such that:
\begin{itemize}
\item $r=|OPT\cap W| > (1-\delta/4)\alpha$. Thus $\alpha \ge \frac{1}{\delta^2} \log(1/\delta)$
\item The total number of slots in $W$ containing at least one element of $OPT$ is at least $(1-\delta)\alpha$.
Thus $(1-\delta/4)\alpha(1-(1-\delta/4)/\beta) > (1-\delta)\alpha$.
Therefore $\beta > (1-\delta/4)^2/(3/4\delta) $, so it suffices to have $\beta>\frac{4}{3\delta}$.
\end{itemize}
Hence we choose constants $(\alpha,\beta)$ with $\alpha \ge \frac{8}{\delta^2} \log(1/\delta)$ and $\beta>\frac{4}{3\delta}$,
so that we have above properties.

Therefore $\sum_{w} \min(\alpha, t_w) \ge (1-\delta)k$, w.h.p.
Now by standard techniques we can deduce that 
\begin{theorem}
$\mathbb{E}[F(S_{1,\ldots, W})] \ge (1-1/e)(\frac{k-\alpha}{k})(1-\delta) OPT$.
\end{theorem}

==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/preliminaries.tex <==
%\subsection{Preliminaries}



%Some useful properties of submodular functions}
 The following properties of submodular functions are well known (e.g., see~\cite{Buchbinder:2014,Feige:2011,Feldman:2015}). %\ref{bookorpaper}). \scomment{add some reference}
\begin{lemma}\label{marginalsum}
Given a monotone submodular function $f$, and subsets $A,B$ in the domain of $f$, we use $\Delta_f(A|B)$ to denote $f(A\cup B)-f(B)$. 
For any set $A$ and $B$, $\Delta_f(A|B) \le \sum_{a\in A\setminus B} \Delta_f(a|B)$
\end{lemma}
\begin{lemma}\label{sample}
Denote by $A(p)$ a random subset of $A$ where each element has probability at least $p$ to appear in $A$ (not necessarily independently). Then $E[f(A(p))] \ge (1-p) f(\emptyset) + (p)f(A)$
\end{lemma}

%\scomment{Doesn't Lemma \ref{constssample} follow from Lemma \ref{sample} by setting $p=|A|/k$}

We will use the following well known deviation inequality for martingales (or supermartingales/submartingales).

%\mcomment{also we should add freedman}
%\scomment{Where is that being used?}
%\mcomment{appendix proof of m-submodular} \scomment{anything that is only being used in appendix should be added to appendix}
\begin{lemma}[Azuma-Hoeffding inequality]
\label{lem:azuma}
Suppose $\{ X_k : k = 0, 1, 2, 3, ... \}$ is a martingale (or super-martingale) and ${\displaystyle |X_{k}-X_{k-1}|<c_{k},\,} $
almost surely. Then for all positive integers N and all positive reals $r$,
$${\displaystyle P(X_{N}-X_{0}\geq r)\leq \exp \left(\frac{-r^{2}}{2\sum _{k=1}^{N}c_{k}^{2}}\right).} $$
And symmetrically (when $X_k$ is a sub-martingale):
$$
{\displaystyle P(X_{N}-X_{0}\leq -r)\leq \exp \left(\frac{-r^{2}}{2\sum _{k=1}^{N}c_{k}^{2}}\right).} 
$$
\end{lemma}
\begin{lemma}[Chernoff bound for Bernoulli r.v.]
\label{lem:Chernoff}
Let $X = \sum_{i=1}^N X_i$, where $X_i = 1$ with probability $p_i$ and $X_i = 0$ with
probability $1 - p_i$, and all $X_i$ are independent. Let $\mu = \Ex(X) = \sum_{i=1}^N p_i$. Then, 
$$P(X \geq (1 + \delta)\mu) \le e^{{-\delta^2\mu}/{(2+\delta)}} $$
for all $\delta>0$, and
$$P(X \leq (1 - \delta)\mu) \le e^{-\delta^2\mu/2}$$
for all $\delta\in(0,1)$. 
\end{lemma}

\begin{definition}
(\textbf{Matroids}). A matroid is a finite set system $\mathcal{M} = (\mathcal{N} , \mathcal{I})$, where $\mathcal{N}$ is a set and $\mathcal{I}\subseteq 2^{\mathcal{N}}$
is a family of subsets such that: (i) $\emptyset \in I$, (ii) If $A \subseteq B \subseteq N$ , and $B \in I$, then $A \in I$,
(iii) If $A, B \in I$ and $|A| < |B|$, then there is an element $b \in B\setminus A$ such that $A + b \in I$. In a matroid $\mathcal{M} = (\mathcal{N} , \mathcal{I})$, $N$ is called the ground set and the members of $\mathcal{I}$ are called independent sets of the matroid. The bases of $\mathcal{M}$ share a common cardinality, called the
rank of $\mathcal{M}$.
\end{definition}

\begin{lemma} 
\label{lem:Brualdi} (\textbf{Brualdi} )
If $A, B$ are any two bases of matroid $M$ then there exists a
bijection $\pi$ from $A$ to $B$, fixing $A\cap B$, such that $A - x + \pi(x) \in M$ for all $x \in A$.
\end{lemma}


\subsection{Some useful properties of $(\alpha, \beta)$ windows}
In~\cite{us}, we proved some useful properties of $(\alpha, \beta)$ windows, defined in Definition~\ref{def:windows} and used in Algorithm \ref{alg:main}. 
which we summarize it in this section.

The first observation is that every item will appear uniformly at random in one of the $k\beta$ slots in $(\alpha,\beta)$ windows. 

\begin{definition}
For each item $e\in I$, define $Y_e\in [k\beta]$ as the random variable indicating the slot in which $e$ appears. We call vector $Y\in [k\beta]^n$ a \textit{configuration}.
\end{definition}
%Since the length of each slot is coming from $B(n,\frac{1}{k\beta})$, random variables $\{Y_e\}_{e\in I}$ are i.i.d. with uniform distribution on all $k\beta$ slots. 


\begin{lemma} \label{lem:indep}
Random variables $\{Y_e\}_{e\in I}$ are i.i.d. with uniform distribution on all $k\beta$ slots. 
\end{lemma}

This follows from the uniform random order of arrivals, and the use of the balls in bins process to determine the number of items in a slot during the construction of $(\alpha,\beta)$ windows. 
%A proof is provided in Appendix \ref{app:windows}.

%Further, we define the following new quantities to aid the analysis. 
%\scomment{Earlier $T_w$ was defined as $T_w:= \bigcup_{\tau} (\tau, \gamma(\tau))$. I am not sure how one would define  union over such things. }
Next, we make important observations about the probability of assignment of items in $S^*$ in the slots in a window $w$, given the sets $R_{1,\ldots, w-1}, S_{1,\ldots, w-1}$ (refer to \eqref{eq:Rw}, \eqref{eq:Sw} for definition of these sets). 
To aid analysis, we define the following new random variable $T_w$ that will track all the useful information from a window $w$.  
\begin{definition}
Define $T_w:= \{(\tau, \gamma(\tau))\}_\tau$, for  all $\alpha$-length subsequences $\tau=(s_1,\ldots, s_\alpha)$ of the $\alpha\beta$ slots in window $w$. Here, $\gamma(\tau)$ is a sequence of items as defined in \eqref{eq:gamma}. Also define  $Supp(T_{1,\cdots ,w}) :=\{e| e\in\gamma(\tau) \text{ for some } (\tau, \gamma(\tau))\in T_{1,\cdots, w} \} $ (Note that $Supp(T_{1,\cdots, w})=R_{1,\ldots, w}$).
%take the union of $(\gamma(\tau), \tau)$
%$T_{1,\cdots, w} := \bigcup_{\omega \le w, \tau \in w} (\tau, \gamma(\tau)) $
\end{definition}

%\begin{obs}
%For $1\le w\le W$,  $T_{1,\ldots, w}$ and $S_{1, \ldots, w}$  are independent of ordering of elements within a slot.
%\end{obs}
\begin{lemma}
\label{config}
For any window $w\in [W]$,  $T_{1,\ldots, w}$ and $S_{1, \ldots, w}$ \toRemove{are uniquely defined for each configuration $Y$.}
are independent of the ordering of elements within any slot, and 
are determined by the configuration $Y$.
\end{lemma}
\toRemove{
\begin{proof}
Given the assignment of items to each slot, it follows from the definition of $\gamma(\tau)$ and $S_w$ (refer to \eqref{eq:gamma} and \eqref{eq:Sw}) that $T_{1,\ldots, w}$ and $S_{1, \ldots, w}$ are independent of the ordering of items within a slot. Now, since  the assignment of items to slot are determined by the configuration $Y$, we obtain the desired lemma statement.
%and the position of each reassignments that are determined by $(Y,Z)$.
\end{proof}
}

Following the above lemma, given a configuration $Y$, we will some times use the notation $T_{1,\ldots, w}(Y)$ and $S_{1, \ldots, w}(Y)$ to make this mapping explicit.


\begin{lemma}
\label{lem:pijBound}
For any item $i\in S^*$, window $w \in \{1,\ldots, W\}$, and slot $s$ in window $w$, define
\begin{equation}
\label{eq:pijBound}
p_{is}:=\mathbb{P}(i \in s \cup Supp(T) | T_{1,\ldots, w-1}=T).
\end{equation}
Then, for any pair of slots $s',s''$ in windows $w, w+1, \ldots, W$,
\begin{equation}
p_{is'}=p_{is''} \ge \frac{1}{k\beta} \ .
\end{equation}
\end{lemma}
\toRemove{
\begin{proof}
%Let $s$ be a slot in the first $w-1$ windows and $s'$ be a slot in window $w$.
If $i\in Supp(T)$ then the statement of the lemma is trivial, so consider $i\notin Supp(T)$. For such $i$, $p_{is}=\mathbb{P} (Y_i=s  | T_{1,\ldots, w-1}=T)$. 
%Now, consider any pair of slots $s,s'$ with $s$ in windows $1,\ldots, w-1$ and $s'$ in window $w$.

%begin{lemma}
%label{beforeafterw}
%label{afterw}
%or $w\in [W]$, consider any $i\in S^*$ and $i\notin Supp(T_{1,\ldots, w-1})$. 
We show that for any pair of slots $s,s'$, where $s$ is a slot in first $w-1$ windows and $s'$ is a slot in window $w$, 
\begin{equation}\label{eq1}
\mathbb{P}(T_{1,\ldots, w-1}=T|Y_i=s) \le \mathbb{P}(T_{1,\ldots, w-1}=T|Y_i=s') \ .
\end{equation}
And, for any %Similarly we can show the following:
%\begin{lemma} \label{afterw}
pair of slots $s', s''$ in windows $\{w, w+1 ,\cdots, W\}$, 
\begin{equation}
\label{eq:afterw}
\mathbb{P} ( T_{1,\ldots, w-1}=T | Y_i=s' ) =\mathbb{P} ( T_{1,\ldots, w-1}=T | Y_i=s'').
\end{equation}
%end{lemma}
%begin{proof}
To see \eqref{eq1}, suppose for a configuration $Y$ we have $Y_i=s$ and $T_{1,\cdots, w-1}(Y)=T $. 
Since $i\notin Supp(T)$, then by definition of $T_{1,\ldots, w-1}$ we have that $i\notin \gamma(\tau)$ for any  $\alpha$ length subsequence $\tau$ of slots in any of the windows $1,\ldots, w-1$. Therefore, if we remove $i$ from windows ${1,\cdots, w-1}$ (i.e., consider another configuration where $Y_i$ is in windows $\{w, \ldots, W\}$) then $T_{1,\cdots, w-1}$ would not change. This is because $i$ is not the output of argmax in definition of $\gamma(\tau)$ (refer to  \eqref{eq:gamma}) for any $\tau$, so that its removal will not change the output of argmax. 
Also by adding $i$ to slot $s'$, $T_{1,\cdots, w-1}$ will not change since $s'$ is not in window $1,\cdots, w-1$.
Suppose configuration $Y'$ is a new configuration obtained from $Y$ by changing $Y_i$ from $s$ to $s'$. 
Therefore $T_{1,\cdots ,w-1}(Y') = T$. 
Also remember that from lemma~\ref{eqprob}, $\mathbb{P} (Y) = \mathbb{P}(Y')$.
%Now consider this mapping that take a configuration $Y$ with $Y_i=s$ and map it to configuration $Y'$ with $Y'=s'$.
%This mapping is 
This mapping shows that $\mathbb{P}(T_{1,\ldots, w-1}=T|Y_i=s) \le \mathbb{P}(T_{1,\ldots, w-1}=T|Y_i=s')$. 

The proof for \eqref{eq:afterw} is similar.
%end{proof}


%Now, consider any slot $s$ in window $1,\ldots, w-1$.
By applying Bayes' rule to \eqref{eq1} we have 
\[
\mathbb{P} (Y_i=s  | T_{1,\ldots, w-1}=T) \frac{ \mathbb{P}(T_{1,\ldots, w-1}=T) }{\mathbb{P}(Y_i=s) } 
\le \mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) \frac{ \mathbb{P}(T_{1,\ldots, w-1}=T) }{\mathbb{P}(Y_i=s') } \ .
\]
Also from Lemma~\ref{lem:indep}, $\mathbb{P}(Y_i=s)  = \mathbb{P}(Y_i=s')$ thus 
\[
\mathbb{P} (Y_i=s  | T_{1,\ldots, w-1}=T) 
\le \mathbb{P} (Y_i=s'| T_{1,\ldots, w-1}=T)  \ .
\]
Now, for any pair of slots $s',s''$ in  windows $w, w+1, \cdots, W$, by applying Bayes' rule to the equation \eqref{eq:afterw},
we have $p_{is'}=\mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) =\mathbb{P} (Y_i=s''  | T_{1,\ldots, w-1}=T)=p_{is''}$.
That is, $i$ has as much probability to appear in $s'$ or $s''$ as any of the other (at most $k\beta$) slots in windows $w, w+1, \ldots, W$. 
As a result $p_{is''}=p_{is'} \ge \frac{1}{k\beta}$.
\end{proof}
}

\begin{lemma}
\label{lem:ijindep}
For any window $w$,  $i,j\in S^*, i\ne j$ and $s,s'\in w$, the random variables $\mathbf{1}(Y_i=s|T_{1,\cdots, w-1}=T)$ and $ \mathbf{1}(Y_j=s'|T_{1,\cdots, w-1}=T)$ are independent. That is, given $T_{1,\cdots, w-1}=T$,  items $i,j\in S^*, i\ne j$ appear in any slot $s$ in $w$ independently.
\end{lemma}
\toRemove{
\begin{proof}
To prove this, we show that $\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T)=\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T \text{ and } Y_j =s')$. Suppose $Y'$ is a configuration such that $Y'_i=s$ and $Y'_j=s'$, and $T_{1,\cdots, w-1}(Y')=T$. Assume there exists another feasible slot assignment of $j$, i.e., there is another configuration $Y''$ such that $T_{1,\cdots, w-1} (Y'') =T$ and $Y''_j=s''$ where $s''\ne s'$. (If no such configuration $Y''$ exists, then $\mathbf{1}(Y_j=s')|T$ is always $1$, and the desired lemma statement is trivially true.) Then, we prove the desired independence by showing that there exists a feasible configuration where slot assignment of $i$ is $s$, and $j$ is $s''$. This is obtained by changing $Y_j$ from $s'$ to $s''$ in $Y'$, to obtain another configuration $\bar{Y}$. In Lemma~\ref{addtoslot}, we show that this change will not effect $T_{1,\cdots, w-1}$, i.e., $T_{1,\cdots, w-1} (\bar Y)=T $. 
Thus configuration $\bar Y$ satisfies the desired statement.
\end{proof}
}

%\mcomment{why did you remove the following lemma? added back}\scomment{yes, we need it. }
\begin{lemma} \label{addtoslot}
Fix a slot $s'$, $T$, and $j\notin Supp(T)$. Suppose that there exists  some configuration  $Y'$ such that $T_{1,\cdots, w-1} (Y') =T$ and $Y_j'=s'$. Then, given any configuration $Y''$ with $T_{1,\ldots, w-1}(Y'')=T$, we can replace  $Y''_j$ with $s'$ to obtain a new configuration $\bar Y$ that also satisfies $T_{1,\ldots, w-1}(\bar Y)=T$.
\toRemove{
Suppose there exists at least one configuration $\bar{Y}$ such that   $T_{1,\cdots, w-1} (\bar{Y}) =T$ and $\bar{Y}_j=s$ for $j\notin Supp(T)$.
Then for any configuration $Y$ with  $T_{1,\cdots, w-1} (Y) =T$, by setting $Y_j=s$, we get a new configuration $Y'$
such that $T_{1,\cdots, w-1} (Y') =T$.}
\end{lemma}
\toRemove{
\begin{proof}
%Suppose $Y$ is a configuration such that $T_{1,\cdots, w-1} (Y) =T$. 
Suppose the slot $s'$ lies in window $w'$.
If $w' \ge w$ then the statement is trivial. So suppose $w' < w$.
Create an intermediate configuration by {\it removing} the item $j$ from $Y''$, call it $Y^-$. Since $j\notin Supp(T_{1,\cdots, w-1}(Y'')) = Supp(T)$ we have $T_{1,\cdots, w-1} (Y^-) =T$. In fact, for every subsequence $\tau$, the greedy subsequence for $Y''$, will be same as that for $Y^-$, i.e.,   $\gamma_{Y''}(\tau) = \gamma_{Y^-}(\tau)$.
Now add item $j$ to slot $s'$ in $Y^-$, to obtain configuration $\bar Y$. We claim $T_{1,\cdots, w-1} (\bar Y) =T$.
%We only need to show that $j$ will not get selected in slot $s$ in configuration $Y'$.
%Suppose not, then there is a subsequence $\tau$  in the algorithm ending in slot $s$ such that $\gamma_{Y'} (\tau) =\{i_1, \cdots, i_{t-1}, j\}$


By construction of $T_{1,\ldots, w}$, we only need to show that $j$ will not be part of the greedy subsequence $\gamma_{\bar Y}(\tau)$ for any subsequence $\tau, |\tau| = \alpha$ containing the slot $s'$ when the input is in configuration $\bar Y$. To prove by contradiction, suppose that $j$ is part of greedy subsequence for some $\tau$ ending in the slot $s'$. \toRemove{We only need to show that $j$ will not get selected in slot $s$ in configuration $Y'$.
Suppose $j$ gets selected in slot $s$ for some subsequence $\tau$ ending in slot $s$.}
%Thus $\gamma_{Y'}(\tau) = \{i_1, \cdots, i_{t-1}, j\}$. Note that since slots before $s$ are the same as $Y^-$ and $T_{1,\cdots, w-1} (Y^-) =T$, $\gamma_{Y^-}(\tau) = \{i_1, \cdots, i_{t-1}, i_t\}$.
\toRemove{Suppose that $\gamma_{Y^-}(\tau)  := \{i_1, \cdots, i_{t-1}, i_t\} = \gamma_{Y''}(\tau) $.} 
For this $\tau$, let $\gamma_{Y^-}(\tau)  := \{i_1, \cdots, i_{\alpha-1}, i_\alpha\} = \gamma_{Y''}(\tau) $. Note that since the items in the  slots  before $s'$ are identical for $\bar Y$ and $Y^-$, \toRemove{and $T_{1,\cdots, w-1} (Y^-) =T$,} we must have that $\gamma_{\bar Y}(\tau) = \{i_1, \cdots, i_{\alpha-1}, j\}$, i.e.,
$\Delta_f(j | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{\alpha-1}\} ) \ge \Delta_f(i_\alpha | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{\alpha-1}\} ) $.
%$j=\arg \max_{i\in j\cup U_s \cup T_{1, \ldots, w-1}} \Delta_f(i | S_{1,\ldots,w-1} \cup \{i_1,\ldots, i_{t-1}\} \cup \{i\}) $
%$i_t=\arg \max_{i\in U_s \cup T_{1, \ldots, w-1}} \Delta_f(i | S_{1,\ldots,w-1} \cup \{i_1,\ldots, i_{t-1}\} \cup \{i\}) $
On the other hand, since $T_{1,\cdots, w'-1} (Y') = T_{1, \cdots, w'-1}(Y'') = T (\text{restricted to $w'-1$ windows})$,  we have that $\gamma_{Y'} (\tau) =\{i_1, \cdots, i_\alpha\}$.
However, $Y'_j=s'$. Therefore $j$ was not part of the greedy subsequence $\gamma_{Y'}(\tau)$ even though it was in the last slot in $\tau$, implying $\Delta_f(j | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{t-1}\} ) < \Delta_f(i_t | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{t-1}\} ) $. This  contradicts the earlier observation.
\end{proof}
}


==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/sizeBound.tex <==
Given the algorithm description, it is not very difficult to show that %\scomment{in expectation or with high probability?} \mcomment{Neither. It is exact. the max alg should terminate after selecting $O(\log(1/\delta))$ elements. the gaurantee is w.h.p.} 
our algorithm uses a shortlist of size at most $O(k)$ if $\alpha, \beta$ are constants. 
The number of items selected by Algorithm \ref{alg:SIIImax} is at most $L$.
By choosing appropriate size $L$ for shortlist $A$,
%$L=\ln (1/\epsilon)+\ln(1/\delta)+\sqrt{\ln^2{1/\delta}+2m\ln(1/\delta)\ln(1/\epsilon)}$ 
w.h.p. we can gaurantee  that $A$ contains the maximum element $M$.
%A key observation here is that the expected number of items selected by Algorithm \ref{alg:SIIImax} 
%\ref{alg:tmp} 
%\mcomment{1?} 
%is bounded by $\log(1/\delta)$. 
\scomment{Change $\epsilon,\delta$ to get max with probability $1-\epsilon$.}
%\begin{theorem}
%\label{maxanalysis}
%Algorithm~\ref{alg:SIIImax}, with parameter $u=n\epsilon$,  
%and shortlist of size $L= \ln(1/\epsilon)+\ln(1/\delta)+\sqrt{\ln^2{1/\delta}+2\ln(1/\delta)\ln(1/\epsilon)}$
%selects the maximum element with 
%probability $(1-\epsilon-\delta)$, \end{theorem}



%This result can be further extended to high probability bounds using standard techniques:

%\scomment{add appropriate lemma about Algorithm 1.}
Now, we can deduce the desired bound on the size of shortlist returned by Algorithm \ref{alg:tmp}
\begin{prop}
The size of shortlist $A$ selected by Algorithm~\ref{alg:tmp} is $O(k)$.
%\scomment{proposition about size of shortlist returned by Algorithm \ref{alg:tmp}.}
\end{prop}
\begin{proof}
Note that for each window $w=1,\ldots, k/\alpha$, and for each of the $\alpha\beta$ slots in this window, the subroutine in Algorithm \ref{alg:tmpWindow} runs  Algorithm \ref{alg:SIIImax} for ${\alpha \beta \choose \alpha}$ times (for all $\alpha$ length subsequences) to add at most $\log(1/\delta)$ items each time to . Therefore, the above algorithm selects $ k \beta {\alpha \beta \choose \alpha} = O(k)$ items as part of the shortlist.
\end{proof}



==> Submodular Matroid Secretary Problem with Shortlists (arxiv)citation/streaming.tex <==
%\label{sec:streaming}
%\ccomment{Put here a short section explaining on how extend the algorithm to work for streaming.}
In this section, we show that Algorithm \ref{alg:main} can be implemented in a way that it uses a memory buffer of size at most $\eta(k)=O(k)$; also we compute the number of objective function evaluations for each arriving item as follows. % is $O(1+\frac{k^2}{n})$. %This will allow us to obtain  Theorem \ref{thm:streaming} (restated below) as a corollary of Theorem \ref{opttheorem}.
%\thmStreaming*



\thmStreamingMatroid

Similarly for $p$-matchoid constraint we have the following result for the streaming setting:

%\thmStreamingMatroid
\thmStreamingMatchoid
\begin{proof}
Th difference between Algorithm~\ref{alg:main} in this paper and the main Algorithm  in~\cite{us} is that, we remove elements of $\bar{S}_w$  from $S$ at the end of each window $w$. Therefore, with the same argument in the proof of Theorem 2 in~\cite{us}, we keep track of all parameters in Algorithm~\ref{alg:main} including $\bar{S}_w, S_w, R_w, \hat{S}_w$ in a memory efficient way using memory $O(k)$. 
The other difference between the two algorithms is in the subroutine~\ref{alg:matroidmax} that finds the element with maximum $g$ in a slot. 
In~\cite{us}, $g(e,S)$ can be computed using only one oracle access, whereas in the new definition of $g$ in equation~\ref{eq:newg}, we need access to independence oracle of $p$ matroids that $e$ belongs to, in order to check the independence of $S+e-e'$ for each $e' \in S$. At most $p \kappa$ elements of $S$ are eligible (they are in the ground set of a matroid that $e$ also member of). Hence, 
in order to create $\Omega_{\ell}(e,S)$, 
 for each arriving element $e$ in the input, we need $O(p\kappa)$ access to Independence oracle. Similarly the total access to the value oracle is $O(p\kappa)$. 
 In order to compute 
$\lambda(e,S)$, we need to consider all $\kappa^p$ combinations and have access to value oracle. Therefore the  number of access to the value oracle is $O(p\kappa+\kappa^p)$ per element. 
But, since the first element $a_0$ is computed in the beginning of each slot
for each $\tau$, we would have in average an additional $O(k^2/n)$ function evaluation per element.
\end{proof}

\toRemove{
\subsection{Max-Coverage}
One important monotone submodular function is max-coverage. 
\begin{definition} (max-coverage)
\end{definition}


Oracle access 

memory required to store each set.
}

 In the next section, we empirically compare our streaming algorithms with the state of the art algorithms in the streaming setting.
\toRemove{
In the current description of Algorithm \ref{alg:main}, there are several steps in which the algorithm potentially needs to store $O(n)$ previously seen items in order to compute the relevant quantities. 
%We discuss how to modify those steps to obtain an equivalent implementation but with memory buffer requirement of only $O(k)$. 
First, in Step \ref{li:subb}, in order to be able to compute $\gamma(\tau)$ for all less than $\alpha$ length subsequences $\tau$ of slots $s_1, \ldots, s_{j-1}$, the algorithm should have stored all the items that arrived in the slots $s_1, \ldots, s_{j-1}$. However, this memory requirement can be reduced by a small modification of the algorithm, so that at the end of iteration $j-1$, the algorithm has already computed  $\gamma(\tau)$ for all such $\tau$, and stored them to be used in iteration $j$. In fact, this can be implemented in a memory efficient manner, in the following way. For every subsequence $\tau$ of slots $s_1, \ldots, s_{j-1}$ of length $<\alpha$, consider prefix $\tau'=\tau\backslash s_{j-1}$. Assume $\gamma(\tau')$ is available from iteration $j-2$. 
If $\tau'=\tau$, then $\gamma(\tau)=\gamma(\tau')$. Otherwise, in Step 6 of iteration $j-1$, the algorithm must have considered the subsequence $\tau'$ while going through all subsequences of length less than $\alpha$ of slots $s_1, \ldots, s_{j-2}$. Now, modify the implementation of Step 6 so that  the algorithm also tracks the (true) maximum $M_{j-1}(\tau')$ of $a_0, a_1, \ldots, a_N$ for each $\tau'$. Then, $\gamma(\tau)$ can be obtained by extending $\gamma(\tau')$ by $M_{j-1}(\tau')$, i.e.,  $\gamma(\tau)=\{\gamma(\tau'), M_{j-1}(\tau')\}$. Thus, at the end of iteration $j-1$, $\gamma(\tau)$ would have been computed for all subsequences $\tau$ relevant for iteration $j$, and so on. In order to store these $\gamma(\tau)$ for every subsequence $\tau$ (of  at most $\alpha$ slots from $\alpha \beta$ slots), we require a memory buffer of size at most $\alpha^2{\alpha \beta \choose \alpha} = O(1)$.  

%In order to implement steps 6--9 for window $w$, and for every slot $s_j$, the algorithm needs a buffer to store $\tau, \gamma(\tau)$ for every subsequence  $\tau$ of length at most $\alpha$, of the $j-1$ slots in window $w$. This requires a memory buffer of size at most $\alpha \beta \times 2\alpha{\alpha \beta \choose \alpha}$. 
Secondly, across windows and slots, the algorithm keeps track of $R_w, S_w, w=1,\ldots, k/\alpha$ where $W=k/\alpha$. In the current description of Algorithm \ref{alg:main}, these sets are computed after seeing all the items in window $w$ in Step~\ref{li:Rw}. Thus, all the items arriving in that window would be needed to be stored in order to compute them, requiring $O(n)$ memory buffer. However, the alternate implementation discussed in the previous paragraph reduces this memory requirement to $O(k)$ as well. Using the above implementation, at the end of iteration $\alpha \beta$ for the last slot $s_{\alpha\beta}$ in window $w$, we would have computed and stored $\gamma(\tau)$ for all the subsequences  $\tau$ of length $\alpha$ of slots $s_1,\ldots, s_{\alpha\beta}$. 
$R_w$ is simply defined as union of all items in  $\gamma(\tau)$ over all such $\tau$ (refer to \eqref{eq:Rw}). And, $S_w = \gamma(\tau^*)$  for the best subsequence $\tau^*$ among these subsequences (refer to \eqref{eq:Sw}). 
Thus, computing $R_w$ and $S_w$ does not require any additional memory buffer. Storing $R_w$ and $S_w$ for all windows requires a buffer of size at most $\sum_w |R_w| + |S_w| = \frac{k}{\alpha} \times \alpha {\alpha \beta \choose \alpha}+ k = O(k).$
%Thus the subsequences considered in   to either add slot $s_j$. , by using the observation  that $R_w$ (as defined in \eqref{eq:Rw}) can be formed simply by adding all the union of all items in $A_j(\tau)$ The union of items these subsequences form $R_w$. Further, it needs to store $S_w$ for each window, which is of size $\alpha$. 
Therefore, the total buffer required to implement Algorithm \ref{alg:main} is of size $ O(k)$. 

%Finally, let's bound the number of objective function evaluations for each arriving item. Each arriving item is processed in Step 6, where objective function is evaluated twice for each $\tau$ to compute the corresponding $a_i$. Since there are atmost ${\alpha \beta \choose \alpha}$ subsequences $\tau$ for which this quantity is computed, the total number of objective function evaluations is  bounded by $2 {\alpha \beta \choose \alpha}=O(1)$. 
%This concludes the proof of Theorem \ref{thm:streaming}.

Finally, let's bound the number of objective function evaluations for each arriving item. Each arriving item is processed in Step 6, where objective function is evaluated twice for each $\tau$ to compute the corresponding $a_i$. Since there are atmost ${\alpha \beta \choose \alpha}$ subsequences $\tau$ for which this quantity is computed, the total number of times 
%the %Algorithm~\ref{alg:SIIImax} is called is 
%objective function evaluations is  
this computation is performed is bounded by $2 {\alpha \beta \choose \alpha}=O(1)$. However, for each $\tau$, we also compute $a_0$ in the beginning of the slot. Computing $a_0$ for each $\tau$ involves taking max over all items in $R_{1,\ldots, w-1}$, and requires $2|R_{1,\ldots,w-1}|\le 2k {\alpha \beta \choose \alpha}$ evaluations of the objective function. Due to this computation, in the worst-case, the update time for an item can be $ 2k {\alpha \beta \choose \alpha}^2 + 2 {\alpha \beta \choose \alpha}= O(k)$. However, since $a_0$ is computed {\it once} in the beginning of the slot for each $\tau$, the  total update time over all items is bounded by $2k {\alpha \beta \choose \alpha}^2 \times k\beta + {\alpha \beta \choose \alpha} \times n = O(k^2+n)$. Therefore the amortized update time for each item is $O(1+\frac{k^2}{n})$.
\scomment{replaced by above:Also each subroutine call on a slot $s_j$ goes over all elements in $s_j$ and also $R_{1,\cdots, w-1}$ to find the maximum element. 
%In the current format of the algorithm  
%The update time can be made to be at most $\frac{O(k^2)}{n}$ in this way. 
When we pass elements of $s_j\cup R_{1,\cdots, w-1}$ to the online subroutine~\ref{alg:SIIImax} one by one, for each element $e\in  s_j$ we can also pass $\frac{|R_{1,\cdots, w-1}|}{|s_j|}$ elements from $R_{1,\cdots, w-1}$. %Therefore, the expected update time for each element in $s_j$ would be  $\frac{O(k^2)}{n}$.
Therefore the amortized update time
would be $O(1+\frac{k^2}{n})$.
%in the beginning of each slot when we pass
Also note that the worst case update time can be $O(k)$.}
This concludes the proof of Theorem \ref{thm:streaming}.

Similarly for the $p$-matchoid constraints we have

%To conclude,  the following is obtained as a corollary of Theorem \ref{alg:main}.

%\noindent {\bf Theorem 2 (restated)}
%{\em For any constant $\epsilon>0$, there exists an algorithm for the \nameStreaming that uses a memory of size at most $\eta_\epsilon(k)=O(k)$, and achieves $1-\frac{1}{e} -\epsilon -O(\frac{1}{k})$ approximation to $\OPT$.
%Also it processes each arriving item with $O(1)$ evaluations
%of the objective function.}
}

%\subsection{Max-Coverage}




\subsection{Experiment}
In this section, we consider different types of constraints including uniform matroid, intersection of partition matroids and $p$-matchoid constraints. We compare our algorithm with state of the art algorithm for each type of constraint using YouTube dataset and Twitter dataset described in the next section.


\subsubsection{DataSets}
The experiments will be on a Twitter stream summarization task and a YouTube Video
summarization task similar to the one in Kazemi et al.~\cite{kazemi2019submodular}.


\paragraph{\textbf{Twitter Stream Summarization}} In this application, we want to produce real-time summaries
for Twitter feeds. 
%Whether we want to provide a periodic synopsis of major
%events or simply to reduce the clutter in a user’s feed, 
%it would be very valuable if we could
It is valuable to create
a succinct summary that contains all the important information.
We use the dataset created by~\cite{kazemi2019submodular}.
They gather recent tweets from 30 different popular news accounts, to collect
a total of 42,104 unique tweets. 
They also define a monotone submodular function $f$ 
that measure the redundancy of important stories in a set $S$.
%that covers the important stories of the day without redundancy. 
It is defined as follows on a set $S\subseteq V$ of tweets:
$$
f(S):=\sum_{w\in W} \sqrt{\sum_{e \in S} score(w,e)}
$$

function f defined over a ground set $V$ of tweets. Each tweet $e\in V$ consists of a positive value
vale denoting its number of retweets and a set of $\ell_e$ keywords $W_e = \{w_{e,1}, \cdots, w_{e,\ell_e}\}$
from a general
set of keywords $W$. The score of a word $w\in W_e$ for a tweet $e$ is defined by $score(w, e) = vale_e$. If
$w\notin W_e$. Define $score(w, e) = 0$.


\paragraph{\textbf{YouTube Video Summarization}}
For the YouTube dataset, we want to select a subset of frames from video feeds which are representative of the entire video.
We use the same dataset as in~\cite{kazemi2019submodular}, which is YouTube videos of
New Year’s Eve celebrations from ten different cities around the world.

%Using the first 30 seconds of each video, they train an autoencoder that 
They compresses each frame into
a 4-dimensional representative vector. Given a ground set $V$ of such vectors,  define a matrix $M$
such that $M_{ij}=e-dist(v_i,v_j)$
, where $dist(v_i, v_j )$ is the euclidean distance between vectors 
$v_i, v_j \in V$.
Intuitively, $M_{ij}$ encodes the similarity between the frames represented by $v_i$ and $v_j$. 
They define a function  that intuitively measure the diversity of the
vectors in a set $S$ as follows: $f(S) =
\log det(I + \alpha M_S)$, where $I$ is the identity matrix, $\alpha > 0$ and $M_S$ is the principal sub-matrix of $M$
indexed by $S$. 

%The utility of a set $S\subseteq V$ is defined as a non-negative monotone submodular objective $f(S) =
%\log det(I + \alpha M_S)$, where $I$ is the identity matrix, $\alpha > 0$ and $M_S$ is the principal sub-matrix of $M$ indexed by $S$. 

\subsubsection{\textbf{Uniform Matroid}}
The simplest constraint that we can impose is the uniform matroid or equivalently the cardinality constraint.
In the simplest form our algorithm is similar to~\cite{us}.
We compare our algorithm to the state of the art algorithm in the streaming setting~\cite{kazemi2019submodular}.
As we established
an upper bound on the constant factor $\eta_{\epsilon}(k)$ in theorem~\ref{opttheoremmatchoid}, the performance of our algorithm crucially depends on the choice of 
$\alpha$ and $\beta$. The running time also is a function of $\alpha$ and $\beta$, and it grows rapidly as we increase $\alpha$ and $\beta$. 
Surprisingly, our algorithm outperforms~\cite{kazemi2019submodular}
substantially even with relatively small choices of $\alpha=6$ and $\beta=2$.
We also observe that the utility of the output returned by our algorithm can be very  close to  what the optimal offline algorithm, namely the Greedy algorithm achieves. In Figure~\ref{fig:uniform}, we have plotted the performance of all three algorithms on the YouTube dataset.
Note that in our experiment we use a simplistic version of our algorithm in which we subsample from the shortlist in beginning of each window and only use that subsample rather than the entire shortlist. Furthermore we observe that our algorithm is slower than~\cite{kazemi2019submodular}, but the interesting fact about our algorithm as stated in Theorem~\ref{opttheoremmatchoid} is that it is highly parallel thus it has the potential to become $\eta_{\epsilon}(k)$  times faster.
%using parallelization. %(here roughly 1000 times).  
\begin{figure}[ht!]
\centering
\includegraphics[width=120mm]{correctFig.png}
\caption{The plot is for unifrom matroid, $\alpha =6$ and $\beta=2$}
\label{fig:uniform}
\end{figure}



%\subsubsection{$p$-matchoid constraints}
%\subsubsection{Intersection of Two Matroids}
\subsubsection{\textbf{$p$-matchoid constraints}}
For the case of $p$-matchoid constraints, state of the art algorithm for general streaming setting is due to Feldman et al.~\cite{feldman2018streaming}.
In our experiment, we divide the elements of input into $q$ categories $\mathcal{N}= \mathcal{N}_1 \cup \cdots, \cup  \mathcal{N}_q$. 
We assign $p$ tags to each element $e$.
Each tag belongs to one of the catergories $1,\cdots, q$ (generated randomly). 
Further, we impose a cardinality constraint $3$ for each category (i.e, $\mathcal{I}_{\ell} $ is a cardinality constraint).
The objective is to select at most $3$ elements from each category. In other words, an independent set of $p$-matchoid is defined as 
$$\mathcal{I}=\{S\subseteq \mathcal{N}: |S\cap \mathcal{N}_i|\le 3, \forall i\in [q] \}$$
In our algorithm, we  set $\alpha=3$ and $\beta=2$. We have plotted the performance of our algorithms and~\cite{feldman2018streaming} on the Twitter dataset below.
The first plot, Figure~\ref{fig:p3}, is for fixed $p=3$ and different number of categories $q$.
The second plot, Figure~\ref{fig:pmatchoid}, is for fixed number of categories $q=30$ and different values of $p$ from $1,\cdots, 10$. As the competitive ratio of our algorithm suggests, by  increasing $p$ the ratio of our utility versus the utility of~\cite{feldman2018streaming} increases.

%In order to create partitions we assign a label to each tweet, which represent the category it belongs to (generated randomly). We consider a $3$-matchoid constraint that is the intersection of a partition matroid with rank $k$.
%The goal is to choose at most 3 items from each partition.  We  set $\alpha=3$ and $\beta=2$. 
%We have plotted the performance of our algorithms and~\cite{feldman2018streaming} on the Twitter dataset below.


\begin{figure}[ht!]
\centering
%\includegraphics[width=100mm]{matroid.png}
\includegraphics[width=120mm]{tw3uni.png}
\caption{ The plot is for 3-matchoid constraint, and $\alpha =3$, $\beta=2$}
\label{fig:p3}
\end{figure}






\begin{figure}[ht!]
\centering
\includegraphics[width=120mm]{pmatchoidmany.png}
\caption{ The plot is for $p$-matchoid constraint, for $p=1,\cdots, 10$, and $\alpha =3$, $\beta=2$ and fixed $k=30$.}
\label{fig:pmatchoid}
\end{figure}

==> algorithms1.tex <==
%\section{Algorithms}
%\subsection{Simpler but unimplementable, offline version}
%\subsection{Algorithm description}

Before giving our algorithm for \nameOfProblemSL, we describe a simple technique for \nameSecSL~
that achieves a  $1-\delta$ competitive ratio for  with shortlists of size logarithmic in $1/\delta$.
Recall that in the \nameSec, the aim is to select an item with expected value close to the maximum among a pool of items $I=(a_1, \ldots, a_N)$ arriving sequentially in a uniformly random order. 
We will consider the variant with shortlists, where we now want to pick a shortlist which contains an item with expected value close to the maximum.
%\ccomment{why are we using $\epsilon$ in the text and $\delta$ in the Algorithm below}\scomment{fixed}
We propose the following simple algorithm. For the first $n\delta/2$ rounds, don't add any items to the shortlist, but just keep track of the maximum value seen so far.
For all subsequent rounds, 
for any arriving item $i$ that has a value $a_i$ greater than or equal to the maximum value seen so far, add it to the shortlist if the size of shortlist is less than or equal to $L=4\ln(2/\delta)$. This algorithm is summarized as Algorithm \ref{alg:SIIImax}. Clearly, for contant $\delta$, this algorithm uses a shortlist of size $L=O(1)$. Further, under a uniform random ordering of input, we can show that the maximum value item will be part of the shortlist with probability $1-\delta$. (See Proposition \ref{maxanalysis} in Section \ref{sec:analysis}.)
%that the expected number of items in the shortlist $A$ is at most $\log(1/\epsilon)$, i.e., $O(1)$, and the maximum value item will be part of the shortlist with probability $1-\epsilon$. %analysis is presented in Section \ref{sec:max}. 
%--------------------------------------
\begin{algorithm*}[ht]
  %\caption{~\bf{Select-If-it-Improves}($I , u$)}
  \caption{~\bf{Algorithm for secretary with shortlist} (finding max online)}
  \label{alg:SIIImax} 
\begin{algorithmic}[1]
\State Inputs: number of items $N$, items in $I=\{a_1, \ldots, a_N\}$ arriving sequentially, $\delta \in (0,1]$. 
\State Initialize: $A\leftarrow \emptyset$,  $u=n\delta/2$, $M = -\infty$ %$M\leftarrow \max\{a_1, \cdots, a_{u-1}\}$
%\scomment{Should initialization of $u$ be changed to $n\delta/2$?}
%\mcomment{yes}
\State $L \leftarrow 4\ln(2/\delta)$ %\scomment{I changed (3+$\sqrt{2}$) to $4$}

\For {$i= 1$ to $N$}
%\If {$F(S\cup \{a_i\}) > F(S) $}
\If {$ a_i > M$}
\State $M \leftarrow  a_i$
\If {$i \geq u$ and $|A|<L$}
\State $A\leftarrow A\cup \{a_i\}$
\EndIf
\EndIf
\EndFor
%\State return $S\setminus \{a_1,\cdots, a_u\}$

%\mcomment{
%cleaner:
%\For {$i= u$ to $N$}
%\If {$ a_i > \max_{1\le j <i} a_j$ and $|A|<L$}
%\State $A\leftarrow A\cup \{a_i\}$
%\EndIf
%\EndFor
%}

\State return $A$, and $A^*:= \max_{i\in A} a_i$
\end{algorithmic}
\end{algorithm*}
%--------------------------------------------

%-----------------------------------------
\begin{algorithm*}[h!]
  %\caption{~\bf{Select-If-it-Improves}($I , u$)}
  \caption{~\bf{Algorithm for {\bf submodular} $k$-secretary with shortlist}}
  \label{alg:main} 
  \label{alg:tmp} 
\begin{algorithmic}[1]
\State Inputs: set $\bar I=\{\bar{a}_1,\ldots, \bar{a}_n\}$ of $n$ items arriving sequentially, submodular function $f$, parameter $\epsilon \in (0,1]$. 
\State Initialize: $S_0 \leftarrow \emptyset, R_0 \leftarrow \emptyset, A \leftarrow \emptyset, A^* \leftarrow \emptyset$, constants $\alpha \ge 1, \beta \ge 1$ which depend on the constant $\epsilon$.
\State Divide indices $\{1,\ldots, n\}$ into $(\alpha, \beta)$ windows as prescribed by Definition \ref{def:windows}.
%Divide the sequence of candidates into consecutive groups of $\frac{n}{\beta k}$ candidates, referred to as slots (or buckets). And, divide the sequence of slots into consecutive groups of $\alpha \beta$ slots, referred to as {\it windows}.
%===========================
\For {window $w= 1, \ldots, k/\alpha$} 
%\State For every $\alpha$-length subsequence $\tau=(s_1,\ldots, s_\alpha) \subseteq [\alpha\beta]$ of slots in window $w$, define 
%$$\gamma(\tau):=\{i_1, \ldots, i_\alpha\}$$
%where 
%$$i_j := \arg \max_{i\in V_{s_j,w} \cup R_{1,\ldots, w-1}} f(S_{1,\ldots,w-1} \cup \{i_1\ldots, i_{j-1}\} \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \{i_1\ldots, i_{j-1}\})$$
%\State Define $R_w:=\{\cup_{\tau} \gamma(\tau)\}.$ 
 

%\State Process the online inputs in window $w$ using the subroutine in Algorithm \ref{alg:tmpWindow} to select a subset $H_w$ of items. 
 \For {every slot $s_j$ in window $w$, $j=1,\ldots, \alpha\beta$}
  \State Concurrently for all subsequences of previous slots $\tau\subseteq \{s_1, \ldots, s_{j-1}\}$ of length $|\tau|<\alpha$ \label{li:subb}   \hspace{0.44in} in window $w$, call the online algorithm in Algorithm \ref{alg:SIIImax} with the following inputs: 
  %\begin{center}
  \begin{itemize}[leftmargin=0.7in]
  \item   number of items $N=|s_j|+1$, $\delta=\frac{\epsilon}{2}$, and
%  \scomment{You have to use $\delta$ smaller than $\epsilon$ to get $1-\frac{1}{e}-\epsilon$ in the final result.}
  \item item values $I=(a_0, a_1, \ldots, a_{N-1})$, with 
     \begin{eqnarray*} 
  a_0 & := & \max_{x\in R_{1,\ldots, w-1}} \Delta(x|S_{1,\ldots,w-1} \cup \gamma(\tau)) \\
  %\max_{x\in R_{1,\ldots, w-1}} f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{x\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\}$
     a_\ell & := & \Delta(s_j(\ell)| S_{1,\ldots,w-1} \cup \gamma(\tau) ),  \forall \ell=1,\ldots, N-1
     \end{eqnarray*}
    %f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\})$
 where $s_j(\ell)$ denotes the $\ell^{th}$ item in the slot $s_j$. 
% \item $\delta = \frac{\epsilon}{{\alpha \beta \choose \alpha}}$.
  \end{itemize}
   %\end{center}
   %\mcomment{why do you divide by... the erros do not add up}  \scomment{Please add the required theorem showing this}  \mcomment{added lemma~\ref{online}}
\State Let $A_{j}(\tau)$ be the shortlist returned by  Algorithm \ref{alg:SIIImax} for slot $j$ and subsequence $\tau$. Add 
\label{li:tmp} \hspace{0.44in} all items except the dummy item $0$ to the shortlist $A$. Let's $A(j)=\bigcup_{\tau} A_j(\tau)$.
%for all $\tau$,
%  $$A(j) \leftarrow A(j)\cup (A_{j}(\tau))$$
%$H_w$, i.e, for all $\tau$,
 % $$H_w \leftarrow H_w\cup (A_{j}(\tau) \cap s_j)$$
 That is, \label{li:sube}
 $$A\leftarrow A\cup  (A(j)\cap s_j)$$
 \EndFor
%\State return $H_w$
% \State $A\leftarrow A\cup H_w$
 \State \label{li:Rw} After seeing all items in window $w$, compute $R_w, S_w$ as defined in \eqref{eq:Rw} and \eqref{eq:Sw} respectively.
 \State $A^* \leftarrow A^*\cup (S_w \cap A)$
\EndFor
\State return $A$, $A^*$. %$A=T_1 \cup \cdots  \cup T_{W}$
\end{algorithmic}
\end{algorithm*}

%==========================


%\begin{algorithm*}[ht]
  %\caption{~\bf{Subroutine of Algorithm \ref{alg:tmp} for window $w$}}
  %\label{alg:tmpWindow} 
  \toRemove{
  \begin{algorithmic}[1]
  \For {every slot $s_j$ in window $w$, $j=1,\ldots, \alpha\beta$}
  \State Concurrently for all subsequences of previous slots $\tau\subseteq \{s_1, \ldots, s_{j-1}\}$ in window $w$, of length $|\tau|<\alpha$, call the online algorithm in Algorithm \ref{alg:SIIImax} with the following inputs: number of items $N=|s_j|+1$, $\delta = \frac{\epsilon}{{\alpha \beta \choose \alpha}}$, \mcomment{why do you divide by... the errors do not add up} and values of arriving items $(a_0, a_1, \ldots, a_{N-1})$ defined as 
  $$a_0:=\max_{x\in R_{1,\ldots, w-1}} f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{x\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\}$$
    $$a_i :=f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\})$$
 where $i$ denotes the $i^{th}$ item in slot $s_j$.
  \State Let $A_{j}(\tau)$ be the shortlist returned by  Algorithm \ref{alg:SIIImax} for slot $j$ and subsequence $\tau$. Add all items except the dummy item $0$ to $H_w$, i.e, for all $\tau$,
  $$H_w \leftarrow H_w\cup (A_{j}(\tau) \cap s_j)$$
 \EndFor
\State return $H_w$
\end{algorithmic}
}
%\end{algorithm*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
There are two main difficulties in extending this idea to the \nameOfProblemSL. First, instead of one item, here we aim to select a set $S$ of $k$ items using an $O(k)$ length shortlist. Second, the contribution of each new item $i$ to the objective value, as given by the submodular function $f$, depends on the set of items selected so far. 

The first main concept we introduce to handle these difficulties  is that of dividing the input into sequential blocks that we refer to as $(\alpha, \beta)$ windows. Below is the precise construction of $(\alpha, \beta)$ windows, for any postivie integers $\alpha$ and $\beta$, such that $k/\alpha$ is an integer.
%\ccomment{This definition is imprecise.  Needs to be made technically crisp.}
%\ccomment{What exactly is this distribution?  Are we drawing with replacement or without and do the $X_i$ sum to $n$?}

We use a set of random variables $X_1,\ldots,X_m$ defined in the following way.  Throw $n$ balls into $m$ bins uniformly at random.  Then set $X_j$ to be the number of balls in the $j$th bin.  We call the resulting $X_j$'s a {\em $(n,m)$-ball-bin random set}.


\begin{definition}[$(\alpha,\beta)$ windows]
\label{def:windows}
Let $X_1,\ldots,X_{k\beta}$ be a $(n,k\beta)$-ball-bin random set.
Divide the indices $\{1,\ldots, n\}$ into $k\beta$ slots, where the $j$-th slot, $s_j$, consists of $X_j$ consecutive indices in the natural way, that is, slot $1$ contains the first $X_1$ indices, slot $2$ contains the next $X_2$, etc.
 %, $X_i$ would be the number of balls in the $i$-th bin.
 Next, we define $k/\alpha$ windows, where window $i$ consists of $\alpha \beta$ consecutive slots, in the same manner as we assigned slots.
\end{definition}
%\ccomment{Would an example or a figure help here to define slots and windows?}
Thus, $q^{th}$ slot is composed of indices $\{\ell, \ldots, r\}$, where $\ell=X_1+...+X_{q-1}+1$ and  $r=X_1+...+X_q$. 
Further, if the ordered the input is $\bar a_1, \dots, \bar a_n$ then we say that the items inside the slot $s_q$ are $\bar a_{\ell}, \bar a_{\ell+1}, \dots, \bar a_{r}$ 
To reduce notation, when clear from context, we will use $s_q$ and $w$ to also indicate the {\it set of items} in the slot $s_q$ and window $w$ respectively.

%The idea is to divide the inputs into $k/\alpha$ blocks (i.e., windows) for a constant $\alpha\ge 1$ such that 
%\ccomment{Shouldn't we say what alpha is because the intuition depends on it}
When $\alpha$ and $\beta$ are large enough constants, some useful properties can be obtained from the construction of these windows and slots. First, roughly $\alpha$ items from the optimal set $S^*$ are likely to lie in each of these windows; and further, it is unlikely that two items from $S^*$ will appear in the same slot. (These statements will be made more precise in the analysis where precise setting of $\alpha,\beta$ in terms of $\epsilon$ will be provided.) Consequently, our algorithm can focus on identifying a constant number (roughly $\alpha$) of optimal items from each of these windows, with at most one item coming from each of the $\alpha \beta$ slots in a window. The core of our algorithm is a subroutine that accomplishes this task in an online manner using a shortlist of constant size in each window. 

To implement this idea, we use a greedy selection method that considers all possible $\alpha$ sized subsequences of the $\alpha\beta$ slots in a window, and aims to identify the subsequence that maximizes the increment over the best items identified so far. 
More precisely, for any subsequence $\tau=(s_1,\ldots, s_\ell)$ of the $\alpha\beta$ slots in window $w$, we define a `greedy' subsequence $\gamma(\tau)$ of items as:
\begin{equation}
\label{eq:gamma}
\gamma(\tau):=\{i_1, \ldots, i_\ell\}
\end{equation}
where
\begin{equation}
\label{eq:ij}
i_j := \arg \max_{i\in s_j \cup R_{1, \ldots, w-1}} f(S_{1, \ldots,w-1} \cup \{i_1,\ldots, i_{j-1}\} \cup \{i\}) - f(S_{1, \ldots, w-1} \cup \{i_1\ldots, i_{j-1}\}).
\end{equation}
In ({\ref{eq:ij}) and in the rest of the paper, we use shorthand $S_{1,\ldots, w}$ to denote $S_1\cup \cdots \cup S_{w}$, and $R_{1,\ldots, w}$ to denote $R_1\cup \cdots \cup R_{w}$, etc.  We also will take unions of subsequences, which we interpret as the union of the elements in the subsequences.
%\ccomment{Are we bothered by taking the union of a sequence rather than a set?}
We also define $R_w$ to be  the union of all greedy subsequences of length $\alpha$, and $S_w$to be  the best subsequence among those. That is,
\begin{equation}
\label{eq:Rw}
R_w = \cup_{\tau: |\tau|=\alpha} \gamma(\tau)
\end{equation}
and 
\begin{equation}
\label{eq:Sw}
S_w=\gamma(\tau^*),
\end{equation} where
\begin{equation}
\label{eq:taustar}
\tau^*:=\arg \max_{\tau: |\tau|=\alpha} f(S_{1,\ldots,w-1} \cup \gamma(\tau)) - f(S_{1,\ldots,w-1}).
\end{equation}
Note that $i_j$ (refer to \eqref{eq:ij}) can be set as  either an item in slot $s_j$ or an item {\it from a previous greedy subsequence} in $R_1\cup \cdots \cup R_{w-1}$. The significance of the latter relaxation will become clear in the analysis.
%Here, $s_j \cup R_1 \cup \cdots \cup R_{w-1}$ denotes the union of items in slot $s_j$ and 

%$S_w$ represents the best subsequence among all the subsequences in $R_w$.
As such, identifying the sets $R_w$ and $S_w$ involves looking forward in a slot $s_j$ to find the best item (according to the given criterion in \eqref{eq:ij}) among all the items in the slot. To obtain an online implementation of this procedure, we use an online subroutine that employs the algorithm (Algorithm \ref{alg:SIIImax}) for the basic secretary problem described earlier. This online procedure will result in selection of a set $H_w$ potentially larger than $R_w$, while ensuring that each element from $R_w$ is part of $H_w$ with a high probability $1-\delta$ at the cost of adding extra $\log(1/\delta)$ items to the shortlist. Note that $R_w$ and $S_w$ can be computed {\it exactly at the end} of window $w$. 

Algorithm \ref{alg:tmp} summarizes the overall structure of our algorithm. 
%The  following notation is used for brevity. For any collection of sets $V_1, \ldots, V_\ell$, we use $V_{1,\ldots, \ell}$ to denote $V_1 \cup \cdots \cup V_\ell$. 
In the algorithm, for any item $i$ and set $V $, we define $\Delta_f(i|V):=f(V\cup \{i\})- f(V)$.
%The subroutine to compute $H_w$ for window $w$ uses Algorithm \ref{alg:SIImax} for each subsequence $\tau$ and each slot $s_j$ in that subsequence. Consequently, the parameters for Algorithm \ref{alg:SIImax} for slot $j$ are: number of items $X_j$ which is $n/k\beta$ in expectation, $\delta >0$, and value $a_i$ of an item $i\in [X_j]$ is as given by the expression inside maximizer in \eqref{eq:ij}.
%\scomment{I will come back to make this more precise with parameter specifications, after finishing the subroutine description and analysis.}

The algorithm returns both the shortlist $A$ which we show to be  of size $O(k)$ in the following proposition, as well as a set $A^*=\cup_w (S_w \cap A)$ of size at most $k$ to compete with $S^*$. In the next section, we will show that $\Ex[f(A^*)] \ge (1-\frac{1}{e} - \epsilon -O(\frac{1}{k})) f(S^*)$ to provide a bound on the competitive ratio of this algorithm. 

\begin{prop}
\label{prop:size}
Given $k,n$, and any constant $\alpha, \beta$ and $\epsilon$, the size of shortlist $A$ selected by Algorithm~\ref{alg:main} is at most $4k \beta {\alpha \beta \choose \alpha}\log(2/\epsilon) = O(k)$. 
%\scomment{proposition about size of shortlist returned by Algorithm \ref{alg:tmp}.}
\end{prop}
\begin{proof}
For each window $w=1,\ldots, k/\alpha$, and for each of the $\alpha\beta$ slots in this window, lines \ref{li:subb} through \ref{li:sube} in  Algorithm \ref{alg:main} runs  Algorithm \ref{alg:SIIImax} for ${\alpha \beta \choose \alpha}$ times (for all $\alpha$ length subsequences). By construction of  Algorithm \ref{alg:SIIImax}, for each run it will add at most $L\le 4\log(2/\epsilon)$ items each time to the shortlist. 
%\scomment{Here, we need to fix what $ \delta$ is in terms of $\epsilon$. I have waiting for your precise theorem about this.} \mcomment{lemma~\ref{online}}
Therefore, over all windows, Algorithm \ref{alg:main} adds at most $ \frac{k}{\alpha} \times \alpha\beta  {\alpha \beta \choose \alpha} L = O(k)$ items to  the shortlist. 
\end{proof}
%Later, in the proof of Theorem \ref{opttheorem}, we show that we set $\alpha=O(\frac{1}{\epsilon^4}\log(1/\epsilon)), \beta=O(\frac{1}{\epsilon^2})$ to get the desired competitive ratio. This setting of $\alpha, \beta$ results in the specific dependence of function $\eta_\epsilon(k)$ on $\epsilon$, as  stated in Theorem \ref{opttheorem}.
%\scomment{Add some sentences regarding the changes in implementation required for the streaming version.}


%\subsection{Preliminary: Algorithm for finding max online}
%Add details about online Algorithm for picking $\log(1/\delta)$ items from a sequence of $n$ items such that max lies in the picked items with probability $1-\delta$.
%Consider the simple greedy algorithm described in algorithm~\ref{alg:SIIImax}.

%\begin{algorithm*}[ht]
%  \caption{~\bf{Select-If-it-Improves}($I , u$)}
%  \label{alg:SIII} 
%\begin{algorithmic}[1]
%\State $S\leftarrow \emptyset$
%\For {i=0 to n}
%%\If {$\max(S\cup \{a_i\}) > \max(S) $}
%\If {$F(a_i) > \max_{a\in S} F(a) $}
%\State $S\leftarrow S\cup \{a_i\}$
%\EndIf
%\EndFor
%\State return $S\setminus \{a_1,\cdots, a_u\}$
%\end{algorithmic}
%\end{algorithm*}




%\begin{theorem}
%Suppose $S$ is the output of above algorithm on the input $I=\{a_1,\cdots, a_n\}$ then $F(S) = F(I)$
%\end{theorem}
%\begin{proof}

%%Suppose $F(I)=f(T)$,  where $|T|=m$. The above algorithm never miss  any element of $T$.
%%Since $F$ is submodular if the marginal increae

%Suppose $S_i$ is the subset selected at iteration $i$. Since $F$ is submodular, if $F(S_i\cup \{a_i\}) \le F(S_i)$ 
%then $F(S\cup\{a_i\}) \le F(S)$. Therefore every $e\in I\setminus S$ has marginal value 0 with respect to $S$, i.e., $F(S)=F(I)$.
%\end{proof}

%\paragraph{Bounds on size of shortlist maintained by Algorithm \ref{alg:tmp}.}



==> bib.tex <==
@misc{kazemi2019submodular,
    title={Submodular Streaming in All its Glory: Tight Approximation, Minimum Memory and Low Adaptive Complexity},
    author={Ehsan Kazemi and Marko Mitrovic and Morteza Zadimoghaddam and Silvio Lattanzi and Amin Karbasi},
    year={2019},
    eprint={1905.00948},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}
\bibitem{kleinberg} R. Kleinberg, A Multiple-Choice Secretary Algorithm with Applications to Online Auctions
\bibitem{vondrak} V. Feldman, J. Vondrak, Optimal Bounds on Approximation of Submodular and XOS Functions by Juntas
\bibitem{kleh} T. Kesselheim, A. Tönnis, Submodular Secretary Problems: Cardinality, Matching, and Linear Constraints
\bibitem{mirzasoleiman} A. Badanidiyuru, B. Mirzasoleiman, A. Karbasi, A. Krause, Streaming Submodular Maximization: Massive Data Summarization on the Fly
\bibitem{bateni} M. Bateni, M. Hajiaghayi, M, Zadimoghaddam,  Submodular Secretary Problem and Extensions
%\bibitem{distr} B. Mirzasoleiman, A. Karbasi, R. Sarkar, A. Krause, Distributed Submodular Maximization
\bibitem{recent}  T. Hess, S. Sabato, The monotone submodular secretary problem under a cardinality constraint with limited resources
\bibitem{norouzi} Beyond 1/2-Approximation for Submodular Maximization on Massive Data Streams
\bibitem{linear} B. Mirzasoleiman, A. Badanidiyuru, A Karbasi, J. Vondrak, A. Krause, Lazier Than Lazy Greedy
%\bibitem{swm} M. Kapralov, I. Post, J. Vondrak, Online Submodular Maximization: Beating 1/2 Made Simple
\bibitem{vahab} N. Korula, V. Mirrokni, M. Zadimoghaddam, Online Submodular Welfare Maximization Greedy Beats 1/2 in random order



@article{buchbinder2018online,
  title={Online Submodular Maximization: Beating 1/2 Made Simple},
  author={Buchbinder, Niv and Feldman, Moran and Garg, Mohit},
  journal={arXiv preprint arXiv:1807.05529},
  year={2018}
}


==> conclusion.tex <==
In this paper, we defined a relaxation of the submodular secretary problem with cardinality constraint. We allow the algorithm
to select more than $k$ elements, and the algorithm should output a subset of size $k$ among selected items.
We designed an algorithm with asymptotic
competitive ratio $R$ for any $R<1-1/e$. The total number of selections is only $O(k)$ elements. 
It is open  whether we can generalize this result to more general constraints such as matroid constraints.


==> impossible.tex <==
%\section{Impossibility Result}

In this section we provide an upper bound showing the following:

\hardness*

%\begin{theorem}
%There is no algorithm achieving asymptotic competitive ratio $7/8+\epsilon$ for submodular secretary problem using $o(n)$ selections. 
%\end{theorem}

%\mcomment{In the following proof we will consider a submodular $k+1$-secretary} problem. 
In the following proof, for simplicity of notation, we prove the desired bound for submodular $(k+1)$-secretary problem. %Since $k+1=O(k)$, the upper bound derived will imply the stated bound for the  submodular $k$-secretary problem. 
For any given $n, k$, we construct a set of instances of the  \nameOfProblemSLplus~such that any online algorithm that uses a shortlist of size $\eta(k+1)$ will have competitive ratio of at most $\frac{7}{8} + \frac{\eta(k+1)}{2n}$ on a randomly selected instance from this set. 

First, we define a monotone submodular function $f$ as follows. 
%For $n>0$, we define a  monotone submodular function $f$. 
The ground set consists of $\frac{n}{2k}+n-1$ items. There are two types of items, $C$ and  $D$, with $L:=n/2k$ items of type $C$ and
$n-1$ items of type $D$. We define $f(\phi):=0$, $f(\{c\}):=k$ for $c\in C$, and $f(\{d\}):=1$ for all $d\in D$. 
%There are infinitely many elements of $C$ and $D$. 
%\scomment{Don't you just need $L$ items of type $C$ and $n-1$ items of type $D$?}
%There are
Also there is a collection of $L$ {\it disjoint} sets $T_{\ell}=\{c^{\ell}, d_1^{\ell},\cdots, d^{\ell}_{k}\}$, $\ell=1,2, \ldots L$, such that $c^{\ell}\in C$ and $d_j^{\ell}\in D$. We define $f(T_{\ell}):=2k$ for all $\ell=1,\ldots, L$.
%\scomment{infinite number of such sets? or will $L$ suffice?} 
%\mcomment{in the definition of function it should be infinite but in the input we use $n/2k$ of them}
%\scomment{After going through the proof, I don't see why you need infinite number, it seems just $L=n/2k$ will suffice. Where are you using that there are infinte number of $T^\ell$?}
%\mcomment{
%The reason is that you should give one functions $f$ that works for all $n$. Otherwise one may claim that for any given function $f$ there is large enough $N_f$ so that we can go beyond 7/8, for $n>N_f$. 
%}
Now, let
$$g(t):=k+\frac{k}{2}+\cdots+ \frac{k}{2^{i-1}} + \frac{(t-ik)}{2^i},$$
where $i=\floor{t/k}$. It is easy to see that $g$ is a monotone submodular function. 

Now, define $f$ on the remaining subsets of the ground set as follows. For all $S$ with $|S|\ge 1$, 
\begin{itemize}
\item $|S\cap C| \ge 2 \implies f(S):=2k+1$
\item $|S\cap C|=0 \implies f(S):=1+g(|S|-1)$
\item $|S\cap C|=1$ $\implies S\cap C=\{c^\ell\}$ for some $\ell\in [L]$   $\implies$
%$$f(S):=\min\{2k+1, k+\frac{1}{2} g(|S|-1)+\frac{k'}{2} (g(|S|-1)-g(|S|-2))\},$$ 
%$$f(S):=\min\{2k+1, k+\frac{1}{2} g(|S|-1)+\frac{k'}{2^{i+1}}\},$$ 
$$f(S):= \min\{2k+1, k+\frac{1}{2} g(|S|-1)+\frac{k'}{2^{i+1}}\},$$ 
%\mcomment{so can we remove min above? }\scomment{yes, actually, you don't use $f(S)\le 2k+1$ anywhere, do you?} 
where $k'=|S\cap\{d^{\ell}_1,\cdots, d_k^{\ell}\} |$, $i=\lfloor(|S|-1)/k\rfloor$.
\end{itemize}

%\scomment{$i$ was not defined in above, please check if I defined it correctly.}
%\mcomment{yes}
%\scomment{isn't the first case in the below gone now?}
%\mcomment{no why?} \scomment{because all items in $C$ are $c^\ell$ for some $\ell$}
%\mcomment{yes correct}
%\scomment{removed below
%\begin{itemize}
%\item ..
%\begin{itemize}
%\item $S\cap C\notin\{c^{\ell}\}_{\ell=1, \ldots, L} \implies f(S):=k+\frac{1}{2} g(|S|-1)$
%\item $S\cap C= \{c_1^{\ell}\}$ for some $\ell$  $\implies f(S):=\min\{2k+1, k+\frac{1}{2} g(|S|-1)+k'/2^{i+1}\}$, where $k'=|S\cap\{d^{\ell}_1,\cdots, d_k^{\ell}\} |$.
%\end{itemize}
%\end{itemize}
%}
%Observe that for any subset $S$, $f(S)\le 2k+1$. 
Observe that since $g(k)=k$, for any subset $S$ of size at most $k+1$, we have $f(S)\le k+\frac{k}{2} + \frac{k}{2} = 2k$.

\begin{lemma}
$f$ is a monotone submodular function.
\end{lemma}
\begin{proof}
We have to show that for any item $x$ and subsets $S\subseteq T$, $\Delta_f(x|S) \ge \Delta_f(x|T)$.
We consider the following cases:
\begin{itemize}
\item if $|T\cap C| \ge 2 \implies \Delta_f(x|T)=0$, so it is trivial.
\item if $|T\cap C| =0 \implies |S\cap C|=0 \implies \Delta_f(x|S) \ge \Delta_f(x|T)$ because of submodularity of $g$.
\item if $|T\cap C|=1 \implies |S\cap C|\le 1$
\begin{itemize}
\item if $|S\cap C|=1 $ then $S\cap C = T\cap C = \{c^{\ell}\}$ for some $\ell$:
\begin{itemize}
\item $x\in \{d_1^{\ell},\cdots, d_k^{\ell}\} \implies \Delta_f(x|S)=1/2^{i+1}+1/2^{i+1}$ for $i=\lfloor (|S|-1)/k\rfloor$, and $\Delta_f(x|T)=1/2^j+1/2^j$ for some $j=\lfloor (|T|-1)/k\rfloor$ and $j\ge i+1$.
\item $x\notin \{d_1^{\ell},\cdots, d_k^{\ell}\} \implies \Delta_f(x|S)=1/2^{i+1}$ for $i=\lfloor (|S|-1)/k\rfloor$ and $\Delta_f(x|T)=1/2^j$ for some $j\ge i+1$.
\end{itemize} 
%\item $S\cap C = T\cap C \notin \{c_1^{\ell}\}_{\ell} \implies \Delta_f(x|S) \ge \Delta_f(x|T)$ because of submodularity of $g$.

\item if $|S\cap C|=0 \implies \Delta_f(x|T) \le 1/2^{j+1}+1/2^{j+1}$ for $j=\lfloor (|T|-1)/k\rfloor$ and $\Delta_f(x|S)= 1/2^i$ for some $i\le j$. 
\end{itemize}
Thus $\Delta_f(x|S) \ge \Delta_f(x|T)$.
\end{itemize} 
Monotonicity follows trivially from the definition of $f$.
\end{proof}

\toRemove{
Also for any subset of $S$ with at least two elements of $C$, $f(S)=2k$. 
For subset $S$ with no element in $C$, if $i=\floor*{\frac{|S|}{k}}$, 
$f(S)$ is defined as 
\[
f(S)= k+k/2+ \dots +(|S|-ik)/2^{i}.
\]
For subset $S$ with exactly one element $c\in C$ such that $c\neq c_1$, if if $i=\floor*{\frac{|S|-1}{k}}$, 
$f(S)$ is defined as 
\[
f(S)= k+ k/2+ \dots +(|S|-1-ik)/2^{i+1}.
\]
Thus if $|S|=k+1$ and it contains exactly one element of $c\in C$ such that $c\neq c_1$ then $f(S)=k+k/2$.
Now suppose $S$  contains $c'$. 
For $S=T$, $f(S)=2k$.  Suppose $S$ contains $k'<k$ elements of $\{b_1, \dots, b_k\}$  and $\ell$ other elements of $D$. 
Let's $t=k'+\ell$, and $i=\floor*{\frac{t}{k}}$, then
\[
f(S)= \min\{2k, k'/2+(k+ k/2+ \dots +(t-ik)/2^{i+1})\}
\]
}
%\scomment{this proof is very vague, especially the claim any algorithm will select $k/2$ of $D$? Phrases like algorithm is not "aware" of something cannot be stated as a fact. You need to prove that the algorithm will not be able to distinguish between the two scenarios. We need to discuss.}



%Let $ {\cal T}^L$ be a collection of (any) $L=n/2k$ sets from $T^\ell, \ell=1,2, \ldots$. W.l.o.g., let's assume ${\cal T}^\ell = \{T_1, \ldots, T_L\}$.   

Now, denote $D^{\ell} := T^\ell \cap D = \{d_1^{\ell},\cdots, d_k^{\ell}\}$ for $\ell=1,2, \ldots, L$. Also, let 
$D'=D\setminus (\bigcup_{\ell=1}^L D^{\ell})$. % where $L:=n/2k$. 
%\scomment{Do you need $T^\ell, \ell =1,\ldots, L$ to be disjoint?} \mcomment{yes}
% $B'=B\setminus (\bigcup_{\ell }^{L} B^{\ell})$ for $L:=n/2k$.
Now define $L$ input instances $\{I_{\ell}\}_{\ell =1,\ldots, L}$, each of size $n$, as follows. For
any arbitrary subset $\tilde{D}\subseteq D'$ of size $n-Lk-1$, 
%\scomment{Which subset $\tilde{B}$? any arbitrary subset?} \mcomment{arbitrary}
define $I_{\ell}=\bigcup_{i=1,\ldots, L}  D^{i} \cup \tilde{D} \cup \{c^{\ell}\}$, for  $\ell=1,\ldots, L$.
%and $I_2=B^1 \cup B^2 \cup \tilde{B} \cup \{a_1^2\}$ (the difference is $a_1^1$ and $a_1^2$).
%Now suppose the input consists of the following:  $T^{\ell}=\{a_1^{\ell}, b_1^{\ell}, \cdots b_k^{\ell} \}$, no other element of $C$ and the remaining elements are from $B':=B\setminus \{b_1^{\ell}, \cdots, b_k^{\ell}\}$. 
Thus, for instance $I_{\ell}$, the the optimal $k+1$ subset is $T^\ell$ with value $f(T^{\ell})=2k$. 
%\scomment{earlier we stated $T^\ell$ is optimal, but we have never proven that none of the $k+1$ subset can take value $2k+1$. We actually do not need to show $T^\ell$ is optimal.}
%\scomment{$T^\ell$ is of size $k+1$, optimal should be of size $k$. If making $T_\ell$ to be of size $k$ makes it messy, you can initially state that you will consider submodular $k+1$ secretary problem.}


Now consider any algorithm for the submodular \nameSecSL\ and cardinality constraint $k+1$. We denote by $Alg$ the set of $\eta(k+1)$ items selected by the algorithm as part of the shortlist. % (all elements in the shortlist of size $\eta(k)$).
%\scomment{We have  used $C$ to denote shortlist in the algorithm. May be you can use a different symbol instead of type $A$ and $B$. }
Let $\bar I$ denote an instance chosen uniformly at random from $I_\ell, \ell=1,\ldots, L$.  
%We choose one of $I_{\ell}$ randomly. \scomment{randomly or arbitrarily?} 
Let $\pi$ denote a random ordering of $n$ items in $\bar I$. 
%We give a random order of $I_{\ell}$, say $\pi$ to the algorithm as input,
%(note that in the secretary problem the elements of input can be selected adversarially but the order should be random).
We denote by random variable $(\bar{I},\pi)$ the randomly ordered input instance to the algorithm. Also we denote by $\bar{T}, \bar{D}$ and $\bar c$, the corresponding $T^{\ell}$, $D^{\ell}$ and $c^\ell$.

Now we claim 

%Note that algorithm is not aware of $\ell$.
%Consider an algorithm $Alg$.
%Suppose $a_1^{\ell}$ is the $t$-th elements in the input, and
%elements of input are ordered as $I=(I_1,\cdots, I_n)$.
%Suppose $Alg$ is the set of elements selected by an algorithm.
%Denote by $\bar{B}=\{b_1,\cdots, b_k\}$.

\begin{lemma}
$\mathbb{E}_{(\bar{I},\pi)}[|Alg\cap \bar{D}|] \le k/2+\eta(k+1)/L$.
\end{lemma}
\begin{proof}
Suppose $(e_1,\cdots, e_n)$ indicates the ordered input according to random ordering $\pi$ on $\bar{I}$. %for some $0<\ell<L$.
Now let $t$ be the random variable indicating the index of $c^{\ell}$ in $(e_1,\cdots, e_n)$, i.e., $e_t=c^{\ell}$. 
%Define $R:=\mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}|]$.
Then, due to random ordering, and random choice of $\bar I$ from $I_1, \ldots, I_\ell$, we have
$$\mathbb{E}_{(\bar I, \pi)}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap D^1|]= \cdots = \mathbb{E}[|Alg\cap\{e_1,\cdots, e_{t-1}\}\cap D^{L}|]\ .$$
Also, since $D^\ell, \ell=1,\ldots, L$ are disjoint,
$$\sum_{\ell=1}^L \mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap D^{\ell}|] \le \eta(k+1)\ .$$
Since $\bar D=D^\ell$ with probability $1/L$,  we have
$$H:=\mathbb{E}[|Alg\cap\{e_1,\cdots, e_{t-1}\}\cap \bar{D}|]=  \frac{1}{L} \sum_{\ell=1}^L \mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap D^{\ell}|] \le \frac{1}{L} \eta(k+1)\ . $$ 
%\rightarrow 0$ as $n/\eta(k) \rightarrow \infty$.
Now define
$G:=\mathbb{E}[|Alg\cap\{e_t,\cdots, e_{n}\}\cap \bar{D}|]$.
We have
$$G\le \mathbb{E} [|\bar{D}\cap\{e_t,\cdots, e_n\}|]  \le k/2\ .$$
%Also define $H:=\mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\cap \bar{B}\}|]$.
%Also, $H\le k-G$.
Thus $$\mathbb{E}[|Alg\cap \bar{D}|] \le G+H\le k/2+\eta(k+1)/L\ .$$
%\rightarrow G$$
%\le k/2$$
%G+(k-G)/2 \le k/2+G/2\le k/2+k/4=3/4k$$.
\end{proof}
Now on input $\bar{I}$, if the algorithm doesn't select $\bar c$ as part of shortlist $Alg$, then by definition of $f$ for sets that do not contain any item of type $C$, we have 
$$f(A^*):=\max_{S \subseteq Alg:|S|\le k+1} f(S) \le 1+ g(k) = k+ \frac{k}{2}$$ 

Otherwise, if algorithm selects $\bar c$ then by definition of $f$ 
$$f(A^*):=\max_{S \subseteq Alg:|S|\le k+1} f(S) \le \max_{S \subseteq Alg \backslash (\bar D \cup \{\bar c\}):|S|\le k-|Alg \cap \bar D|} f(S \cup \bar D \cup \{\bar c\}) 
= k+ \frac{k}{2} +\frac{1}{2} |Alg\cap \bar{D}|$$ 
therefore $$\mathbb{E}[f(A^*)] \le k+\frac k 2+ \frac k 4+ \frac{\eta(k+1)}{2L} = \frac{7k}{4} + \frac{k\eta(k+1)}{n} \ .$$

%Hence $\mathbb{E}[f(Alg)]  \rightarrow k+k/2+k/4$ as $n\rightarrow \infty$, since $\eta(k)=o(n)$.
Since the optimal is equal to $\Ex[f(\bar T)]=2k$, the competitive ratio is upper bounded by
$$ 
%\left(\frac{7k}{4} + \frac{k\eta(k)}{n}\right)\left/\right. 2k = 
\frac{7}{8} + \frac{\eta(k+1)}{2n}$$

This proves competitive ratio upper bound of $\frac{7}{8} + o(1)$ when $\eta(k+1)=o(n)$, to complete the proof of Theorem \ref{hardness}.
%\scomment{I think we need to change the upper bound in theorem statement to $7/8 + o(1)$}
%Before arriving $a_1^{\ell}$ algorithm can not distinguish between elements of $B'=\{b_1^{\ell},\dots, b_k^{\ell}\}$
%and the rest of $D$ thus the expected number of elements in $B'$ selected by algorithm before observing $a_1$ goes to $0$ as $n/k\rightarrow \infty$.

%Therefore an online algorithm would select $k/2$ elements of set $B'$ in expectation and also it selects $a_1^{\ell}$ (and $k/2$ other elements from $B\setminus B'$).  Therefore, its $f$ value is $k+k/2+k/4$.
%Hence the competitive ratio is at most $7/8$.


==> introduction.tex <==
%\section{Introduction}



In the classic \textit{secretary problem}, 
$n$ items appear in random order.  We know $n$, but don't know the value of an item until it appears.   
Once an item arrives we have to irrevocably and immediately decide whether or not to select it. Only one item is allowed to be selected, and the objective is to  select the most valuable item, or perhaps to 
%\ccomment{Is this really equivalent, or just related}
%\mcomment{not equivalent but related. }
maximize the expected value of the selected item  
%The origin of the secretary problem is hard to track
~\cite{Dynkin:SovMath:1963,ferguson1989solved, 10.2307/2985407}. 
It is well known that the optimal policy is to observe the first $n/e$ items without making any selection and then select the first item whose value is larger than the value of the best item in the first $n/e$ items~\cite{Dynkin:SovMath:1963}. This algorithm, given by ~\citet{Dynkin:SovMath:1963},
is asymptotically optimal, and hires the best secretary with probability at least $1/e$. Hence it
is also $1/e$-competitive for the expected value of the chosen item, and
%\ccomment{Is this true?}
%\mcomment{Yes, but the original paper shows the probability not the expectation Dynkin provided an asympotically optimal algorithm for this problem, which hires the best secretary with probability at least 1/e}
it can be shown that no algorithm can beat $1/e$-competitive ratio in expectation.
%

Many variants and generalizations of the secretary problem have been studied in the literature, see e.g., \cite{Ajtai:2001,WILSON1991325,vanderbei1980optimal, wilson1991optimal, kleinberg, Babaioff:2008}.  
%\ccomment{We should have more variants hear} The secretary problem has been generalized.  
\cite{kleinberg, Babaioff:2008} introduced a 
{multiple choice secretary problem}, where the goal is to select $k$ items in a randomly ordered input so as to maximize  the {\it sum} of their values; and  \citet{kleinberg} gave an algorithm with an asymptotic competitive ratio of $1-O(1/\sqrt{k})$. Thus as $k\to \infty$, the competitive ratio approaches  1. Recent literature studied several generalizations of this setting to multidimensional knapsacks \cite{moser1997algorithm}, and proposed algorithms for which the expected online solution approaches the best offline solution as the knapsack sizes becomes large~(e.g., \cite{FHKMS10, devanur-hayes, AgrawalWY14}). 
%\scomment{add citations, Cliff's paper, Devanur and Hayes, my paper on online linear programming etc.}
%\ccomment{I added some of these references to bibtex to the bib file because I had it handy.  Mohammad, you need to add the text and references.}
%\ccomment{Does multiple choice secretary only refer to the case of sum?}
%\mcomment{no it can be any function}


In another variant of multiple-choice secretary problem, \citet{Bateni} and ~\citet{Gupta:2010} introduce 
the \textit{\nameOfProblem}. In this secretary problem, the algorithm again selects $k$ items, but 
the value of the selected items is given by a monotone submodular function 
%It is an online variant of monotone submodular maximization subject to cardinality constraints. 
%The objective function is designed by an adversary, but the order of the items is uniformly at random.
$f$. The algorithm has a value oracle access to the function, i.e., for any given set $T$, an algorithm can query an oracle to find its value $f(T)$~\cite{oracle}.
The algorithm can select at most $k$ items $a_1 \cdots, a_k$, from a randomly ordered sequence of $n$ items. The goal is to maximize $f(\{a_1,\cdots, a_k\})$.
%Now imagine we are allowed to select several items instead of one item. Would that let us to improve $1/e$?
%Assuming a value oracle access to the submodular function; i.e., for a given set $T$, an algorithm can query an oracle to find its value $f(T)$~\cite{oracle}.
Currently, the best result for this setting is due to ~\citet{kesselheim}, who achieve a $1/e$-competitive ratio in exponential time, or $\frac{1}{e}(1-\frac{1}{e})$ in polynomial time. In this case, the offline problem is NP-hard and hard-to approximate beyond the factor of $1-1/e$ achieved by the greedy algorithm \cite{nemhauser1978best}. 
%\scomment{need a reference for lower bound of $1-1/e$ for offline monotone submodular maximization}
However, it is unclear if a competitive ratio of $1-1/e$ can be achieved by an online algorithm for the {\nameOfProblem} even when $k$ is large. 

\paragraph{Our model: \nameSecSL.}
In this paper, we consider a relaxation of the secretary problem 
%.  What if  the online algorithm for secretary problem 
where the algorithm is allowed to  select a {\it shortlist} of items that is larger than the number of items that ultimately need to be selected. That is, in a multiple-choice secretary problem with cardinality constraint $k$, the algorithm is allowed to choose more than $k$ items as part of a shortlist. Then, after seeing the entire input, the algorithm can choose a subset of size $k$ from the bigger set of items in the shortlist. 
%when seeing items online, and ultimately maximizes a function of $k$ elements, 
%we are allowed to choose more than $k$ elements, and then after seeing the entire input, choose a  a subset of size $k$ from our bigger set.  

This new model is motivated by some practical applications of secretary problems, such as hiring (or assignment problems),  where in some cases it may be possible to tentatively accept a larger number of candidates (or requests), while deferring the choice of the final $k$-selections to after all the candidates have been seen. Since there may be a penalty for declining candidates who were part of the shortlist, one would prefer that the shortlist is not much larger than $k$.

Another important motivation is theoretical: we wish to understand to what extent this relaxation of the secretary problem can improve the achievable competitive ratio. This question is in the spirit of several other methods of analysis that allow an online algorithm to have additional power, such as {\em resource augmentation} \cite{KalyanasundaramP00,PhillipsSTW97}.

The potential of this relaxation is illustrated by the basic secretary problem, where the aim is to select the item of maximum value among randomly ordered inputs. There, it is not difficult to show that if an algorithm  picks every item that is better than the items seen so far, the true maximum will be found, while the expected number of items picked under randomly ordered inputs will be $\log(n)$. Further, we show that this approach can be easily modified to get the maximum with $1-\epsilon$ probability while picking at most  $O(\ln(1/\epsilon))$ items for any constant $\epsilon>0$. Thus, with just a constant size shortlist, we can break the $1/e$ barrier for the secretary problem and achieve a competitive ratio that is arbitrarily close to $1$.

%For the secretary problem, we can imagine choosing not one secretary, but several, and then taking the best one at the end.  
Motivated by this observation, we ask if a similar improvement can be achieved by relaxing the \nameOfProblem~to allow a shortlist. That is, instead of choosing $k$ items, the algorithm is allowed to chose  $\eta(k)$ items as part of a shortlist, for some function $\eta$;
and at the end of all inputs, the algorithm chooses $k$ items from the $\eta(k)$ selected items. Then, what is the relationship between $\eta(\cdot)$ and the competitive ratio for this problem? Can we achieve a solution close to the best offline solution when $\eta(k)$ is not much bigger than $k$, for example  when 
 $\eta(k)=O(k)$?  

%We answer this question affirmatively in this paper, and provide an algorithm 
%What is the relationship between $\eta$ and the competitive ratio. 
%In other words, we have a {\em shortlist} of size $\eta(k)$, where $\eta(k)$ is independent of $n$, and the output is subset of this shortlist.
%We wish to understand how much this relaxation can improve the competitive ratio.   In other words, what is the relationship between $\eta$ and the competitive ratio.
 
%For exmaple, when the  it is possible to approach the optimal offline solution by some function $\eta$ as $k\to \infty$.  Can we obtain a similar results for the \nameOfProblemSL.


%\ccomment{Is there a practical-ish motivation for this model?}
%A motivation for this model is that for the $k$-secretary problem instead of restricting ourselves to make irrevocable decisions for each item, we may add items to a shortlist and defer the final decision to the end (choosing $k$ elements from shortlist). We want the size of shortlist to be as small as possible.

In this paper, we answer this question affirmatively by giving a polynomial time algorithm that achieves $1-1/e-\epsilon-O(k^{-1})$ competitive ratio for the \nameOfProblem~using a shortlist of size $\eta(k)=O(k)$. This is surprising since $1-1/e$ is the best achievable approximation (in polynomial time) for the offline problem. Further, for some special cases of submodular functions, we demonstrate that an $O(1)$ shortlist allows us to achieve a $1-\epsilon$ competitive ratio. These results demonstrate the power of (small) shortlists for closing the gap between online and offline (polynomial time) algorithms. 
%size we give a new algorithm and show several positive (and one negative) results that capture the power of these shortlists and  show that they are (surprisingly) powerful. 

We also discuss connections of {\nameSecSL} to the related streaming settings. While a streaming algorithm does not qualify as an online algorithm (even when a shortlist is allowed), we show that our algorithm can in fact be implemented in a streaming setting to use $\eta(k)=O(k)$ memory buffer; and our results significantly  improve  the available results for the \streamingProblem.
Furthermore since the upperbound given in ~\cite{mcgregor2017better} holds for random order streams, our result is asymptotically tight in this setting.

\subsection{Problem Definition}
%In the well-studied submodular $k$-secretary problem, applicants from a set ${\cal U} = \{a_1, a_2, \ldots, a_n\}$  (pool of applicants) arrive in a uniformly random order over $n$ sequential rounds. In each round, an online algorithm irrevocably decides whether to select an applicant or not. The algorithm can select at most $k$ applicant. The goal is to maximize the value of the selected $k$ applicants, as given by a submodular function $f$. 

%More formally, let $S, |S|\le k$ denote the subset of candidates selected by the algorithm, then the expected utility of the algorithm is given by $\ALG:=\Ex[f(S)]$, where $f$ is a monotone submodular function, and the expectation taken both over random order and possible randomness in the algorithm's selection of subset $A$ given an order. The competitive ratio of the online algorithm is then defined as $\frac{\ALG}{\OPT}$, where $\OPT$ is the optimal offline utility defined as 
%$$\OPT=f(S^*), \text{ where, } S^*=\arg \max_{S \subseteq [n], |S|\le k} f(S).$$

%\scomment{edited by me on 8/21}
We now give a more formal definition.
Items from a set ${\cal U} = \{a_1, a_2, \ldots, a_n\}$  (pool of items) arrive in a uniformly random order over $n$ sequential rounds. The set ${\cal U}$ is apriori fixed but unknown to the algorithm, and the total number of items $n$ is known to the algorithm. In each round, the algorithm irrevocably decides whether to add the arriving item to a {\it shortlist} $A$ or not. %The goal is to return,  at the end of $n$ rounds, a shortlist $A$ of size at most $\eta(k) \ge k$ to maximize the  `value' of best $k$ subset of this shortlist. More formally, 
%We are given a monotone submodular function $f:2^{\cal U} \rightarrow \mathbb{R}$, in a value oracle model. %Let the set $A \subseteq {\cal U}, |A|\le \eta(k)$ denote the shortlist of items selected by the online algorithm,  then 
The algorithm's value at the end of $n$ rounds is given by 
$$\ALG = \Ex[\max_{S\subseteq A, |S|\le k} f(S)]$$ 
where $f(\cdot)$ is a monotone submodular function. The algorithm has value oracle access to this function.

The optimal offline utility is given by
$$\OPT:=f(S^*), \text{ where } S^*=\arg \max_{S \subseteq [n], |S|\le k} f(S).$$ 
We say that an algorithm for this problem achieves a competitive ratio  $c$ using shortlist of size $\eta(k)$, if at the end of $n$ rounds, $|A|\le \eta(k)$ and $\frac{\ALG}{\OPT}\ge c$.

Given the shortlist $A$, since the problem of computing the solution $\arg \max_{S\subseteq A, |S|\le k} f(S)$ can itself be computationally intensive, our algorithm will also track and output a subset $A^* \subseteq A, |A^*| \le k$. We will lower bound  the competitive ratio by bounding $\frac{f(A^*)}{f(S^*)}$.

The above problem definition has connections to some existing problems studied in the literature. The well-studied online \nameOfProblem~described earlier is obtained from the above definition by setting $\eta(k)=k$, i.e., it is same as the case when no extra items can be selected as part of a shortlist. 
%\scomment{Did a pass on the para below on 8/30 after our discussion regarding streaming problem}
Another related problem is {\it  \streamingProblem}~studied in~\cite{norouzi}. In this problem, items from a set $\cal U$ arrive online in random order and the algorithm aims to select a subset $S \subseteq {\cal U}, |S|\le k$ in order to maximize $f(S)$. The streaming algorithm is allowed to maintain a {\it buffer} of size $\eta(k)\ge k$. 
However, this streaming problem is distinct from the \nameOfProblemSL\ in several important ways. On one hand, since an item previously selected in the memory buffer can be discarded and replaced by a new items, a memory buffer of size $\eta(k)$ does not imply a shortlist of size at most $\eta(k)$. On the other hand, in the secretary setting, we are allowed to memorize/store more than $\eta(k)$ items without adding them to the shortlist. Thus an algorithm for \nameOfProblem with shortlist of size $\eta(k)$ may potentially use a buffer of size larger than $\eta(k)$. 
Our algorithms, as described in the paper, do use a large buffer, but we will show
%\ccomment{Where do we show that the streaming actually works}
that the algorithm presented in this paper can in fact be implemented to use only $\eta(k)=O(k)$ buffer, thus obtaining matching results for the streaming problem. 
%imply the same competitive ratio for random order streaming problem with buffer of size $\eta(k)$, but not vice-versa. We will discuss the corollary of our algorithm design and analysis for the  submodular random order streaming problem. 
%Because shortlists can be used as a buffer for memory but not vice versa. ( we are allowed to delete from memory and reduce the size but we can not remove from a shortlist)







%In the new `submodular $k$-secretary with shortlist' problem considered in this paper, we allow the online algorithm to select a shortlist of more than $k$ candidates, and pick the final subset of $k$ candidates from this shortlist at the end. Specifically,  we allow the online algorithm to select a subset $A$ of size $|A|\le \eta(k)$, where $\eta(k)\ge k$. The competitive ratio of the online algorithm is then defined with respect to the best $k$-subset of $A$. That is, competitive ratio is given by $ \frac{\ALG_{\eta}}{\OPT}$, where $\OPT$ as defined before, and 
%$$\ALG_\eta = \Ex[\max_{S\subseteq A, |S|\le k} f(S)],$$ 
%with $A$ being the subset of items selected by the online algorithm, of size at most $\eta(k)$. 

\subsection{Our Results}
Our main result is an online algorithm  for \nameOfProblemSL\ that, for any constant $\epsilon>0$, achieves a competitive ratio of $1-\frac{1}{e} - \epsilon-O(\frac{1}{k})$ with $\eta(k) = O(k)$. 
Note that for \nameOfProblem\ there is an upper bound of $1-1/e$ on the achievable aproximation factor, even in the offline setting, and this upper bound applies to our problem for arbitrary size $\eta(\cdot)$ of shortlists. On the other hand for online monotone \nameOfProblem, i.e., when $\eta(k)=k$, the best competitive ratio achieved in the literature is $1/e-O(k^{-1/2})$~\cite{kesselheim} 
%\scomment{is there an upper bound? } \mcomment{ No} 
Remarkably, with only an $O(k)$ size shortlist, our online algorithm is able to achieve a competitive ratio that is arbitrarily close to the offline upper bound of $1-1/e$.

In the theorem statements below, big-Oh notation $O(\cdot)$ is used to represent asymptotic behavior with respect to $k$ and $n$. We assume the standard  value oracle model:  the only access to the submodular function is through a black box
returning $f(S)$ for a given set $S$, and  each such queary can be done in $O(1)$ time. 
%\ccomment{Define value oracle model and state thm.1 appropriately}
\begin{theorem} \label{opttheorem}
For any constant $\epsilon>0$, there exists an online algorithm (Algorithm \ref{alg:main}) for the \nameOfProblemMatroidSL\ that achieves a competitive ratio of $1-\frac{1}{e} -\epsilon -O(\frac{1}{k})$, with shortlist of size $\eta_\epsilon(k)=O(k)$. Here,  $\eta_\epsilon(k)=O(2^{poly(1/\epsilon)}k)$.  
%$$\eta_\epsilon(k) =c k\log(1/\epsilon) {\frac{1}{\epsilon^3} \log(1/\epsilon)  \choose {\frac{1}{\epsilon^2} \log(1/\epsilon)}} =O(2^{poly(1/\epsilon)}) \ ,$$
%for some absolute constant $c$.
% for submodular secretary problem with cardinality constraints, such that it selects $O(k)$ elements. %, where $C(a)$ is a constant depending only on $a$.
  The running time of this online algorithm is $O(n)$.
\end{theorem}
%\scomment{Can we add a compact description of dependence of  $\eta_\epsilon(k)$ on $\epsilon$ in this theorem statement? What is this function: exponential or super-exponential in $1/\epsilon$?}
%\scomment{Should we say $O(n)$ evaluations of the objective function instead of time?}
%\scomment{After fixing the proof in section 3, I am getting a different (much bigger) dependence on $1/\epsilon$. Mohammad, can you check? May be considering this, we should leave it here as $\eta_\epsilon(k)=O(2^{poly(1/\epsilon)}$?}
%\scomment{I see that the theorem statement was changed, but we still need to provide the exact function, may be right after the theorem statement. Adding below:}

%Specifically, we have $\eta_\epsilon(k)=$\etaMacro$k$ for some constant $c$.
%The running time  of our algorithm is linear in $n$, the size of the input, which 
%is significant as, until recently, it was not known if there exists a linear time algorithm achieving a $1-1/e-\epsilon$ approximation even for the offline monotone submodular maximization problem under cardinality constraint\cite{linear}. 
Similar to~\cite{us}, an interesting aspect of our algorithm is that it is highly parallel. Even though the decision for each arriving item may take time that is exponential in $1/\epsilon$ (roughly  $\eta_\epsilon(k)/k$), it can be readily parallelized among multiple (as many as $\eta_\epsilon(k)/k$) processors. 
%The  operations required to make a decision for each item can be divided between available processors. (the running time will be divided by $\min(c,p)$ where $c=k\log(1/\delta) {\frac{1}{\delta^3} \log(1/\delta)  \choose {\frac{1}{\delta^2} \log(1/\delta)}}$ is the hidden constant in $O(k)$ and $p$ the number of processors )


%More precisely, we design a $1-1/e-\epsilon-O(k^{-1})$ competitive algorithm that selects $O(k\log(1/\delta) {\frac{1}{\delta^3} \log(1/\delta)  \choose {\frac{1}{\delta^2} \log(1/\delta)}})$ elements, i.e., the dependency on $k$ is linear and on $\delta$ is exponential.



%\scomment{Add a formal corollary of Theorem 1 for random-order streaming problem here. Also, will be good to add a few lines in problem definition section describing how our problem relates to random order streaming.} \mcomment{done done}


%As discussed earlier, by definition, a corollary of our results is an algorithm for the submodular random order streaming problem with the same competitive ratio.
Further, we show an implementation of Algorithm 2 that uses a memory buffer of size at most $\eta_\epsilon(k)$ to get the following result for the problem of {\it \streamingProblem} described in the previous section. 
%\ccomment{Make terminology for evaluations consistent with previous work}
\begin{restatable}{theorem}{thmStreaming}
\label{thm:streaming}
For any constant $\epsilon\in (0,1)$, there exists an algorithm for the \streamingProblem  that achieves $1-\frac{1}{e} -\epsilon -O(\frac{1}{k})$ approximation to $\OPT$ while using a memory buffer of size at most $\eta_\epsilon(k)=O(k)$. Also, the number of objective  function evaluations for each item, amortized over $n$ items, is $O(1+\frac{k^2}{n})$.
%Also, decision for each arriving item requires $O(1)$ evaluations of the objective function.
%Also in amortized time, it processes each arriving item with $O(1+\frac{k^2}{n})$ evaluations of the objective function.
%Also the amortized time to processes each arriving item requires $O(1+\frac{O(k^2)}{n})$ evaluations of the objective function.
% The running time of this online algorithm is $O(n)$.
\end{restatable}
%The above result significantly improves over the state-of-the-art results in random order streaming model \cite{norouzi}, which are an approximation ratio of $\frac 1 2+8\times 10^{-14}$ using a memory of size $O(k\log k)$. 
%uses $O(k)$ memory and achieves asymptotic $R<1-1/e$ approximation.

%\scomment{I don't understand the upper bound stated below - by arbitrary $\eta$, couldn't we get at best the the offline problem. I can just select everything into shortlist. So, is the below giving an upper bound for the offline problem?  } \mcomment{using $o(n)$ selections. No it is for online problem}

%As a result, we show that in our model $\eta(k)=\gamma.k$, where $\gamma$ is a constant. It is optimal up to a constant factor.
%The constant factor $\gamma$ is growing as the competitive ratio gets closer to $1-1/e$. 
%Because of the known upper bound for offline submodular maximization with cardinality constraint.
%It is obvious that we can not get better than $1-1/e$ competitive algorithm if we only consider  polynomial time algorithms. 

%It is natural to ask whether these $k$-lists are, in fact, too powerful.  Maybe they could actually allow us to always match the best offline algorithm.  We give a negative result in this direction and 
%show that even if we have unlimited computation power, for any function $\eta(k)=o(n)$, we can get no better than $7/8$-competitive algorithm using a shortlist of size $\eta(k)$. Note that with unlimited computational power, the offline problem can be solved exactly. This result demonstrates that 
%having a shortlist does not make the online problem too easy - 
%even with a shortlist (of size $o(n)$) there is an information theoretic gap between the online and offline problem. Note that the $1-1/e$ upperbound for streaming model~\cite{mcgregor2017better} 
%does not imply an upper bound for the shortlist model.

\toRemove{
%\mcomment{we should emphasize the upper bound is for any $k$, i.e., it holds asymptotically}
\begin{restatable}{theorem}{hardness}
%\begin{theorem} 
\label{hardness}
No online algorithm (even with unlimited computational power)   can achieve a competitive ratio better than $7/8+o(1)$ for the \nameOfProblemSL, while using a shortlist of size $\eta(k)=o(n)$.
%by selecting $\eta(k)$ elements for any function $\eta$ (independent of $n$).
\end{restatable}
%\end{theorem}

%\scomment{By independent of $n$, do you mean $\eta(k)$ does not grow with $n$, i.e., $\eta(k)=O(1)$ if $O(\cdot)$ denotes asymptotic with respect to $n$? This is not same as $o(n)$, e.g.. $\eta(k)=\sqrt{n}$ would also be $\eta(k)=o(n)$.} \scomment{We need to discuss this issue}
 
 % It also improves~\cite{Badanidiyuru2014StreamingFly} on random order inputs.
%(Note that in our algorithm we keep extra items in the shortlist only for a limited time $O(n/k)$, and then we are able to release them.
%That is why the extra memory is $O(1)$ instead of $O(k)$).

%Another interesting aspect of our algorithm is that it is highly parallel. In order to decide whether or not to select an item in a slot $s_i$ in window $W$ which consists of $\{s_1, \dots, s_{\alpha \beta}\}$,
%the algorithm concurrently run several online maximum algorithms to find the maximum marginal value with respect to %different subsets.
% $S\cup \gamma(\tau)$, where $\tau$ is a subset of slots $\{s_1,\dots, s_{i-1}\}$ with $|\tau|<\alpha$.
%We select a new item if any of the maximum algorithms (for some $\tau$) select it, otherwise we do not select it. All the maximum algorithms for different subsets $\tau$ can be run in parallel. 

%Although the update time in our algorithm is $O(1)$, the constant can be very large. Consequently it may not be desirable for large streams. 
%We take two approaches to improve it. The first approach is parallel algorithms. The interesting fact about our algorithm is that it is highly parallel, i.e. the  operations required for each element can be divided between as many processor as it is available. 
%The running time will be divided by the number of processors. 

%In addition, we design a fast  thresholding algorithm that requires only one function evaluation per element.
%It achieves competitive ratio $1/2-O(1/\sqrt{k})$ by selecting $k\log^2k$ elements. The competitive ratio and the update time of this algorithm is still better than~\cite{kesselheim} and~\cite{Hess}. In ~\cite{kesselheim}  update time is $O(n^2)$. 
%In terms of memory, our thresholding algorithm uses less memory than~\cite{Badanidiyuru2014StreamingFly} but more than~\cite{Hess}.


%We also provide an upper bound showing that it is not possible to achieve any competitive ratio better than $7/8$ by selecting $O(g(k))$ elements, where $g$ is an arbitrary function, even if we have free computation.
%\scomment{Can you add a theorem statement for the results discussed below?} \mcomment{added}
Finally, for some special cases of monotone submodular functions, we can asymptotically approach the optimal solution.
%\ccomment{Don't mention this as a thm.}
%\begin{theorem}
%Suppose $F$ is a monotone submodular function and $F(a_1,\cdots, a_i+\alpha,\cdots, a_k)  \ge  F(a_1, \cdots, a_i, \cdots, a_k  )$, for any  $\alpha >0$ and $1\le i \le k$.
%Let $S$ be the elements selected by Kleinberg's algorithm~\cite{kleinberg}, then
%$E[F(S)]>(1-5/\sqrt{k})OPT$.
%%Let $T$ be the $k$ largest elements of $S$, and $OPT=f(T)$.
%The expected number of elements of $T$ selected by the algorithm is at least $(1 -5/\sqrt{k})k$.
%\end{theorem}
%\begin{enumerate}
%\item $F$ is a monotone submodular function, and $F(a_1,\cdots, a_i+\alpha,\cdots, a_k)  \ge  F(a_1, \cdots, a_i, \cdots, a_k  )$, for $\alpha >0$ and $1\le i \le k$.
%\end{enumerate}
%We show Kleinberg's algorithm asymptotically approaches optimal solution.
%We prove that the Kleinberg algorithm works under this assumption which means that the competitive ratio of the algorithm asymptotically approaches 1.
The first one is the family of functions we call $m$-submdular. 
A function $f$ is $m$-submodular if it is submodular and there exists a submodular function $F$ such that for all $S$:
%\begin{itemize}
%\item 
\[ 
f(S)= \max_{T\subseteq S, |T|\le m} F(T) \ .
\]
%\end{itemize}
\scomment{This needs to be rewritten, I don't have time right now, so removing: Example of $m$-submodular functions are   maximum node weighted bipartite matching and  maximum edge weighted bipartite matching defined on $G=(X\times Y)$ with $|Y|=m$.  (the assignments will be done at the end of algorithm after all the selections are made).}

%\scomment{
%What is $\epsilon, \delta$? I removed this and restated inline with our rest of the results.
%\begin{theorem}
%For any $m$-submodular function $F$ there is an Algorithm that selects a set $S$ with $|S|<m\ln (1/\epsilon)+\ln(1/\delta)+\sqrt{\ln^2{1/\delta}+2m\ln(1/\delta)\ln(1/\epsilon)}$ and $E[F(S)]=(1-\epsilon-\delta)OPT$.
%\end{theorem}
%}
%\begin{restatable}{theorem}{msub}
\begin{theorem}
\label{thm:msub}
If $f$ is an $m$-submodular function, there exists an online algorithm for the \nameOfProblemSL~that achieves a competitive ratio of $1-\epsilon$ with shortlist of size $\eta_{\epsilon,m}(k)=O(1)$. Here, 
$\eta_{\epsilon,m}(k) = (2m+3) \ln(2/\epsilon)$.
\end{theorem}
%\end{restatable}
A proof of Theorem~\ref{thm:msub} along with the relevant algorithm (Algorithm \ref{alg:SIII}) appears in the appendix.

Another special case  is  monotone submodular functions $f$ satisfying the following property:
$f(\{a_1,\cdots, a_i+\alpha,\cdots, a_k\})  \ge  f(\{a_1, \cdots, a_i, \cdots, a_k \})$, for any $\alpha >0$ and $1\le i \le k$.
We can show that the algorithm by \citet{kleinberg} asymptotically approaches optimal solution for such functions, but we omit the details.

}





%We call an algorithm $ALG$ c-competitive if for any objective function $F$ chosen by the adversary, the
%set of selected items $ALG$ satisfies $E [F(ALG)] \ge (c ? o(1)) · OPT$, where $OPT$ is a feasible
%(offline) solution that maximizes v and the o(1)-term is asymptotical with respect to the length of
%the sequence n. 










%What is the minimum size shortlist to get a  $c$-competitive algorithm?
%These are questions that we consider in this paper.



%The submodular secretary problem, introduced by Bateni2013SubmodularExtensions et al. and Gupta et al., is an
%online variant of monotone submodular maximization subject to cardinality constraints. In this
%problem, we are allowed to select up to k items from a set of n items.
%The value of a set is represented by a monotone, submodular function.
%The values of the submodular function are only known on subsets of the items that have already arrived.
%The objective function is designed by an adversary, but the order of the items is uniformly at random.




%It is well-known since 1963 [10]
%that the optimal policy is to interview the first t ? 1 applicants, then hire the next one whose quality exceeds that of
%the first t ? 1 applicants, where t is defined by ; as $n \to \infty$, the probability of hiring
%the best applicant approaches 1/e, as does the ratio t/n.
%Note that a solution to the secretary problem immediately
%yields an algorithm for a slightly different objective function optimizing the expected value of the chosen element.





%In secretary problem, we are given a random order input and we are going to select the maximum element.
%In the classic secretary problem, one is presented a sequence of items with different scores online in
%random order. Upon arrival of an item, one has to decide immediately and irrevocably whether to
%accept or to reject the current item.  The objective is to accept the best of these items. 




%Multiple Choice secretary problem:


%Submodular Secretary problem:



%Our extension


%Streaming model:





% Imagine that you
%manage a company, and you want to hire a secretary from a pool of n applicants. You are very keen on hiring only
%the best and brightest. Unfortunately, you cannot tell how good a secretary is until you interview him, and you must
%make an irrevocable decision whether or not to make an offer at the time of the interview. The problem is to design
%a strategy which maximizes the probability of hiring the most qualified secretary. It is well-known since 1963 [10]
%that the optimal policy is to interview the first t ? 1 applicants, then hire the next one whose quality exceeds that of
%the first t ? 1 applicants, where t is defined by ; as $n \to \infty$, the probability of hiring
%the best applicant approaches 1/e, as does the ratio t/n. Note that a solution to the secretary problem immediately
%yields an algorithm for a slightly different objective function optimizing the expected value of the chosen element.




%In this paper, we consider general monotone submodular functions.



%The submodular secretary problem, introduced by Bateni2013SubmodularExtensions et al. and Gupta et al., is an
%online variant of monotone submodular maximization subject to cardinality constraints. In this
%problem, we are allowed to select up to k items from a set of n items.
%The value of a set is represented by a monotone, submodular function.
%The values of the submodular function are only known on subsets of the items that have already arrived.
%The objective function is designed by an adversary, but the order of the items is uniformly at random.

%We call an algorithm c-competitive if for any objective function v chosen by the adversary, the
%set of selected items ALG satisfies $E [v(ALG)] \ge (c ? o(1)) · v(OPT)$, where $OPT$ is a feasible
%(offline) solution that maximizes v and the o(1)-term is asymptotical with respect to the length of
%the sequence n. 

\scomment{The susection "Our techniques" was describing analysis and algorithm design techniques that are not being used in the proof anymore, there is no time to revise it, so I am removing it. Most of this intuition appears in algorithm description and proof overview anyway.}
\toRemove{
\subsection{Our techniques}
First we design a simple algorithm for the classic secretary problem  (finding the maximum element) that achieves a competitive ratio  of $1-\epsilon$ (for any $\epsilon>0$)  using a shortlist of size $O(\log(1/\epsilon))$.
%for a class of submodular functions that we call them $m$-submodular,
%for any $m>0$. 
The algorithm  ignores an $\epsilon$-fraction of the input and then selects an item if it is greater than the maximum element seen so far. 
We show that with probability $1-\epsilon$, the total number of selections made by this algorithm is at most $O(\log (1/\epsilon))$.
%A special $m$-submodular function for $m=1$ is the function $\max$. 
%As a result we 
We will use this online algorithm as a subroutine in our proposed algorithm for \nameOfProblemSL, for repeatedly finding (with probability $1-\epsilon$) the  item with maximum marginal value with respect to a subset of items, under submodular function $f$.  %It requires $\log(1/\epsilon)$ selections.
The main idea of the algorithm for \nameOfProblemSL\ is to divide the input into some blocks that we call them $(\alpha,\beta)$ \textit{windows}.  In this procedure, we partition the input into slots, where the sizes of the slots follow a balls-and-bins distribution.  We then group these slots into windows.
%Divide the input into $k\beta$ slots. The $i$-th slot, $s_i$, consists of $X_i$ consecutive elements of the input.
%Random variables $\{X_i\}$  for $i\in [k\beta]$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
%A \textit{window}, represented by parameters $(\alpha,\beta)$, consists of $\alpha \beta$ consecutive slots.
%\begin{definition} 
%A \textit{window}, represented by parameters $(\alpha,\beta)$, consists of $\alpha$ consecutive intervals, 
%of length $n/k$. 
%each interval is divided into $\beta$ slots. The length of $i$-th slot is a random variable denoted by $X_i$.
%Random variables $\{X_i\}$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
%random sample from the binomial distribution $B(n,\frac{1}{k\beta})$.
%of length $\frac{n}{k\beta}$.
%\end{definition}
%It consists of $\alpha$ consecutive intervals, 
%%of length $n/k$. 
%each interval is divided into $\beta$ slots. The length of $i$-th slot is a random variable denoted by $X_i$.
%Random variables $\{X_i\}$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
%%random sample from the binomial distribution $B(n,\frac{1}{k\beta})$.
%%of length $\frac{n}{k\beta}$.
%%Each window consists of smaller subintervals that we call them \textit{slots}.
Applying concentration inequalities for each {window}, and show that each window  has  roughly $\alpha$ elements of $OPT$ (the optimal solution), w.h.p.,
%the probability increases as $\alpha$ increases.
and that the fraction of elements of $OPT$ in a window that lie in different slots is at least $1-1/\beta$.
Therefore by choosing $\beta$ large enough most of the items in a window are in different slots, roughly speaking.\newline
For each window $w$ the algorithm \textit{guesses} the slots in which elements of $OPT$ in  $w$ lie in. 
By \text{guess} we mean that the algorithm enumerates over all subsets of size $\alpha$ of all $\alpha\beta$  slots in  $w$, and choose 
the one with the maximum marginal gain with respect to previously selected items. This can be done in an online manner.\newline
In the analysis of the algorithm for each window $w$,
we define an event $T_{1,\cdots, w-1}$ which conditions on the elements selected by the algorithm and also the positions in which they get selected by the algorithm. 
By conditioning on $T_{1,\cdots, w-1}$, we prove a lower bound for the expected marginal gain in the next window $w$.
Suppose $S_{1,\cdots, w-1}$ is output of the algorithm in windows $1,\cdots ,w-1$.
The crucial idea is that we show  conditioned on $T_{1,\cdots, w-1}$, each element $e\in OPT\setminus S_{1,\cdots, w-1}$
is more likely to appear in a slot in $w$ than in a slot in $1,\cdots, w-1$. 

We then have a normalization step in which we make all the elements of $OPT\setminus S_{1,\cdots, w-1}$ "appear" with the same probability in $w$. 
Therefore given that one slot in window $w$ contains an element of $OPT$, it can be any of $OPT\setminus S_{1,\cdots, w-1}$ with probability at least $1/k$. Hence the marginal gain for that slot is at least $\frac{1}{k}(OPT-F(S))$. 
We then repeat the argument for all the slots in window $w$  containing elements of the normalized sample.
\newline
The algorithm we describe uses $O(n)$ memory, in addition to the shortlist, but we can show how to modify the algorithm so that the amount of memory used is roughly the same as the size of the shortlist, and therefore the algorithm can be implemented in a streaming model.
} 

\subsection{Comparison to related work}
%There are two main frameworks  for \nameOfProblem: online algorithms and streaming algorithms.
%In the online framework,  we assume the input has random order. %(in adversarial order we can not guarantee anything)
%All of the previous algorithms in this framework irrevocably select a subset of size $k$, whose value is close to OPT~\cite{Bateni, kesselheim,Naor,smspm}.
We compare our results (Theorem \ref{opttheorem} and Theorem \ref{thm:streaming}) to the best known results for {\it \nameOfProblem}~and {\it \streamingProblem}, respectively.

The best known algorithm so far for \nameOfProblem~is by \citet{kesselheim}, with asymptotic competitive ratio of $1/e-O(k^{-1/2})$. 
In their algorithm, after observing each element, they use an oracle to compute optimal offline solution on the elements seen so far.
Therefore it requires exponential time in $n$. The best competitive ratio that they can get in polynomial time is 
$\frac{1}{e}(1-\frac{1}{e})-O(k^{-1/2})$.
In comparison, by using a shortlist of size $O(k)$ our (polynomial time) algorithm achieves a competitive ratio of $1-\frac{1}{e}-\epsilon-O(k^{-1})$. In addition to substantially improves the above-mentioned results for \nameOfProblem, this closely matches the best possible offline approximation ratio of $1-1/e$ in polynomial time. Further, our algorithm is linear time. Table \ref{table:t1} summarizes this comparison. 
Here, $O_\epsilon(\cdot)$ hides the dependence on the constant $\epsilon$. The hidden constant in $O_{\epsilon}(.)$ is %$c\frac{\log(1/\epsilon)}{\epsilon^2}  {\frac{1}{\epsilon^6} \log(1/\epsilon)  \choose {\frac{1}{\epsilon^4} \log(1/\epsilon)}}$ 
\etaMacro for some absolute constant $c$.
%~\cite{Badanidiyuru2014StreamingFly} and~\cite{kesselheim}.

\begin{table}[h!]
\centering
\begin{tabular}{ |c c c c c| }
\hline
 & \#selections & Comp ratio & Running time & Comp ratio in poly(n) \\%&  Comp ratio in poly(n,k)  \\ 
\hline
\cite{kesselheim} & $k$ & $1/e-O(k^{-1/2})$ & $exp(n)$ & $\frac{1}{e}(1-1/e)$ \\ %& $(1-1/e)1/e$ \\ 
this & $O_{\epsilon}(k)$ & $1-1/e-\epsilon-O(1/k) $ & $O_{\epsilon}(n)$ &  $1-1/e-\epsilon-O(1/k)$ \\%&  $1-1/e-\epsilon$ \\
%2nd & $k\log^2 k$ & $1/2-O(k^{-1/4})$ & $poly(n), exp(k)$ & $1/2-O(k^{-1/4})$ & $(1/2-O(k^{-1/4}))(1-1/e)$ \\
\hline    

\end{tabular}
\caption{\nameOfProblem~settings}
\label{table:t1}
\end{table}
%On the other hand, in the streaming framework the decision to select an element is not irrevocable, and there is a buffer of limited size and you can add or remove elements from the buffer, i.e., you can deselect some elements that you have already selected. The random order assumption in this model is not necessary.
In the streaming setting, \citet{Chakrabarti2015} provided a single pass streaming algorithm for monotone submodular function maximization under $k$-cardinality constraint, that achieves a $0.25$ approximation under adversarial ordering of input. Further, their algorithm requires $O(1)$ function evaluations per arriving item and $O(k)$ memory.
The currently best known approximation  under  adversarial order streaming model is by~\citet{Badanidiyuru2014StreamingFly}, who achieve a $1/2-\epsilon$ approximation with a memory of size $O(\frac{1}{\epsilon}k\log k)$. 
%\scomment{no known? or is it not possible?}\mcomment{not possible}
%Any algorithm for streaming submodular
%maximization that only queries the value of the
%submodular function on feasible sets (i.e., sets of cardinality
%at most k) and is an α-approximation for a
%constant α > 0.5 must use Ω(n/k) memory, where n is
%the length of the stream.
There is an upper bound of $1/2+o(1)$ on the competitive ratio achievable by 
any algorithm for streaming submodular
maximization that only queries the value of the submodular function on feasible sets while using $o(n)$ memory~\cite{norouzi}.
%any streaming algorithm for this problem under adversarial order, while using $o(n)$ memory~\cite{norouzi}.
%It does not need random order assumption. 
%Also note that this algorithm can not be converted into an online algorithm. 
%Streaming algorithm with random order assumption has been considered for other problems. 
%But nothing better than~\cite{Badanidiyuru2014StreamingFly} is known for this problem under random order setting. 

\citet{Hess} initiated the study of  \streamingProblem.
Their algorithm uses $O(k)$ memory and a total of $n$ function evaluations to achieve $0.19$ approximation. 
%This result is  worse than the result of~\cite{kesselheim}  in the stricter online model. But note that~\cite{kesselheim} requires $\Omega(nk)$ function evalutation and $\Omega(n)$ memory.
The state of the art result in the random order input model is due to \citet{norouzi} who achieve a $1/2+8\times 10^{-14}$ approximation, while using a memory buffer of size $O(k\log k)$.
%Badanidiyuru et al.~\cite{Badanidiyuru2014StreamingFly} design the first efficient streaming algorithm
%with constant factor $1/2-\epsilon$ approximation guarantee, requiring only a single pass through the data, and memory $O(\frac{1}{\epsilon}k\log k )$.
%Recently~\cite{norouzi} showed that it is impossible to get ratio better than $1/2+o(1)$ in the adversarial order input using memory $o(n)$.
%Our algorithm is in the intersection of the above frameworks. 
%It generalizes the online framework in the way that we are allowed to select more than $k$ elements. 
%We generalize the online model in the way that we are allowed to select more than $k$ elements, and output a subset of size $k$ whose  value is close to OPT.  Note that we are only interested in returning a subset of size at most $k$ as our output.  
%In algorithms like ~\cite{Vondrak}, although the output is close to OPT, it is not restricted to $k$ elements, and we can't guarantee that it contains a subset of size $k$ whose value is close to OPT.
%In comparison, our algorithm selects $O(k)$ elements and guarantees that there is a subset of size $k$ whose value is $R-O(k^{-1})$ times $OPT$, for $R<1-1/e$.Thus by relaxing the number of selections we improve upon the best competitive ratio $1/e$, while only using $O(n)$ running time.  These bounds compare favorably to~\cite{kesselheim}, which  needs to find the optimal offline solution $n$ times, or to use an $1-1/e$ approximation to find each offline optimal solution. In the latter case, the running time is  $O(n^2)$ and the competitive ratio is  $\frac{1}{e} (1-1/e)$.
 
%It is asymptotically a $1/2-O(k^{-1/4})$ approximation algorithm.
%In terms of memory size, it improves upon the previous $k\log k$~\cite{norouzi}. %$\frac{1}{\epsilon}k\log k$.%, for $k>(1/\epsilon)^4$.
%(Note that the approximation ratio of our algorithm is asymptotic and for a fixed $k$ we can not decrease error more than $k^{-1/4}$)
%Also in terms of running time it is polynomial in $n$, but it requires exponential time in $k$.
%Also note that the online algorithm~\cite{kesselheim} can not be converted into a streaming algorithm with nontrivial memory size.

%The goal is to partition the items between agents so as to maximize the sum of their valuation functions.
%The well known greedy algorithm gives a 1/2 approximation for this problem. Also for the adversarial order 1/2 is the best we can achieve~\cite{Kapralov:2013}.
%\cite{vahab},~\cite{swm}  slightly improve the analysis of the greedy algorithm to just above 1/2 for  random order input (0.505, 0.509 competitive ratio respectively). The later result can be generalized to maximizing monotone sumobular functions subject to  a partition matroid. It is incomparable with \nameOfProblemSL.

%Table~\ref{table:t1} and 
Table~\ref{table:t2} provides a detailed comparison of our result in Theorem \ref{thm:streaming} to the 
%, we compare our algorithm to some of the previous works to show the tradeoffs in the various parameters for both the online algorithms model and the streaming model.
above-mentioned results for  \streamingProblem, showing that our algorithm substantially improves the existing results on most aspects of the problem. 

\begin{table}[h!]
\centering
\begin{tabular}{ |c c c c c | }
\hline
 & Memory size & Approximation ratio & Running time & update time \\ 
 \hline
\cite{Hess} & $O(k)$ &  $0.19$ & $O(n)$ & O(1) \\ 
\cite{norouzi} & $O(k\log k)$ &  $1/2+8\times 10^{-14}$ & $O(n\log k)$ & $O(\log k)$ \\ 
\cite{Badanidiyuru2014StreamingFly} & $O(\frac{1}{\epsilon}k\log k)$ & $1/2-\epsilon$ & $poly(n,k, 1/\epsilon)$ & $O(\frac{1}{\epsilon}\log k)$ \\ 
this & $O_{\epsilon}(k)$ & $1-1/e-\epsilon-O(1/k)$ & $O_{\epsilon}(n)$ & amortized $O_{\epsilon}(1+\frac{k^2}{n})$ \\
%2nd & $k\log^2 k$ & $1/2-O(k^{-1/4})$ & $poly(n), exp(k)$ &  \text{amortize one operation}\\
\hline    
\end{tabular}
\caption{\streamingProblem
}
%$\log(1/\epsilon) {\frac{1}{\epsilon^3} \log(1/\epsilon)  \choose {\frac{1}{\epsilon^2} \log(1/\epsilon)}}$.}
\label{table:t2}
\end{table}



There is also a line of work studying the online variant of the submodular welfare maximization problem (e.g., \cite{vahab,swm,Kapralov:2013}). In this problem, 
the items arrive online, and each arriving item should be allocated  to one of $m$ agents with a submodular valuation functions $w_i(S_i)$ where $S_i$ is the subset of items allocated to $i$-th agent). The goal is to partition the arriving items into $m$ sets to be allocated to $m$ agents, so that the sum of valuations over all agents is maximized. This setting is incomparable with the \nameOfProblem~setting considered here.

==> olderProof.tex <==
\begin{lemma}
\label{lem:piBound}
For any element $i\in S^*$, and $w \in \{1,\ldots, W\}$
\begin{equation}
p_i:=\mathbb{P}(i\in U_w \cup Supp(T_{1,\ldots, w-1}) | T_{1,\ldots, w-1}=T) \ge \frac{\alpha}{k}
\end{equation}
\end{lemma}
\begin{proof}
%Remember that from lemma~\ref{eqprob}, for every configuration $Y \in [k\beta]^n$, we have $\mathbb{P}(Y)=(k\beta)^{-n}$.
%Also from above lemma, for $1\le w\le W$,  $T_{1,\ldots, w}$ and $S_{1, \ldots, w}$ are uniquely defined for each configuration $Y$.
%Suppose $T_{1,\cdots, w-1}=T$ and 
Let $s$ be a slot in the first $w-1$ windows and $s'$ be a slot in window $w$.
If $i\in Supp(T)$ then the statement of the lemma is trivial, so suppose $i\notin Supp(T)$.
By applying Bayes' rule to equation~\ref{eq1} we have
\[
\mathbb{P} (Y_i=s  | T_{1,\ldots, w-1}=T) \frac{ \mathbb{P}(T_{1,\ldots, w-1}=T) }{\mathbb{P}(Y_i=s) } 
\le \mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) \frac{ \mathbb{P}(T_{1,\ldots, w-1}=T) }{\mathbb{P}(Y_i=s') } 
\]
Also from Lemma~\ref{indep}, $\mathbb{P}(Y_i=s)  = \mathbb{P}(Y_i=s')$ thus 
\[
\mathbb{P} (Y_i=s  | T_{1,\ldots, w-1}=T) 
\le \mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) 
\]
Furthermore, for slot $s"$ in  windows $w, w+1, \cdots, W$, by applying Bayes' rule to lemma~\ref{afterw}
we have $\mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) =\mathbb{P} (Y_i=s"  | T_{1,\ldots, w-1}=T)$.
As a result $\mathbb{P}(i \in U_w \cup R_{1,\ldots, w-1} | T_{1,\ldots, w-1}) \ge \frac{\alpha}{k}$.

\end{proof}
%And, for every  $i\in S^*$, define
%\begin{equation}
%p_i :=\mathbb{P}(i\in U_w \cup R_{1,\ldots, w-1} | T_{1,\ldots, w-1})
%\end{equation}
%Then, a corollary of Lemma \ref{lem:piBound} is that $p_i \ge \alpha/k$. 

\begin{lemma}
\label{JIN}
Fix a window $w$. Now, given $U_w, T_{1, \ldots, w-1}$, create $\tilde{S}$ by accepting each item $i\in S^* \cap (U_w \cup R_{1,\ldots, w-1})$ independently with probability $\alpha/(kp_i)$. Then,
the indicator random variables $\{{\mathbf 1}(i\in \tilde S)|T_{1,\ldots, w-1} \}$ for all $i\in S^*$ are independent with  expected value $\alpha/k$.
\end{lemma}
\begin{proof}
Using Lemma \ref{lem:piBound}, the expected value can be derived as
$$\mathbb{P}(i\in \tilde{S}| T_{1, \ldots, w-1}) = \mathbb{P}(i\in \tilde{S}| i\in U_w\cup R_{1,\ldots, w-1},T_{1, \ldots, w-1} )\mathbb{P}(i\in U_w\cup R_{1,\ldots, w-1}| T_{1, \ldots, w-1}) = \alpha/(kp_i) \times p_i = \alpha/k.$$
Next, we show that for any $i,j\in S^*$, random variables ${\mathbf 1}(i\in \tilde S)|T_{1,\ldots, w-1}$ and ${\mathbf 1}(j\in \tilde S)|T_{1,\ldots, w-1}$ are independent. Given the construction of $\tilde S$, it suffices to prove that the random variables ${\mathbf 1}(i\in U_w \cap R_{1,\ldots, w})|T_{1,\ldots, w-1}$ and ${\mathbf 1}(j\in U_w \cap R_{1,\ldots, w})|T_{1,\ldots, w-1}$ are independent. Now, given $T_{1,\ldots, w-1}=T$, if $i \in Supp(T)$ then this is trivial since $R_{1,\ldots, w} =Supp(T)$ so that $\mathbb{P}(i\in U_w \cap R_{1,\ldots, w} | T_{1,\ldots, w-1}=T)=1$. Similarly for $j\in Supp(T)$.

So, assume $i,j  \notin Supp(T)$. Then, the problem reduces to proving that  ${\mathbf 1}(i\in U_w)|T$ and ${\mathbf 1}(j\in U_w)|T$ are independent, i.e., given $T$, $i$ and $j$ will appear in the window $w$ independently. 
To prove this, we show that $\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T)=\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T \text{ and } Y_j =s')$, i.e., slot assignment of $i$ is independent of the slot assignment of $j$. 

Suppose $Y'$ is a configuration such that $Y'_i=s$ and $Y'_j=s'$, and $T_{1,\cdots, w-1}(Y')=T$. To show the required independence, we show that for every other feasible slot assignment of $j$, there exists a feasible configuration where slot assignment of $i$ is $s$.
More precisely, consider any configuration $Y''$ such that $T_{1,\cdots, w-1} (Y'') =T$ and $Y''_j=s''$ where $s''\ne s'$. (If no such configuration $Y''$ exists, then $Y_j|T$ is always $s'$ so that $s'$ is the only feasible assignment of $j$ given $T$, and the desired statement is trivially true.)
Then by changing $Y_j$ from $s'$ to $s''$ in $Y'$, we can obtain another configuration $\bar{Y}$. In Lemma~\ref{addtoslot}, we show that this change will not effect $T_{1,\cdots, w-1}$, i.e., $T_{1,\cdots, w-1} (\bar Y)=T $. 
Thus configuration $\bar Y$ satisfies the desired statement.
\end{proof}
\scomment{I replaced the proof below with the proof of Lemma 7}
\toRemove{
\begin{proof}
Suppose $i,j \in S^*$. 
If $i \in Supp(T) $ then this is trivial since $\mathbf{1}(i\in \tilde S) | T=1$. \scomment{the preceding statement is not correct, in that case, we just have $p_i=1$.}
So suppose $i,j  \notin Supp(T)$. 
%Now we show that $\mathbb{P}(J_i=1|T_{1,\cdots, w-1}=T)=\mathbb{P}(J_i=1|T_{1,\cdots, w-1}=T \text{ and } J_j =s')$.
Now we show that $\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T)=\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T \text{ and } Y_j =s')$.
Suppose $Y$ is a configuration in which $Y_i=s$ and $Y_j=s'$, and $T_{1,\cdots, w-1} (Y)=T$.
Also suppose there exists at least one configuration $\bar{Y}$ such that $T_{1,\cdots, w-1} (\bar{Y}) =T$ and $\bar{Y}_j=s"$. \scomment{what if no such configuration exists?}
Then by changing $Y_j$ from $s'$ to $s"$ we obtain a configuration $Y'$. Also from lemma~\ref{addtoslot}, we have  $T_{1,\cdots, w-1} (Y')=T $. 
%It is because in configuration $Y$, $j$ has not been selected in slot $s'$ and its removal will not change $T_{1,\cdots, w-1}$.
%Furthermore since there is a configuration $\bar{Y}$ as described above, adding $j$ to $s"$ will not change $T_{1,\cdots, w-1}$.
Hence the mapping from $Y$ to $Y'$ proves lemma.
\end{proof}
}

\begin{lemma} \label{addtoslot}
Fix a slot $s'$, $T$, $j\notin Supp(T)$. Suppose that there exists  some configuration  $Y'$ such that $T_{1,\cdots, w-1} (Y') =T$ and $Y_j'=s'$. Then, given any configuration $Y''$ with $T_{1,\ldots, w-1}(Y'')=T$, we can replace  $Y''_j$ with $s'$ to obtain a new configuration $\bar Y$ that also satisfies $T_{1,\ldots, w-1}(\bar Y)=T$.
\toRemove{
Suppose there exists at least one configuration $\bar{Y}$ such that   $T_{1,\cdots, w-1} (\bar{Y}) =T$ and $\bar{Y}_j=s$ for $j\notin Supp(T)$.
Then for any configuration $Y$ with  $T_{1,\cdots, w-1} (Y) =T$, by setting $Y_j=s$, we get a new configuration $Y'$
such that $T_{1,\cdots, w-1} (Y') =T$.}
\end{lemma}
\begin{proof}
%Suppose $Y$ is a configuration such that $T_{1,\cdots, w-1} (Y) =T$. 
Suppose the slot $s'$ lies in window $w'$.
If $w' \ge w$ then the statement is trivial. So suppose $w' < w$.
Create an intermediate configuration by {\it removing} the item $j$ from $Y''$, call it $Y^-$. Since $j\notin Supp(T_{1,\cdots, w-1}(Y'')) = Supp(T)$ we have $T_{1,\cdots, w-1} (Y^-) =T$. In fact, for every subsequence $\tau$, the greedy subsequence for $Y''$, will be same as that for $Y^-$, i.e.,   $\gamma_{Y''}(\tau) = \gamma_{Y^-}(\tau)$.
Now add item $j$ to slot $s'$ in $Y^-$, to obtain configuration $\bar Y$. We claim $T_{1,\cdots, w-1} (\bar Y) =T$.
%We only need to show that $j$ will not get selected in slot $s$ in configuration $Y'$.
%Suppose not, then there is a subsequence $\tau$  in the algorithm ending in slot $s$ such that $\gamma_{Y'} (\tau) =\{i_1, \cdots, i_{t-1}, j\}$


By construction of $T_{1,\ldots, w}$, we only need to show that $j$ will not be part of the greedy subsequence $\gamma_{\bar Y}(\tau)$ for any subsequence $\tau, |\tau| = \alpha$ containing the slot $s'$ when the input is in configuration $\bar Y$. To prove by contradiction, suppose that $j$ is part of greedy subesquence for some $\tau$ ending in the slot $s'$. \toRemove{We only need to show that $j$ will not get selected in slot $s$ in configuration $Y'$.
Suppose $j$ gets selected in slot $s$ for some subsequence $\tau$ ending in slot $s$.}
%Thus $\gamma_{Y'}(\tau) = \{i_1, \cdots, i_{t-1}, j\}$. Note that since slots before $s$ are the same as $Y^-$ and $T_{1,\cdots, w-1} (Y^-) =T$, $\gamma_{Y^-}(\tau) = \{i_1, \cdots, i_{t-1}, i_t\}$.
\toRemove{Suppose that $\gamma_{Y^-}(\tau)  := \{i_1, \cdots, i_{t-1}, i_t\} = \gamma_{Y''}(\tau) $.} 
For this $\tau$, let $\gamma_{Y^-}(\tau)  := \{i_1, \cdots, i_{\alpha-1}, i_\alpha\} = \gamma_{Y''}(\tau) $. Note that since the items in the  slots  before $s'$ are identical for $\bar Y$ and $Y^-$, \toRemove{and $T_{1,\cdots, w-1} (Y^-) =T$,} we must have that $\gamma_{\bar Y}(\tau) = \{i_1, \cdots, i_{\alpha-1}, j\}$, i.e.,
$\Delta_f(j | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{\alpha-1}\} ) \ge \Delta_f(i_\alpha | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{\alpha-1}\} ) $.
%$j=\arg \max_{i\in j\cup U_s \cup T_{1, \ldots, w-1}} \Delta_f(i | S_{1,\ldots,w-1} \cup \{i_1,\ldots, i_{t-1}\} \cup \{i\}) $
%$i_t=\arg \max_{i\in U_s \cup T_{1, \ldots, w-1}} \Delta_f(i | S_{1,\ldots,w-1} \cup \{i_1,\ldots, i_{t-1}\} \cup \{i\}) $
On the other hand, since $T_{1,\cdots, w'-1} (Y') = T_{1, \cdots, w'-1}(Y'') = T (\text{restricted to $w'-1$ windows})$,  we have that $\gamma_{Y'} (\tau) =\{i_1, \cdots, i_\alpha\}$.
However, $Y'_j=s'$. Therefore $j$ was not part of the greedy subsequence $\gamma_{Y'}(\tau)$ even though it was in the last slot in $\tau$, implying $\Delta_f(j | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{t-1}\} ) < \Delta_f(i_t | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{t-1}\} ) $. This is  is a contradiction to the earlier observation.


\end{proof}
%Now let  indicator random variable $J_i$ for $i\in S^*$ indicates whether or not $i \in \tilde{S}$ 
%indicates whether or not $e$ appears in $U_w$, i.e., whether or not $U_i^e\in W_{i+1}$.



%Also if $V_e$ is a random variable indicating whether or not $e\in \mathcal{A}$ for $e\in OPT'$,
%we show $\{V_e|Snapshot(i)\}_{e\in OPT'}$ are i.i.d.  with $\mathbb{P}[V_e=1] = \alpha/k$.

%\begin{lemma}
 % %$\mathbb{P}[e=b_j| e\in \mathcal{A}]=1/k$ for $j\in[k]$.
% Random variables $\{V_e|Snapshot(i)\}$,  $ \forall e\in OPT'$ are i.i.d. with $\mathbb{P}[V_e=1]=\alpha/k$.
%\end{lemma}

%\begin{prop}\label{uni}
% Given $i \in \tilde{S}$, we have $\mathbb{P}(i=j)=1/k$, $\forall j\in S^*$.
%\end{prop}

%\scomment{The lemma statement below is not precise- it seems you actually mean uniformly at  random over $\tilde S|T_{1,\ldots, w-1}$, i.e., random also over $U_w$, but given $T_{1, \ldots, w-1}$. We can discuss.}
\begin{prop}\label{uni}
For element $i$ drawn uniformly at random from $\tilde{S}$, we have $\mathbb{P}(i=e)=1/k$, $\forall e\in S^*$.
\end{prop}




Now each element in $\tilde{S}\cap U_w$ has a unique slot in $w$. 
\begin{prop}
Suppose $p_1, \dots, p_{\ell}$ are the slots in $w$ containing at least one element of $\tilde{S}\cap U_w$ (in the same order that they appear in $w$). 
In addition, suppose $b_j\in p_j\cap \tilde{S}$, is the element of $\tilde{S}\cap U_w$ in slot $p_j$ (in case there are more than one element choose one randomly).
%$a_1 ,\cdots, a_t$ are $t$ samples without replacement drawn uniformly at random from $\tilde{S}$.
Then $b_1, \cdots, b_{\ell}$ is a random order of $\{b_1, \cdots, b_{\ell}\}$, and $\{b_1, \cdots, b_{\ell}\}$ are drawn uniformly at random from $\tilde{S}\cap U_w$.
\end{prop}
\scomment{Is Proposition 3 same as saying that $\{Y_i, i\in \tilde S\cap U_w\}$ are i.i.d. and uniformly distributed over slots in $w$? Where is the proof of this proposition?}
\mcomment{Yes, it follows from lemma 7 and the fact that we showed in lemma 6: for slot $s"$ in  windows $w$, by applying Bayes' rule to lemma~\ref{afterw}
we have $\mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) =\mathbb{P} (Y_i=s"  | T_{1,\ldots, w-1}=T)$.}
%\begin{prop}\label{rord}
%%$a_1 ,\cdots, a_t$ are $t$ samples without replacement drawn uniformly at random from $\tilde{S}$.
%$a_1, \cdots, a_t$ is a random order of $\{a_1, \cdots, a_t\}$, and $\{a_1, \cdots, a_t\}$ are drawn uniformly at random from $\tilde{S}$.
%\end{prop}

On the other hand, elements of $\tilde{S}\cap R_{1,\ldots, w-1}$ 
are not assigned to a  unique slot in $w$ (in the algorithm they were compared against the maximum marginal value in all the slots of $w$).
So we can assign each of them to a unique random slot in $w$.

\begin{prop}
Suppose $q_1, \dots, q_{m}$ are the slots in $w$ assigned to at least one element of $\tilde{S} \cap R_{1,\ldots, w-1}$ (in the same order that they appear in $w$). 
Furthermore, suppose $c_j\in q_j\cap \tilde{S}$, is the element of $\tilde{S}\cap R_{1,\ldots, w-1}$ in slot $q_j$ (in case there are more than one element choose one randomly).
%$a_1 ,\cdots, a_t$ are $t$ samples without replacement drawn uniformly at random from $\tilde{S}$.
Then $c_1, \cdots, c_m$ is a random order of $\{c_1, \cdots, c_m\}$, and $\{c_1, \cdots, c_m\}$ are drawn uniformly at random from $\tilde{S}\cap R_{1,\ldots, w-1} $.
\end{prop}


Now suppose $\{i_1, \cdots, i_t\}=\{p_1, \dots, p_{\ell}\} \cup \{q_1, \dots, q_{m}\}$ (in the same order that they appear in $w$).
From above propositions we have
\begin{prop}\label{rord}
Suppose $a_j \in i_j$  is an element of $i_j \cap (\{p_1, \dots, p_{\ell}\} \cup \{q_1, \dots, q_{m}\})$ (in case there are more than one element choose one randomly).Then
% $a_1, \cdots, a_m$ is a random order of $\{c_1, \cdots, c_m\}$, and $\{c_1, \cdots, c_m\}$ are drawn uniformly at random from $\tilde{S}\cap R_{1,\ldots, w-1} $.
%$a_1 ,\cdots, a_t$ are $t$ samples without replacement drawn uniformly at random from $\tilde{S}$.
$a_1, \cdots, a_t$ is a random order of $\{a_1, \cdots, a_t\}$, and $\{a_1, \cdots, a_t\}$ are drawn uniformly at random from $\tilde{S}$.
\end{prop}





%Consider the set $\mathcal{A}$ we create using the blackbox algorithm. It is a set that we create only for the purpose of argument. Algorithm~\ref{alg:khod} is not aware of this set. 
%Its existence is enough for the algorithm.
The algorithm \textit{guess} the position of elements of $\tilde{S}$, %$OPT\cap W_{i+1}$, 
i.e., slots $i_1, \cdots, i_t$. %, where $t \ge (1-\delta)\alpha$ w.h.p.
In other words, for some $\tau$ in the enumeration of algorithm,  the elements of $\tilde{S}$ lie in the slots of $\tau$. i.e., $\{i_1, \cdots, i_t\} \subseteq \tau$.
%Suppose $a_j\in i_j\cap \tilde{S}$, is the element of $\tilde{S}$ in slot $i_j$.
Suppose $s_j$ is the maximum element selected by the algorithm in $i_j$.
i.e., %$s_j=\omega(\{i_1,\dots,i_j\})$.
$s_j=argmax_{a\in i_j} \Delta_F(a| \gamma{(i_1,\ldots, i_{j-1})})$.
Also let's define $A(j)=\{a_1, \cdots, a_j\} $ and $S(w,j)= S_{1,\ldots, w-1} \cup \{s_1,\cdots, s_j\}$.

\begin{lemma}
%$\mathbb{E}[\Delta_F(S_w | S_{1,\ldots, w-1})] \ge \frac{t}{k} (\frac{k-\alpha}{k}OPT-\mathbb{E}[F(S_{1,\ldots, w-1})])$.
$\mathbb{E}[\Delta_F(s_{j+1}|S(w,j))] \ge \frac{1}{k} (\frac{k-\alpha}{k}OPT-\mathbb{E}[F(S(w,j))])$
\end{lemma}

\begin{proof}
\scomment{What is $OPT'$? What is $P$?}
\mcomment{$P:=S^*\setminus S_{1,\dots, w-1}$, Replaced}
From proposition~\ref{uni} and~\ref{rord}, $a_1$ can be any element in $S^*$, % $OPT\setminus P$, 
w.p. at least $1/k$.
Thus,
\[
\mathbb{E}[\Delta_F(a_1|S_{1,\ldots, w-1}) | T_{1,\ldots, w-1}] \ge \frac{1}{k} \sum_{e\in S^*} \Delta_F(e|S_{1,\ldots, w-1}) %=\frac{1}{k} \sum_{e\in OPT\setminus %P} \Delta_F(e|S_{1,\ldots, w-1}).
\]

%\[
%\mathbb{E}[\Delta_F(a_1|S_{1,\ldots, w-1}) | T_{1,\ldots, w-1}] \ge \frac{1}{k} \sum_{e\in OPT'} \Delta_F(e|S_{1,\ldots, w-1}) =\frac{1}{k} \sum_{e\in OPT\setminus P} \Delta_F(e|S_{1,\ldots, w-1}).
%\]
% (OPT-F(S(i)))$.


Now we use the following well known lemma:
\begin{lemma}%\label{marginalsum}
For any set $A$ and $B$, $\Delta_F(A|B) \le \sum_{a\in A\setminus B} \Delta_F(a|B)$
\end{lemma}
%(Note that in the original version of this lemma the sum is over $A$ instead of $A\setminus B$. But the above format is  stronger if  $A$ and $B$ have intersection. It is the reason we can assign value zero to dummy elements which represent the intersection).
Therefore,
\[
%OPT-F(S(i)) \le \sum_{e\in OPT} \Delta_F(e|S(i)) = \sum_{e\in OPT\setminus P} \Delta_F(e|S(i)) 
OPT-F(S_{1,\ldots, w-1}) \le  \sum_{e\in S^*}  %OPT\setminus P} 
\Delta_F(e|S_{1,\ldots, w-1})  %=  \sum_{e\in OPT'} \Delta_F(e|S(i)) 
\]
Hence,  
\[
\mathbb{E}[\Delta_F(a_1|S_{1,\ldots, w-1})|T_{1,\ldots, w-1}] \ge \frac{1}{k} (OPT-F(S_{1,\ldots, w-1})).
\]
%Now let's define $A(j)=\{a_1, \cdots, a_j\} $ and $S(w,j)= S_{1,\ldots, w-1} \cup \{s_1,\cdots, s_j\}$.
%denote $S(i)\cup \{s_1, \cdots, s_j\} $ by $S(i,j)$. 
Similarly, we can see that 
%$E[\Delta_F(a_{j+1}|S(i,j))] \ge \frac{1}{k} (OPT-F(S(i,j)))$.
\[
\mathbb{E}[\Delta_F(a_{j+1}|S(w,j)) | T_{1,\ldots, w-1}] \ge  \frac{1}{k} \sum_{e\in S^*\setminus A(j)} \Delta_F(e|S(w,j)) 
%=\frac{1}{k} \sum_{e\in OPT\setminus (P\cup A(j))} \Delta_F(e|S(w,j)) 
%\ge \frac{1}{k} \sum_{e\in OPT\setminus (P\cup A)} \Delta_F(e|S(i,j))
\]
Also we have,
\begin{align*} %\label{eq1}
%\begin{split}
%A & = \frac{\pi r^2}{2} \\
% & = \frac{1}{2} \pi r^2
\sum_{e\in S^*\setminus A(j) } %OPT\setminus {(P\cup A(j))}} 
\mathbb{E}[\Delta_F(e|S(w,j)) | T_{1,\ldots, w-1}]  %= \sum_{e\in OPT\setminus P} \Delta_F(e|S(i,j)) 
&\ge \mathbb{E}[F(S^*\setminus A(j)) | T_{1,\ldots, w-1}]-\mathbb{E}[F(S(w,j)) | T_{1,\ldots, w-1}] \\
&\ge \frac{k-\alpha}{k}OPT-\mathbb{E}[F(S(w,j)) | T_{1,\ldots, w-1}] 
%\end{split}
\end{align*}
The last inequality coming from the fact that given $T_{1,\ldots, w-1}$, the set $A(j)$ is a random subset of $S^*$ of size at most  $\alpha$,
so we can apply the following lemma%~\ref{randomsubset}.
\begin{lemma}\label{randomsubset}
For a random subset $A$ of $R$, the expected value of $f(A)$ is at least $\frac{|A|}{k}.f(R)$.
\end{lemma}
Thus 
\[
\mathbb{E}[F(S^*\setminus A(j)) | T_{1,\ldots, w-1}] \ge \frac{k-\alpha}{k}OPT .
\]
Hence, 
\begin{align*}
\mathbb{E}[\Delta_F(s_{j+1}|S(w,j)) | T_{1,\ldots, w-1}] &\ge \mathbb{E}[\Delta_F(a_{j+1}|S(w,j)) | T_{1,\ldots, w-1}] \\
& \ge \frac{1}{k} (\frac{k-\alpha}{k}OPT-\mathbb{E}[F(S(w,j)) | T_{1,\ldots, w-1}]) 
\end{align*}
Now by taking expectation over all possible realizations of $T_{1,\ldots, w-1}$,
\[
\mathbb{E}[\Delta_F(s_{j+1}|S(w,j))] \ge \frac{1}{k} (\frac{k-\alpha}{k}OPT-\mathbb{E}[F(S(w,j))])
\]
%Now by standard techniques we can deduce that $\mathbb{E}[F(S_{1,\ldots, W})] \ge (1-1/e)(\frac{k-\alpha}{k})(1-\delta) OPT$.

 \end{proof}

 
 
Now we prove 
elements of $\tilde{S}$ cover at least  $(1-\delta)\alpha$ slots in $w$, w.h.p. Let $t_w$  denote the number of these slots in $w$.

\begin{theorem}
%Elements of $\tilde{S}$ cover at least  $(1-\delta)\alpha$ slots in $w$, w.h.p.
$(1-\delta)\alpha \le t_w \le (1+\delta)\alpha$, w.h.p. 
\end{theorem}


%Therefore,
%$$\Ex[f(\tilde S \cup S_{1,\ldots, w-1}) - f(S_{1,\ldots, w-1})] \ge \frac{\alpha}{k} f(S^* \cup S_{1,\ldots, w-1}) - f(S_{1,\ldots, w-1}) $$
%INCOMPLETE: the expected size of $\tilde{S}$ is $\alpha$, but the realized size could be larger, and will be truncated to $\alpha$. We need to account for the decrease in objective due to this truncation.
By Chernouf bound, we can show that with high probability each window contains roughly $\alpha$ elements of $\tilde{S}$.

\begin{lemma}\label{bern}
%Suppose $W$ is a $(\alpha,\beta)$ window then
For window $w$
\[
\mathbb{P}(|\tilde{S}| < (1-\delta)\alpha ) %\le exp(-\frac{ (1/2)\alpha^{3/2}}{\alpha+1}) \le exp(-\sqrt{\alpha}/4)
\le \exp(-\delta^2 \alpha/2)
\]
\end{lemma}

Also we can show that roughly $\alpha-2\alpha/\beta$ slots in a window contain at least one element of $\tilde{S}$.

\begin{lemma}\label{slotlemma}
%The probability that one slot has two or more elements is at most $1-e^{-1/\beta}$.
%The fraction of nonempty slots with more than one elements of $OPT$ is at most $\beta(1-e^{1/\beta})$.
%The total number of slots  with more than one element of $OPT$  is at most $2\alpha/\beta$, w.h.p.
Given $|\tilde{S}|=r$,
the total number of slots in $W$ containing at least one element of $\tilde{S}$ is greater than %\alpha-2\alpha/\beta$  w.h.p.
$r(1-r/\alpha \beta)$  w.h.p.
%The total number of elements $e\in OPT\cap W$ such that $Y_e\cap OPT=\{e\}$ is at least $\alpha-2\alpha/\beta$.
%with more than one element of $OPT$  is at most $2\alpha/\beta$, w.h.p.
%$\beta(1-e^{1/\beta})$, w.h.p.
\end{lemma}
\begin{proof}

Suppose $\tilde{S}=\{a_1,\dots, a_r\}$.
%From previous lemma $r\le 2\alpha$, w.p. at least $1-\exp(-\sqrt{\alpha}/3)$.
Let $Z_i$ be a random variable indicating whether or not %$Y_{a_j}\cap OPT\neq \{a_j\}$.
$|Y_{a_j}\cap \{a_1,\dots, a_{j-1}\}| \ge 1$.
%indicating whether $a_k$ is alone in its slot or not.
We have at most $r$ occupied slots, thus the probability that $Z_i=1$ is at most $ r/(\alpha \beta) $ or $\mathbb{E}[Z_i]\le r/\alpha\beta$. Furthermore let $X_i=\sum_{j=1}^{i} Z_j$, then $\mathbb{E}[X_i] \le ri/\alpha\beta$.
%Also let $\mathcal{F}_i$ be the slots elements $1,\cdots, i$  are in, then $L\le \alpha/\beta$. 
Also define the set of filtration $\{\mathcal{F}_i\}$ to be the slots containing elements $\{a_1,\cdots, a_i\}$.
Then $\mathcal{F}_0 \subseteq \dots \subseteq \mathcal{F}_r$.
In addition, $L=\sum_{i\le r}  Var(Z_i|\mathcal{F}_{i-1}) \le r^2/\alpha\beta$.
By Freedman's inequality $\mathbb{P}( X_r > r^2/\alpha\beta + \epsilon )  \le exp(-\frac{\epsilon^2}{4r^2/\alpha\beta +2\epsilon})$.
\end{proof}

Suppose $\delta=1-1/e-R$.
From the above lemmas there are large enough constants $\alpha$ and $\beta$ such that:
\begin{itemize}
\item $r=|OPT\cap W| > (1-\delta/4)\alpha$. Thus $\alpha \ge \frac{1}{\delta^2} \log(1/\delta)$
\item The total number of slots in $W$ containing at least one element of $OPT$ is at least $(1-\delta)\alpha$.
Thus $(1-\delta/4)\alpha(1-(1-\delta/4)/\beta) > (1-\delta)\alpha$.
Therefore $\beta > (1-\delta/4)^2/(3/4\delta) $, so it suffices to have $\beta>\frac{4}{3\delta}$.
\end{itemize}
Hence we choose constants $(\alpha,\beta)$ with $\alpha \ge \frac{8}{\delta^2} \log(1/\delta)$ and $\beta>\frac{4}{3\delta}$,
so that we have above properties.

Therefore $\sum_{w} \min(\alpha, t_w) \ge (1-\delta)k$, w.h.p.
Now by standard techniques we can deduce that 
\begin{theorem}
$\mathbb{E}[F(S_{1,\ldots, W})] \ge (1-1/e)(\frac{k-\alpha}{k})(1-\delta) OPT$.
\end{theorem}
